A Library of Mirrors: Deep Neural Nets in Low Dimensions are Convex Lasso Models with Reflection Features

We prove that training neural networks on 1-D data is equivalent to solving convex Lasso problems with discrete, explicitly defined dictionary matrices. We consider neural networks with piecewise linear activations and depths ranging from 2 to an arbitrary but finite number of layers. We first show that two-layer networks with piecewise linear activations are equivalent to Lasso models using a discrete dictionary of ramp functions, with breakpoints corresponding to the training data points. In certain general architectures with absolute value or ReLU activations, a third layer surprisingly creates features that reflect the training data about themselves. Additional layers progressively generate reflections of these reflections. The Lasso representation provides valuable insights into the analysis of globally optimal networks, elucidating their solution landscapes and enabling closed-form solutions in certain special cases. Numerical results show that reflections also occur when optimizing standard deep networks using standard non-convex optimizers. Additionally, we demonstrate our theory with autoregressive time series models.

==> siamonline_220329/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Example Article\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> unused/3lyrReLUfeaturesfig.tex <==
%these figures got incorporated into one figure, so not needed. Correct though
\begin{figure}
    \centering
    \begin{tikzpicture}
    \pgfmathsetmacro{\hint}{12}
    \pgfmathsetmacro{\vint}{-6}
    \pgfmathsetmacro{\scale}{0.5}
    \pgfmathsetmacro{\xi}{4}
    \pgfmathsetmacro{\xj}{11}
    \pgfmathsetmacro{\xk}{15}
    \pgfmathsetmacro{\len}{26}
    \pgfmathsetmacro{\reflectkink}{\xj+\xk-\xi}
    \begin{scope}[scale=\scale,shift={(0*\hint,0)}]
    \draw[dashed] (0,0) -- (\len,0);
    \draw (0,\xi) -- (\xi,0) -- (\reflectkink,0) -- (\len,\len-\reflectkink);
    %\node (a1) at (3,0) [circle,fill=green, label=below left:$x_j$]{};
    %\node (zero) at (0,0) [circle,fill=red, label=below:$0$]{}; 
    \node (xi) at (\xi,0) [circle,fill=green, label=below:$x_i$]{}; 
    \node (xj) at (\xj,0) [circle,fill=red, label=below:$x_j$]{};
    \node (xk) at (\xk,0) [circle,fill=blue, label=below:$x_k$]{};
    \node (avg) at (0.5*\xk+0.5*\xj,0) [circle,fill=purple, label=below:$\frac{x_j+x_k}{2}$]{};
    \node (reflect) at (\reflectkink,0) [circle,fill=green, label=below:$x_j+x_k-x_i$]{};
    \end{scope}
    \end{tikzpicture}
    \caption{$\text{wedge}_{x_i,x_j+x_k-x_i}$ features for $3$-layer ReLU NNs with $2$ neurons but 
    %no 
    bias in the second layer. The non-data \kink{} occurs at the reflection of a data point $x_i$ about the average of two data points: $x_j+x_k-x_i=\reflect{x_i}{\frac{x_j+x_k}{2}}$}.
    \label{wedge_3lyrReLU}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \pgfmathsetmacro{\hint}{12}
    \pgfmathsetmacro{\vint}{-6}
    \pgfmathsetmacro{\scale}{0.5}
    %\begin{scope}[scale=\scale,shift={(0*\hint,0)}]
    %    \draw[dashed] (0,0) -- (10,0);
    %\draw (0,0) -- (5,0) -- (7,4) -- (10,7);
    %\node (a1) at (3,0) [circle,fill=green, label=below left:$x_j$]{};
    %\node (a2) at (5,0) [circle,fill=red, label=below:$x_i$]{}; 
    %\node (a3) at (7,0) [circle,fill=green, label=below:$\reflect{x_j}{x_i}$]{};
    %\end{scope}
    \begin{scope}[scale=\scale,shift={(1*\hint,0)}]
    \draw[dashed] (0,0) -- (10,0);
    \draw (0,0) -- (5,0) -- (7,4) -- (10,7);
    %\node (a1) at (3,0) [circle,fill=green, label=below left:$x_j$]{};
    \node (a2) at (5,0) [circle,fill=red, label=below:$x_i$]{}; 
    \node (a3) at (7,0) [circle,fill=green, label=below:$x_j$]{};
    \end{scope}
    \end{tikzpicture}
    \caption{$\hill_{x_i,x_j}$ features for $3$-layer ReLU NNs with $2$ neurons. The first slope is $2$, and the second slope is $1$. }
    \label{fig:3lyrelunobias2neurons}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
    \pgfmathsetmacro{\hint}{12}
    \pgfmathsetmacro{\vint}{-6}
    \pgfmathsetmacro{\scale}{0.5}
    \begin{scope}[scale=\scale,shift={(0*\hint,0)}]
   \draw[dashed] (0,0) -- (9,0);
    \draw (0,0) -- (2,0) -- (5,3) -- (7,3) -- (9,5);
    \node (a1) at (2,0) [circle,fill=red, label=below left:$x_j$]{};
    \node (a2) at (5,0) [circle,fill=green, label=below:$x_i$]{}; 
    
    \node (a3) at (7,0) [circle,fill=blue, label=below:$x_k$]{};
    \end{scope}
    \begin{scope}[scale=\scale,shift={(1*\hint,0)}]
    \draw[dashed] (0,0) -- (9,0);
    \draw (0,0) -- (2,0) -- (5,3) -- (7,7) -- (9,9);
    \node (a1) at (2,0) [circle,fill=red, label=below left:$x_i$]{};
    \node (a2) at (5,0) [circle,fill=green, label=below:$x_j$]{}; 
    
    \node (a3) at (7,0) [circle,fill=blue, label=below:$x_k$]{};
    \end{scope}
    \end{tikzpicture}
    \caption{Features $t_{x_i<x_j<x_k}$ (left) and $s_{x_i<x_j<x_k}$ (right) for $3$-layer ReLU NNs with $2$ neurons and bias in the middle layer.  In $t_{x_i<x_j<x_k}$ , the first slope is $1$, the second slope is $0$, and the third slope is $1$. In $s_{x_i<x_j<x_k}$ , the first slope is $1$, the second slope is $2$, and the third slope is $1$. }
    \label{fig:s}
\end{figure}

==> unused/background.tex <==


\section{Background: Convex optimization for neural networks in $D \geq 1$ dimensions }\label{app_section:NN_cvx_background}

%Convex analysis of neural networks was studied in several prior works. As an example, \cite{bengio2005convex,bach2017breaking,fang2019convex} studied infinite-width neural networks to enable the convexification of the overall model. However, due to the infinite-width assumption, these results do not reflect the training of finite-width neural networks in practice. Recently, a series of papers \cite{ergen2020aistats, ergen2021convex,pilanci2020neural} developed a convex analytic framework to train two-layer neural networks with ReLU activation. 

Recent papers have approached two layer networks from a convex analyis lens. \cite{pilanci2020neural} considers the following regularized training problem:
\begin{align}\label{eq:background_relu}
	 & p^*:=\min_{w,b,\alpha} \frac{1}{2}\sum_{n=1}^N \left(\sum_{i=1}^m\alpha_i\sigma(x_n w_i+b_i)-y_n \right)^2 + \frac{\beta}{2}\sum_{i=1}^m(|\alpha_i|^{2}+\|w_i\|_2^{2}).
\end{align}
Here, $x_i \in \mathbb{R}^d$ are row vectors, $w_i \in \mathbb{R}^d$ are column vectors, $\sigma(z) = \max \{0,z\}$ is the ReLU activation function and $\beta>0$ is a regularization parameter. Then using the convex duality arguments, they characterize the optimal solutions via the following dual problem of (a rescaled version of) \eqref{eq:background_relu}:
\begin{align}\label{eq:background_relu_dual}
	p^*\geq d^*:=\max_\lambda & -\frac{1}{2}\|\lambda-y\|_2^2+\frac{1}{2}\|y\|_2^2, \nonumber \\
	                          & \text{ s.t. }
	%\max_{\substack{w,b \\ \|w\|_2 \leq  1}}
	|\lambda^T\sigma(Xw+b)|\leq   \beta \,\,\forall w:\|w\|_2\le1,\,\beta\in\mathbb{R}.
\end{align}
After proving the strong duality for \eqref{eq:background_relu} and \eqref{eq:background_relu_dual}, i.e., $p^*=d^*$, they then take the dual of \eqref{eq:background_relu_dual} to obtain the convex bidual of \eqref{eq:background_relu} as follows:
\begin{align}\label{eq:background_relu_bidual}
	p^*= \min_{u_i,u_i',b_i,b_i'} & \norm{\sum_{i=1}^P D_i(X(u_i-u_i')+b_i\bone-b_i'\bone)-y}_2^2 + \beta\sum_{i=1}^P(\|u_i\|_2+\|u_i'\|_2), \nonumber \\
	\text{ s.t. }                 & D_i(Xu_i+b_i\bone)\geq 0, D_i(Xu_i'+b_i'\bone)\geq 0,
\end{align}
where $\{D_i\}_{i=1}^P$ is the enumeration of hyperplane arrangements for the data matrix $X$, which is detailed below.


%\subsection{Hyperplane arrangements}
First define the hyperplane arrangements set for $X \in \mathbb{R}^{N \times d}$ as,
%
%\begin{align*}
%\mathcal{H} := \bigcup \big \{ \%{\mathrm{sign}(X w)\} \,:\, w \in \mbR^d %\big \},
%\end{align*}
\begin{align}%\label{eq:Hdef}
	\mathcal{H}(X) :=  \big \{ \mathrm{sign}([X, \mathbf{1}] w) \,:\, w \in \mbR^{d+1} \big \},
\end{align} %making bias explicit

where the cardinality of the set $\mathcal{H}(X) $ can be upper bounded as $\vert \mathcal{H}(X) \vert \le 2^n$. Here, the set $\mathcal{H}(X)$ denotes all possible $\{+1,-1\}$ labelings of the samples $\{x_i\}_{i=1}^N$ by a linear classifier $w \in \mathbb{R}^{d+1}$. Next, define a new set to denote the indices with positive signs of the elements in $\mathcal{H}(X)$ as $
	\mathcal{S} := \big\{ \{ \cup_{h_i=1} \{i\}  \} \,:\, h \in \mathcal{H}(X) \big\}$. Now, for every for index set $S \in \mathcal{S}$, define a diagonal matrix $\diag(S) \in \mathbb{R}^{N\times N}$ of zeros and ones as follows:
\begin{align*}
	\diag(S)_{ii}:=\begin{cases} 1 & \text{ if } i \in S \\
              0 & \text{ otherwise }
	               \end{cases}.
\end{align*}
The matrix $\diag(S)$ represents a hyperplane arrangement, one for each $S \in \mathcal{S}$. Let $P = |\mathcal{S}|$ be the number of such hyperplane arrangements. We enumerate them to form ${D_i}_{i=1}^P = \{ \diag(S): S \in \mathcal{S} \}$. The number of arrangements can be bounded more tightly by,
\begin{align*}
	P\le 2 \sum_{k=0}^{r-1} {n-1 \choose k}\le 2r\left(\frac{e(n-1)}{r}\right)^r,
\end{align*}
where $r:=\mbox{rank}(X)\leq \min(N,d)$ \cite{cover1965geometrical, stanley2004introduction}.


Although the problem in \eqref{eq:background_relu_bidual} is convex and therefore eliminates several optimization related issues attributed to the nonconvexity of \eqref{eq:background_relu}, it still requires exhaustive enumeration of hyperplane arrangement matrices $\{D_i\}_{i=1}^P$. Thus, \eqref{eq:background_relu_bidual} is usually a high dimensional convex optimization constraints with a prohibitively large number of constraints. This issue precludes application of the convex approach to practical scenarios. Alternatively, problem \eqref{eq:background_relu} must be approximated by subsampling the hyperplane arrangements.

As a follow-up work, \cite{ergen2023globally} adapted a similar convex duality approach to neural networks with threshold activations and proved that \eqref{eq:background_relu} can be, equivalently cast as the following LASSO problem
\begin{align}\label{eq:background_threshold_bidual}
	\min_{w } \frac{1}{2}\|Dw-y\|_2^2+\beta\|w\|_1,
\end{align}
where $D \in \{0,1\}^{N\times P}$ is the matrix of all possible hyperplane arrangements. In other words, the diagonal entries of $\{D_i\}_{i=1}^P$ in \eqref{eq:background_relu_bidual} corresponds to the columns of $D$ in \eqref{eq:background_threshold_bidual}. Although modifying the activations as threshold function simplifies the training problem \eqref{eq:background_threshold_bidual} as a standard unconstrained Lasso problem, computing the $D$ matrix still requires an exhaustive search over all subsets of the data to determine valid hyperplane arrangement patterns. Therefore, the equivalent convex problems proposed in \cite{pilanci2020neural,ergen2023globally} may not be suitable to provide a complete description of the optimal solutions as a result of the training process in general.

However, for low dimensional data, we show that there is no need to perform an exhaustive search over all data subsets to form the hyperplane arrangements in $D$. In particular, we introduce a novel convex analytic approach to describe and understand the optimal solutions of low dimensional datasets using a fixed size dictionary matrix. Additionally, we extend the Lasso formulation from threshold activations to other activations such as ReLU and absolute value.



==> unused/extra2DinputReLUfeatetc.tex <==

\section{extra analysis for absolute value number of features}
%SCRATCH
For $x\geq2$, let $z(x)=x-1$ and $k(x)=x+z(x)=2x-1$ be the maximum number of zeros; and \kink{}s after passing through an activation; respectively, of a piecewise linear function with $x$ \kink{}s and which has constant value beyond the outermost \kink{}s.

%don't count until get to final layer b
First, for $l=1$,

\[\xl{L}_n\left(\bl{L-1}\right)= \sigma \left( \mathbf{X}_n^{(L-1)} \wl{L-1} + \bl{L-1}\right).\]

Then $\left|\mathcal{K}\left(\xl{L}_n\left(\bl{L-1}\right)\right) \right| = 1 = l$. Namely, $\mathcal{K}\left(\xl{L}_n\left(\bl{L-1}\right)\right) = -\xl{L-1}_{n}\wl{L-1}$. So $\xl{L}_n(\bl{L-1})$ has $l$ \kink{}, $l$ of which are of the form $-\xl{L-1}_{i}\wl{L-1}.$ So \\
$\mathcal{K} \left( \sum_{n=1}^N \lambda_n \left(\xl{L}_n\left(\bl{L-1}\right)\right) \right) \subset \left\{ -\xl{L-1}_{n^{(L-1)}}\wl{L-1}:n^{(L-1)} \in [N]   \right\}$. Fix $n^{(L-1)} \in [N]$. Plugging in $\bl{L-1}=-\xl{L-1}_{n^{(L-1)}} \wl{L-1}$ gives for $l=2$,


%Note 
%$\xl{L}\left(\bl{L-1}\right)= \sigma \left( \mathbf{X}^{(L-1)}_n \wl{L-1} +b^{(L-1)}\right)$ has one $\sigma$ and therefore has $1$ kink which happens to be its zero. Plugging this in gives 

\[\xl{L}_n\left(\bl{L-2}\right)=\sigma \left( \Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\cdot \wl{L{-}1}\right)\]

where

\[\Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)=\sigma \left( \mathbf{X}^{(L{-}2)}_n \wl{L{-}2}{+} \bl{L{-}2}\right)-\sigma \left( {\mathbf{X}^{(L{-}2)}_{n^{(L{-}1)}}} \wl{L{-}2}  {+} \bl{L{-}2}\right).\]

Then $\left| \mathcal{K}\left( \Tilde{\xl{L-1}}\left(\bl{L-2}\right)\right)\right|=2=l$. Namely, \\ $\mathcal{K}\left( \Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\right) = \left\{ -\xl{L-2}_{n}\wl{L-2},   -\xl{L-2}_{n^{(L-1)}}\wl{L-2}\right\}$.  %So  \\
%$-\xl{L-2}_{n^{(L-2)}}\wl{L-2} \in \arg \max_{\bl{L-2}} \left| \sum_{n=1}^N \lambda_n \left(\xl{L}_n\left(\bl{L-2}\right)\right) \right| $ for some $n^{(L-2)} \in [N]$. 
%
%Observe $\Tilde{\xl{L-1}}\left(\bl{L-2}\right)$ has $2$ \kink{}s, which are of the same form $\xl{L}_{n^{(L-2)}}$. 
Also, \\ $\lim_{\bl{L-2} \to \infty} \Tilde{\xl{L-1}_n}\left(\bl{L-2}\right) = -\lim_{\bl{L-2} \to -\infty} \Tilde{\xl{L-1}_n}\left(\bl{L-2}\right) \in (-\infty,\infty)$. So \\ $\left|\mathcal{Z}\left( \Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\right) \right| =  
\left \lfloor \left| \mathcal{K}\left( \Tilde{\xl{L-1}}\left(\bl{L-2}\right)\right)\right|-1 \right \rfloor_{odd} = l-1= 1$. Namely, \\ $\mathcal{Z}
\left(\Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\right)=\left\{-\midpt{\xl{L-2}_n\wl{L-2}}{\xl{L-2}_{n^{(L-1)}}\wl{L-2}}\right\}$.
So $\xl{L}_n(\bl{L-2})$ has \\
$ \left| \mathcal{K}\left( \Tilde{\xl{L-1}}\left(\bl{L-2}\right)\right)\right|+\left| \mathcal{Z}\left( \Tilde{\xl{L-1}}\left(\bl{L-2}\right)\right)\right|=l+(l-1)=3$ \kink{}s, $l$ of which are of the form $-\xl{L-2}_i \wl{L-2}$.
Therefore for fixed $n^{(L-1)}\in [N]$, \\
$\mathcal{K} \left( \sum_{n=1}^N \lambda_n \left(\xl{L}_n\left(\bl{L-2}\right)\right) \right) {\subset} \left\{ -\xl{L{-}2}_{n^{(L{-}1)}}\wl{L{-}2}, \midpt{\xl{L{-}2}_n\wl{L{-}2}}{\xl{L{-}2}_{n^{(L{-}1)}}\wl{L{-}2}} :n^{(L{-}2)} \in [N]  \right\}.$ Fix $n^{(L-2)} \in [N]$.
%Observe that $\Tilde{\xl{L-1}}\left(\bl{L-2}\right)$ is of constant value beyond its (outer) \kink{}s, and therefore has at most $z\left(2\right)=1$ zero, which contributes another \kink{} of a different form to $\xl{L}\left(\bl{L-2}\right)$. So $\Tilde{\xl{L-1}}\left(\bl{L-2}\right)$ has at most $2$ forms of \kink{}s. 
%
Plugging in these \kink{} $\bl{L-2}$ for $l=3$ gives 

\[\Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)= \xl{L-1}_n\left(\bl{L-3}\right) - \xl{L-1}_{n^{(L-1)}}\left(\bl{L-3}\right)\]
%
where
\[\xl{L-1}\left(\bl{L-3}\right)=
\sigma\left( \Tilde{\xl{L-2}} \left( \bl{L-3} \right) \cdot \wl{L-2} \right)\]
%
where
%
\[\Tilde{\xl{L{-}2}}\left( \bl{L{-}3} \right){=}\sigma\left(\xl{L-3}\wl{L-3}{+}\bl{L-3} \right) {-} \sigma\left( \xl{L-3}_{n^{(L-2)}}\wl{L-3}{+}\bl{L-3}\right)\] 
%
or
%
\[\Tilde{\xl{L{-}2}}\left( \bl{L{-}3} \right){=}\sigma\left(\xl{L-3}\wl{L-3}{+}\bl{L{-}3} \right) {-} \frac{\sigma\left( \xl{L{-}3}_{n^{(L{-}2)}}\wl{L{-}3}{+}\bl{L-3}\right) {+} \sigma\left( \xl{L{-}3}_{{n^{(L{-}1)}}}\wl{L{-}3}{+}\bl{L{-}3}\right)}{2}.\] 

Then $\left|\mathcal{K}\left(\Tilde{\xl{L-2}_n}\left( \bl{L-3}\right) \right) \right| \in \{l-2,3\},\left|\mathcal{K}\left(\Tilde{\xl{L-2}}_{n^{(L-1)}}\left( \bl{L-3}\right) \right) \right| =2$. So \\ $\left|\mathcal{K}\left(\Tilde{\xl{L-2}}\left( \bl{L-3}\right) \right) \right| \leq 3=l$. Also, \\ $\lim_{\bl{L-3} \to \infty} \Tilde{\xl{L-2}}\left(\bl{L-3}\right) = -\lim_{\bl{L-3} \to -\infty} \Tilde{\xl{L-2}}\left(\bl{L-3}\right) \in (-\infty,\infty)$. So \\ $\left|\mathcal{Z}\left(\Tilde{\xl{L-2}}\left( \bl{L-3}\right) \right) \right| =\left \lfloor  \left|\mathcal{K}\left(\Tilde{\xl{L-2}}\left( \bl{L-3}\right) \right) \right| -1 \right \rfloor_{odd} \leq \left \lfloor l -1\right \rfloor_{odd} = 1 $. 
%So $\left|\mathcal{K}\left(\xl{L-1}\left(\bl{L-3}\right)\right)\right|\in \{2+1,3+1\}=\{3,4\}$. 
%Also, \\ $\lim_{\bl{L-3} \to \infty} \Tilde{\xl{L-1}_n}\left(\bl{L-3}\right) = \lim_{\bl{L-3} \to -\infty} \Tilde{\xl{L-1}_{n^{(L-1)}}}\left(\bl{L-3}\right) \in (-\infty,\infty)$. 
So \\ $\left| \mathcal{K}\left(\Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\right) \right| \leq l + 2\left|\mathcal{Z}\left( \tilde{\xl{L-2}}\left(\bl{L-3}\right)\right)\right|= l + 2\lfloor l-1 \rfloor_{odd}=5$. Also, \\ $\lim_{\bl{L-3} \to \infty} \xl{L-1}_n\left(\bl{L-3}\right) = \lim_{\bl{L-3} \to -\infty} \xl{L-1}_{n^{(L-1)}}\left(\bl{L-3}\right) \in (-\infty,\infty)$. So \\$\left|\mathcal{Z}\left(\xl{L}_n\left(\bl{L-2}\right)\right)\right|\leq \left \lfloor \left| \mathcal{K}\left(\Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\right) \right|-1 \right \rfloor_{even}= \left\lfloor l+ 2\lfloor l-1 \rfloor_{odd}-1 \right\rfloor_{even} = 4$. So $\left| \mathcal{K}\left(\xl{L}\left(\bl{L-3}\right)\right)\right|\leq \left| \mathcal{K}\left(\Tilde{\xl{L-1}_n}\left(\bl{L-2}\right)\right) \right| + \left| \mathcal{Z}\left(\xl{L}_n\left(\bl{L-2}\right)\right)\right| = l+ 2\lfloor l-1 \rfloor_{odd} + \left\lfloor l+ 2\lfloor l-1 \rfloor_{odd}-1 \right\rfloor_{even}  = 9$.

So there are at most $9$ optimal $\bl{L-3}$, of which $2\left|\mathcal{Z}\left( \tilde{\xl{L-2}}\left(\bl{L-3}\right)\right)\right|+\left| \mathcal{Z}\left(\xl{L}_n\left(\bl{L-2}\right)\right)\right|=6$ are linear combinations of $\xl{L-3}_n,\xl{L-3}_{n^{(L-1)}},\xl{L-3}_{n^{(L-2)}}$ and $3$ are just $\xl{L-3}_n,\xl{L-3}_{n^{(L-1)}},\xl{L-3}_{n^{(L-2)}}$. Since there were two options for $\bl{L-2}$, the number of linear combinations is doubled. In the next layer, 

Count the number of zeros created. This plus the number of $\xl{L-l}$;s ie $l+1$ is the number of \kink{}s. And each zero consists of $l+1$ $\xl{L-l}$'s.

Observe in the first case, $\Tilde{\xl{L{-}2}}_n\left( \bl{L-3} \right)$ and $\Tilde{\xl{L{-}2}}_{n^{(L-1)}}\left( \bl{L-3} \right)$ each have $2$ \kink{}s. In the second case, $\Tilde{\xl{L{-}2}}_n\left( \bl{L-3} \right)$  and $\Tilde{\xl{L{-}2}}_{n^{(L-1)}}\left( \bl{L-3} \right)$ have $2$ and $3$ \kink{}s. Now, we use the same argument as above. In all cases, the \kink{}s of $\Tilde{\xl{L{-}2}}\left( \bl{L-3} \right)$ are all of the same form $\xl{L-3}_{n^{(L-3)}}$, and $\Tilde{\xl{L{-}2}}\left( \bl{L-3} \right)$ is constant after its outermost \kink{}s. In the first case, $\xl{L-1}_n\left( \bl{L-3}\right)$ and $\xl{L-1}_{n^{(L-1)}}\left( \bl{L-3}\right)$ each have at most $z(2)=1$ zero but of the same \midptname{} form, so $\Tilde{\xl{L-1}}\left(\bl{L-2}\right)$ has at most $2(2+z(2))=6$ \kink{}s. However the \kink{} $-\xl{L-3}_{n^{(L-2)}}\wl{L-3}$ is shared between $\xl{L-1}_n$ and $\xl{L-1}_{n^{(L-1)}}$, so $\Tilde{\xl{L-1}}\left(\bl{L-2}\right)$ has at most $2(2+z(2))-1=5$ \kink{}s. It can be seen that $\Tilde{\xl{L-1}}\left(\bl{L-2}\right)$ is constant beyond its outer \kink{}s, so $\xl{L}\left(b^{(L-3)}\right)$ has $k(2(2+z(2))-2)=9$ \kink{}s. These are $9$ new \kink{} forms. 

In the second case, 

\begin{equation}
    \begin{aligned}
        \left| \left|\left| \xl{L-3}_n + \bl{L-3}\right| - \left| \xl{L-3}_{n^{(L-2)}} + \bl{L-3}\right| \right| - \left| \left| \xl{L-3}_{n^{(L-1)}} + \bl{L-3}\right| - \left| \xl{L-3}_{n^{(L-2)}} + \bl{L-3}\right| \right| \right|
    \end{aligned}
\end{equation}



For each component of $\bl{L-2}$, the innnermost argument linear combination has $2$ $\sigma$'s and therefore $k=2$ kinks (however they are of the same form). How many zeros does the innermost argument have? An unbounded piecewise linear function with $k_0=2$ kinks, if it is monotone, has exactly one zero, and otherwise has at most $k_0+1=3$ zeros. (For absolute value, $2$ of the zeros and kinks are the same, so there is just one extra $b^{(L-2)}$ to consider. And for ReLU, the zero and the kink are shared, so there are no extra $b^{(L-2)}$ to consider). The zeros of any layer are the kinks of the next outer layer. Suppose one neuron per layer, so zeros are a function of just one variable (and therefore finite number of them.) Therefore the second innermost layer (in this case the outer layer) has at most $k_0+1=3$ kinks. Therefore the total number of possible $b^{(L-1)}$ to consider is for non-monotone, $k+(k+1)$. Now, $b^{(L-2)}$ can either be of the form $\xl{L-2}_i$ if it came from a kink of the innermost layer, or a linear combination of $\xl{L-2}_n, \xl{L-2}_{n^{(L-1)}}$ if it came from a zero (kink of the next layer). However $2$ of those cases overlap. In the former case,


In the non-monotone case there are $2$ forms of $b^{(L-2)}$, either being another $\xl{(L-2)}_i$ or a linear combination of them. Plugging in the usual $b^{(L-2)}$ gives $2$ kinks in each of the $2$ innermost layers and hence $3$ kinks in each of their next layers (but so far, just $3$ types: the usual and the average). When $k_0=2$ $k_0+1=3$-kink functions are added, this is  $k_0(k_0+1)=6$ kinks and hence $k_0(k_0+1)+1=7$ zeros in the outermost layer. Some of these zeros are shared with the zeros of the previous layer. Each time, only one new type of $b$ is created, when both $\sigma$'s are active - no, that does not need to be the case, need to check if sol is valid.
But plugging in the non-usual average $b^{(L-2)}$ gives $3$ $\sigma$'s in the innermost layer, which is $3$ kinks. 

The non-monotone difference of $2$ $\sigma$'s, with the same variable $b$ and coefficient in front of $b$, has $2$ kinks however the graph is flat beyond the first and last kink, so there is only one zero. $k_0+1$ is the total number of possible zeros. This is why only $z_1=(k_0+1)-2=1$ one zero and hence additional kink is created from the next outer layer, so the total number of kinks in the next outer layer is $k_0+z_1=k_0+1=3$. When these $k_0+1$ are then subtracted, again $b$ beyond the first and last kink is constant, so the number of zeros and hence new kinks is at most $2(k_0+((k_0+1)-2))-2=2*3-2=4$. Are any of these the same form? Ignoring same form in the later layers, we get the total number of types is $1+1+4=6$. I think actually the first 2 and last 2 kinks will not be kinks and flat.
%
If the average is used, then still flat at ends. So for $k_0'=3$ (from the average contributing $k_0+1=2$ extra b's), $z_1' = k_0'+1-2=k_0'-1=k_0=2$ zeros and hence extra kinks are in the next outer layer. So the total number of kinks in the next layer is  $k_0'+z_1'=2k_0+1=5$. When these $2k_0+1$ functions are then subtracted, the endpoints are still flat, so the number of zeros and hence new kinks is at most $2*5-2=8$. Ignoring same form in the later layers, we get the total number of types is $2+2+8=12$.

Todo: show flatness, and then subtract that from number of zeros in each layer, which is the number of new kinks (I think these don't overlap with previous kinks since they will be like the averages). Add up total number of zeros in each layer for total number of kinks caused by $b$ of that depth.
\section{3 layer, 1D ReLU NN}


\begin{definition}
    Let 
    \begin{equation*}
        \begin{aligned}
            \hill_{a,b}(x)=
            \begin{cases}
                0 &\mbox{ if } x \leq a \\
                2(x-a) &\mbox{ if } a \leq x \leq b \\
                x + b-2a &\mbox{ else }
            \end{cases}
        \end{aligned}
    \end{equation*}
\end{definition}

\begin{lemma}\label{lemma:relucombo}
For $\sigma(x)=(x)_+$ and $a,b \in \mathbb{R}$,
    \begin{equation*}
        \begin{aligned}
            \sigma(\sigma(x-a)-\sigma(b-x)) = 
            \begin{cases}
                \relu{+}{a}(x)&\mbox{ if } a \geq b \\
                \hill_{\frac{a+b}{2},b}(x) &\mbox{ else }
            \end{cases}
        \end{aligned}
    \end{equation*}
    %
    %And if  $a \geq b$, $\sigma(\sigma(x-a)-\sigma(b-x))=\relu{+}{a}(x)$.
    In particular, $ \sigma(\sigma(x-a)-\sigma(b-x))$ has a \kink{} at $\max\{a,b\}$.
\end{lemma}

\begin{proof}
    If $a\leq b$,
\begin{equation*}
    \begin{aligned}
        \sigma(x-a)-\sigma(b-x)&=
        \begin{cases}
            x-b &\mbox { if } x \leq a \\
            2x-a-b &\mbox{ if } a \leq x \leq b \\
            x-a &\mbox{ else}, 
        \end{cases}
    \end{aligned}
\end{equation*}
%
which is monotone nondecreasing and is zero exactly when $x = \frac{a+b}{2}$, so
\begin{equation*}
    \begin{aligned}
        \sigma(\sigma(x-a)-\sigma(b-x))&=
        \begin{cases}
                0 &\mbox{ if } x \leq \frac{a+b}{2} \\
                2x-a-b &\mbox{ if } \frac{a+b}{2} \leq x \leq b \\
            x-a &\mbox{ else}.
        \end{cases}
    \end{aligned}
    \end{equation*}
%
If $a \geq b$,
%
\begin{equation*}
    \begin{aligned}
        \sigma(x-a)-\sigma(b-x)&=
        \begin{cases}
            x-b \leq 0 &\mbox { if } x \leq b \\
            0 &\mbox{ if } b \leq x \leq a \\
            x-a \geq 0 &\mbox{ else}, \\
        \end{cases}
    \end{aligned}
\end{equation*}
so the result follows.
\end{proof}


Suppose $L=3, \Wul{i}{1} = \left(w^{(i,1)},\tilde{w}^{(i,1)}\right),  \Wul{i}{2} = \left(w^{(i,2)},\tilde{w}^{(i,2)}\right)^T, \bul{i}{1}=\left(b^{(i,1)},\tilde{b}^{(i,1)}\right), \bul{i}{2}=\left(b^{(i,2)}\right)$, where $w^{(i,1)},\tilde{w}^{(i,1)},w^{(i,2)},\tilde{w}^{(i,2)},b^{(i,1)},\tilde{b}^{(i,1)},b^{(i,2)},\tilde{b}^{(i,2)}\in\mathbb{R}$ . So, the neural network is

\begin{equation*}
    \nn{3}{\mathbf{x}} = \sum_{i=1}^m \sigma \left( \sigma \left( \mathbf{x} w^{(i,1)}+ b^{(i,1)}\right) w^{(i,2)}+ \sigma \left( \mathbf{x} \tilde{w^{(i,1)}}+ \tilde{b}^{(i,1)}{1}\right)\tilde{w}^{(i,2)} +b^{(i,2)}\right)\alpha_i + \xi.
\end{equation*}

Let the regularization be $l_2$ norm: $\regfunc_{(i,l)}\left(\Wul{i}{1}\right)=\left\|\Wul{i}{1}\right\|_2 = \sqrt{(w^{(i,1)})^2+(\tilde{w}^{(i,1)})^2}$ for $l < L$ and $\regfunc_{(i,L)}\left(\Wul{i}{L}\right)=\left| \Wul{i}{L}\right|$. So, the training problem is

\begin{equation*}
    \min_{\theta \in \Theta} \mathcal{L}_y \left(\nn{3}{\mathbf{X}} \right) + \frac{\beta}{3} \sum_{i=1}^{m_3}\left( \left|\alpha_i\right|^3_1 + \left \| \left(w^{(i,1)}, \tilde{w}^{(i,1)}\right)\right\|_{2}^3  + \left \| \left(w^{(i,2)}, \tilde{w}^{(i,2)}\right)\right\|_{2}^3 \right).
\end{equation*}

Then the rescaled problem \eqref{eq:gen_rescaled} is 

% The training problem is equivalent to the rescaled problem 

    \begin{equation*}
    \min_{\theta \in \Theta:  \left(w^{(i,l)}\right)^2+\left(\tilde{w}^{(i,l)}\right)^2=1: l < L} \mathcal{L}_y \left(\nn{3}{\mathbf{X}} \right) + \beta \sum_{i=1}^{m_3}\left|\alpha_i\right|_1,
    \end{equation*}

\textbf{Assume} For $l<L=3$, let $|w^{(i,l)}|=|\tilde{w}^{(i,l)}|$ in the original training problem. 
Then replacing ${w^{(i,l)}}' = \sqrt{2} w^{(i,l)}, \alpha' = \frac{1}{2}\alpha, {b^{(i,1)}}'=\sqrt{2}b^{(i,1)},  {b^{(i,2)}}'=2b^{(i,1)},\beta' = \frac{\beta}{2}$ and then renaming back, the rescaled problem is equivalent to

    \begin{equation*}
    \min_{\theta \in \Theta:  \left | w^{(i,1) } \right|= \left | w^{(i,2) } \right|= \left | \tilde{w}^{(i,1) } \right|= \left | \tilde{w}^{(i,2) } \right|=1} \mathcal{L}_y \left(\nn{3}{\mathbf{X}} \right) + \beta' \sum_{i=1}^{m_3}\left|\alpha_i\right|_1.
    \end{equation*}


%\begin{equation*}
%    \min_{\theta \in \Theta} \mathcal{L}_y \left(\nn{3}{\mathbf{X}} \right) + \frac{\beta}{3} \sum_{i=1}^{m_3}\left( \left|\alpha_i\right|^3_1 + \left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{2}^3  + \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{2}^3 \right).
%\end{equation*}

%\begin{lemma}
%    The training problem is equivalent to the rescaled problem 

%    \begin{equation*}
%    \min_{\theta \in \Theta: \left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}= \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}=1} \mathcal{L}_y \left(\nn{3}{\mathbf{X}} \right) + \beta \sum_{i=1}^{m_3}\left|\alpha_i\right|_1 .
%\end{equation*}
%\end{lemma}

%\begin{proof}


%By the AM-GM inequality, $\frac{\beta}{3} \sum_{i=1}^{m_3}\left( \left|\alpha_i\right|^3_1 + \left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}^3  + \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}^3 \right) \geq \beta \sum_{i=1}^{m_3} \left|\alpha_i\right|_1 \left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}  \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty} $. So a lower bound is

%\begin{equation}\label{eq:rescaled}
%    \min_{\theta \in \Theta} \mathcal{L}_y \left(\nn{3}{\mathbf{X}} \right) + \frac{\beta}{3} \sum_{i=1}^{m_3}  \left|\alpha_i\right|  \left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}   \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}.
%\end{equation}

%By rescaling $\Wul{i}{l}$ by $\left \| \left(\Wul{1}{l}, \tWul{i}{l}\right)\right\|_{\infty}$, and $\alpha_i$ by $\left \| \left(\Wul{1}{1}, \tWul{i}{1}\right)\right\|_{\infty}\left \| \left(\Wul{1}{2}, \tWul{i}{2}\right)\right\|_{\infty}$, \eqref{eq:rescaled} remains equivalent with the constraint that $\left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}= \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}=1$. Finally, the lower bound \eqref{eq:rescaled} meets the training problem with equality by scaling $|\alpha_i|^{\frac{1}{3}}$ to the weights.

%and equality is achieved when $\left| \alpha_i \right| = \left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}=\left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}$.

%By rescaling $\bul{i}{l},\tbul{i}{l}$, the neural net in the training problem \eqref{eq:rescaled} is equivalent to 

%\begin{equation*}
%\begin{aligned}
%    \nn{3}{\mathbf{X}} &= \sum_{i=1}^m \sigma \left( \sigma \left( \mathbf{X} \frac{\Wul{i}{1}}{\left \| \left(\Wul{1}{1}, \tWul{i}{1}\right)\right\|_{\infty}} + \bul{i}{1}\right) 
%    \frac{\Wul{i}{2}}{\left \| \left(\Wul{i}{2}, \tWul{i}{1}\right)\right\|_{\infty}} \right. \\
%    &+ \sigma \left( \mathbf{X} \frac{\Wul{i}{1}}{\left \| \left(\Wul{1}{1}, \tWul{i}{1}\right)\right\|_{\infty}}+\tbul{i}{1}\right) \frac{\Wul{i}{2}}{\left \| \left(\Wul{i}{2}, \tWul{i}{1}\right)\right\|_{\infty}} 
%    \Bigg)\\
%    & \cdot \alpha_i\left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty} \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}+ \xi
%\end{aligned}
%\end{equation*}

%So in the training problem \eqref{eq:rescaled} , the neural net is equivalent to 

%\begin{equation*}
%\begin{aligned}
%    \nn{3}{\mathbf{X}} &= \sum_{i=1}^m \sigma \left( \sigma \left( \mathbf{X} \Wul{i}{1}+ \bul{i}{1}\right) 
%    \Wul{i}{2} \right. \\
%    &+ \sigma \left( \mathbf{X}\Wul{i}{1} +\tbul{i}{1}\right)\Wul{i}{2} 
%    \Bigg)\\
%    & \cdot \alpha_i\left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty} \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}+ \xi
%\end{aligned}
%\end{equation*}

%with the constraint that $\left \| \left(\Wul{i}{1}, \tWul{i}{1}\right)\right\|_{\infty}= \left \| \left(\Wul{i}{2}, \tWul{i}{2}\right)\right\|_{\infty}=1$
    
%\end{proof}

\textbf{With second layer bias:}

The dual of the rescaled problem is \eqref{gen_parallel_dual}, where

\begin{equation*}
    \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(x_n w^{(1)} + b^{(1)}\right)w^{(2)} + \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)\Tilde{w}^{(2) }+b^{(2)}\right).
\end{equation*}

As a function of $b^{(2)}$, $\mathbf{X}^{(3)}_n$ has a \kink{} when $b^{(2)}=-\sigma \left(x_n w^{(1)} + b^{(1)}\right)w^{(2)} - \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)\Tilde{w}^{(2) }$. Plugging in $b^{(2)}$ gives 

\begin{equation*}
\begin{aligned}
    \mathbf{X}^{(3)}_n &{=}\sigma \left( \left( \sigma \left(x_n w^{(1)} {+} b^{(1)}\right)-\sigma\left(x_i w^{(1)} {+} b^{(1)} \right) \right) w^{(2)} {+} \left( \sigma\left(x_n \tilde{w}^{(1)}{+}\tilde{b}^{(1)} \right) {-} \sigma\left(x_i \tilde{w}^{(1)}{+}\tilde{b}^{(1)} \right) \right) \Tilde{w}^{(2)}\right)\\
    &{=} \sigma \left( w^{(2)} \text{sign}\left((x_n{-}x_i)w^{(1)}\right)\ramp{+}{{-}\max \left\{x_n w^{(1)}, x_i w^{(1)} \right\}}{{-}\min \left\{x_i w^{(1)}, x_n w^{(1)} \right\}}\left(b^{(1)} \right) \right. \\
    & \quad {+}\tilde{w}^{(2)}\text{sign}\left((x_n{-}x_i)\tilde{w}^{(1)}\right)  
    \ramp{+}{{-}\max \left\{x_n \tilde{w}^{(1)}, x_i \tilde{w}^{(1)} \right\}}{{-}\min \left\{x_i \tilde{w}^{(1)}, x_n \tilde{w}^{(1)} \right\}} \left(\tilde{b}^{(1)}\right)\Big),
\end{aligned}
\end{equation*}

which is monotone in $b^{(1)}$ and monotone in $\tilde{b}^{(1)}$. Since \rampname{}s have constant value outside of their \kink{}s, $\mathbf{X}^{(3)}_n $ has \kink{}s there, hence at $b^{(1)} \in \left \{-x_n w^{(1)}, -x_i w^{(1)}
 \right \}$ and  $\tilde{b}^{(1)} \in \left\{-x_n \tilde{w}^{(1)}, -x_i \tilde{w}^{(1)}\right\}$. Plugging this in gives features 

 \begin{equation*}
     \begin{aligned}
          \sigma \left( \left( \sigma \left((x {-} x_j) w^{(1)} \right)-\sigma\left((x_i-x_j) w^{(1)}  \right) \right) w^{(2)} {+} \left( \sigma\left((x-x_k) \tilde{w}^{(1)} \right) {-} \sigma\left( (x_i -x_k) \tilde{w}^{(1)}\right) \right) \Tilde{w}^{(2)}\right)\\
     \end{aligned}
 \end{equation*}

  By symmetry, the set of features generated by $w^{(2)}=1=-\tilde{w}^{(2)}$ and  $w^{(2)}=-1=-\tilde{w}^{(2)}$ are the same.
 The set of features generated by negating both  $w^{(1)}$ and $\tilde{w}^{(1)}$ are the same but reflected, ie opposite monotonicity. %I think?
 Therefore it suffices to find the following cases:

\textbf{Case 0}: If $-w^{(2)} =-\tilde{w}^{(2)}= w^{(1)} = \tilde{w}^{(1)}$ then the feature are 

\begin{equation*}
    \begin{aligned}
        \sigma \left( \sigma\left(x_i-x_j   \right) {+}   \sigma\left( x_i -x_k \right) - \sigma \left(x {-} x_j  \right) -\sigma\left(x-x_k \right)  \right)
    \end{aligned}
\end{equation*}

\textbf{Case 0}: If $-w^{(2)} =-\tilde{w}^{(2)}= w^{(1)} = -\tilde{w}^{(1)}$ then the feature are

\begin{equation*}
    \begin{aligned}
        \sigma \left( \sigma\left(x_i-x_j   \right) {+}   \sigma\left( x_i -x_k \right) - \sigma \left(x {-} x_j  \right) -\sigma\left(x_k -x \right)  \right)
    \end{aligned}
\end{equation*}

\textbf{Case 1}: If $w^{(2)}=\tilde{w}^{(2)}=w^{(1)}=\tilde{w}^{(1)}=1$ the features are:

\begin{equation*}
    \begin{aligned}
        \sigma \left( \sigma \left(x  {-} x_j \right) {+} \sigma\left( x {-} x_k \right) {-} \sigma\left(x_i {-} x_j \right)   {-} \sigma\left(x_i  {-} x_k \right) \right) {=}
        \begin{cases}
            \hill_{x_j,x_k}(x)&\mbox{ if } x_i = \min\{x_i,x_j,x_k\}\\
            \hill_{x_i,x_k}(x)&\mbox{ if } x_j < x_i < x_k \\
            \hill_{x_i,x_j}(x)&\mbox{ if } x_k < x_i < x_j \\
            2\relu{+}{x_i}(x)&\mbox{ if } x_i = \max\{x_i,x_j,x_k\}
        \end{cases}
    \end{aligned}
\end{equation*}



\textbf{Case 2}: If $w^{(2)}=-\tilde{w}^{(2)}=w^{(1)}=\tilde{w}^{(1)}=1$
the features are: %ramps are in order indices

\begin{equation*}
    \begin{aligned}
        \sigma \left( \sigma \left(x  {-} x_j \right) {-} \sigma\left( x {-} x_k \right) {-} \sigma\left(x_i {-} x_j \right)   {+} \sigma\left(x_i  {-} x_k \right) \right) {=}
        \begin{cases}
            \ramp{+}{\min\{x_j,x_k\}}{\max\{x_j,x_k\}}(x)&\mbox{ if } x_i {=} \min\{x_i,x_j,x_k\}\\
            \ramp{+}{x_i}{x_k}(x)&\mbox{ if } x_j {<} x_i {<} x_k \\
            \ramp{-}{x_k}{x_i}(x)&\mbox{ if } x_k {<} x_i {<} x_j \\
           \ramp{-}{\min\{x_j,x_k\}}{\max\{x_j,x_k\}}(x)&\mbox{ if } x_i {=} \max\{x_i,x_j,x_k\}
        \end{cases}
    \end{aligned}
\end{equation*}


\textbf{Case 3}: If $w^{(2)}=-\tilde{w}^{(2)}=w^{(1)}=-\tilde{w}^{(1)}=1$
the features are: %ramps are in order indices

\begin{equation*}
    \begin{aligned}
        &\sigma \left( \sigma \left(x  {-} x_j \right) {-} \sigma\left( x_k {-} x \right) {-} \sigma\left(x_i {-} x_j \right)   {+} \sigma\left(x_k  {-} x_i \right) \right) \\
        &{=} \begin{cases}
            s_{x_i < x_j < x_k}(x)&\mbox{ if } x_i < x_j < x_k \\
            t_{x_i < x_k < x_j }(x)&\mbox{ if } x_i < x_k < x_j \\
            \hill_{x_i < x_k}(x)&\mbox{ if } x_j < x_i < x_k \\
           % \relu{+}{x_j}&\mbox{ if } x_k < x_i < x_j \\
           %\relu{+}{x_i}(x)&\mbox{ if } x_j < x_k < x_i \\
           \relu{+}{\max\{x_j,x_i\}}(x)&\mbox{ else. } 
        \end{cases}
    \end{aligned}
\end{equation*}

%\begin{equation*}
 %       \mathbf{X}^{(3)}_n =\sigma \left( \sigma \left(x_n  + b^{(1)}\right)-\sigma\left(x_i + b^{(1)} \right)   +  \sigma\left(-x_n +\tilde{b}^{(1)} \right)- \sigma\left(-x_i +\tilde{b}^{(1)} \right)  \right)
%\end{equation*}

%If  $-x_n \geq -x_i$, ie $x_i \geq x_n$, then $\mathbf{X}^{(3)}_n=0$. So suppose $-x_n \leq -x_i$, ie $x_i \leq x_n$. Then $\sigma \left(x_n  + b^{(1)}\right)-\sigma\left(x_i + b^{(1)} \right) = \ramp{+}{-x_n}{-x_i}\left( b^{(1)}\right) \geq 0$ and $ \sigma\left(-x_n +\tilde{b}^{(1)} \right)- \sigma\left(-x_i +\tilde{b}^{(1)} \right) = \ramp{-}{x_i}{x_n} \left( \Tilde{b}^{(1)}\right) \geq 0$. So $\mathbf{X}^{(3)}_n = \ramp{+}{-x_n}{-x_i}\left( b^{(1)}\right) +\ramp{-}{x_i}{x_n} \left( \Tilde{b}^{(1)}\right)$.
%As a function of $b^{(1)}, \Tilde{b}^{(1)}$, $\mathbf{X}^{(3)}$ has \kink{}s at $b^{(1)} \in \{ -x_i,  -x_n\}, \tilde{b}^{(1)} \in \{ x_i,  x_n\}$. So for all $n$,

%\begin{equation*}
%    \mathbf{X}^{(3)}_n = \sigma\left(\sigma \left(x_n  - x_j \right)-\sigma\left(x_i - x_j \right)   +  \sigma\left(-x_n + x_k \right)- \sigma\left(-x_i + x_k \right) \right) .
%\end{equation*}
%

\textbf{Case 4}: If $w^{(2)}=\tilde{w}^{(2)}=w^{(1)}=-\tilde{w}^{(1)}=1$:

Note that $\sigma \left(x  - x_j \right) +  \sigma\left( x_k - x \right) = \text{wedge}_{x_j,x_k}(x)+\max\{0,x_k-x_j\}$.
Observe that 
\begin{equation*}
    \begin{aligned}
        \sigma \left(x  - x_j \right) +  \sigma\left( x_k - x \right) &= \text{wedge}_{x_j,x_k}(x)+\max\{0,x_k-x_j\} \\
        &= \begin{cases}
            \text{wedge}_{j < k}(x) + x_k-x_j&\mbox{ if } x_k > x_j \\
            \text{wedge}_{k < j}(x)&\mbox{ else.}
        \end{cases}
    \end{aligned}
\end{equation*}


%this is true but not necessary, reader can do
%Observe that 
%
%\begin{equation*}
%    \begin{aligned}
%        \sigma\left(x_i - x_j \right)   +\sigma\left(x_k -x_i  \right) &= 
%        \begin{cases}
%            x_k - x_i &\mbox{ if } x_i = \min\{x_i,x_j,x_k\}\\
%             x_k - x_j &\mbox{ if } x_j < x_i < x_k \\
%            0 &\mbox{ if } x_k < x_i < x_j \\
%            x_i - x_j  &\mbox{ if } x_i = \max\{x_i,x_j,x_k\}
%        \end{cases}\\
%        & \geq 0.
%    \end{aligned}
%\end{equation*}
%


So the features are 
%
\begin{equation*}
    \begin{aligned}
        &\sigma \left( \sigma \left(x  - x_j \right) +  \sigma\left( x_k - x \right) -\sigma\left(x_i - x_j \right)   - \sigma\left(x_k -x_i  \right) \right) \\
        &=\begin{cases}
            (\text{wedge}_{x_j < x_k}(x)+x_k-x_j)-(x_k-x_i) =  \text{wedge}_{x_j < x_k}(x)-(x_j-x_i) &\mbox{ if } x_i < x_j < x_k \\
            \text{wedge}_{x_k < x_j}(x)-(x_k-x_i) &\mbox{ if } x_i < x_k < x_j \\
            (\text{wedge}_{x_j<x_k}(x)+x_k-x_j)-(x_k-x_j)  &\mbox{ if } x_j < x_i < x_k \\
            (\text{wedge}_{x_j<x_k}(x)+x_k-x_j)-(x_i-x_j) =\text{wedge}_{x_j<x_k}(x)-(x_i-x_k)&\mbox{ if } x_j < x_k < x_i \\
            \text{wedge}_{x_k<x_j}(x) &\mbox{ if } x_k < x_i < x_j \\
            \text{wedge}_{x_k<x_j}(x)-(x_i-x_j)&\mbox{ if } x_k < x_j < x_i 
        \end{cases}\\
        &=
        \begin{cases}
            \text{wedge}_{x_i<x_k+x_j-x_i}(x) &\mbox{ if } x_i = \min\{x_i,x_j,x_k\}\\
            \text{wedge}_{x_k+x_j-x_i<x_i}(x) &\mbox{ if } x_i = \max\{x_i,x_j,x_k\}\\
            \text{wedge}_{x_j,x_k} &\mbox{ else. }
        \end{cases}
    \end{aligned}
\end{equation*}

%Note that if $x_k < x_j$, $x_i -x_j > 0$ and $x_k-x_i>0$ cannot both hold. Otherwise if $x_k > x_j$, then both hold. 



\textbf{Without second layer bias:}

The dual of the rescaled problem is \eqref{gen_parallel_dual}, where

\begin{equation*}
    \begin{aligned}
        \mathbf{X}^{(3)}_n &=\sigma \left(\sigma \left(x_n w^{(1)} + b^{(1)}\right)w^{(2)} + \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)\Tilde{w}^{(2) }\right) \\
        &= \sigma \left(w^{(2)}\relu{+}{-x_nw^{(1)}}\left(b^{(1)}\right) + \tilde{w}^{(2)}\relu{+}{-x_n\tilde{w}^{(1)}}\left( \tilde{b}^{(1)}\right)\right),
    \end{aligned}
\end{equation*}

which is monotone in $b^{(1)}$ and monotone in $\tilde{b}^{(1)}$. Therefore the \kink{}s are at the \kink{}s of $\relu{+}{-x_n w^{(1)}}\left(b^{(1)}\right), \relu{+}{-x_n\tilde{w}^{(1)}}\left( \tilde{b}^{(1)}\right)$ and hence $b^{(1)} = -x_n w^{(1)}, \tilde{b}^{(1)} = -x_n \tilde{w}^{(1)} $. Plugging this in gives features

\begin{equation*}
    \sigma \left(\sigma \left(\left(x - x_j \right) w^{(1)} \right)w^{(2)} + \sigma\left( \left(x -x_k \right) \tilde{w}^{(1)} \right)\Tilde{w}^{(2) }\right) = \sigma \left(w^{(2)} \relu{w^{(1)}}{x_j}(x)  + \tilde{w}^{(2)} \relu{\tilde{w}^{(1)}}{x_k}(x)\right)
\end{equation*}


We consider cases: \\

\textbf{Case 1}: If $w^{(2)} = -1=\tilde{w}^{(2)}$ then $\mathbf{X}^{(3)}_n=0$. \\

\textbf{Case 2}:
If $w^{(2)}=1=\tilde{w}^{(2)}$ then %$\mathbf{X}^{(3)}_n = \sigma \left(x_n w^{(1)} + b^{(1)}\right) + \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)$ as a function of 
%$b^{(1)}, \Tilde{b}^{(1)}$ has a \kink{} exactly when $b^{(1)}=-x_n w^{(1)}, \Tilde{b}^{(1)}=-x_n \tilde{w}^{(1)}$. Plugging in $b^{(1)}$ makes $\mathbf{X}^{(3)}_n=\sigma \left(\left( x_n -x_i \right)w^{(1)} \right) + \sigma\left(\left(x_n - x_j \right) \tilde{w}^{(1)} \right)$. So 
the features are 

\begin{equation*}
\begin{aligned}
        \sigma \left(\left( x -x_j \right)w^{(1)} \right) + \sigma\left(\left(x - x_k \right) \tilde{w}^{(1)} \right) &= 
        \begin{cases}
            \hill^{w^{(1)}}_{x_j,x_k}(x) & \mbox{ if } w^{(1)} = \Tilde{w}^{(1)}\\
            \text{wedge}_{x_j,x_k} + \max\{0,w^{(1)}(x_j-x_k)\} & \mbox{ else}. 
        \end{cases}
\end{aligned}
\end{equation*}

\textbf{Case 3}: By symmetry, the range of $\mathbf{X}^{(3)}_n$ is the same when $w^{(2)} = 1 = -\tilde{w}^{(2)}$ or $w^{(2)} = -1 = -\tilde{w}^{(2)}$. So without loss of generality suppose $w^{(2)} = 1 = -\tilde{w}^{(2)}$. Then 
%$
%    \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(x_n w^{(1)} + b^{(1)}\right) - \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)\right).
%$
%
%So as a function of $b^{(1)}$, $\mathbf{X}^{(3)}_n$ has \kink{}s when $b^{(1)}=-x_n w^{(1)} + \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)$. Plugging this in makes \\ 
%$
%    \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(\sigma\left(x_i \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)+(x_n  -x_i) w^{(1)} \right) - \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)\right).
%$
%If $\text{sign}(w^{(1)})=\text{sign}\left(\tilde{w}^{(1)}\right)$ then $\mathbf{X}^{(3)}_n$ has no dependence on and hence no \kink{}s as a function of $\tilde{b}^{(1)}$. 

%If $(x_n-x_i)w^{(1)} \leq 0$ then $  \sigma\left(\sigma\left(x_i \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)+(x_n  -x_i) w^{(1)} \right) \neq 0$ if only if $\tilde{b}^{(1)} \geq -x_n w^{(1)} + x_i w^{(1)} - x_i \tilde{w}^{(1)} = -x_n \tilde{w}^{(1)} + 2(x_i-x_n)w^{(1)} \geq -x_n \tilde{w}^{(1)}$, if and only if $\sigma(x_n\tilde{w}^{(1)}+\tilde{b}^{(1)}) \neq 0$, if and only if $\sigma \left(\sigma\left(x_i \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)+(x_n  -x_i) w^{(1)} \right) - \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right) = 2(x_n-x_i)w^{(1)} \leq 0$, if and only if $\mathbf{X}^{(3)}_n = 0$. So suppose $(x_n - x_i)w^{(1)} \geq 0$. Then $
%    \mathbf{X}^{(3)}_n = \sigma\left(x_i \tilde{w}^{(1)}+\tilde{b}^{(1)} \right)+(x_n  -x_i) w^{(1)}  - \sigma\left(x_n \tilde{w}^{(1)}+\tilde{b}^{(1)} \right) = \ramp{+}{-x_i\Tilde{w}^{(1)}}{-x_n\Tilde{w}^{(1)}}(\tilde{b}^{(1)})+(x_n-x_i)w^{(1)} \geq 0
%$
%and has \kink{}s at $\Tilde{b}^{(1)} \in \{-x_i\Tilde{w}^{(1)},-x_n\Tilde{w}^{(1)}\}$. Plugging this in makes for all $n \in [N]$,
%
%$
%    \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(\sigma\left((x_i -x_j )\tilde{w}^{(1)}\right)+(x_n  -x_i) w^{(1)} \right) - \sigma\left((x_n-x_j) \tilde{w}^{(1)}\right)\right).
%$
%
%So by \cref{lemma:relucombo}, 
the features are 
\begin{equation*}
    \begin{aligned}
%        &\sigma \left(\sigma \left((x  -x_i) w^{(1)}+\sigma\left((x_j -x_i ){w}^{(1)}\right) \right) - \sigma\left((x_j-x) {w}^{(1)}\right)\right) \\
%        &=
%        \begin{cases}
%            \sigma\left(\sigma \left(\left(x-\reflect{x_j}{x_i}\right)w^{(1)}\right) - \sigma((x_j-x)w^{(1)})\right) 
            %= 
            %\ramp{+}{\reflect{x_j}{x_i}}{x_j}(x)
%            &\mbox{ if } (x_j-x_i)w^{(1)} \geq 0 \\
            %\ramp{+}{x_j}{x_i}(x)
            %\sigma\left(\sigma\left((x-x_i)w^{(1)}\right) - \sigma\left((x_j-x)w^{(1)}\right)\right) 
%            &\mbox{ else }
%        \end{cases} \\
        &= \begin{cases}
            \hill^{w^{(1)}}_{x_j,x_k}(x) &\mbox{ if } (x_k-x_j)w^{(1)} \geq 0 \\
            \relu{w^{(1)}}{x_j}(x) &\mbox{ else}.
        \end{cases}
    \end{aligned}
\end{equation*}
%
%%%%%%%%%%%%%%%
%Additionally suppose $w^{(1)}=1=-\tilde{w}^{(1)}$. %Then 
%$
%    \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(  \sigma\left(\tilde{b}^{(1)} -x_i \right) + x_n  -x_i \right) - \sigma\left(\tilde{b}^{(1)} -x_n\right)\right).
%$
%%
%If $x_n \leq x_i$ then $\mathbf{X}^{(3)}_n=0$. So suppose $x_n \geq x_i$. Then $\mathbf{X}^{(3)}_n= \sigma\left(\tilde{b}^{(1)} -x_i \right) + x_n  -x_i   - \sigma\left(\tilde{b}^{(1)} -x_n\right) = \ramp{+}{x_i}{x_n}(\Tilde{b}^{(1)}) + x_n - x_i $ which has \kink{}s at $\tilde{b}^{(1)} \in \{x_n, x_i\}$. Plugging this in makes, for all $n$, \\
%$
%     \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(  \sigma\left(x_j-x_i \right) + x_n  -x_i \right) - \sigma\left(x_j -x_n\right)\right).
%$
%So by \cref{lemma:relucombo}, the features are 
%\begin{equation*}
%    \begin{aligned}
%        \sigma \left(\sigma \left( x + \sigma\left(x_j-x_i \right)  -x_i \right) - \sigma\left(x_j -x\right)\right) &=
%        \begin{cases}
%            \sigma\left(\sigma \left(x-\reflect{x_j}{x_i}\right) - \sigma(x_j-x)\right) 
%            %= 
%            %\ramp{+}{\reflect{x_j}{x_i}}{x_j}(x)
%            &\mbox{ if } x_j \geq x_i \\
 %           %\ramp{+}{x_j}{x_i}(x)
 %           \sigma\left(\sigma\left(x-x_i\right) - \sigma\left(x_j-x\right)\right) 
%            &\mbox{ else }
%        \end{cases} \\
%        &= \begin{cases}
%            \hill_{x_i<x_j}(x) &\mbox{ if } x_j \geq x_i \\
%            \relu{+}{x_i}(x) &\mbox{ else}.
%        \end{cases}
%    \end{aligned}
%\end{equation*}
%

%$\mathbf{X}^{(3)}_n=0\relu{+}%{\reflect{x_n}{x_i}}(\Tilde{b}^{(1)})$  which has \kink{}s at $\tilde{b}^{(1)} = \reflect{x_n}{x_i}$. Plugging this in makes 
%$
%    \mathbf{X}^{(3)}_n =\sigma \left(\sigma \left(  \sigma\left(\reflect{x_j}{x_i} -x_i \right) + x_n  -x_i \right) - \sigma\left(\reflect{x_j}{x_i} -x_n\right)\right).
%$
%So by \cref{lemma:relucombo}, the features are 
%\begin{equation*}
%    \begin{aligned}
%        \sigma \left(\sigma \left(  x{+}\sigma\left(\reflect{x_j}{x_i} {-}x_i \right)  {-}x_i \right) {-} \sigma\left(\reflect{x_j}{x_i} {-}x\right)\right) &=
%        \begin{cases}
%            \sigma\left(\sigma(x{-}x_i)-\sigma\left(\reflect{x_j}{x_i} {-}x\right) \right)
%            %=0
%            &\mbox{ if } x_j \geq x_i \\
%             \sigma \left(\sigma(x{-}x_j)-\sigma\left(\reflect{x_j}{x_i}{-}x \right)\right)&\mbox{ else }
%        \end{cases} \\
%        &= \begin{cases}
%            \relu{+}{x_i}(x) &\mbox{ if } x_j \geq x_i \\
%            \hill_{x_i,\reflect{x_j}{x_i}}(x) &\mbox{ else }.
%        \end{cases}
%    \end{aligned}
%\end{equation*}




\section{4 layers with $d$ dimensional input}

%%%%%%%%%
Consider the $4$-layer deep narrow ReLU 
%or absolute value
network with training samples of dimension $d \geq 1$.
%There is one neuron in each hidden layer (ie, the layers preceded and followed by activations). 
In other words, the network is 

\begin{equation*}
    \nn{4}{\mathbf{x}} = \xi + \sum_{i=1}^{m_4} \alpha_i \sigma \left( \sigma \left( \sigma \left(\mathbf{x} \Wul{i}{1} + b^{(i,1)} \right) w^{(i,2)} + b^{(i,2)}  \right) w^{(i,3)} + b^{(i,3)}  \right),
\end{equation*}
%
with parameters $\Wul{i}{1} \in \mathbb{R}^d$, $w^{(i,l)} \in \mathbb{R}$  and $b^{(i,l)}, \alpha_i, \xi \in \mathbb{R}$ for $l \geq 1$.
%
Consider the training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro} but where the weight regularization is with $1$-norm, ie 

\begin{equation*}
    \min_{\params \in \Theta}  \frac{1}{2} \| \nn{L}{\mathbf{X}}  - \mathbf{y} \|^2_2 + \frac{\beta}{L} \left(\sum_{i=1}^{m_4}|\alpha_i|_1^L + \|\Wul{i}{1}\|_1^L + |w^{(i,2)} |^L  + |w^{(i,3)} |^L \right). 
\end{equation*}

%As before, bias parameters are unregularized.
By a similar argument as Lemma 27 in \citep{pilanci2023complexity}  and \cref{lemma:rescale}, %Lemma 8 in the 1D NN paper
the training problem can be rescaled to \cref{eq:noncvxtrain_genLlyrLLnorm_rescale}
%Equation (20) in the 1D NN paper,
but with $L$ changed to $1$ in the norm constraint $\|\Wul{i}{l}\|_{L}$. Its dual is \cref{gen_parallel_dual}.
%Equation (27) in the 1D NN paper. 
Note that for $\mathbf{w} \in \mathbb{R}^d$ and $\mathbf{a}, \mathbf{b} \in \mathbb{R}^{1 \times d}$, the "reflections" are $\reflect{\mathbf{a}}{\mathbf{b}} = 2\mathbf{b}-\mathbf{a} \in \mathbb{R}^{1 \times d}$ and $\reflect{\mathbf{aw}}{\mathbf{bw}} = 2\mathbf{bw}-\mathbf{aw}=(2\mathbf{b}-\mathbf{a})\mathbf{w}=\reflect{\mathbf{a}}{\mathbf{b}}\mathbf{w} \in \mathbb{R}$. The only difference from before is $\mathbf{W}^{(1)}$ and $\mathbf{x}_n$ are of length $d$ instead of being scalars. However, $\mathbf{x}_n \mathbf{W}^{(1)} \in \mathbb{R}$. Therefore \cref{lemma:max_constr_Llyrl}
% Lemma 10 in the 1D NN paper 
still holds with the same proof. By redefining the domains $s_1 \in \mathbb{R}^d$ instead of $s_1 \in \{-1,1\}$ and $\mathcal{\Tilde{M}}^{(1)} = \mathcal{M}^{(1)} = \mathbb{R}^{d} \times \{-1,1,\}^{L-2}$ instead of $ \{-1,1\}^{L}$ in \cref{def:tempreludicfunc} and \cref{def:dicindexset},
%Definition (10) in the 1D NN paper, 
\cref{lemma:L234constr_recursive}
% Lemma 11 in the 1D NN paper
holds. Now plug in optimal candidates for $b^{(1)}$ in the last equation in the proof of \cref{lemma:max_constr_Llyrl}. Let $\mathbf{j}=(j_1,j_2,j_3)$. The maximization constraint in the dual is 

\begin{equation*}
     \max_{\mathbf{j}, \mathbf{w}^{(i)}, \mathbf{a}\in \tilde{\params} }  \left | \sum_{n=1}^N \lambda_n f_n \right| \leq \beta,
\end{equation*}
where 
\begin{equation}\label{eq:fn}
    \begin{aligned}
        f_n &=  \sigma \left(  \left( \sigma \left(   \left( \sigma \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right)\mathbf{w}^{(1)} \right)  {-} \sigma \left(\left( {\mathbf{x}_{j_2}} {-} \mathbf{a} \right)\mathbf{w}^{(1)}  \right) \right) w^{(2)} \right) \right. \right. \\
     &   \qquad  {-}\sigma \left(  \left( \sigma \left(\left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right) \mathbf{w}^{(1)} \right)  {-} \sigma \left( \left( {\mathbf{x}_{j_2} } {-} \mathbf{a} \right)\mathbf{w}^{(1)} \right)  w^{(2)}\right) \right) \Big) w^{(3)} \Big)
    \end{aligned}
\end{equation}
%
%\begin{equation*}
%\begin{aligned}
%     \max_{\mathbf{j}, \mathbf{w}^{(i)}, a\in \tilde{\params} } & \Bigg | \sum_{n=1}^N \lambda_n \sigma \left(  \left( \sigma \left(   \left( \sigma \left( \left( \mathbf{x}_n {-} {a} \right)\mathbf{w}^{(1)} \right)  {-} \sigma \left(\left( {\mathbf{x}_{j_2}} {-} a \right)\mathbf{w}^{(1)}  \right) \right) w^{(2)} \right) \right. \right. \\
%     &  \qquad \qquad  {-}\sigma \left(  \left( \sigma \left(\left( {\mathbf{x}_{j_3}} {-} a \right) \mathbf{w}^{(1)} \right)  {-} \sigma \left( \left( {\mathbf{x}_{j_2} } {-} a \right)\mathbf{w}^{(1)} \right)  w^{(2)}\right) \right) \Big) w^{(3)} \Big) \Bigg | \leq \beta. 
%\end{aligned}
%\end{equation*}
%
and $\tilde{\params} = \left \{\mathbf{j}, \mathbf{w}, \mathbf{a}: j_1, j_2, j_3 \in [N], \mathbf{a} \in \left \{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right \}, w^{(3)} = \pm 1, w^{(2)} = \pm 1, \|\mathbf{w}^{(1)}\|_1=1 \right\}$. Note that $\mathbf{a}$ depends on $\mathbf{j}$.
Now, we make the constraints finite and the objective linear in $\mathbf{w}^{(1)}$ by optimizing $\mathbf{w}^{(1)}$ over polytopes defined by hyperplane arrangements. Denote $\mathbf{1}\{z\}$ as the threshold function outputting $1$ if $z \geq 0$ and $0$ otherwise, and extend it componentwise for vector inputs.
Define the following sets of  hyperplane arrangement patterns. 

%For  $j \in [N]$,
%\begin{equation*}
%   \mathcal{D}_j = \left \{ \text{Diag} \left( \mathbf{1} \left\{ \left(\mathbf{X}- \mathbf{1}\mathbf{x}_j \right) \mathbf{w} \right\} \right): \mathbf{w} \in \mathbb{R}^d \right\} 
%\end{equation*}
%and for $j_1, j_2 \in [N]$, 
%\begin{equation*}
%    \mathcal{D}^{R}_{(j_1,j_2)} = \left\{ \text{Diag} \left(
%\mathbf{1}\left\{ \left(\mathbf{X}- \mathbf{1}\reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}}\right) \mathbf{w}  \right \} \right): \mathbf{w} \in \mathbb{R}^d \right \}.
%\end{equation*}

For $\mathbf{j},a \in \tilde{\theta}$, let $\mathcal{D}_{\mathbf{j},\mathbf{a}} = \left \{ \text{Diag} \left( \mathbf{1} \left\{ \left(\mathbf{X}- \mathbf{1a} \right) \mathbf{w} \right\} \right): \mathbf{w} \in \mathbb{R}^d \right\} $. Enumerate $\left \{D_{\mathbf{j},\mathbf{a},1}, \cdots D_{\mathbf{j},\mathbf{a}, P} \right \} = \mathcal{D}_{\mathbf{j},\mathbf{a}}$. For $p \in [P]$, let $\mathcal{C}_{\mathbf{j},\mathbf{a},p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D_{\mathbf{j},\mathbf{a},p} -I\right) \left( \mathbf{X}-\mathbf{1}\mathbf{a} \right) \mathbf{w} \geq 0  \right \}$. 
Then, we have $\sigma \left(\left(\mathbf{X} - \mathbf{1}\mathbf{a} \right) \mathbf{w}^{(1)}  \right) = D_{\mathbf{j},\mathbf{a},p} \left(\mathbf{X}-\mathbf{1}\mathbf{a}\right) \mathbf{w}^{(1)} $  iff $\mathbf{w}^{(1)} \in \mathcal{C}_{\mathbf{j},\mathbf{a},p} $. 

As a special case when $\mathbf{a}$ is a data sample, for $j \in [N]$ and $w \in \mathbb{R}^d$, let $\mathcal{D}_{j} $ be $ \mathcal{D}_{\mathbf{j},\mathbf{a}}$ where $\mathbf{a}=\mathbf{x}_j$. For $j \in [N] $, enumerate $\left \{D_{j,1}, \cdots, D_{j,P_j} \right \} = \mathcal{D}_{j}$. As similar to above, let $\mathcal{C}_{j,p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D_{j,p} -I\right)\left( \mathbf{X}-\mathbf{1}\mathbf{x}_j \right) \mathbf{w} \geq 0  \right \}$.  
%
%Let $\left \{D_{j,1}, \cdots D_{j,P_j} \right \} = \mathcal{D}_j$. For $j \in [N]$, $p \in [P_j]$, let $\mathcal{C}_{j,p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D_{j,p} -I\right) \mathbf{X} \mathbf{w} \geq 0  \right \}$. Then, for $j \in [N]$, $p \in [P_j]$, we have $\sigma \left(\left(\mathbf{X} - \mathbf{1}\mathbf{x}_j \right) \mathbf{w}^{(1)}  \right) = D_{j,p} \left(\mathbf{X}-\mathbf{1}\mathbf{x}_j \right) \mathbf{w}^{(1)} $  iff $\mathbf{w}^{(1)} \in \mathcal{C}_{j,p} $.
%
%Similarly let $\left \{ D^R_{(j_1,j_2),1}, \cdots D^R_{(j_1,j_2),P_{(j_1,j_2)}} \right\} = \mathcal{D}^R_{(j_1, j_2)}$. For $j_1, j_2 \in [N]$, $p \in [P_{(j_1, j_2)}]$, let $\mathcal{C}^R_{(j_1, j_2),p} = \left \{\mathbf{w} \in \mathbb{R}^d: \left(2D^R_{(j_1,j_2),p} -I\right) \mathbf{X} \mathbf{w} \geq 0  \right \}$. Then, for $j_1, j_2 \in [N]$, $p \in [P_{(j_1, j_2)}]$, we have $\sigma \left(\left(\mathbf{X} - \mathbf{1}\reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right) \mathbf{w}^{(1)}  \right) = D^R_{(j_1, j_2),p} \left(\mathbf{X}-\mathbf{1}\reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}}\right) \mathbf{w}^{(1)} $  iff $\mathbf{w}^{(1)} \in \mathcal{C}^R_{(j_1, j_2),p} $.
%
%Therefore, for fixed $\mathbf{j}$, if $a =x_{j_1}$ then for $\mathbf{w}^{(1)} \in \mathcal{C}_{j_1,p} $,
%
%\begin{equation*}
%    \begin{aligned}
%        f_n &=  \sigma \left(  \left( \sigma \left(   \left( \left( \mathbf{x}_n {-} {a} \right)\mathbf{w}^{(1)}{\left(D_{j_1,p}\right)}_n   {-} \left( {\mathbf{x}_{j_2}} {-} a \right)\mathbf{w}^{(1)}  {\left(D_{j_1,p}\right)}_{j_2} \right) w^{(2)} \right) \right. \right. \\
%     &   \qquad  {-}\sigma \left(  \left( \left( {\mathbf{x}_{j_3}} {-} a \right) \mathbf{w}^{(1)} {\left(D_{j_1,p}\right)}_{j_3}  {-}  \left( {\mathbf{x}_{j_2} } {-} a \right)\mathbf{w}^{(1)} {\left(D_{j_1,p}\right)}_{j_2} \right) w^{(2)}\right) \Big) w^{(3)} \Big) \\
%     & = \sigma \left(  \left( \sigma \left(   \left(  \mathbf{x}_n {-} {a}   {-} \left( {\mathbf{x}_{j_2}} {-} a \right) {\left(D_{j_1,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{j_1,p}\right)}_n \right) \right. \right. \\
%     &    \qquad {-}\sigma \left(  \left(  {\mathbf{x}_{j_3}} {-} a     {-}  \left( {\mathbf{x}_{j_2} } {-} a \right){\left(D_{j_1,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{j_1,p}\right)}_{j_3}\right) \Big) w^{(3)} \Big) \\
%    \end{aligned}
%\end{equation*}
%
%and similarly with $D^R_{j_1, j_2, p}$ instead of $D_{j_1, p}$ if $a = \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}}$.
%
%Let $D_{\mathbf{j},a,p}$ be $D_{j_1,p}$

For $w \in \{-1,1\}$, and $d \in \{0,1\}$, let $\Bar{d}=1-d$ and $d^{w}$ be $d$ if $w=1$ and $1-d$ if $w=-1$.

Fix $\mathbf{j},\mathbf{w},\mathbf{a} \in \Tilde{\theta}$. Fix $p \in [P], p_{j_2} \in [P_{j_2}], p_{j_3} \in [P_{j_3}]$. For $i \in [N]$, let $d_{\mathbf{a},i} = \left(D_{\mathbf{j},\mathbf{a},p}\right)_{i,i} \in \{0,1\}$. For $j,i\in [N]$, let $d_{j, i} = \left(D_{j,p_j}\right)_{i,i} \in \{0,1\}$. 
 When $\mathbf{w}^{(1)} \in \mathcal{C}_{\mathbf{j},\mathbf{a},p} \cap \mathcal{C}_{j_2, p_{j_2}} \cap \mathcal{C}_{j_3, p_{j_3}}$, we have

\begin{equation*}
    \begin{aligned}
    f_n &=  \sigma \left(  \left( \sigma \left(   \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right)\mathbf{w}^{(1)}d_{\mathbf{a,n}}   {-} \left( {\mathbf{x}_{j_2}} {-} \mathbf{a} \right)\mathbf{w}^{(1)} d_{\mathbf{a},j_2}  \right) w^{(2)} \right) \right. \right. \\
     &   \qquad  {-}\sigma \left(  \left( \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right) \mathbf{w}^{(1)} d_{\mathbf{a},j_3} {-}  \left( {\mathbf{x}_{j_2} } {-} \mathbf{a} \right)\mathbf{w}^{(1)} d_{\mathbf{a},j_2} \right) w^{(2)}\right) \Big) w^{(3)} \Big) \\
     %
     %& = \sigma \left(  \left( \sigma \left(   \left(  \mathbf{x}_n {-} {a}   {-} \left( {\mathbf{x}_{j_2}} {-} a \right) {\left(D_{\mathbf{j},a,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{\mathbf{j},a,p}\right)}_n \right) \right. \right. \\
     %&    \qquad {-}\sigma \left(  \left(  {\mathbf{x}_{j_3}} {-} a     {-}  \left( {\mathbf{x}_{j_2} } {-} a \right){\left(D_{\mathbf{j},a,p}\right)}_{j_2} \right) \mathbf{w}^{(1)} w^{(2)} {\left(D_{\mathbf{j},a,p}\right)}_{j_3}\right) \Big) w^{(3)} \Big) \\
     %
     &= \sigma \left(  \left( \sigma \left(   \left(  \left( \mathbf{x}_n {-} {\mathbf{a}} \right)d_{\mathbf{a},n} \Bar{d}_{\mathbf{a},j_2}+ (\mathbf{x}_n {-} \mathbf{x}_{j_2})d_{\mathbf{a},n} d_{\mathbf{a},j_2} - \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{a},j_2} \right) \mathbf{w}^{(1)} w^{(2)}  \right)  \right. \right. \\
     &    \qquad {-}\sigma \left(  \left(  \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right)d_{\mathbf{a},j_3}\Bar{d}_{\mathbf{a},j_2}  + \left( \mathbf{x}_{j_3} {-}\mathbf{x}_{j_2}\right)d_{\mathbf{a},j_3}d_{\mathbf{a},j_2} - \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{a,j_3}d_{\mathbf{a},j_2}  \right) \mathbf{w}^{(1)} w^{(2)} \right) \Big) w^{(3)} \Big) \\
     %
      %&= \sigma \left(  \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right) d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_2} d^{w^{(2)}}_{\mathbf{a},n}  + (\mathbf{x}_n {-} \mathbf{x}_{j_2})d_{\mathbf{a},n}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,n} + \left( \mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{a},j_2} d^{-w^{(2)}}_{\mathbf{a},j_2} 
     %   \right. \right.  \\
     %&   \qquad {-}   \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right)d_{\mathbf{a},j_3}\Bar{d}_{\mathbf{a},j_2}d^{w^{(2)}}_{\mathbf{a},j_3}  - \left( \mathbf{x}_{j_3} {-}\mathbf{x}_{j_2}\right)d_{\mathbf{a},j_3}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,j_3} - \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right)  \Bar{d}_{a,j_3} d_{\mathbf{a},j_2} d^{-w^{(2)}}_{\mathbf{a},j_2}   \Big) \mathbf{w}^{(1)} w^{(3)} \Big) \\
     %
    &= \sigma \left(  \left( \left( \mathbf{x}_n {-} {\mathbf{a}} \right) d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}1\right\}
    + (\mathbf{x}_n {-} \mathbf{x}_{j_2})d_{\mathbf{a},n}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,n} 
    + \left( \mathbf{x}_{j_2} {-} \mathbf{a} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}-1\right\}
        \right. \right.  \\
     &   \qquad {-}   \left( {\mathbf{x}_{j_3}} {-} \mathbf{a} \right)d_{\mathbf{a},j_3}\Bar{d}_{\mathbf{a},j_2}\mathbf{1}\left\{w^{(2)}{=}1\right\} 
     - \left( \mathbf{x}_{j_3} {-}\mathbf{x}_{j_2}\right)d_{\mathbf{a},j_3}d_{\mathbf{a},j_2}d^{w^{(2)}}_{j_2,j_3} -
     \left(\mathbf{x}_{j_2} {-} \mathbf{a} \right)  \Bar{d}_{\mathbf{a},j_3} d_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}{-}1\right\}   \Big) \mathbf{w}^{(1)} w^{(3)} \Big) \\ 
     %
     & \scalemath{0.8}{
     {=} \left( \left(\left(\mathbf{x}_n {-} \mathbf{a}\right)d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_3}\mathbf{1}\left \{w^{(3)}{=}1 \right\} 
     {+} \left(\mathbf{x}_n {-} \mathbf{x}_{j_3}\right)d_{\mathbf{a},n}d_{\mathbf{a},j_3}d^{w^{(3)}}_{j_3,n} {-} \left(\mathbf{x}_{j_3} {-} \mathbf{a}\right)\Bar{d}_{\mathbf{a},n}d_{\mathbf{a},j_3}\mathbf{1}\left\{w^{(3)}{=}{-}1\right\} \right)\Bar{d}_{\mathbf{a},j_2} \mathbf{1}\left\{w^{(2)}{=}1\right\} \right.
     }\\
     & \scalemath{0.8}{ 
     {+} \left(\left(\mathbf{x}_n {-} \mathbf{x}_{j_2} \right) d_{\mathbf{a},n} \Bar{d}_{\mathbf{a},j_3}d_{j_2, n} \mathbf{1}\left \{ w^{(3)}{=}1\right\}{+} \left(\mathbf{x}_n {-}\mathbf{x}_{j_3} \right) d_{\mathbf{a},n} d_{\mathbf{a},j_3}d_{j_2,n}d_{j_2,j_3}d_{j_3,n}^{w^{(3)}} {+} \left(\mathbf{x}_{j_3} {-} \mathbf{x}_{j_2} \right) \Bar{d}_{\mathbf{a},n} d_{\mathbf{\mathbf{a}},j_3}d_{j_2,j_3} \mathbf{1}\left\{ w^{(3)}{=}{-}1\right\}\right) d_{\mathbf{a},j_2} \mathbf{1} \left\{ w^{(2)}{=}1\right\}
     } \\
     & {+} \left(\mathbf{x}_{j_2}{-}\mathbf{a} \right)\left(\bar{d}_{\mathbf{a},n}d_{\mathbf{a},j_3} \mathbf{1}\left\{ w^{(3)}{=}1\right\}{+} d_{\mathbf{a},n}\Bar{d}_{\mathbf{a},j_3}  \mathbf{1}\left\{ w^{(3)}{=-}1\right\}\right)d_{\mathbf{a},j_2} \mathbf{1}\left \{w^{(2)}{=}{-}1 \right \} \Big) \mathbf{w}^{(1)} 
    \end{aligned}
\end{equation*}
%
which is linear in $\mathbf{w}^{(1)}$.
%and in every case, the argument of $\sigma(\cdot)$ will be of the form $(\mathbf{x}_{j}-\mathbf{a})\mathbf{w}^{(1)}\mathbf{w}^{(3)}$ where $\mathbf{a}$ is a data point or a reflection of data points, so the $\sigma$ can be removed by inserting hyperplane arrangement matrices.
Let $\mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}} = \mathcal{C}_{\mathbf{j},\mathbf{a},p} \cap \mathcal{C}_{j_2, p_{j_2}} \cap \mathcal{C}_{j_3, p_{j_3}} \cap \{\mathbf{w} \in \mathbb{R}^{d}: \|\mathbf{w}^{(1)}\|_1=1 \}$.
Therefore the maximization constraint in the dual is

\begin{equation*}
    \max_{j_1, j_2, j_3 \in [N] } 
    \max_{\mathbf{a} \in \left\{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}} 
    \max_{w^{(2)}, w^{(3)} \in \{-1,1\}} \max_{p \in [P], p_{j_2} \in [P_{j_2}], p_{j_3} \in [P_{j_3}]}
    \max_{\mathbf{w}^{(1)} \in \mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}} }  \left | \sum_{n=1}^N \lambda_n f_n \right| \leq \beta.
\end{equation*}
%
Since a linear function $\pm \sum_{n=1}^N \lambda_n f_n$ is being maximized over a polytope $\mathcal{E}_{\mathbf{j},\mathbf{a},\mathbf{p}}$, it suffices to maximize 
$f_n$ over the finite set of extremal points of $\mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}}$. By Lemma 19 in \citep{pilanci2023complexity}, the set of extremal points of $\mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}}$ are

\begin{equation*}
\mathcal{E}_{\mathbf{j},\mathbf{a},\mathbf{p}} = \left \{w \in  \mathcal{T}_{\mathbf{j},\mathbf{a},\mathbf{p}}: \exists S \subset [N], |S| = d-1, \text{ s.t. } \mathbf{M}_s w =\mathbf{0}, \text{ rank}(\mathbf{M}_s)=d-1 \right \},
\end{equation*}
where 

\begin{equation*}
\mathbf{M} = 
    \begin{pmatrix}
        \mathbf{X} - \mathbf{1}\mathbf{a} \\
         I
    \end{pmatrix}.
\end{equation*}
%
Note that $\mathbf{M}$ depends on $\mathbf{j}$ and $\mathbf{a}$. Writing $f_n$ in its equivalent form \eqref{eq:fn}, the objective and $\mathcal{E}_{\mathbf{j},\mathbf{a},\mathbf{p}}$ depend on $\mathbf{j}$ and $\mathbf{a}$ but not on $\mathbf{p}$. For each $\mathbf{j},\mathbf{a}$, the union of the regions $\mathcal{C}_{\mathbf{j},\mathbf{a},p} \cap \mathcal{C}_{j_2, p_{j_2}} \cap \mathcal{C}_{j_3, p_{j_3}} $ over $\mathbf{p}$ cover all of $\mathbb{R}^N$. So the maximization constraint is equivalent to  

\begin{equation*}
    \max_{j_1, j_2, j_3 \in [N] } 
    \max_{\mathbf{a} \in \left\{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}} 
    \max_{w^{(2)}, w^{(3)} \in \{-1,1\}} 
    \max_{\mathbf{w}^{(1)} \in \mathcal{E}_{\mathbf{j},\mathbf{a}} }  \left | \sum_{n=1}^N \lambda_n f_n \right| \leq \beta,
\end{equation*}
%
where
%
\begin{equation*}
\mathcal{E}_{\mathbf{j},\mathbf{a}} = \left \{w \in \mathbb{R}^d: \exists S \subset [N], |S| = d-1, \text{ s.t. } \mathbf{M}_s w =\mathbf{0}, \text{ rank}(\mathbf{M}_s)=d-1 \right \}.
\end{equation*}

Consider the \lasso{} problem

\begin{equation*}
\min_{\mathbf{z}, \xi}  \frac{1}{2} \| \Amat{} \mathbf{z} + \xi \mathbf{1} - \mathbf{y} \|^2_2 + \beta \|\mathbf{z}\|_1,
	%\min_{\mathbf{z}} \mathcal{L}_{\mathbf{y}} (\mathbf{A}\mathbf{z} + \xi \mathbf{1}) + \frac{\beta}{2} \|\mathbf{z}\|_1,
\end{equation*}
%
where $\mathbf{A}$ is a dictionary matrix with columns of length $N$ whose $n^{\text{th}}$ element is $f_n$ as defined in \eqref{eq:fn}, for each $j_1,j_2,j_3 \in [N], \mathbf{a} \in \left \{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}$, $\mathbf{w}^{(1)} \in \mathcal{E}_{\mathbf{j},\mathbf{a}}$, and $w^{(2)}, w^{(3)} \in \{-1,1\}$.
%
As the bidual of the training problem, the \lasso{} problem is a lower bound for the training problem. We now describe a reconstruction from a \lasso{} solution $\mathbf{z}^*, \xi^*$ to a neural net that is optimal in the training problem, as similar to \cref{def:reconstructfunc}. We assume that $m_4 \geq \|\mathbf{z}^*\|_0$.
%For each $j_1,j_2,j_3 \in [N], \mathbf{a} \in \left \{\mathbf{x}_{j_1}, \reflect{\mathbf{x}_{j_1}}{\mathbf{x}_{j_2}} \right\}$, $\mathbf{w}^{(1)} \in \mathcal{E}_{\mathbf{j},\mathbf{a}}$, and $w^{(2)}, w^{(3)} \in \{-1,1\}$, the corresponding \lasso{} feature is a column in $\mathbb{R}^N$ with $n^{\text{th}}$ element \eqref{eq:fn}.
For each $i^{\text{th}}$ selected feature of the \lasso{} problem and corresponding $\mathbf{w}^{(1)}, w^{(2)}, w^{(3)}$ and feature coefficient $z^*_i$, let $\mathbf{a}_1 = \mathbf{a} \in \mathbb{R}^{1 \times N}$, $a_2 = \left(\left(\mathbf{x}_{j_2} -\mathbf{a}_1 \right)\mathbf{w}^{(1)} \right)_+ \in \mathbb{R}$, $a_3 = \left(  \left(\left(  \left( \mathbf{x}_{j_3} - \mathbf{a}_1 \right)\mathbf{w}^{(1)} \right)_+ - a_2\right)w^{(2)} \right)_+ \in \mathbb{R}$.
  Let  $ \boldsymbol{\alpha} = \mathbf{z}^*$ and $\xi=\xi^*$. 
  Let $\Wul{i}{1} = \mathbf{w}^{(1)}, w^{(i,l)} = w^{(l)} 
  %\in \{-1,1\}$
  $, $\bul{i}{1} = - \mathbf{a}_1 \mathbf{w}^{(1)}, b^{(i,l)} = - a_l w^{(l)}
  %\in \mathbb{R}
  $.
  Finally, let $\gamma_i = |\alpha_i|^{\frac{1}{4}}$ and apply the transformation $q \to \gamma_i \frac{q}{\|q\|_1}$ for $q \in \left\{\alpha_i, \Wul{i}{1}, w^{(i,2)}, w^{(i,3)}  \right\}$, and $b^{(i,l)} \to b^{(i,l)} \left(\gamma_i\right)^l $. 
Let these be weights for that $i^{\text{th}}$ parallel unit. This reconstructs a neural net that achieves the same objective, showing that the \lasso{} problem is equivalent to the training problem. %: 
%$a^{(1)} = \mathbf{a}, b^{(i,2)} = -\left(\left(\mathbf{x}_{j_2} - b^{(i,1)} \right)\mathbf{w}^{(1)} \right)_+ w^{(2)}$, $b^{(i,3)} = -\left(  \left(\left(  \left( \mathbf{x}_{j_3} - a^{(i)}_1 \right)\mathbf{w}^{(1)} \right)_+ - a^{(i)}_2\right)s_{2} \right)_+ w^{(3)}$ for the third layer.

While $w^{(2)}, w^{(3)} \in \{-1,1\}$ (up to rescaling the network), the values of $\mathbf{w}^{(1)}$ are the elements of $\mathcal{E}_{\mathbf{j},\mathbf{a}}$. By the orthogonality characterization,

\begin{equation*}
   \mathcal{E}_{\mathbf{j},\mathbf{a}} = \left\{ \frac{\times_{\tilde{\mathbf{x}}_n \in \Tilde{\mathbf{X}}} \Tilde{\mathbf{x}}_n }{\|\times_{\Tilde{\mathbf{x}}_n \in \Tilde{\mathbf{X}}} \Tilde{\mathbf{x}}_n \|_1} \right\},
\end{equation*}
%
where $\Tilde{\mathbf{X}}$ is a set of $d-1$ linearly independent vectors in $\{\mathbf{x}_1-\mathbf{a}, \cdots, \mathbf{x}_N-\mathbf{a}, \mathbf{e}_1, \cdots, \mathbf{e}_d\}$. For each first layer weight $\mathbf{w}^{(1)}$, there is a training sample or its reflection for which $\mathbf{w}^{(1)}$ is orthogonal to at least $d-1$ other training samples shifted by it.

\section{2 layers with $>1$ neuron}

Suppose $\mathbf{w}^{(1)} \in \mathbb{R}^{d \times M}, \mathbf{b}^{(1)} \in \mathbb{R}^{1 \times M}, \mathbf{w}^{(2)} \in \mathbb{R}^{M \times 1}$ and $b^{(2)}, w^{(3)}, b^{(3)}  \in \mathbb{R}$. Then optimizing the maximization constraint in the dual over $b^{(3)}, b^{(2)}$ gives

\begin{equation*}
    \begin{aligned}
        f_n &=  \sigma \left(  \left( \sigma \left(   \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)} {+} \mathbf{b}^{(1)}\right)  {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}  {+}  \mathbf{b}^{(1)}  \right) \right) \mathbf{w}^{(2)} \right) \right. \right. \\
     &   \qquad  {-}\sigma \left(  \left( \sigma \left({\mathbf{x}_{j_3}}\mathbf{w}^{(1)}  {+} \mathbf{b}^{(1)}  \right)  {-} \sigma \left( {\mathbf{x}_{j_2} } \mathbf{w}^{(1)}{+} \mathbf{b}^{(1)}\right) \right)  \mathbf{w}^{(2)} \right) \Big) w^{(3)} \Big) \\
     %
     &=  \sigma \left(  \left( \sigma \left(  \sum_{m=1}^M  \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,m} {+} b^{(1)}_m  \right) {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,m}  {+}  b^{(1)}_m  \right) \right) w^{(2)}_m \right) \right. \right. \\
     &   \qquad  {-}\sigma \left( \sum_{m=1}^M \left( \sigma \left({\mathbf{x}_{j_3}}\mathbf{w}^{(1)}_{:,m}  {+} b^{(1)}_m  \right)  {-} \sigma \left( {\mathbf{x}_{j_2} } \mathbf{w}^{(1)}_{:,m}{+} b^{(1)}_m\right) \right) w_m^{(2)} \right) \Bigg) w^{(3)} \Bigg)
    \end{aligned}
\end{equation*}

Suppose there are $3$ layers and $2$ neurons in each layer. Let 
\begin{equation*}
    c_m = \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,m} 
     {+} b^{(1)}_m \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,m}  
     {+}  b^{(1)}_m \right) \right) w^{(2)}_m \in \mathbb{R}.
\end{equation*}
%
     Then

\begin{equation*}
    \begin{aligned}
     f_n &=  \sigma \left(c_1 + c_2 \right).
    \end{aligned}
\end{equation*}
%
For fixed $\mathbf{w}^{(1)},\mathbf{w}^{(2)}_2$, note that $c_2$ does not depend on $b^{(1)}$ and $f_n$ is a capped ramp vertically shifted by $-c_2$. Then the \kink{}s of the piecewise linear function $\sum_{n=1}^N \lambda_n f_n$ as a function of $b^{(1)}_1 \in \mathbb{R}$ are at $b^{(1)}_1 \in \left\{-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1},-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1}-c_2  : j_1 \in [N] \right\} $.

%Feature shapes below. Also get as linear as possible with w
\textbf{Case 1}: If $b^{(1)}_1 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1}$ then $c_1$ is fixed for fixed $\mathbf{w}^{(1)},w^{(2)}$ and does not depend on $b^{(2)}$ and the \kink{}s of $\sum_{n=1}^N \lambda_n f_n$ as a function of $b^{(1)}_2 $ are $b^{(1)}_2 \in \left\{-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2},-\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}-c_1  : j_1 \in [N] \right\} $. If moreover $b^{(1)}_2 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}$ then 

\begin{equation*}
    f_n = \sigma \left(\sum_{m=1}^2 \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,m} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,m} \right)\right) w^{(2)}_m   \right).
\end{equation*}
%
%this is a vector equation in terms of $\mathbf{x}_n$. Hard to call it a ramp, more like a 2D ramp
which is like a vertically shifted capped ramp in $2D$ in terms of $\mathbf{x}_n$ with \kink{} lines at \\ $\mathbf{x} \in \left \{ \mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1},\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}, \sum_{m=1}^2 \sigma \left( \left({\mathbf{x}_{j_2}} 
{-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,m} \right) w^{(2)}_m  \right \}$. 
If on the other hand 
$b^{(1)}_2 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,2}-c_1$ then

\begin{equation*}
   \begin{aligned}
    f_n &= \sigma \left( \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1 \right. \\  
     & \qquad {+} \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,2} -  \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1\right) \right. \\
     & \qquad {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,2}
     {-} \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1 \right)\Big) w^{(2)}_2 \Big) \Big) \\
     %
    % &=\sigma \left( \left( \sigma \left( \left( \mathbf{x}_n 
     %{-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} \right)
     %{-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     %{-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)\right) w^{(2)}_1 \right. \\  
     %& \qquad {+} \left( \sigma \left( \left( \mathbf{x}_n 
     %{-} \mathbf{x}_{j_1} \right) \left(\mathbf{w}^{(1)}_{:,2} {-} \mathbf{w}^{(1)}_{:,1}w^{(2)}_1 \right)   
     %{+} \sigma \left( \left({\mathbf{x}_{j_2}} 
     %{-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} \right)w^{(2)}_1 \right) \right. \\
   \end{aligned}
\end{equation*}

\textbf{Case 2}: If $b^{(1)}_1 = -\mathbf{x}_{j_1}\mathbf{w}^{(1)}_{:,1}-c_2$ then $c_1$ depends on $b^{(1)}_2$ and in terms of $b^{(1)}_2$, we have

\begin{equation*}
\begin{aligned}
    f_n &= \sigma \left( \left( \sigma \left( \left( \mathbf{x}_n 
     {-} \mathbf{x}_{j_1} \right) \mathbf{w}^{(1)}_{:,1} -\left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,2} 
     {+} b^{(1)}_2 \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,2}  
     {+}  b^{(1)}_2 \right) \right) w^{(2)}_2 \right. \right. \right) \\ 
     &\qquad {-} \sigma \left( \left({\mathbf{x}_{j_2}} 
     {-} \mathbf{x}_{j_1}  \right) \mathbf{w}^{(1)}_{:,1} {-} \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,2} 
     {+} b^{(1)}_2 \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,2}  
     {+}  b^{(1)}_2 \right) \right) w^{(2)}_2  \right) \Big) w^{(2)}_1   \\
     &\qquad {+} \left( \sigma \left(  \mathbf{x}_n \mathbf{w}^{(1)}_{:,2} 
     {+} b^{(1)}_2 \right) 
     {-} \sigma \left({\mathbf{x}_{j_2}}\mathbf{w}^{(1)}_{:,2}  
     {+}  b^{(1)}_2 \right) \right) w^{(2)}_2 \Big).
\end{aligned}
\end{equation*}
which has \kink{}s and hence optimal $b^{(1)}_2$ when $b^{(1)}_2 \in ...$. 


If there were $M=2$ neurons in the second layer, I think this can be simplified.


Or 5 layers - add another layer. Need to get recursive?


==> unused/future.tex <==
Consider sigma = sign activation. In the 2-layer nn, the hidden weights lie inside sigma, which erases their magnitude. The 2-layer nn grows a 3rd layer by expanding its vector of 2nd layer (outermost) weights into a matrix W, and appending a new vector of outermost 3rd-layer weights. This addition of parameters raises dangers of overfitting if the weight penalty is too small. On the other hand, the outer (third) layer throws away magnitude information away from the new weights in W by enclosing them in sigma. This makes the weight penalty shift from the inner (second) to the outermost (third) layer. This vector multiplies entire units, so the training problem chooses the best sparse (sigma-activated) combination of 2-layer nn's. It will not sacrifice matching the overall shape in order to fit to small local details.  The weight penalty is like a group regularization where the groups are nns.   So when the weight penalty is significant (ie large beta), deeper NNs want to fit the data in as few (big) features as possible, so  Also at each layer the activation amplitudes s get absorbed by multiplying with weights. So the product form of activations that remove information from parameters, and weight penalty makes the penalized weights bubble up to the last layer as the ones that matter. 

==> unused/intro_conclusion_yifei.tex <==



The complexity and non-linearity of deep neural networks presents challenges in fully understanding a trained model, as the current methodology does not provide a precise mathematical definition for the model, which is determined by the entire training trajectory, including various heuristically chosen optimizer hyperparameters. In contrast, weights in a generalized linear model such as linear or logistic regression are mathematically defined through convex optimization theory, and have clear statistical interpretations.  To bridge this disconnect, we develop a convex optimization formulation for characterizing deep neural network training problems on low dimensional datasets and establish an exact connection via $\ell_1$ penalized linear models.

We recast the training problem of deep neural networks as convex LASSO problems. LASSO (Least Absolute Shrinkage and Selection Operator) is a convex optimization technique that is used to solve linear regression problems with a penalty on the sum of the absolute values of the coefficients, which is known as the $\ell_1$ norm. By analyzing the inequality constraints in the convex dual problem, we show that the regularized training problem of deep neural networks corresponds to convex LASSO problems.


%

The connection between DNNs and LASSO implies new results on the structure of non-convex DNN training problems. For instance, it is known that LASSO problems can have multiple optimal solutions. This implies that the corresponding DNN problem has multiple equivalent global minima. However, we will show that neural networks with symmetric activations such as sign and absolute value correspond to LASSO models with a unique optimum. In contrast, ReLU and threshold activation may yield non-unique optima.  Additionally, LASSO also has a regularization parameter $\beta$ and a continuous path of solutions can be generated. This path can be mapped back to the corresponding DNN problem to get a continuous family of neural networks as the norm penalty varies.



In particular, we construct explicit dictionary matrices for the Lasso model which is shown to be equivalent to a DNN model. This dictionary matrix contains a fixed set of basis signals that are computed from the input 1D data. This interpretation provides valuable insights into to inner workings of the DNN model.

Additionally, when weight regularization approaches zero, for activation functions such as those that are symmetric, the problem has a closed-form solution. This implies that the explicit dictionary matrices found for 1-D data can be used to train the neural network efficiently with a variety of activation functions and for different levels of weight regularization.

Overall, the explicit dictionary matrices for 1-D data provide a way to understand the fundamental mechanisms behind a black-box DNN, which can be useful for interpreting the model's predictions and for designing more effective architectures and corresponding optimizers.

% \subsection{Motivation}
% The motivation for studying low-dimensional datasets (e.g., 1D, 2D, 3D data) in the context of deep neural networks could be that these types of data often appear in many real-world applications such as signal processing, audio processing, and physics-informed engineering problems. These types of data are also relatively simple and easy to visualize, which makes them useful for understanding the behavior of neural networks.

% Additionally, studying low-dimensional data can provide a deeper understanding of the underlying principles of neural networks and how they work. By studying simple cases, it can be easier to understand the complex behavior of neural networks when applied to high-dimensional datasets.

% Furthermore, studying low-dimensional data can also provide a way to test the limitations of neural networks and identify problems that need to be addressed. This can be useful for developing more effective neural networks that can be applied to a wide range of tasks.

% In summary, studying low-dimensional datasets is important in understanding the behavior of deep neural networks and for making them more effective in a wide range of applications. It can also help in identifying the limitations of the models and how to overcome them.


\subsection{Our contribution}

\emi{Insert main informal theorems.}

In this paper, we study two-layer neural networks with a variety of activation functions and deeper neural networks with sign activation on low-dimensional datasets via the lens of convex optimization. We analyze the inequality constraints in the convex dual problem and derive that the regularized training problem of deep neural network corresponds to convex LASSO (Least Absolute Shrinkage and Selection Operator) problems. By carefully analyzing the inequality constraints in the convex dual
problem, we show that the weight decay regular-
ized training problem of deep neural networks
corresponds to convex LASSO problems with a
fixed dictionary of basis signals. We provide ex-
plicit descriptions of this basis set, which serve as a clear and transparent explanation of. When the weight decay regularization parameter
approaches zero, the problem has a closed-form
solution for symmetric activation functions

We aim to give a complete and rigorous theoretical description of a deep neural network model with arbitrary depth by recasting the training problem as a convex LASSO problem. This can provide a white-box explanation of how the neural network is processing the input data, as the LASSO problem can be interpreted as a linear regression problem with a constraint on the sum of the absolute values of the coefficients.

Our method of using convex optimization to analyze the inequality constraints in the convex dual problem allows them to derive that the regularized training problem of deep neural network corresponds to convex LASSO problems. This provides a way to understand the internal workings of the neural network and how it is processing the input data.

Additionally, by providing explicit formulations for the parameters of the LASSO problems, the authors are able to give a complete and rigorous theoretical description of how the neural network is processing the input data. This can provide valuable insight into how the neural network is functioning and can be used to design more effective neural networks.

Overall, by recasting the training problem as a convex LASSO problem, we provide a way to understand the internal workings of a deep neural network model with arbitrary depth, which can be useful for interpreting the model's predictions and for designing more effective neural networks. It transforms the "black box" neural network model to a "white box" model, where the internal workings of the model can be understood and explained.


\section{Conclusion}

In conclusion, our results have shown that 2-layer and L-layer neural networks with certain activation functions are equivalent to convex LASSO models. Furthermore, when the weight decay regularization parameter tends to zero, the problem simplifies to a closed-form solution. Furthermore, when the width of the network exceeds a critical threshold, the LASSO problem takes the form of a simple convex projection. These findings have significant implications for both the theoretical understanding of deep neural networks and their practical applications. They provide a clear and rigorous theoretical description of deep neural networks, which can be used to better interpret and understand these models. Additionally, our results demonstrate that neural networks can be used effectively in low-dimensional data settings. Overall, the pedagogical value of these findings is high, as they offer a transparent and exact explanation of deep neural networks.


However, it is important to note that LASSO problems can be difficult to solve for high-dimensional data, where the dimensionality of the space is large. In this case, the dictionary matrices, which are used to represent the input data in the LASSO problem, making the problem challenging. One possible solution to this issue is to use subsampling methods to select a smaller subset of the data to use in the LASSO problem. This can reduce the dimensionality of the input space, making the problem more tractable. However, this approach may not be ideal as it can introduce bias in the solution. An alternative is to use implicit representations of the dictionary matrices which can make the problem more efficient to solve. But these methods also have their own set of limitations and may not be a perfect solution. 
%Overall, it's important to note that solving high-dimensional LASSO problems is a challenging task and that the authors of the paper may have not discussed the limitations of their method in solving such problems in the abstract.


==> unused/junk.tex <==

\section{did not work because subgradient components are not independent when multiplied by a matrix}
As proved in lemma \ref{lemma:A_full_rk}, the inverse of the dictionary matrix is of the form

\begin{equation}
A^{-1}=\frac{1}{2}
    \begin{pmatrix}
        1 & -1 & 0 & 0 & 0 & \cdots & 0 & 0 \\
        0 & 1 & -1 & 0 &  0 & \cdots & 0 & 0\\
        0 & 0 & 1 & -1 &  0 & \cdots & 0 & 0\\
        0 & 0 & 0 & 1 & -1 & \cdots & 0 & 0\\
        0 & 0 & 0 & 0 & 0 &\cdots & 0 & 0\\
        \vdots & \vdots &\vdots &\vdots &\vdots  &\ddots & \vdots & \vdots\\
        0 & 0 & 0 & 0  & 0 & \cdots & -1 & 1 \\
        1 & 0 & 0 & 0 & 0 & \cdots & 0 & 1 
    \end{pmatrix}.
\end{equation}

So the inverse gram matrix of $A$ is

\begin{equation}\label{eq:inv_gram_dic}
\begin{aligned}
       (A^T A)^{-1} &=  A^{-1} A^{-T} \\
       &= \frac{1}{4}
        \begin{pmatrix}
        1 & -1 & 0 & 0 & 0 & \cdots & 0 & 0 \\
        0 & 1 & -1 & 0 &  0 & \cdots & 0 & 0\\
        0 & 0 & 1 & -1 &  0 & \cdots & 0 & 0\\
        0 & 0 & 0 & 1 & -1 & \cdots & 0 & 0\\
        0 & 0 & 0 & 0 & 0 &\cdots & 0 & 0\\
        \vdots & \vdots &\vdots &\vdots &\vdots  &\ddots & \vdots & \vdots\\
        0 & 0 & 0 & 0  & 0 & \cdots & -1 & 1 \\
        1 & 0 & 0 & 0 & 0 & \cdots & 0 & 1 
    \end{pmatrix}
     \begin{pmatrix}
        1 & 0 & 0 & 0 & 0 & \cdots & 0 & 1 \\
        -1 & 1 & 0 & 0 & 0 & \cdots & 0 & 0 \\
        0 & -1 & 1 & 0 &  0 & \cdots & 0 & 0\\
        0 & 0 & -1 & 1 &  0 & \cdots & 0 & 0\\
        0 & 0 & 0 & -1 & 1 & \cdots & 0 & 0\\
        0 & 0 & 0 & 0 & 0 &\cdots & 0 & 0\\
        \vdots & \vdots &\vdots &\vdots &\vdots  &\ddots & \vdots & \vdots\\
        0 & 0 & 0 & 0  & 0 & \cdots & -1 & 1 \\
    \end{pmatrix}\\
    &= \frac{1}{4}
    \begin{pmatrix}
         2 & -1 & 0 & 0 & 0 & \cdots & 0 &  0 &1 \\
        -1 & 2 & -1 & 0 & 0 & \cdots & 0 & 0 & 0 \\
        0 & -1 & 2 & -1 &  0 & \cdots & 0 & 0 & 0\\
        0 & 0 & -1 & 2 &  -1 & \cdots & 0 & 0 & 0\\
        \vdots & \vdots &\vdots &\vdots &\vdots  &\ddots & \vdots & \vdots & \vdots \\
        0 & 0 & 0 & 0  & 0 & \cdots & -1 & 2 & -1 \\
        1 & 0 & 0 & 0  & 0 & \cdots & 0 & 0 & 2 \\
    \end{pmatrix}.
\end{aligned}  
\end{equation}

Let $g(z)=||z||_1$. The subgradient  $\delta g $ has components for $i \in [N]$,

\begin{equation}
    (\partial g(z))_i = 
    \begin{cases}
        &\{1\} \mbox{ if } z_i > 0 \\
        &\{-1\} \mbox{ if } z_i < 0 \\
       & [-1,1] \mbox{ if } z_i = 0. 
    \end{cases}
\end{equation}

The subgradient (set) of the Lasso objective is

\begin{equation}
    \begin{aligned}
        \delta f(z) &= A^T (Az-y) + \beta \partial g(z) \\
        &= A^T A \left(z - A^{-1}y + \beta (A^T A)^{-1} \delta g(z) \right) \\
    \end{aligned}
\end{equation}

where addition and multiplication of scalars with sets are defined pointwise.

We have $0 \in \delta f(z)$  if and only if there exists $w \in \delta g(z)$ such that $A^T A \left(z - A^{-1}y + \beta (A^T A)^{-1} w\right)=0$, if and only if there exists  $w \in \delta g(z)$ such that 

\begin{equation} \label{eq:subgrad0_signact}
    z - A^{-1}y + \beta (A^T A)^{-1}w=0,
\end{equation}

 if and only if $0 \in z - A^{-1}y + \beta (A^T A)^{-1} \delta g(z) = (A^TA)^{-1} \delta f(z)$, if and only if
 
\begin{equation}\label{eq:z_in_subgrad}
    z \in A^{-1}y + \beta (A^T A)^{-1}\delta g(z).
\end{equation}

For $i \in [N]$, let $a_i = (A^{-1}y)_i$. As shown in the proof of lemma \ref{lemma:A_full_rk}, we have

\begin{equation}\label{def_ai}
    \begin{aligned}
       a_i = 
       \begin{cases}
           \frac{y_i - y_{i+1}}{2} &\mbox{ if } i \in [N-1] \\
           \frac{y_1 + y_{N}}{2}& \mbox{ if } i = N.
       \end{cases}
    \end{aligned}
\end{equation}

Let 

\begin{equation}\label{def:betatilde}
    \tilde{\beta} := \frac{1}{4}\beta
\end{equation}


%From equation \eqref{eq:inv_gram_dic}, for $i \in \{2, \cdots, N-1\}$,

%\begin{equation}
%     -\beta (A^T A)^{-1} w = \Tilde{\beta}(w_{i-1} - 2w_{i} + w_{i+1}).
%\end{equation}



Plug equation \eqref{eq:inv_gram_dic} into equation \eqref{eq:z_in_subgrad}. Then  $\mathbf{0} \in [\delta f(z)]$, if and only if 

    \begin{align} 
     z_1 &\in a_1 + \tilde{\beta}(2 \delta g(z_1) - \delta g(z_2) + \delta g(z_N))
        \label{eq:gradz_inclusion_condition_signact_1} \\ 
        z_i & \in a_i + \Tilde{\beta}(\delta g(z)_{i-1} - 2\delta g(z)_{i} + \delta g(z)_{i+1}) \quad i \in \{2, \cdots, N-1\} \label{eq:gradz_inclusion_condition_signact_2_N-1} \\
        z_N &\in a_N + \tilde{\beta}(\delta g(z_1) + \delta g(2z_N)) \label{eq:gradz_inclusion_condition_signact_N} 
    \end{align}

    Let $Q: \{-1,0,1\}^N \times [N]$ be defined as follows. For $w \in \{-1,0,1\}^N, i \in [N]$:

    \begin{equation}\label{eq:def_Q(w,i)}
        \begin{aligned}
            Q(w,i):= 
            \begin{cases}
            2 \delta g(w_{i}) - \delta g(w_{i+1}) + \delta g(w_N)  &\mbox{ if }  i =1 \\
              \delta g(w)_{i-1} - 2\delta g(w)_{i} + \delta g(w)_{i+1} &\mbox{ if }  i \in \{2, \cdots, N-1\} \\
              \delta g(w_1) + \delta g(2w_i) &\mbox{ if }  i =N \\
            \end{cases}
        \end{aligned}
    \end{equation}

By equations  \eqref{eq:gradz_inclusion_condition_signact_1}, \eqref{eq:gradz_inclusion_condition_signact_2_N-1}, \eqref{eq:gradz_inclusion_condition_signact_N}, the stationarity condition $\mathbf{0} \in \delta f(z)$ holds if and only if for all $i \in [N]$

\begin{equation}\label{eq:gradz_inclusion_condition_signact}
    z_i \in a_i +  \tilde{\beta}Q(\textrm{sgn}(z),i).
\end{equation}
    
If we can find a sign pattern $w   \in \{-1,0,1\}^N$ such that $a_i+\tilde{\beta}Q(w,i)$ contains an element $z_i'$ with $\textrm{sgn}(z_i')=w_i$ then setting $z_i = z_i'$ satisfies equation \eqref{eq:gradz_inclusion_condition_signact} for index $i$.

\begin{remark}\label{rmk:condn_on_ai}
   First, $a_i + \tilde{\beta}Q(w,i)$ contains a positive element if and only if $a_i + \tilde{\beta}\max Q(w,i) > 0$, if and only if $a_i > -\tilde{\beta}\max Q(w,i)$.
Similarly, $a_i + \tilde{\beta}Q(w,i)$ contains a negative element if and only if $a_i + \tilde{\beta}\min Q(w,i) < 0$, if and only if $a_i < - \tilde{\beta}\min Q(w,i)$.
Finally, $a_i + \tilde{\beta}Q(w,i)$ contains $0$ if and only if $a_i \in - \tilde{\beta}Q(w,i)$, if and only if $- \tilde{\beta}\max Q(w,i) \leq a_i \leq  -\tilde{\beta}\min Q(w,i)$. 
\end{remark}

Fix $i \in \{2,\cdots, N-1\}$. Suppose $w_{i-1} \in \{+,-,0\}$ is given. We will enumerate all possible pairs of the next two sign patterns $w_i, w_{i+1} \in \{+,-,0\}$. %, each of which determines the subgradient pair $\delta g(w)_{i-1}, \delta g(w)_{i}, \delta g(w)_{i+1}$. 
For each possible sign pattern $w_{i-1},w_i,w_{i+1}$, remark \ref{rmk:condn_on_ai} gives the necessary and sufficient condition on $a_i$ for $a_i + Q(w,i)$ to contain an element $z_i'$ with the same sign as $w_i$. Hence, given $w_{i-1}$,   this condition would make setting $z_i = z_i'$ and setting $\textrm{sgn}({z_{i+1}}) = w_{i+1}$ satisfy \eqref{eq:gradz_inclusion_condition_signact} for index $i$. 

On the other hand, since $\textrm{sgn}(z_i), \textrm{sgn}(z_{i+1})$ appear in equation \eqref{eq:gradz_inclusion_condition_signact} for index $i+1$ as well, fixing a particular $\textrm{sgn}(z_{i+1})$ and setting $z_i = z_i'$ from the result might make \eqref{eq:gradz_inclusion_condition_signact} unsatisfiable for index $i+1$, since the only free variable left is $w_{i+2}$. 

However, suppose for this paragraph there exists a sign pattern $w_i \in \{-,0,+\}$ such that for all possible signs of $w_{i+1} \in \{-,0,+\}$ there exists $z_i' \in a_i + Q(w,i)$ with the same sign as $w_i$. Then assigning $\textrm{sgn}(z_i) = w_i$ with no assumption on $\textrm{sgn}(z_{i+1})$ will always satisfy equation \eqref{eq:gradz_inclusion_condition_signact} for index $i$. And the assignment will leave two free variables $w_{i+1}, w_{i+2}$ in equation \eqref{eq:gradz_inclusion_condition_signact} for index $i+1$. 

$\mathbf{w_{i-1}=0}$

$ w_i= + $ 
\begin{equation}
    \begin{aligned}
        Q(w,i) = [-1,1]-2+w_{i+1} 
        = [-3,-1]+w_{i+1} =
        \begin{cases}
            [-2,0] \mbox { if } w_{i+1}= + \\
            [-4,2] \mbox { if } w_{i+1}= - \\
            [-4,0] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

By remark \eqref{rmk:condn_on_ai} if $a_i > \max -[-2,0] = \max[0,2]$, $a_i > \max -[-4,2]=\max[-2,4]$, and $a_i > \max -[-4,0]=\max[0,4]$ then for any $w_{i+1}$, setting $w_i=+$ will admit a solution to equation \eqref{eq:gradz_inclusion_condition_signact} for index $i$. In other words, the equation \eqref{eq:gradz_inclusion_condition_signact} criteria is for $a \geq \tilde{\beta}\max\{-(-2),-(-4),-(-4)\}=4\tilde{\beta}$.


$w_i = -$

\begin{equation}
    \begin{aligned}
        Q(w,i) = [-1,1]+2+w_{i+1} 
        = [-1,1]+2+w_{i+1}
        =[1,3]+2+w_{i+1} =
        \begin{cases}
            [2,4] \mbox { if } w_{i+1}= + \\
            [0,2] \mbox { if } w_{i+1}= - \\
            [0,4] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \leq \tilde{\beta}\min\{-(4),-(2),-(4)\}=-4\tilde{\beta}$.

$w_i = 0$

\begin{equation}
    \begin{aligned}
        Q(w,i) = [-1,1]-2[-1,1]+w_{i+1}
        = [-3,3]+w_{i+1} =
        \begin{cases}
            [-2,4] \mbox { if } w_{i+1}= + \\
            [-4,2] \mbox { if } w_{i+1}= - \\
            [-4,4] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \in \tilde{\beta}[-2,2]$.

$\mathbf{w_{i-1}=+}$

$w_i = +$

\begin{equation}
    \begin{aligned}
        Q(w,i) = -1 + w_{i+1} =
        \begin{cases}
            \{0\} \mbox { if } w_{i+1}= + \\
            \{-2\}  \mbox { if } w_{i+1}= - \\
            [-2,0] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \geq 2 \tilde{\beta}$.

$w_i = -$

\begin{equation}
    \begin{aligned}
        Q(w,i) = 3 + w_{i+1} =
        \begin{cases}
            \{4\} \mbox { if } w_{i+1}= + \\
            \{2\}  \mbox { if } w_{i+1}= - \\
            [2,4] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \leq -4 \tilde{\beta}$.

$w_i = 0$

\begin{equation}
    \begin{aligned}
        Q(w,i) = 1+2[-1,1]+w_{i+1} 
        = [-1,3]+w_{i+1} =
        \begin{cases}
            [0,4] \mbox { if } w_{i+1}= + \\
            [-2,2] \mbox { if } w_{i+1}= - \\
            [-2,4] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \in \tilde{\beta}[-2,0]$.

$\mathbf{w_{i-1}=-}$

$w_i = +$

\begin{equation}
    \begin{aligned}
        Q(w,i) = -3 + w_{i+1} =
        \begin{cases}
            \{-2\} \mbox { if } w_{i+1}= + \\
            \{-4\}  \mbox { if } w_{i+1}= - \\
            [-4,-2] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \geq 4\tilde{\beta}$.

$w_i = -$

\begin{equation}
    \begin{aligned}
        Q(w,i) = 1 + w_{i+1} =
        \begin{cases}
            \{2\} \mbox { if } w_{i+1}= + \\
            \{0\}  \mbox { if } w_{i+1}= - \\
            [0,2] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \leq -2\tilde{\beta}$.

$w_i = 0$

\begin{equation}
    \begin{aligned}
        Q(w,i) = -1+2[-1,1]+w_{i+1} 
        = [-3,1]+w_{i+1}=
        \begin{cases}
            [-2,2] \mbox { if } w_{i+1}= + \\
            [-4,0] \mbox { if } w_{i+1}= - \\
            [-4,2] \mbox { if } w_{i+1}= 0 \\
        \end{cases}
    \end{aligned}
\end{equation}

Equation \eqref{eq:gradz_inclusion_condition_signact} criteria is $a \in \tilde{\beta}[0,2]$.

\begin{assumption}\label{Assump:a1am=0}
    Suppose $y_1 = y_2$ and $y_N = -y_1$. Equivalently, from equation \ref{def_ai},  assume $a_1 = a_N = 0$. 
\end{assumption}

\begin{remark}
    Assumption \ref{Assump:a1am=0} can be achieved by adding another point $x_0 > x_1$ with label $y_0 = y_1$ and then another point $x_{N+1} < x_N$ with label $y_{N+1}=-y_0$, and then relabeling indices.
\end{remark}

\begin{lemma}\label{lemma:any_w1}
    Under assumption \ref{Assump:a1am=0}, for any $w_1, w_2 \in \{+,-,0\}$, if $w_N=w_1$ then equation \eqref{eq:gradz_inclusion_condition_signact} is satisfied for $i\in \{1,N\}$. 

\end{lemma}

\begin{proof}
From the definition \eqref{eq:def_Q(w,i)} of $Q(w,i)$, it suffices to show that

 $1$) there exists $z_1$ with $\textrm{sgn}(z_1)=w_1$ and
    \begin{equation}
        z_1 \in a_1 + \tilde{\beta}(2 \delta g(w_1) - \delta g(w_2) + \delta g(w_N)) \\
    \end{equation}

    $2$) there exists $z_N$ with $\textrm{sgn}(z_N)=w_N$ and
    \begin{equation}
        z_N \in a_N + \tilde{\beta}(\delta g(w_1) + \delta g(2w_N)). \\
    \end{equation}
    
   The right hand side of $1$) becomes $\tilde{\beta}(3 \delta g(w_1) - \delta g(w_2))$ and the right hand side of $2$) becomes $2\tilde{\beta}(\delta g(w_1))$. Both cases always contains an element of the same sign as $w_1$. So $1$) is satisfied.
\end{proof}

Equivalently,



\begin{assumption}\label{assump:bigjumps}
%For $i \in \{2, \cdots, N-1\}$ let $\Delta_i := y_{i+1}-y_i$. 

Suppose that for every $i \in \{2, \cdots, N-1\}$, 
  if $ |y_{i+1} - y_i| < 2 \beta $ then 

\begin{equation}
\begin{aligned}
     y_i <  &y_{i+1} < y_i + \beta &\mbox{ if } y_{i} < y_{i-1}  \\
    y_i -\beta <  &y_{i+1} < y_i &\mbox{ if } y_{i} > y_{i-1}  \\
    y_i -\beta <  &y_{i+1} < y_i + \beta &\mbox{ if } y_{i} = y_{i-1}  \\
\end{aligned}
\end{equation}


%Suppose that for every $i \in \{2, \cdots, N-1\}$, the labels $y_i$ satisfy the following:

% 1) If $y_{i+1} < y_i $ then $y_{i+2}  \in y_{i+1} + \beta((-\infty, -2] \cup [0,1] \cup [2, \infty))$. 
    
 %   2) If $y_{i+1} > y_i$ then $y_{i+2}  \in y_{i+1} + \beta((-\infty, -2] \cup [-1,0] \cup [2, \infty))$. 
    
  %  3) If $y_{i+1} = y_i$ then $y_{i+2}  \in y_{i+1} + \beta((-\infty, 2] \cup [-1,1] \cup [2, \infty))$.

    

    Equivalently, from equations \eqref{def_ai} and \eqref{def:betatilde}, 
    assume for every $i \in \{2, \cdots, N\}$:
    
   1) If $a_{i-1} > 0$ then $a_i \in \tilde{\beta}((-\infty, -4] \cup [-2,0] \cup [4, \infty))$. %[2, \infty) change to 4 to allow start from 0
    
    2) If $a_{i-1} < 0$ then $a_i \in \tilde{\beta}((-\infty, -4] \cup [0,2] \cup [4, \infty))$. %(-\infty, -2]  change to -4 to allow start from 0
    
    3) If $a_{i-1} = 0$ then $a_i \in \tilde{\beta}((-\infty, 4] \cup [-2,2] \cup [4, \infty))$.
\end{assumption}

\begin{remark}
Note by assumption \ref{} the labels correspond to data sorted in descending order: $x_1 > x_2 > \cdots > x_N$.

Assumption \ref{assump:bigjumps} places no restrictions on the data labels if consecutive labels $y_i$ and $y_{i+1}$ are far enough apart, more than $2\beta$ gap. If the jump $|y_{i+1}-y_i|$ between labels is small enough, under $2\beta$ then the labels must alternate between back and forth between increasing and decreasing by up to $\beta$. So, the data labels either fluctuate within a small range of $\beta$ about a plateau or make jumps larger than $2\beta$ to a new plateau. 

    %We have for $i \in [N-1]$ that 
   % Assumption \ref{assump:bigjumps} can hold if the data is sufficiently step-like. If the data label has just increased from $y_{i}$ to $y_{i+1} > y_i$ at index $i$, it will only increase again in the next index if it makes a sufficiently large jump to a new pulse. It can decrease a little bit and oscillate slightly. It can also jump down to a lower step if the gap is large enough. See figure \ref{fig:pulse_ex}.
\end{remark}

Figure \ref{fig:pulse_ex} is a plot of example training data $(x_i, y_i)$ satisfying assumption \ref{assump:bigjumps} for $\tilde{\beta}=1$. The data either oscillates within $2\tilde{\beta}$ around a plateau, or jumps to another plateau that is $4\tilde{\beta}$ away.

\begin{figure}[ht]
\begin{tikzpicture}
\centering
\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_i$}, ylabel = $y_i$]
\addplot[ycomb,color=black,solid,mark=*] 
plot coordinates{
(1,10) 
(2,10) 
(3,11) 
(4,10.5)
(5,11.5)
(6,11.1)
(7,7)
(8,7)
(9,6.9)
(10,7.5)
(11,6.5) 
(12,2) 
(13,2.2) 
(14,2.1)
(15,8)
(16,7.9)
(17,7.9)
(18,8.1)
(19,7.8)
(20,8.2)
(21,-3)
(22,-2.2)
(23,9.3)
(24,9)
(25,9)
(26,9.1)
(27,9.3)
(28,8.9)
(29,9.2)
(30,9.05)
(31,8.8)
(32,9.4)
(33,7.6)
(34, 12)
(35, 8)
(36, 13)
(37, -5)
(38, -4.9)
(39, -6)
(40, -5.5)
(40, -5.5)
(41, -10)
(42, -10)
};
\end{axis}
\end{tikzpicture}
\caption{Example training data pairs $(x_1,y_1), \cdots, (x_N, y_N)$ satisfying assumption \ref{assump:bigjumps} for $\tilde{\beta}=1$.}
\label{fig:pulse_ex}
\end{figure}

Figure \ref{fig:fsm} is a possible transition diagram between states ${-,+,0}$ representing the sign of $z_i$. The label on the edge from node $w_{i-1}$ to node $w_i$ is the criteria for $a_i$ guaranteeing that regardless of $z_{i+1}$, if we are given the previous state $\textrm{sgn}(z_{i-1})=w_{i-1}$, setting the sign of $z_i$ to be $w_i$ satisfies equation \eqref{eq:gradz_inclusion_condition_signact} for index $i$. If assumption \ref{assump:bigjumps} holds, then from every state $w_i$, there is another state $w_{i}$ that it can transition to in diagram \ref{fig:fsm}. Note we only transition out of a state $w_{i-1}$ if $a_i$ has a different sign than $w_{i-1}$ in \ref{fig:fsm}. 

\begin{lemma}\label{lemma:az_sign_match} 
    Let $i \in \{2, \cdots, N-1\}$. Suppose we chose $\textrm{sgn}(z_i)$ based on $\textrm{sgn}(z_{i-1})$ and $a_i$ from the transition diagram \ref{fig:fsm}.
    Then \ref{fig:fsm} is well-defined to find $\textrm{sgn}(z_{i+1})$.
\end{lemma}

\proofsketch{
    $z_i$ is approximately $a_i$ (this holds with equality when $\beta \to zero$). So the signs of $z_i$ and $a_i$ should be similar. 
}

\begin{proof}
    First suppose $z_i=0$. Then no matter $a_{i}$, assumption \ref{assump:bigjumps} gives a range of $a_{i+1}$ that is included among the edges transitioning from node $0$ in figure \ref{fig:fsm}. 
 
   Now suppose $z_i \neq 0$. The value of $a_i$ for every incoming edge to state $w_i \in \{+,-\}$ has the same sign as $w_i$. SO if $z_i \neq 0$, then $\textrm{sgn}(z_i)=\textrm{sgn}(a_i)$. Then assumption \ref{assump:bigjumps} guarantees a range of $a_{i+1}$ that is among one of the outgoing edges from $\textrm{sgn}(z_i)$. 
   
   So in both cases, \ref{fig:fsm} is well-defined to find $\textrm{sgn}(z_{i+1})$ from $\textrm{sgn}(z_{i}), \textrm{sgn}({a_{i+1}})$.
\end{proof}

 

%\begin{figure}[ht] % ’
%    \centering 
%    \begin{tikzpicture}[]
%description
%        \node[circle, draw, minimum size=1.7cm] (prev) at (-9, 6) {$\textrm{sgn}(z_{i-1})$};
%        \node[circle, draw, minimum size=1.7cm] at (-5, 6) (cur) {$\textrm{sgn}(z_{i})$};
 %       \path[->] (prev) edge node [above] {$\frac{1}{\tilde{\beta}}a_i$} (cur);

%        \node[circle, draw, minimum size=1cm] (0) at (0, 6) {$0$};
 %       \node[circle, draw, minimum size=1cm] at (-4, 0) (-) {-};
%        \node[circle, draw, minimum size=1cm] at (4, 0) (+) {+};

        %edges
%    \path[->] (0) edge [bend left] node [right] {$\geq 4$} (+);
%    \path[->] (+) edge [bend left] node [left] {$[-2,0]$} (0);
%     \path[->] (0) edge [bend right] node [left] {$\leq -4$}  (-);
%    \path[->] (-) edge [bend right] node [right] {$[0,2]$} (0);
%     \path[->] (-) edge [bend left] node [above] {$\geq 4$} (+);
 %   \path[->] (+) edge [bend left] node [below] {$\leq -4$} (-);

    %self loops
%     \path (0) edge [loop above] node {$[-2,2]$} (0);
 %    \path (+) edge [loop right] node {$\geq 2$} (+);
 %   \path (-) edge [loop left] node {$\leq -2$} (-);
 %   \end{tikzpicture}
 %   \caption{State transition diagram from $\textrm{sgn}(z_{i-1})$ to  $\textrm{sgn}(z_{i})$ for $i \in \{2, \cdots, N-1\}$ if assumption \ref{assump:bigjumps} holds. The transition conditions for $a_i$ are listed on the edges. All numbers are scaled to $\tilde{\beta}$.}
  %  \label{fig:fsm}
%\end{figure}
%todo: do self loops

\begin{figure}[ht] % ’
    \centering 
    \begin{tikzpicture}[]
%description
        \node[circle, draw, minimum size=1.7cm] (prev) at (-9, 6) {$\textrm{sgn}(z_{i-1})$};
        \node[circle, draw, minimum size=1.7cm] at (-5, 6) (cur) {$\textrm{sgn}(z_{i})$};
        \path[->] (prev) edge node [above] {$\frac{1}{{\beta}}a_i$} (cur);

        \node[circle, draw, minimum size=1cm] (0) at (0, 6) {$0$};
        \node[circle, draw, minimum size=1cm] at (-4, 0) (-) {-};
        \node[circle, draw, minimum size=1cm] at (4, 0) (+) {+};

        %edges
    \path[->] (0) edge [bend left] node [right] {$\geq 1$} (+);
    \path[->] (+) edge [bend left] node [left] {$[-\frac{1}{2},0]$} (0);
     \path[->] (0) edge [bend right] node [left] {$\leq -1$}  (-);
    \path[->] (-) edge [bend right] node [right] {$[0,\frac{1}{2}]$} (0);
     \path[->] (-) edge [bend left] node [above] {$\geq 1$} (+);
    \path[->] (+) edge [bend left] node [below] {$\leq -1$} (-);

    %self loops
     \path (0) edge [loop above] node {$[-\frac{1}{2},\frac{1}{2}]$} (0);
     \path (+) edge [loop right] node {$\geq \frac{1}{2}$} (+);
    \path (-) edge [loop left] node {$\leq -\frac{1}{2}$} (-);
    \end{tikzpicture}
    \caption{State transition diagram from $\textrm{sgn}(z_{i-1})$ to  $\textrm{sgn}(z_{i})$ for $i \in \{2, \cdots, N-1\}$ if assumption \ref{assump:bigjumps} holds. The transition conditions for $a_i$ are listed on the edges. All numbers are scaled to ${\beta}$.}
    \label{fig:fsm}
\end{figure}

\begin{lemma}\label{lemma:fsm}
    Suppose assumptions \ref{Assump:a1am=0} and \ref{assump:bigjumps} hold. Consider the following algorithm.
    
    1) Set the initial and final state $z_1 = z_N = 0$. 
    
    2) For $i \in \{2, N-1\}$:
    Choose $\textrm{sgn}(z_i)$ based on $\textrm{sgn}(z_{i-1})$ and $a_i$ according to diagram \ref{fig:fsm}. 

    3) For $i \in \{2, N-1\}$:
    Set $z_i$ to be the right hand side of \eqref{eq:gradz_inclusion_condition_signact}.\\

    Then the resulting $z$ satisfies the stationarity condition $0 \in \delta f(z)$.
\end{lemma}

\proofsketch{
We only need to know $a_i$ and two signs of $z_{i-1}, z_{i+1}$ to know $z_i$. So we can find the last layer weights $z_i$ sequentially in increasing index $i$. This procedure is essentially the proof of lemma \ref{lemma:fsm}.
}

\begin{proof}
    By lemma \ref{lemma:any_w1}, we can set $z_1 = 0$ and satisfy \eqref{eq:gradz_inclusion_condition_signact} for $i \in \{1,N\}$.  
    
    By assumption \ref{Assump:a1am=0}, $a_1 = 0$.  
    Since $z_1 = a_1$, assumption \ref{assump:bigjumps} guarantees a range on $a_2$ that makes the transition diagram  \ref{fig:fsm} is well-defined. 
    So we choose $\textrm{sgn}({z_2})$ based on $\textrm{sgn}({z_2})$ starting from node $0$ and $a_2$ according to figure \ref{fig:fsm}. 

    Therefore by lemma \ref{lemma:az_sign_match}, we can find $z_3$ from figure \ref{fig:fsm}. Then we set $z_2 $ according to \eqref{eq:gradz_inclusion_condition_signact}.
    Since the transitions guarantee equation  \eqref{eq:gradz_inclusion_condition_signact} is satisfied for any $z_3$, we know that $z_1, z_2, z_3$ satisfy equation \eqref{eq:gradz_inclusion_condition_signact} for $i=2$. 

We repeat this argument for $i \in \{3, \cdots, N-1\}$: since $\textrm{sgn}(z_{i-1})$ was chosen from figure \ref{fig:fsm}, lemma \ref{lemma:az_sign_match} allows us to use figure \ref{fig:fsm} again to choose $\textrm{sgn}(z_i)$ based on $\textrm{sgn}(z_{i-1})$ and $a_i$, and then $\textrm{sgn}(z_{i+1})$ from $\textrm{sgn}(z_{i})$ and $a_{i+1}$. We set $z_i$ to be the right hand side of \eqref{eq:gradz_inclusion_condition_signact}, which is now satisfied by construction in how we chose $z_i$. 
   
So equation  \eqref{eq:gradz_inclusion_condition_signact}   will be satisfied for all $i \in \{2, \cdots, N-1\}$.
    Combining with lemma \ref{lemma:any_w1}, we have $0 \in \delta f(z)$.
\end{proof}


 
% For $i \in [N]$, $w_i \in (\delta g(z))_i$ satisfies $w_i = \textrm{sgn}(z_i)$ if $z_i \neq 0$ and $w_i \in [-1,1]$ otherwise.





%For any $w, i \in \{2, \cdots, N-1\}$ let $Z(w,i) = a_i + \Tilde{\beta}(w_{i-1} - 2w_{i} + w_{i+1})$.

%By plugging in equation \eqref{eq:inv_gram_dic} into equation \eqref{eq:subgrad0_signact},  $\mathbf{0} \in [\delta f(z)]_{2:N-1}$ (in other words, $0 \in \delta f(z)_i$ for $i \in \{2, \cdots, N-1\}$) if and only if there exists $w \in \delta g(z)$ such that for $i \in \{2, \cdots, N-1\}$,

%\begin{equation}\label{eq:z_condition_signact}
%    \begin{aligned}
%        z_i &=  A^{-1}y - \beta (A^T A)^{-1}w \\
%        &= a_i + \Tilde{\beta}(w_{i-1} - 2w_{i} + w_{i+1}) \\
%        &= Z(w, i).\\
%    \end{aligned}
%\end{equation}

%In other words,

%\begin{equation}
%    \begin{aligned}
%        z_i \in a_i + \Tilde{\beta}(\delta |z_{i-1}| - 2 \delta |z_i| + \delta |z_{i+1}|)
%    \end{aligned}
%\end{equation}

%The goal is to find the signs of $z_i$ such that we can find $w \in \delta g(z)$ satisfying for every $i$, \eqref{eq:z_condition_signact}. In other words, to find $w \in [-1,1]^N$ such that setting $z_i=Z(w,i)$ does not contradict $w \in \delta g(z)$.

%Note $w$ satisfies \eqref{eq:z_condition_signact} if and only if $w_{i-1}, w_i, w_{i+1}$ does.

%We can denote $w_{\textrm{max}}(z) = \max \delta g(z)$ which is $1$ if $w_i \geq 0$ and $-1$ otherwise.  And $w_{\textrm{min}}(z) = \min \delta g(z)$ which is $-1$ if $w_i \leq 0$ and $1$ otherwise. 

%Then
%\begin{equation}
%    \begin{aligned}
%     \Tilde{\beta}(-w_{\textrm{max},i-1} + 2w_{\textrm{min,i}} - w_{\textrm{max},i+1}) \leq 
%        \Tilde{\beta}(-w_{i-1} + 2w_{i} - w_{i+1})
%        \leq
%        \Tilde{\beta}(-%w_{\textrm{min},i-1} + 2w_{\textrm{max,i}} - w_{\textrm{min},i+1}). 
%    \end{aligned}
%\end{equation}

%For any $w \in \delta g(z)$, $Z(w,i) > 0$  if and only if 
%\begin{equation}
%    \begin{aligned}
%        a_i &\geq \Tilde{\beta}(-w_{i-1} + 2w_{i} - w_{i+1})
%        \begin{cases}
%            & = \Tilde{\beta}(-w_{i-1} + 2w_{i} + 1) \mbox{ if } z_{i+1}>0 \\
%            &=\Tilde{\beta}(-w_{i-1} + 2w_{i} - 1) \mbox{ if } z_{i+1}<0 \\
%            &\in \Tilde{\beta}(-w_{i-1} + 2w_{i} + [-1,1]) \mbox{ if } z_{i+1}=0 \\
 %       \end{cases}    
%    \end{aligned}
%\end{equation}

%We enumerate all of the possible cases of signs for $z_{i-1},z_i$. Each case determines a possible range of $w_i \in \delta g(z)$. Given a fixed pair of $z_{i-1},z_i$ signs, for each possible sign of $z_{i+1}$, we find necessary and sufficient criteria on $a_i$ that allow us to set $z_i = Z(w,i)$.


==> unused/noisy_squarewave.tex <==
% this works with some sims but doesn't seem to always work. Also, removed it because took a lot of space and to expedite.


\section{$2$-layer networks with sign activation trained on a NOISY square wave label} \label{app_sec:squarewave-2lyrnoise}

In this section (\cref{app_sec:squarewave-2lyrnoise}) we assume the neural net has $L=2$ layers and uses sign activation, and the data is of dimension $d=1$ . We will use the subgradient condition (\cref{rk:strcvx}) to solve \lasso{} \eqref{eqref:Lasso}. 

\begin{lemma}\label{lemma:A^TA_2layer_sign}
	For $L=2$-layer networks with sign activation,
 \iftoggle{long}{ the elements of the gram dictionary matrix  $\mathbf{A}^T \mathbf{A}$ are }
$(\mathbf{A}^T \mathbf{A})_{i,j}= N - 2|i-j|$ for $i,j \in [N]$.
\end{lemma}

\begin{proof}
 \iftoggle{long}{
 	Since the data is sorted in descending order 
 $x_1 > x_2 > \cdots > x_N$ (\cref{section:notation}), the dictionary matrix $A \in \{-1,1\}^{N \times N}$ is of the form

	\begin{equation}\label{mat:A_2layer_sign}
		A =
		\begin{pmatrix}
			1      & 1      & 1      & 1      & \cdots & 1      & 1      \\
			-1     & 1      & 1      & 1      & \cdots & 1      & 1      \\
			-1     & -1     & 1      & 1      & \cdots & 1      & 1      \\
			-1     & -1     & -1     & 1      & \cdots & 1      & 1      \\
			-1     & -1     & -1     & -1     & \cdots & 1      & 1      \\
			\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
			-1     & -1     & -1     & -1     & \cdots & -1     & 1
		\end{pmatrix}.
	\end{equation}
 }
Recall \cref{remk:Asignform}'s description of $\mathbf{A}$.
%Let $\mathbf{a}_i$ be the $i^{th}$ column of $\mathbf{A}$. 
If $1 \leq i \leq j \leq N$ then
$
			(\mathbf{A}^T \mathbf{A} )_{i,j} 
   = \sum_{k=1}^{N} \mathbf{A}_{i,k} \mathbf{A}_{j,k} 
			                = \sum_{k=1}^{i-1} \mathbf{A}_{i,k} \mathbf{A}_{j,k} + \sum_{k=i}^{j-1} \mathbf{A}_{i,k} \mathbf{A}_{j,k} + \sum_{k=j}^{N} \mathbf{A}_{i,k} \mathbf{A}_{j,k} 
			                = \sum_{k=1}^{i-1} (1) (1) + \sum_{k=i}^{j-1} (-1) (1) + \sum_{k=j}^{N} (-1) (-1)        
			                = (i-1) - (j-1-i+1) + (N-j+1)     =N +  2(i-j)                     = N-2|i-j|
$.
\iftoggle{long}{
	For example, if $i=1,j=N$ then $(A^TA)_{i,j}=N+2(1-N) = 2 - N$.
}
Since $\mathbf{A}^T \mathbf{A}$ is symmetric, if  $1 \leq j \leq i \leq N$ then by reversing the roles of $i$ and $j$, $(\mathbf{A}^T \mathbf{A})_{i,j} = (\mathbf{A}^T \mathbf{A} )_{j,i} = N +  2(j-i)=N-2|i-j|$.
So for any $i, j \in [N]$, $(A^T A )_{i,j} =  N - 2|i-j|$.

\end{proof}

\begin{remark}
	We can write $\mathbf{A}^T\mathbf{A}$ in \cref{lemma:A^TA_2layer_sign} as,
 \iftoggle{long}{ the gram matrix
 $A^TA$ for the $L=2$ layer sign activation can be written out as
 }

	\begin{equation}\label{eq:A^TA_writtenout}
		\setcounter{MaxMatrixCols}{20}
		\begin{aligned}
			\mathbf{A}^T \mathbf{A} & =  \begin{pmatrix}
				           N      & N-2    & N-4    & \cdots & 2      & 0      & -2     & \cdots & 6-N    & 4-N    & 2-N    \\
				           N-2    & N      & N-2    & \cdots & 4      & 2      & 0      & \cdots & 8-N    & 6-N    & 4-N    \\
				           N-4    & N-2    & N      & \cdots & 6      & 4      & 2      & \cdots & 10-N   & 8-N    & 6-N    \\
				           \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
				           6-N    & 8-N    & 10-N   & \cdots & 2      & 4      & 6      & \cdots & 10-N   & 8-N    & 6-N    \\
				           4-N    & 6-N    & 8-N    & \cdots & 0      & 2      & 4      & \cdots & 8-N    & 6-N    & 4-N    \\
				           2-N    & 4-N    & 6-N    & \cdots & -2     & 0      & 2      & \cdots & N-4    & N-2    & N
			           \end{pmatrix}.
		\end{aligned}
	\end{equation}

 \iftoggle{long}{
 
	\begin{equation}\label{eq:A^TA_writtenout}
		\setcounter{MaxMatrixCols}{20}
		\begin{aligned}
			A^T A & =
			\begin{pmatrix}
				1      & -1     & -1     & -1     & \cdots & -1     & -1     \\
				1      & 1      & -1     & -1     & \cdots & -1     & -1     \\
				1      & 1      & 1      & -1     & \cdots & -1     & -1     \\
				1      & 1      & 1      & 1      & \cdots & -1     & -1     \\
				1      & 1      & 1      & 1      & \cdots & 1      & -1     \\
				\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
				-1     & -1     & -1     & -1     & \cdots & 1      & 1
			\end{pmatrix}
			\begin{pmatrix}
				1      & 1      & 1      & 1      & \cdots & 1      & 1      \\
				-1     & 1      & 1      & 1      & \cdots & 1      & 1      \\
				-1     & -1     & 1      & 1      & \cdots & 1      & 1      \\
				-1     & -1     & -1     & 1      & \cdots & 1      & 1      \\
				-1     & -1     & -1     & -1     & \cdots & 1      & 1      \\
				\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
				-1     & -1     & -1     & -1     & \cdots & -1     & 1
			\end{pmatrix}                                                \\
			      & =  \begin{pmatrix}
				           N      & N-2    & N-4    & \cdots & 2      & 0      & -2     & \cdots & 6-N    & 4-N    & 2-N    \\
				           N-2    & N      & N-2    & \cdots & 4      & 2      & 0      & \cdots & 8-N    & 6-N    & 4-N    \\
				           N-4    & N-2    & N      & \cdots & 6      & 4      & 2      & \cdots & 10-N   & 8-N    & 6-N    \\
				           \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
				           6-N    & 8-N    & 10-N   & \cdots & 2      & 4      & 6      & \cdots & 10-N   & 8-N    & 6-N    \\
				           4-N    & 6-N    & 8-N    & \cdots & 0      & 2      & 4      & \cdots & 8-N    & 6-N    & 4-N    \\
				           2-N    & 4-N    & 6-N    & \cdots & -2     & 0      & 2      & \cdots & N-4    & N-2    & N
			           \end{pmatrix}.
		\end{aligned}
	\end{equation}

 }
\end{remark}


\begin{figure}[ht]
	\begin{tikzpicture}
		\centering
		\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
			\addplot[ycomb,color=black,solid,mark=*]
			plot coordinates{
					(1,40-70)
					(2,40-68)
					(3,40-66)
					(4,40-64)
					(5,40-62)
					(6,40-60)
					(7,40-58)
					(8,40-56)
					(9,40-54)
					(10,40-52)

					(11,40-50)
					(12,40-48)
					(13,40-46)
					(14,40-44)
					(15,40-42)
					(16,40-40)
					(17,40-38)
					(18,40-36)
					(19,40-34)
					(20,40-32)

					(21,40-30)
					(22,40-28)
					(23,40-26)
					(24,40-24)
					(25,40-22)
					(26,40-20)
					(27,40-18)
					(28,40-16)
					(29,40-14)
					(30,40-12)

					(31,40-10)
					(32,40-8)
					(33,40-6)
					(34,40-4)
					(35,40-2)
					(36,40)
					(37,40-2)
					(38,40-4)
					(39,40-6)
					(40,40-8)
				};
		\end{axis}
	\end{tikzpicture}
	\caption{Column $10$ of $A^T A$, corresponding to a feature that multiplies $z_{10}$. The number of samples is $N=40$. Note the training samples are ordered in descending order, so to correspond to the labels $y$, the elements of $h_{k,T}$ are plotted from right to left.}
	\label{fig:feature_ex}
\end{figure}


\begin{remark}\label{rk:A^Ty}
 \iftoggle{long}{
 The dictionary matrix applied to a label vector is, 
 }
Recall \cref{remk:Asignform}. For $n \in [N]$,
$
			(\mathbf{A}^T \mathbf{y})_n = \sum_{i=1}^n \mathbf{y}_i - \sum_{i=n+1}^N \mathbf{y}_i
$.

    
\end{remark}

\begin{definition}
    For positive integers $a,b$, denote $\textrm{Quot}(a,b)$ and $ \textrm{Rem}(a,b)$ as the quotient and remainder, respectively, when $a$ is divided by $b$. Specifically, $a = \textrm{Quot}(a,b) b + \textrm{Rem}(a,b)$, $\textrm{Rem}(a,b) \in \{0, \cdots, b-1\}$, and  $\textrm{Quot}(a,b) = \frac{a-\textrm{Rem}(a,b)}{b}$.
    Define the modified remainder, 
    \[
\textrm{rem}(a,b) := 
\begin{aligned}
    \begin{cases}
   \textrm{Rem}(a,b)  & \mbox { if }  \textrm{Rem}(a,b) > 0 \\
   b & \mbox { if } \textrm{Rem}(a,b) = 0 
\end{cases}
\quad \in [b].
\end{aligned}
\]

And define the modified quotient,
\begin{equation*}
    \begin{aligned}
        \textrm{quot}(a,b) := \frac{a-\textrm{rem}(a,b)}{b} = 
        \begin{cases}
            \textrm{Quot}(a,b)  & \mbox { if }  \textrm{Rem}(a,b) > 0 \\
             \textrm{Quot}(a,b)-1 & \mbox { if } \textrm{Rem}(a,b) = 0 
        \end{cases}.
    \end{aligned}
\end{equation*} .

%Deno
% Let $Q_n = \frac{n-\mathrm{Rem}(n,T)}{T} \in \{0, \cdots, k\}$. So $n = Q_n T + \mathrm{Rem}(n,T)$.
\end{definition}

\begin{definition}\label{def:h_{k,T}}
	%Let $k \geq 4$ be an integer, and $T \geq 8$ be an even integer. \iftoggle{todos}{\textcolor{red}{might not need}}

	Suppose \iftoggle{long}{ there are}
 $N=kT$
 \iftoggle{long}{ training samples}
 for $k,T \in \mathbb{N}$. %Denote $\textrm{rem}(T,n)$ as the remainder when $T$ is divided by $n$. 
 Define $\mathbf{h_{k,T}} \in \{-1,1\}^N$ by its $n^{\textrm{th}}$ element as,
 \iftoggle{long}{
 the $i^{th}$ element of $h_{k,T}$ is
 }

	\begin{equation}
		\mathbf{h_{k,T}}(n) =
		\begin{cases}
			%-1 & \mbox { if } \quad \textrm{rem}(T,n) < T/2 \\
            -1 & \mbox { if } \quad \textrm{rem}(T,n) \leq T/2 \\
			1  & \mbox { else }
		\end{cases},
  \quad \mbox{ for } n \in [N].
	\end{equation}


	In other words, $\mathbf{h_{k,T}}$ is a discretized square wave with amplitude $1$ and $k$ cycles of period $T$. See  \cref{fig:pulse_ex_appendix}.

 \begin{remark}\label{rk:hkT_per_sum_0}
 Since $\mathbf{h}_{k,T}$ is periodic and centered around $0$, for $i , n \in \mathbf{Z}_{\geq 0}$, 
     $\sum_{j=iT+1}^{nT}  h_{k,T}(j) = 0.$ 
     \iftoggle{long}{
     $=(k-n) \sum_{j=1}^{T}  h_{k,T}(j) = (k-n) \left( \sum_{j=1}^{\frac{T}{2}} (-1) + \sum_{j=\frac{T}{2}+1}^{T} (1) \right)=0$
     }.
 \end{remark}

\end{definition}


\begin{figure}[ht]
	\begin{tikzpicture}
		\centering
		\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
			\addplot[ycomb,color=black,solid,mark=*]
			plot coordinates{
					(1,1)
					(2,1)
					(3,1)
					(4,1)
					(5,1)
					(6,-1)
					(7,-1)
					(8,-1)
					(9,-1)
					(10,-1)

					(11,1)
					(12,1)
					(13,1)
					(14,1)
					(15,1)
					(16,-1)
					(17,-1)
					(18,-1)
					(19,-1)
					(20,-1)

					(21,1)
					(22,1)
					(23,1)
					(24,1)
					(25,1)
					(26,-1)
					(27,-1)
					(28,-1)
					(29,-1)
					(30,-1)

					(31,1)
					(32,1)
					(33,1)
					(34,1)
					(35,1)
					(36,-1)
					(37,-1)
					(38,-1)
					(39,-1)
					(40,-1)
				};
		\end{axis}
	\end{tikzpicture}
	\caption{Noiseless square wave $y=h_{k,T}$ with $k=4$ cycles and period $T=10$. The number of samples is $N=40$. Note the training samples are ordered in descending order, so to correspond to the labels $y$, the elements of $h_{k,T}$ are plotted from right to left.}
	\label{fig:pulse_ex_appendix}
\end{figure}


\begin{lemma}\label{lemma:A^Th_k,T}
	The $L=2$ layer sign activation dictionary applied to the square wave is, for $n \in [N]$,

	\begin{equation}\label{eq:A^Th_k,Tn_cases}
		(\mathbf{A}^T \mathbf{h_{k,T}})_n = 2 \cdot
		\begin{cases}
			-\mathrm{Rem}(n,T)   & \mbox{ if }  \mathrm{Rem}(n,T) \leq \frac{T}{2} \\
			\mathrm{Rem}(n,T) - T & \mbox{ else } %\quad  T/2 \leq \mathrm{rem}(n,T) \leq T \\
		\end{cases}
  = 2
  	\begin{cases}
			-\mathrm{rem}(n,T)     & \mbox{ if }  \mathrm{rem}(n,T) \leq \frac{T}{2} \\
			 \mathrm{rem}(n,T) - T& \mbox{ else } %\quad  T/2 \leq \mathrm{rem}(n,T) \leq T \\
		\end{cases}.
	\end{equation}

	We can also rewrite \eqref{eq:A^Th_k,Tn_cases} compactly as follows.
\iftoggle{long}{	Since $(A^T h_{k,T})_n $ is the same whether $\mathrm{rem}(n,T)$  is $0 $ or $T$ in equation \eqref{eq:A^Th_k,Tn_cases}, the remainder can be defined to be in the range from $0$ to the divisor minus $1$, or from $1$ to the divisor.
	Let the quotient $q_n = \frac{n-\textrm{rem}(n,\frac{T}{2})}{\frac{T}{2}}$  be the half-cycle containing index $n$, where we define the remainder to satisfy $\textrm{rem}(n,\frac{T}{2}) \in [\frac{T}{2}]$. \\
 }
Let $q_n = \mathrm{quot}\left(n,\frac{T}{2}\right) \in \{0, \cdots, 2k-1\}$. Then,

	\begin{equation}\label{eq:A^Th_k,Tn_simp}
		\begin{aligned}
			( \mathbf{A}^T \mathbf{h_{k,T}})_n= 2  (-1)^{q_n+1} \mathrm{rem}\left(n,\frac{T}{2}\right)
			-\mathbf{1}\{q_n \textrm{ odd}\} T .
		\end{aligned}
	\end{equation}
\end{lemma}

\begin{proof}

\iftoggle{long}{
	Denote the remainder when $n$ is divided by $T$  as $ \mathrm{rem}(n,T)$ (the period $T$ is implicit) and let $Q_n = \frac{n-\mathrm{rem}(n,T)}{T}$ be the quotient. So $n$ falls in the $q_n^{th}$ cycle of $h_{n,T}$. \\
 }

 Let $Q_n = \textrm{Quot}(n,T) \in \{0, \cdots, k\}$. So $n = Q_n T + \mathrm{Rem}(n,T)$. Note $Q_n = k$ only if $n=N$.
	For $n \in [N]$, by \cref{rk:A^Ty} (with $\mathbf{y} = \mathbf{h_{k,T}}$) and \cref{rk:hkT_per_sum_0}, 

	\begin{equation}\label{eq:A^Thw}
		\begin{aligned}
			\left( \mathbf{A}^T \mathbf{h_{k,T}} \right)_n & =
			\sum_{j=1}^n \mathbf{h_{k,T}}(j)  - \sum_{j=n+1}^N \mathbf{h_{k,T}}(j)                                          \\
			                & =  \left( \sum_{j=1}^{Q_n T}  \mathbf{h_{k,T}}(j)
			+ \sum_{j=Q_nT+1}^{n}  \mathbf{h_{k,T}}(j) \right)
			- \left( \sum_{j=n+1}^{ (Q_n+1) T} \mathbf{h_{k,T}} (j) +   \sum_{j=(Q_n+1) T + 1}^{ k T} \mathbf{h_{k,T}} (j)  \right) \mathbf{1} \{n < N\}\\
			                & = \sum_{j=Q_n T+1}^{n}  \mathbf{h_{k,T}}(j)
			-   \left( \sum_{j=n+1}^{ (Q_n+1) T} \mathbf{h_{k,T}} (j) \right) \mathbf{1} \{n < N\} .                          
		\end{aligned}
	\end{equation}

If $\mathrm{Rem}(n,T) >0$, then  $\mathrm{Rem}(n,T) = \mathrm{rem}(n,T) \in [T-1]$, and $n < N$.
Specifically, if $1 \leq \mathrm{Rem}(n,T) \leq T/2$ then,

	\begin{equation}\label{eq:Rem<T/2}
		\begin{aligned}\
			(\mathbf{A}^T \mathbf{h_{k,T}})_n
			 & = \sum_{j=Q_nT+1}^{n}  h_{k,T}(j) - \left( \sum_{j=n+1}^{ Q_n T+T/2}  h_{k,T}(j)
			+  \sum_{j= Q_n T+T/2 +1}^{ (Q_n + 1) T} h_{k,T} (j) \right)                                   \\
			 & = \sum_{j= Q_n T+1}^{n} (-1) - \left( \sum_{j=n+1}^{ Q_n T+T/2} (-1 )
			+  \sum_{j= Q_n T+T/2 +1}^{ (Q_n+1) T} (1 )\right)                                           \\
			 & = -\mathrm{Rem}(n,T) - \left( -(\frac{T}{2}- \mathrm{Rem}(n,T)) + \frac{T}{2} \right)                  \\
			 & = -2 \mathrm{Rem}(n,T).
		\end{aligned}
	\end{equation}

	Similarly if $T/2 + 1 \leq \mathrm{Rem}(n,T) \leq T-1$ then,


	\begin{equation}\label{eq:Rem>T/2}
		\begin{aligned}
			A^T (h_{k,T})_n
			 & = \sum_{j=Q_n T+1}^{Q_n T + T/2}  h_{k,T}(j) + \sum_{j=Q_n T + T/2 +1}^{n}  h_{k,T}(j) - \sum_{j=n+1}^{(Q_n + 1) T} h_{k,T} \\
			 & = \sum_{j=Q_n T+1}^{Q_n T + T/2}  (-1) + \sum_{j=Q_n T + T/2 +1}^{n}  (1) - \sum_{j=n+1}^{(Q_n + 1) T} (1)                  \\
			 & = -\frac{T}{2} + \left(\mathrm{Rem}(n,T) - \frac{T}{2} \right) - (T- \mathrm{Rem}(n,T))                                                                   \\
			 & = -2 T + 2\mathrm{Rem}(n,T).
		\end{aligned}
	\end{equation}

When Rem$(n,T)=0$, we have rem$(n,T)=T$, ie $n = Q_n T$, so \eqref{eq:A^Thw} implies that $\left( \mathbf{A}^T \mathbf{h_{k,T}} \right)_n = 0 = -2\mathrm{Rem}(n,T) = 2(\mathrm{rem}(n,T)-T)$.
Combining this with \eqref{eq:Rem<T/2} and \eqref{eq:Rem>T/2} proves \eqref{eq:A^Th_k,Tn_cases}. 

To show \eqref{eq:A^Th_k,Tn_simp}, observe if $ \mathrm{rem}(n,T) \leq \frac{T}{2}$, then $q_n$ is even and rem$(n,T) = \mathrm{rem}\left(n,\frac{T}{2}\right)$.
If $\frac{T}{2} < \mathrm{rem}(n,T) < T$, then $q_n$ is odd and $\mathrm{rem}(n,T)= \frac{T}{2} + \mathrm{rem}(n,\frac{T}{2})$. So if $\mathrm{rem}(n,T) < T$ then \eqref{eq:A^Th_k,Tn_simp} is equivalent to \eqref{eq:A^Th_k,Tn_cases}. If $\mathrm{rem}(n,T)=T$, then $q_n$ is odd and $\mathrm{rem}(n,\frac{T}{2}) = \frac{T}{2}$ and so the expression in \eqref{eq:A^Th_k,Tn_simp} evaluates to $0$, which is consistent with \eqref{eq:A^Th_k,Tn_cases}.
\end{proof}

\begin{definition}
	Let $i \in [N], s \in \mathbb{R}$. Define the impulse noise vector $\delta_{s,i} \in \mathbb{R}^N$ by its $n^{\textrm{th}}$ element as, 

	\begin{equation}\label{def:delta_si}
		\delta_{s,i}(n) :=
		\begin{cases}
			s & \mbox { if } \quad n = i \\
			0 & \mbox { else }.
		\end{cases},
 \quad n \in [N].
	\end{equation}

\end{definition}

%Define the vector $w_i \in \{-1,1\}^N$ which when multiplied elementwise to a vector changes the element at index $i$ to $s$. For $j \in [N]$, 

%\begin{equation}
%    w_{s,i}(j) := 
%    \begin{cases}
%        s &\mbox { if } \quad j \in [I] \\
%        1  &\mbox { else }.
%    \end{cases}
%\end{equation}

\begin{observation}

	If $s=0$ then for any $i \in [N]$, adding the vector $\delta_{s,i}$ to the label vector $y$ does not change $y$, and $\delta_{s,i}$ represents zero noise. If $y=h_{k,T}$, $i \in [N]$ and $s=-2y_i$ then adding $\delta_{s,i}$ to $y$ flips the sign of $y_i$.

\end{observation}

\begin{figure}[ht]
	\begin{tikzpicture}
		\centering
		\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
			\addplot[ycomb,color=black,solid,mark=*]
			plot coordinates{
					(1,1)
					(2,1)
					(3,1)
					(4,1)
					(5,1)
					(6,-1)
					(7,-1)
					(8,-1)
					(9,-1)
					(10,-1)

					(11,1)
					(12,1)
					(13,1)
					(14,1)
					(15,1)
					(16,-1)
					(17,-1)
					(18,-1)
					(19,-1)
					(20,-1)

					(21,1)
					(22,1)
					(23,1)
					(24,0.5)
					(25,1)
					(26,-1)
					(27,-1)
					(28,-1)
					(29,-1)
					(30,-1)

					(31,1)
					(32,1)
					(33,1)
					(34,1)
					(35,1)
					(36,-1)
					(37,-1)
					(38,-1)
					(39,-1)
					(40,-1)
				};

			%special point
			\addplot[ycomb, color=red,solid,mark=*]
			plot coordinates{
					(24,0.5)
				};

		\end{axis}
	\end{tikzpicture}
	\caption{Noisy square wave $y=h_{k,T}$ with $k=4$ cycles and period $T=10$, and additive noise $\delta_{s,i}$ at index $i=17$ and amplitude $s=-0.5$. The number of samples is $N=40$. Note the training samples are ordered in descending order, so to correspond to the labels $y$, the elements of $h_{k,T}$ are plotted from right to left.}
	\label{fig:pulse_ex_noise}
\end{figure}

%If $s=1$ then for any $i \in [N]$, $w_{s,i} = \mathbf{1}$ does not change the vector it multiplies, acting as no noise.
%%When multiplied to $h_{k,T}$, $w_I$ acts as a bit flip noise, switching $-1$ to $1$ or $1 $ to $-1$ at the locations specified by $I$.  
%For vectors $w,h \in \mathbb{R}^N$, denote $w \cdot h \in \mathbb{R}^N$ to be the elementwise product of $w$ and $h$. For index $i \in [N]$, let $q_i$ be the period of $h_{k,T}$ it occurs in, ie $i=q_iT+r_i$ where $0 \leq r_i = \mathrm{rem}(T,i) < T$. Note $kT=N$, and the sum of elements of $h_{kT}$ over any period, or consecutive $T$ indices, is $0$. If $n \leq i$ then $q_n \leq q_i$. We get,


\begin{lemma}\label{lemma:A^Tdelta_si}
	For $n \in [N], s\in \mathbb{R}$, the $L=2$ layer sign activation dictionary matrix applied to the impulse noise $\delta_{s,i}$ is

	\begin{equation}
		\begin{aligned}
			(A^T\delta_{s,i})_n & =
			\begin{cases}
				-s & \textrm{ if } n < i \\
				s  & \textrm{ else }     \\
			\end{cases}
		\end{aligned}
	\end{equation}


\end{lemma}

\begin{proof}
	Apply \cref{rk:A^Ty} to $\delta_{s,i}$ as defined in equation \eqref{def:delta_si}.
\end{proof}

\begin{lemma}\label{}
	Suppose $y=h_{k,T}+\delta_{s,i}$. In other words, the label vector $y$ consists of a square wave $h_{k,T}$ possibly corrupted by noise at a single index $i \in [N]$. Then the $L=2$ layer sign activation dictionary matrix applied to the labels is given by, for $n \in [N]$,

	\begin{equation}
		\begin{aligned}
			(A^T y)_n & =
			\begin{cases}
				(A^T h_{k,T})_n -s \textrm{ if } n < i \\
				(A^T h_{k,T})_n +s \textrm{ if } n \geq i
			\end{cases} \\
			          & = s \sigma(n-i) + 2 \cdot
			\begin{cases}
				-\mathrm{rem}(n,T)    & \mathrm{ if }  \quad 0 \leq \mathrm{rem}(n,T) \leq T/2 \\
				\mathrm{rem}(n,T) - T & \mathrm{ if } \quad  T/2 \leq \mathrm{rem}(n,T) \leq T \\
			\end{cases}
		\end{aligned}
	\end{equation}

	where $\sigma(x)$ is $1$ if $x\geq 0$ and $-1$ otherwise.
\end{lemma}



\begin{proof}
	Observe
	\begin{equation}
		A^T y
		= A^T h_{k,T} + A^T\delta_{s,i}
	\end{equation}
	Apply lemma \ref{lemma:A^Tdelta_si} and lemma \ref{lemma:A^Th_k,T}.
\end{proof}

\begin{figure}[ht]
	\begin{tikzpicture}
		\centering
		\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
			\addplot[ycomb,color=black,solid,mark=*]
			plot coordinates{
					(1,+0.5)
					(2,-2+0.5)
					(3,-4+0.5)
					(4,-6+0.5)
					(5,-8+0.5)
					(6,-10+0.5)
					(7,-8+0.5)
					(8,-6+0.5)
					(9,-4+0.5)
					(10,-2+0.5)
					(11,+0.5)

					(12,-2+0.5)
					(13,-4+0.5)
					(14,-6+0.5)
					(15,-8+0.5)
					(16,-10+0.5)
					(17,-8+0.5)
					(18,-6+0.5)
					(19,-4+0.5)
					(20,-2+0.5)

					(21,+0.5)
					(22,-2+0.5)
					(23,-4+0.5)
					(24,-6+0.5)
					(25,-8-0.5)
					(26,-10-0.5)
					(27,-8-0.5)
					(28,-6-0.5)
					(29,-4-0.5)
					(30,-2-0.5)

					(31,-0.5)
					(32,-2.5)
					(33,-4.5)
					(34,-6.5)
					(35,-8.5)
					(36,-10-0.5)
					(37,-8-0.5)
					(38,-6-0.5)
					(39,-4-0.5)
					(40,-2-0.5)
				};

			%special point
			\addplot[ycomb, color=red,solid,mark=*]
			plot coordinates{
					(24,-6+0.5)
				};

		\end{axis}
	\end{tikzpicture}
	\caption{$A^Ty$ when $y=h_{k,T}+\delta_{s,i}$ with $k=4$ cycles and period $T=10$, and additive noise $\delta_{s,i}$ at index $i=17$ and amplitude $s=-0.5$. The number of samples is $N=40$. Note the training samples are ordered in descending order, so to correspond to the labels $y$, the elements of $h_{k,T}$ are plotted from right to left.}
	\label{fig:A^T(h+delta)}
\end{figure}

\iftoggle{long}{
\begin{definition}
	For $i \in [N]$, let $e_i \in \mathbb{R}^N$ denote the $i^{th}$ canonical basis vector. For $j \in [N]$,

	\begin{equation}
		\begin{aligned}
			e_i(j) & = \begin{cases}
				           1 & \textrm{ if } i=j \\
				           0 & \textrm{ else }
			           \end{cases}
		\end{aligned}
	\end{equation}
\end{definition}
}

\begin{figure}[ht]
	\begin{tikzpicture}
		\centering
		\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
			\addplot[ycomb,color=black,solid,mark=*]
			plot coordinates{
					(1,0.8)
					(2,0.8)
					(3,0.8)
					(4,0.8)
					(5,0.8)
					(6,-0.6)
					(7,-0.6)
					(8,-0.6)
					(9,-0.6)
					(10,-0.6)

					(11,0.6)
					(12,0.6)
					(13,0.6)
					(14,0.6)
					(15,0.6)
					(16,-0.6)
					(17,-0.6)
					(18,-0.6)
					(19,-0.6)
					(20,-0.6)

					(21,0.6-0.1)
					(22,0.6-0.1)
					(23,0.6-0.1)
					(24,0.6-0.1)
					(25,0.6-0.1)

					(26,-0.6)
					(27,-0.6)
					(28,-0.6)
					(29,-0.6)
					(30,-0.6)

					(31,0.6)
					(32,0.6)
					(33,0.6)
					(34,0.6)
					(35,0.6)
					(36,-0.8)
					(37,-0.8)
					(38,-0.8)
					(39,-0.8)
					(40,-0.8)
				};

			%special point
			\addplot[ycomb, color=red,solid,mark=*]
			plot coordinates{
					(21,0.6-0.1)
					(22,0.6-0.1)
					(23,0.6-0.1)
					(24,0.6-0.1)
					(25,0.6-0.1)
				};

		\end{axis}
	\end{tikzpicture}
	\caption{LASSO solution with $\beta=2$, and the labels being the noisy square wave $y=h_{k,T}$ with $k=4$ cycles and period $T=10$, and additive noise $\delta_{s,i}$ at index $i=17$ and amplitude $s=-0.5$. The number of samples is $N=40$. Note the training samples are ordered in descending order, so to correspond to the labels $y$, the elements of $h_{k,T}$ are plotted from right to left. The magnitude of the first and last half-cycles are $-2w_{bdry}-w_{cycle} = 1-\frac{\beta}{T}=1-\frac{2}{10}=0.8$. The magnitude of the middle cycles (excluding the first, last, and noise-contaminated cycle) are $w_{cycle}=1-2\frac{\beta}{T}=1-2\frac{2}{T}=0.6$.} Note the half-cycle containing noise is $q_i=3$. The magnitude of the noise cycle is $w_{cycle} + 2 w_{noise}= 1-2\frac{\beta}{T}+(-1)^{q_i+1}2\frac{s}{T}=1-2\frac{\beta}{T}+(-1)^{3+1}2\frac{(-0.5)}{10}=1-\frac{4}{10}-\frac{1}{10}=0.5$.
	\label{fig:pulse_ex_noise_sol}
\end{figure}

\begin{definition}\label{def:q_i}
	Given the label vector $y = h_{k,T}+\delta{s,i}$, let $q_i = \frac{i -\textrm{rem}(\frac{T}{2}, i) }{T/2}$ be the half-cycle of $y$ that contains the noise at index $i$.
\end{definition}

\begin{lemma}\label{lemma:switch_ay}
	Let $m \in \mathbb{N}$.
 \iftoggle{long}{Let $\mathbf{y} \in \mathbb{R}^N$.}
  For $\mathbf{v} \in \mathbb{R}^N$, let $\mathcal{I}(\mathbf{v}) = \{i \in \{2,\cdots,N\}: 0 \neq \mbox{sign}(\mathbf{v}_{i-1}) \neq \mbox{sign}(\mathbf{v}_i) \neq 0\}$ be the set of indices at which $\mathbf{v}$ switches sign. Let $\mathcal{A} = \{\mathbf{a} \in \{-1,1\}^N: \mbox{sign}(\mathbf{a}_1)= \mbox{sign}(\mathbf{y}_1), |\mathcal{I}(\mathbf{a})| \leq m \}$ be a set of vectors with at most $m$ switches and having the same sign as $\mathbf{y}$ in the first element. Suppose $\mathbf{a} \in \mbox{argmax}_{\mathbf{a} \in \mathcal{A}}\mathbf{y}^T \mathbf{a}$. Then for every index $i \in \mathcal{I}(\mathbf{a})$, if $\mathbf{y}_i \neq 0 \neq \mathbf{y}_{i-1}$ then $i \in \mathcal{I}(\mathbf{y})$.
\end{lemma}

 \cref{lemma:switch_ay} states that a vector $\mathbf{a}$ that maximizes $\mathbf{y}^T\mathbf{a}$ must switch sign only at indices that $\mathbf{y}$ also switches sign.

\begin{proof}
	Suppose to the contrary there was an index $i \in \mathcal{I}(\mathbf{a}) \cap \mathcal{I}(\mathbf{y})^c$ such that $\mathbf{y}_i \neq 0 \neq \mathbf{y}_{i-1}$. In other words, $\mathbf{a}$ switches sign at index $i$ but $\mathbf{y}$ does not. First, observe that for $j \in \{2, \cdots, N-1\}$, if $\mbox{sign}(\mathbf{a}_j)\neq\mbox{sign}(\mathbf{a}_{j-1})$ or $\mbox{sign}(\mathbf{a}_j)\neq\mbox{sign}(\mathbf{a}_{j+1})$ then flipping the sign of $\mathbf{a}_j$ does not increase the number of switches of $\mathbf{a}$; it merely shifts an index at which $\mathbf{a}$ switches sign. Next, for $k \in [N]$, let $\mathbf{a^{(k)}}$ be the same vector as $\mathbf{a}$ but with its $k^{\textrm{th}}$ element negated: $\mathbf{a^{(k)}}_i=\mathbf{a}_i$ for $i \neq k$ and  $\mathbf{a^{(k)}}_k=-\mathbf{a}_k$. Consider two cases: 

	\textbf{Case 1: $\mbox{sign}(\mathbf{a}_i) \neq \mbox{sign}(\mathbf{y}_i)$}

	%Let $\Tilde{\mathbf{a}}=\mathbf{a^{(i)}}$. %be the same vector as $\mathbf{a}$ but with its $i^{\textrm{th}}$ element negated: $\Tilde{\mathbf{a}}_j=\mathbf{a}_j$ for $j \neq i$ and  $\Tilde{\mathbf{a}}_i=-\mathbf{a}_i$. 
 Since $\mbox{sign}(\mathbf{a}_i) \neq \mbox{sign}(\mathbf{a}_{i-1})$, $|\mathcal{I}(\mathbf{a^{(i)}})| \leq |\mathcal{I}(\mathbf{a})| \leq m $. Observe $\mathbf{y}_i \mathbf{a}_i < 0$. Therefore $\mathbf{y}^T \mathbf{a^{(i)}} =  \left(\sum_{j \neq i} \mathbf{y}_j \mathbf{a}_j \right) - \mathbf{y}_i \mathbf{a}_i = \mathbf{y}^T \mathbf{a} - 2\mathbf{y}_i \mathbf{a}_i > \mathbf{y}^T \mathbf{a}$, contradicting $\mathbf{a} \in \mbox{argmax}_{\mathbf{a} \in \mathcal{A}}\mathbf{y}^T \mathbf{a}$.

	\textbf{Case 2: $\mbox{sign}(\mathbf{a}_i) = \mbox{sign}(\mathbf{y}_i)$}

	Since $i \notin \mathcal{I}(\mathbf{y})$ but $i \in \mathcal{I}(\mathbf{a})$ and $\mathbf{y}_i \neq 0 \neq \mathbf{y}_{i-1}$, we have $\mbox{sign}(\mathbf{y}_{i-1})=\mbox{sign}(\mathbf{y}_{i})=\mbox{sign}(\mathbf{a}_i)=-\mbox{sign}(\mathbf{a}_{i-1})$.  
 %Let $\Tilde{\mathbf{a}}=\mathbf{a^{(i-1)}}$.
 %be $\mathbf{a}$ but with $\mathbf{a}_{i-1}$ negated: $\Tilde{a}_j=a_j$ for $j \neq i-1$ and  $\Tilde{a}_{i-1}=-a_{i-1}$. 
 Since 
 \iftoggle{long}{
 $\mbox{sign}(\mathbf{a}_{1+(i-1)}) = $ 
 }
 $\mbox{sign} \left(\mathbf{a}_{i} \right)  \neq \mbox{sign} \left(\mathbf{a}_{(i-1)} \right)$, $|\mathcal{I}(\mathbf{a^{(i-1)}})| \leq \mathcal{I}(\mathbf{a})\leq m $. And $\mathbf{y}_{i-1} \mathbf{a}_{i-1} < 0$. Therefore  $y^T \mathbf{a^{(i-1)}} = \sum_{j \neq i-1} \mathbf{y}_j \mathbf{a}_j - \mathbf{y}_{i-1} \mathbf{a}_{i-1} = \mathbf{y}^T \mathbf{a} - 2 \mathbf{y}_{i-1}\mathbf{a}_{i-1} > \mathbf{y}^T \mathbf{a}$, a contradiction.
 \iftoggle{long}{
 , contradicting $a \in \mbox{argmax}_{a \in \mathcal{A}}y^T a$.}

	%  Let $i = \min \{ \mathcal{I}(a) \cap \mathcal{I}(y)^c \}$ be the smallest index in $ \{2, \cdots, N\}$, where $a$ switches but $y$ does not. Then $a_{i-1}<0, a_i >0$.
\end{proof}

\begin{remark}
	By a similar argument, \cref{lemma:switch_ay} also holds for minimizing $\mathbf{a}^T \mathbf{y}$.
\end{remark}

%\begin{lemma}
%  Let $\mathcal{I}$, $\mathcal{A}$, $y$ be defined as in lemma \ref{def:q_i}. Let $a \in \{-1,1\}^N$. We can perform the following steps to generate $\Tilde{a} \in \{-1,1\}^N$ such that $\Tilde{a}^T y = a^T y$, $|\mathcal{I}(\Tilde{a})| \leq \mathcal{I}(a)\leq m $ and if $i \in \mathcal{I}(\Tilde{a})$ then $y_{i} \neq 0$.    
%\end{lemma}

%\begin{proof}
%    Let $i_n$ be the $n^{th}$ smallest index in $\mathcal{I}$. Let $i_0 = 1$. For indices $n = 1, 2, \cdots, |\mathcal{I}|$ in ascending order, by definition of $\mathcal{I}$ we have $-\mbox{sign}(a_{i_n }) = \mbox{sign}(a_{i_n -1}) = \mbox{sign}(a_{j}) $ for all indices $j \in \{i_{n-1}, \cdots, i_n -1\}$. Let $a^0 = a$. We will inductively define $a^n$ for $n = 1, 2, \cdots, |\mathcal{I}|$. 


%    Let $P_n$ be the statement that ``$a^{n-1}$ satisfies ${a^{n-1}}^t y = a^T y$, $|\mathcal{I}(a^{n-1})| \leq \mathcal{I}(a)$ and if $i \in [n-1]$ then $y_{i_n} \neq 0$." Note $a^0$ satisfies $P_0$. \\

%    Now, we define $a^n$. Let $n \geq 1$. Suppose $a^{n-1}$ is a vector in $\{-1,1\}^N$ satisfying $P_{n-1}$.

%    If $y_{i_n} \neq 0$, let $a^n = a^{n-1}$. Otherwise, perform the following steps. Let $j = \min\{j \in \{i_{n-1}, \cdots i_n\}: \forall k \in \{j, \cdots, i_n\}, y_k =0\}$ be the smallest index over which $y_{i_n }= \cdots = y_j = 0$.  Let $a^n_j = \cdots = a^n_{i_n} = a_{i_n}$, and let $a^n_k = a^{n-1}_k$ at all other indices $k$. Note $j \neq i_{n-1}$ by $P_{n-1}$. This removed a switch at $i_n$ from $a^{n-1}$ and inserted a switch at $j > i_{n-1}$, so $|\mathcal{I}(a^{n})| \leq |\mathcal{I}(a^{n-1})| \leq \mathcal{I}(a)$. In addition, $a^n$ differs from $a^{n-1}$ only at indices where $y$ was $0$, so ${a^{n}}^T y = {a^{n-1}}^T y = a^T y$. Finally, by definition of $j$, $y_{j}$ \textcolor{red}{uhh there is a switch here but that is okay, cannot avoid, what we want? revise statement.}

%\end{proof}



\subsection{critical $\beta$ for $2$-layer networks}

\begin{lemma}\label{lemma:2lyr_critbeta>=}
	Let $T>2$. Suppose $s > -1$ if $q_i$ is odd and $s<1$ if $q_i$ is even. Suppose the label $y=h_{k,T}+\delta_{s,i}$ is a noisy square wave with $k \geq 3 $ cycles. Let $q_i \in \{0, \cdots, 2k-1\}$ be the quotient when noise index $i$ is divided by $\frac{T}{2}$. Suppose $3 \geq q_i \leq 2k-2$. In other words, the noise is not in the first three half cycles or the last half-cycle.  Let $\beta_c = T - |s|$. If $\beta < \beta_c$ then the optimal bidual variable is $z=\mathbf{0}$, and the neural net is the constant zero function.
\end{lemma}

\begin{proof}
	Let $\mathbf{A}_n$ be the $n^{\textrm{th}}$ column of the dictionary matrix $\mathbf{A}$. By \cref{rk:hkT_per_sum_0}, $\mathbf{1}^T \mathbf{h_{k,T}}=0$. Therefore by \cref{rk:A^Ty}, $|\mathbf{A}_N^T \mathbf{y}| = |\mathbf{1}^T \mathbf{y}| = |\mathbf{1}^T(h_{k,T} + \delta_{s,i})|= |s|$. Consider columns $\mathbf{A}_j$ of $\mathbf{A}$ for $j \in [N-1]$. By  \cref{lemma:switch_ay},  $|\mathbf{A}_j^T \mathbf{y}|$ is maximized if $\mathbf{A}_j$ switches at a switching index of $\mathbf{y}$. Since  $s > -1$ if $q_i$ is odd and $s<1$ if $q_i$ is even, $\mbox{sign}(\mathbf{y})=\mbox{sign}(\mathbf{h_{k,T}})$. So the switchpoints of $\mathbf{y}$ are the same as the switchpoints of $\mathbf{ h_{k,T}}$, which are at multiples of $\frac{T}{2}$. Let $q_j  \in \{0, \cdots, 2k-1\}$ be the quotient when $j$ is divided by $\frac{T}{2}$. For $j$ being a multiple of $\frac{T}{2}$,

	\begin{align*}
		y^T a_j & = (h_{k,T} + \delta_{s,i})^T a_j                                                                                                                                            \\
		        & = h_{k,T}^T a_j + \delta_{s,i}^T a_j                                                                                                                                        \\
		        & = \begin{cases}
			            \frac{T}{2}(1) + \frac{T}{2}(1) + \frac{N-T}{2}(\frac{T}{2}(1) +  \frac{T}{2}(-1) ) + s(-1)^{\mathbf{1}_{q_j\geq q_i}} & \mbox{ if } q_j \mbox { odd } \\
			            \frac{N}{2}(\frac{T}{2}(1) +  \frac{T}{2}(-1) )  + s(-1)^{\mathbf{1}_{q_j\geq q_i}}                                    & \mbox{ if } q_j \mbox {even } \\
		            \end{cases} \\
		        & = \begin{cases}
			            T + s(-1)^{\mathbf{1}_{q_j\geq q_i}} & \mbox{ if } q_j \mbox { odd }   \\
			            s(-1)^{\mathbf{1}_{q_j\geq q_i}}     & \mbox{ if } q_j \mbox { even }.
		            \end{cases}
	\end{align*}

	If $s>0$, since the half cycle $q_i\geq 3$, there exists an odd half cycle $q_j<q_i$, so that $y^Ta_j = T+s=T+|s|$, the largest it can be.

	If $s<0$, since the half cycle $q_i \leq 2k-2$, there exists an odd half cycle $q_j \geq q_i$, so that $y^Ta_j = T-s=T+|s|$, the largest it can be.

	The smallest $y^Ta_j$ can be is $-s$, and $|-s|=|s|<T+|s|$. So the largest $|y^Ta_j|$ can be is $T+|s|$.

	%Since $q_i < k$, if there exists an even half cycle $q_j \geq q_i$ then $y^T a_j = -s$, the smallest it can be.
	%So $\max_j y^T a_j = T+s$.

	%The largest $y^Ta_j$ can be is $T+s$, 

	%Since $T > 2$, $T+ s(-1)^{\mathbf{1}_{q_j\geq q_i}} \in \{T-s, T+s\} \subset [2-s,\infty)$.
	%which is maximized in absolute value \textcolor{red}{(absolute value is the positive?)} by $j$ being an odd multiple of $\frac{T}{2}$ such that $q_n < q_i$ if $s>0$ and $q_n > q_i$ if $s>0$.
	So the critical $\beta$ is $\max_{j \in [N]} |a_j^T y| = T+|s|$.  \cite{Efron:2004}
\end{proof}

\begin{remark}
	If there is no noise, i.e. $s=0$, then lemma \ref{lemma:2lyr_critbeta>=} holds for $k=1$ cycle as well, as the proof is the same.
\end{remark}


\begin{lemma}\label{lemma:2lyr_sign_square_wave_big_beta}
	Suppose the error is not too large: $s > -1$ if $q_i$ is odd and $s<1$ if $q_i$ is even. And assume $y=h_{k,T}$ is a noiseless square wave of $k$ cycles of length $T$. Let $\beta_c = T$. If $\beta \geq \frac{\beta_c}{2} = \frac{T}{2}$ then the optimal bidual variable is

	\begin{equation}
		z = \frac{(\beta_c - \beta)_+}{2T}\left(e_{\frac{T}{2}} + e_{N-\frac{T}{2}}\right).
	\end{equation}

\end{lemma}

\begin{proof}
	By lemma \ref{lemma:2lyr_critbeta>=}, since the noise $s=0$, if $\beta \geq T = \beta_c$ then $z=0$ as desired.

	So assume $\beta \in [\frac{T}{2},T]$. Let $L(z) = \frac{1}{2}||Az-y||^2_2 + ||z||_1$. We will show the subgradient condition for optimality is satisfied, that $0 \in \partial(L)(z)$.

	First suppose $j \in \{\frac{T}{2}, N-\frac{T}{2}\}$. Since $j$ is an odd multiple of $\frac{T}{2}$ and the noise $s=0$, by the proof of lemma \ref{lemma:2lyr_critbeta>=}, $a_j^T y =T= \beta_c$.  Also, $z_j>0$. Therefore for $j \in \{\frac{T}{2}, N-\frac{T}{2}\}$,

	\begin{align*}
		(A^T(Az-y) + \beta \partial g(z))_j & = (A^T(Az-y))_j +\beta \partial g(z)_j                                                                           \\
		                                    & = a_j^T (Az-y) + \beta\partial g(z)_j                                                                            \\
		                                    & = a_j^T (\frac{1}{2T}(\beta_c - \beta)_+(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})-y) + \beta \partial g(z)_j         \\
		                                    & = a_j^T (\frac{1}{2T}(\beta_c - \beta)_+(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})) - a_j^T y + \beta \partial g(z)_j \\
		                                    & = (\frac{1}{2T}(\beta_c - \beta)_+(N+  a_{\frac{T}{2}}^T a_{N-\frac{T}{2}}))   -\beta_c + \beta                  \\
		                                    & = (\frac{1}{2T}(\beta_c - \beta)_+(N+ 2T-N) - \beta_c  + \beta                                                   \\
		                                    & = \frac{1}{2T}(\beta_c - \beta)_+(2T) - \beta_c  + \beta                                                         \\
		                                    & = 0 .
	\end{align*}

	Now, suppose $j \in [N]- \{\frac{T}{2}, N-\frac{T}{2}\}$. Then



	By equation \eqref{2lyr_z_betac}, $Az = \frac{(\beta_c - \beta)_+}{2T}(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})$.
	The vector $a_{\frac{T}{2}} + a_{N-\frac{T}{2}}$ is $2$ for the first $\frac{T}{2}$ indices, $0$ for the next $N-T$ indices, and then $-2$ for the last $\frac{T}{2}$ indices. So

	\begin{equation}\label{remark:2lyr_pred_betac}
		\begin{aligned}
			(Az)_j =\begin{cases}
				        \frac{(\beta_c - \beta)_+}{T}  & \mbox{if} j \leq \frac{T}{2}                  \\
				        0                              & \mbox{if} j \in [\frac{T}{2}+1,N-\frac{T}{2}] \\
				        -\frac{(\beta_c - \beta)_+}{T} & \mbox{if} j > N-\frac{T}{2}                   \\
			        \end{cases}
		\end{aligned}
	\end{equation}



	Let $q_j $ be the quotient when $j$ is divided by $\frac{T}{2}$. So index $j$ is in the $q_j^{th}$ half-cycle (where $h_{k,T}$ is negative), indexing from $0$. Note $a_1$, the first column of (negated) $A$ is $a_1 = (-1, 1, 1, \cdots, 1)^T$, which switches at index $2$. So $a_{\frac{T}{2}}$ switches at index $\frac{T}{2}+1$ and its first $\frac{T}{2}$ elements are $-1$, and the rest are $1$. Note $a_N = -\mathbf{1}$.

	\begin{equation}\label{eq:(Az-y)_j_critzone_beta_2lyr}
		\begin{aligned}
			(Az-y)_j =\begin{cases}
				          \frac{(\beta_c - \beta)_+}{T} -1\leq 0 & \mbox{if} j \leq \frac{T}{2}                  \\
				          (-1)^{q_j+1}                           & \mbox{if} j \in [\frac{T}{2}+1,N-\frac{T}{2}] \\
				          1-\frac{(\beta_c - \beta)_+}{T} \geq 0 & \mbox{if} j \geq N-\frac{T}{2} + 1            \\
			          \end{cases}
		\end{aligned}
	\end{equation}

	Note that  $(Az-y)$ contains zeros if and only if $\beta_c = \beta$, if and only if the set of its zero indices is $\mathcal{Z} = \{j:(Az-y)_j=0\} = \{1, \cdots, \frac{T}{2}\}\cup\{1+N-\frac{T}{2}, \cdots, N\}$. If $\beta_c = \beta$, for any $j \in \{1, \cdots, \frac{T}{2}\}$, $a_j^T y = a_{\frac{T}{2}}^T y$ and for any $j \in \{1+N-\frac{T}{2}, \cdots, N\}$, $a_j^T y = a_{1+N-\frac{T}{2}}^T y$, so for the purposes of maximizing $a_j^T (Az-y)$, if $j \in \mathcal{Z}$ it suffices to consider just $j \in \{ a_{\frac{T}{2}}, a_{1+N-\frac{T}{2}} \} $, which are still switch points of $Az-y$ in \eqref{eq:(Az-y)_j_critzone_beta_2lyr}. Note by symmetry $a_N^T (Az-y)=0$. Every other $a_j$ for $j \in [N-1]$ contains a single switch. Combining the $\beta_c = \beta$ case with lemma \ref{lemma:switch_ay}, $a_k^T (Az-y)$ is maximized if $a_j$ switches at a switch point of $Az-y$. By equation \eqref{eq:(Az-y)_j_critzone_beta_2lyr}, the switch points of $Az-y$ are at multiples of $\frac{T}{2}$. There are two cases, depending on if the switch point occurs at the beginning of an odd or even half cycle. For column $a_j$ of $A$, where $j$ is a multiple of $ \frac{T}{2}$,

	\begin{equation}
		\begin{aligned}
			|a_j^T(Az-y)| & =
			\begin{cases}
				 & \frac{T}{2}(\frac{(\beta_c - \beta)_+}{T}-1)(-1) + \frac{N-T}{2}(\frac{T}{2}(1)+\frac{T}{2}(-1)) + \frac{T}{2}(1-\frac{(\beta_c - \beta)_+}{T})(1)                                           \\ &\mbox{ if } q_j \mbox{ is odd} \\
				 & \frac{T}{2}(\frac{(\beta_c - \beta)_+}{T}-1)(1) + \frac{T}{2}(-1)(-1)+ \frac{T}{2}(1)(1) + \frac{N-2T}{2}(\frac{T}{2}(1)+\frac{T}{2}(-1)) + \frac{T}{2}(1-\frac{(\beta_c - \beta)_+}{T})(-1) \\ &\mbox{ if } q_j \mbox{ is even} \\
			\end{cases} \\
			              & =
			\begin{cases}
				T(1-\frac{(\beta_c - \beta)_+}{T})     & \mbox{ if } q_j \mbox{ is odd}  \\
				T - T(1-\frac{(\beta_c - \beta)_+}{T}) & \mbox{ if } q_j \mbox{ is even} \\
			\end{cases}                                                                                                                                                                     \\
			              & =
			\begin{cases}
				T-(\beta_c - \beta)_+ & \mbox{ if } q_j \mbox{ is odd}  \\
				(\beta_c - \beta)_+   & \mbox{ if } q_j \mbox{ is even} \\
			\end{cases}                                                                                                                                                                                      \\
			              & =
			\begin{cases}
				\beta    & \mbox{ if } q_j \mbox{ is odd}  \\
				T- \beta & \mbox{ if } q_j \mbox{ is even} \\
			\end{cases}
		\end{aligned}
	\end{equation}

	assuming $\beta \leq \beta_c$ and using that $\beta_c = T$ for $2$ layer sign networks.

	Therefore

	\begin{equation}
		\begin{aligned}
			\max_{j \in [N]} |a_j^T(Az-y)| & = \max \{\beta, T -\beta\}.
		\end{aligned}
	\end{equation}

	So $\max_{j \in [N]} |a_j^T(Az-y)| \leq \beta$ if
	$T - \beta \leq \beta \leq \beta_c$, ie $\frac{T}{2} \leq \beta \leq \beta_c $. So the critical region is $\beta \in [\frac{T}{2},T]$.

	Therefore if $\beta \in [\frac{T}{2},T]$ then $|| A^T(Az-y)||_{\infty} \leq \beta$ and hence $0 \in A^T(Az-y) + \beta [-1,1] = \partial L(z)_j$ for $j \in [N]-\{\frac{T}{2}, N-\frac{T}{2}\}$.

\end{proof}

\begin{remark}
	$z$ as defined in lemma \ref{eq:(Az-y)_j_critzone_beta_2lyr} is the minimizer


	\begin{align}\label{eq:subprob}
		\min \frac{1}{2}||\Tilde{A}\Tilde{z}-y||^2_2 + \beta \mathbf{1}^T \Tilde{z} ,
	\end{align}

	where  $\Tilde{A}=A\Tilde{I}$ is the submatrix of $A$, taking the columns with indices odd multiples of $\frac{T}{2}$, $\Tilde{z} = \Tilde{I}^Tz$ denotes a subvector $z$ with only the elements at every odd multiple of $\frac{T}{2}$. Indeed, \eqref{eq:subprob} is

	solved by setting the gradient to $0$:

	\begin{align*}
		\Tilde{A}^T(\Tilde{A}\tilde{z}-y) + \beta\mathbf{1} & =0                                                                 \\
		\tilde{z}                                           & = (\Tilde{A}^T\Tilde{A})^{-1}(\Tilde{A}^Ty-\beta\mathbf{1})        \\
		                                                    & =  (\Tilde{A}^T\Tilde{A})^{-1}(\beta_c \mathbf{1}-\beta\mathbf{1}) \\
		                                                    & (\beta_c - \beta)_+ (\Tilde{A}^T\Tilde{A})^{-1}\mathbf{1}.         \\
	\end{align*}

	To check that $\Tilde{z} \geq 0$ it suffices to show that $(\Tilde{A}^T\Tilde{A})^{-1}\mathbf{1} \geq 0$. Note $\Tilde{I}^T A^T A \Tilde{I}$ subsamples the matrix $A^TA$ at intervals of $T^{th}$ in the columns and then the rows starting at $\frac{T}{2}$.

	From equation \eqref{eq:A^TA_writtenout},

	\begin{equation}
		\setcounter{MaxMatrixCols}{20}
		\begin{aligned}
			\Tilde{I}^T A^T A \Tilde{I}
			 & =  \Tilde{I}^T\begin{pmatrix}
				                 N      & N-2    & N-4    & \cdots & 2      & 0      & -2     & \cdots & 6-N    & 4-N    & 2-N    \\
				                 N-2    & N      & N-2    & \cdots & 4      & 2      & 0      & \cdots & 8-N    & 6-N    & 4-N    \\
				                 N-4    & N-2    & N      & \cdots & 6      & 4      & 2      & \cdots & 10-N   & 8-N    & 6-N    \\
				                 \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
				                 6-N    & 8-N    & 10-N   & \cdots & 2      & 4      & 6      & \cdots & 8-N    & 6-N    & 4-N    \\
				                 4-N    & 6-N    & 8-N    & \cdots & 0      & 2      & 4      & \cdots & 6-N    & 4-N    & 2-N    \\
				                 2-N    & 4-N    & 6-N    & \cdots & -2     & 0      & 2      & \cdots & 4-N    & 2-N    & N
			                 \end{pmatrix}\Tilde{I} \\
			 & =  \begin{pmatrix}
				      N      & N-2T   & N-4T   & \cdots & 2T     & 0      & -2T    & \cdots & 6T-N   & 4T-N   & 2T-N   \\
				      N-2T   & N      & N-2T   & \cdots & 4T     & 2T     & 0      & \cdots & 8T-N   & 6T-N   & 4T-N   \\
				      N-4T   & N-2T   & N      & \cdots & 6T     & 4T     & 2T     & \cdots & 10T-N  & 8T-N   & 6T-N   \\
				      \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
				      6T-N   & 8T-N   & 10T-N  & \cdots & 2T     & 4T     & 6T     & \cdots & 8T-N   & 6T-N   & 4T-N   \\
				      4T-N   & 6T-N   & 8T-N   & \cdots & 0      & 2T     & 4T     & \cdots & 6T-N   & 4T-N   & 2T-N   \\
				      2T-N   & 4T-N   & 6T-N   & \cdots & -2T    & 0      & 2T     & \cdots & N-4T   & N-2T   & N
			      \end{pmatrix}            \\
		\end{aligned}
	\end{equation}

	which has inverse,

	\begin{equation}
		\setcounter{MaxMatrixCols}{20}
		\begin{aligned}
			(\Tilde{I}^T A^T A \Tilde{I})^{-1} & = \frac{1}{4T}
			\begin{pmatrix}
				2      & -1     & 0      & 0      & 0      & \cdots & 0      & 0      & 1      \\
				-1     & 2      & -1     & 0      & 0      & \cdots & 0      & 0      & 0      \\
				0      & -1     & 2      & -1     & 0      & \cdots & 0      & 0      & 0      \\
				0      & 0      & -1     & 2      & -1     & \cdots & 0      & 0      & 0      \\
				\vdots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
				0      & 0      & 0      & 0      & 0      & \cdots & -1     & 2      & -1     \\
				1      & 0      & 0      & 0      & 0      & \cdots & 0      & -1     & 2      \\
			\end{pmatrix}. \\
		\end{aligned}
	\end{equation}



	%Not on diagonal: $-(N-jT) + 2(N-(j+2)T) - (N-(j+4)T) = jT -2(j+2)T +(j+4)T = jT - 2jT -4T +jT + 4T = 0$. 


	So,

	\begin{equation}
		\begin{aligned}
			\Tilde{z} & = (\Tilde{I}^T A^T A \Tilde{I})^{-1}\mathbf{1} \\
			          & = \frac{1}{2T}
			\begin{pmatrix}
				1      \\
				0      \\
				\vdots \\
				0      \\
				1
			\end{pmatrix}
			          & \geq \mathbf{0}
		\end{aligned}
	\end{equation}

	as consistent with lemma \ref{eq:(Az-y)_j_critzone_beta_2lyr}.

\end{remark}



\subsection{pre-critical $\beta$ range for $2$-layer networks}

\begin{lemma}(Informal lemma \ref{lemma:lasso_sol_square_wave_noise}) \\
	Consider training a $2$ layer sign neural network with label vector a square wave of period $T$ corrupted by additive noise of magnitude $|s|$ at one point in the middle. Suppose the regularization parameter $\beta < \frac{T-|s|}{2}$. Then, the beginning of the half cycle of the square wave will produce active neurons. The predicted network will be a square wave of non-uniform amplitude, with the half-cycle that contained the noise modified in the direction of the noise.
\end{lemma}

\begin{lemma}\label{lemma:lasso_sol_square_wave_noise}
	Consider a $L=2$ layer neural network.
	Suppose $y = h_{k,T}+\delta{s,i}$ with $i \in [\frac{T}{2}, N-\frac{T}{2}]$. In other words, the label vector $y$ is a square wave $ h_{k,T}$ consisting of $k$ cycles of period length $T$, and corrupted by noise at a index $i$ that is not in the first or last half-cycle.


	Suppose $s<T$ if $(-1)^{q_i}, s$ have the same sign, where $q_i$ is defined in \ref{def:q_i}. %do we need this always? 



	Suppose the regularization parameter $\beta < \beta_u$, where the upper bound $\beta_u$ is

	\begin{equation}
		\begin{aligned}
			\beta_u & =
			\frac{1}{2}(T + \min \{ 0, (-1)^{q_i+1}s\})                                     \\
			        & = \begin{cases}
				            \frac{T}{2} \mbox{ if } (-1)^{q_i}, s_i \mbox{ have opposite sign } \\
				            \frac{T}{2} -\frac{|s|}{2} \mbox{ else }
			            \end{cases}
		\end{aligned}
	\end{equation}

	\textcolor{red}{check $q_i$ or $q_i+1$}

	Let

	%\begin{equation}
	%    \begin{aligned}
	%         w_{bdry} &= 2\left(1-\frac{3}{2}\frac{\beta}{T}\right)\\
	%         w_{cycle} &= 2(1-2\frac{\beta}{T}) \\
	%         w_{noise} &= -4 \frac{s}{T}
	%    \end{aligned}
	%\end{equation}

	\begin{equation}
		\begin{aligned}
			w_{bdry}  & = -\left(1-\frac{3}{2}\frac{\beta}{T}\right) < 0 \\
			w_{cycle} & = 1-2\frac{\beta}{T}>0                           \\
			w_{noise} & = (-1)^{q_i+1} \frac{s}{T}
		\end{aligned}
	\end{equation}

	Define the following vectors in $\mathbb{R}^N$.

	\begin{equation}
		\begin{aligned}
			z_{bdry}  & = w_{bdry}\left( e_{\frac{T}{2}} + e_{N-\frac{T}{2}}\right)                                     \\
			z_{cycle} & = w_{cycle} \sum_{j=2}^{2k-2} (-1)^{j}e_{j\frac{T}{2}}                                          \\
			z_{noise} & = w_{noise}\left((-1)^{q_i} e_{q_i \frac{T}{2}} + (-1)^{q_i+1} e_{(q_i+1) \frac{T}{2}} \right). \\
			%z_{noise} &= 2\left(1-2\frac{(\beta+1)}{T}\right)\left((-1)^{q_i} e_{q_i \frac{T}{2}} + (-1)^{q_i+1} e_{(q_i+1) \frac{T}{2}} \right) \\
		\end{aligned}
	\end{equation}



	Let $z = z_{bdry}+z_{cycle}+z_{noise}$.

	Then $0 \in A^T(Az-y) + \beta \partial g(z)$.
\end{lemma}

\begin{remark}
	Since the subgradient condition is sufficient for optimality of a convex program, lemma \ref{lemma:lasso_sol_square_wave_noise} gives the optimal solution $z$ to the neural net LASSO problem for a unit square wave with one noisy data point.
\end{remark}

\begin{remark}
	The set of nonzero indices of $z_{bdry}$ and that of $z_{cycle}$ partition the set of indices that are a multiple of $\frac{T}{2}$.
\end{remark}

\begin{remark}\label{remark:pred_2layer}
	The optimal neural net evaluated on the training data, $Az$, has the similar square wave shape as $y$, with the same number of cycles and same cycle length. However, the amplitudes of each half-cycle for $Az$ are less than $y$, which has amplitude $1$. Figure \ref{fig:pulse_ex_noise_sol} plots $Az$.
	The amplitudes of the first and last half cycles are $-2w_{bdry}-w_{cycle}=1-\frac{\beta}{T}$, the amplitudes of the inner half cycles $w_{cycle}=1-2\frac{\beta}{T}$, and the amplitude of the half-cycle with noise ($w_{cycle}+2w_{noise}$) is changed from the inner half cycles by $2\frac{s}{T}$, where $s$ is the amount of noise added.
\end{remark}



\begin{remark}
	Each $z_j$ corresponds to a feature $a_j$ which is a column of $A^TA$ as shown in figure \ref{fig:feature_ex}, and $a_j$ is shaped like a peak. $A^T y$ is a zig-zag pattern as seen in figure \ref{fig:A^T(h+delta)}. The signs of $z_j$ alternate with $j$, corresponding to pointing the peak of $a_j$ up or down, which switches the direction of the zig-zag edge from rising or falling. The cycles in $y$ are all identical and can therefore be expressed by one number, $w_{cycle}$ which is the same coefficeient for all the terms in $z_{cycle}$. The boundary vector $z_{bdry}$ adjusts the beginning and endpoints of $A^T Az$ to match $A^T y$. The $z_i$ for the half-cycle $i$ containing noise is modified to account for the noise by adding $z_{noise}$.
\end{remark}

\begin{proof}

	Note $\beta < \beta_u$ ensures that $w_{bdry}<0, w_{cycle}>0, w_{noise}+w_{cycle}>0$. %we use this later, check with s too.


	%We define $z \in \mathbb{R}^N$ as follows, with $N=kT$. For  $n \in \{1, \frac{T}{2}, T,  3\frac{T}{2}, 2T, \cdots, (2k-1)\frac{T}{2}=N-\frac{T}{2}\}$ let

	%\begin{equation}
	%   z_n = 
	%    \begin{cases}
	%        z_{outer} \textrm{ if } n \in \{\frac{T}{2}, N - \frac{T}{2} \} \\
	%        z_{noise} \textrm{ if } n = q_i \frac{T}{2} \\
	%        -z_{noise} \textrm{ if } n = (q_i + 1) \frac{T}{2} \\
	%        -z_{inner} \textrm{ if } n = j\frac{T}{2}, j  \textrm{ even }, j \notin \{1, 2k-1, q_i, q_i+1 \} \\
	%        z_{inner} \textrm{ if } n = j\frac{T}{2}, j  \textrm{ odd }, \notin \{1, 2k-1, q_i, q_i+1 \} \\
	%    \end{cases}
	%\end{equation}

	%and $z_n=0$ for all other $n \in [N]$ that are not multiples of $\frac{T}{2}$.


	Let $n \in [N]$, with $T/2$ quotient and remainder $q_n, r_n$.

	Then the gram matrix $A^TA$ applied to the boundary solution $z_{bdry}$ is

	\begin{equation}\label{eq:A^TAz_bdry}
		\begin{aligned}
			(A^T A z_{bdry})_n & = w_{bdry}
			\left( (A^T A)_{n,\frac{T}{2}} + (A^T A)_{n,N-\frac{T}{2}} \right)                                         \\
			                   & =  w_{bdry} \left( N-2|n-\frac{T}{2}| +  N-2|n-(N-\frac{T}{2})| \right)               \\
			                   & =2 w_{bdry} \left( N-|n-\frac{T}{2}| -|n-N+\frac{T}{2}| \right)                       \\
			                   & =2 w_{bdry} \cdot
			\begin{cases}
				N + (n-\frac{T}{2}) + (n - N + \frac{T}{2}) = 2n     & \mbox{ if } n \leq \frac{T}{2}                      \\
				N - (n-\frac{T}{2}) + (n - N + \frac{T}{2}) =  T     & \mbox{ if } \frac{T}{2} \leq n \leq N - \frac{T}{2} \\
				N - (n-\frac{T}{2}) - (n - N + \frac{T}{2}) = 2(N-n) & \mbox{ if } n \geq N- \frac{T}{2}
			\end{cases} \\
			                   & =2w_{bdry}
			\begin{cases}
				-(A^T h_{k,T})_n & \mbox{ if } n \leq \frac{T}{2}                      \\
				T                & \mbox{ if } \frac{T}{2} \leq n \leq N - \frac{T}{2} \\
				-(A^T h_{k,T})_n & \mbox{ if } n \geq N- \frac{T}{2}
			\end{cases}.
		\end{aligned}
	\end{equation}

	In the last step of \eqref{eq:A^TAz_bdry}, we used equation \eqref{eq:A^Th_k,Tn_cases} in lemma \ref{lemma:A^Th_k,T}.


	An example of $-A^TAz_{bdry}$ is plotted in figure \ref{fig:z_bdry}.

	\begin{figure}[ht]
		\begin{tikzpicture}
			\centering
			\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
				\addplot[ycomb,color=black,solid,mark=*]
				plot coordinates{
						(1,0)
						(2,-2)
						(3,-4)
						(4,-6)
						(5,-8)

						(6,-10)
						(7,-10)
						(8,-10)
						(9,-10)
						(10,-10)

						(11,-10)
						(12,-10)
						(13,-10)
						(14,-10)
						(15,-10)
						(16,-10)
						(17,-10)
						(18,-10)
						(19,-10)
						(20,-10)

						(21,-10)
						(22,-10)
						(23,-10)
						(24,-10)
						(25,-10)
						(26,-10)
						(27,-10)
						(28,-10)
						(29,-10)
						(30,-10)

						(31,-10)
						(32,-10)
						(33,-10)
						(34,-10)
						(35,-10)

						(36,-10)
						(37,-8)
						(38,-6)
						(39,-4)
						(40,-2)
					};

			\end{axis}
		\end{tikzpicture}
		\caption{$-\frac{1}{2w_{bdry}}A^TAz_{bdry}$ with $T=10$.}
		\label{fig:z_bdry}
	\end{figure}

	The solution $z_{bdry}$ accounts for noise by contributing

	\begin{equation}\label{eq:A^TAz_noise_init}
		\begin{aligned}
			(A^T A z_{noise})_n & = w_{noise}
			\left( (-1)^{q_i} (A^T A)_{n,q_i \frac{T}{2}} + (-1)^{q_i+1}  (A^T A)_{n,(q_i+1)\frac{T}{2}} \right)                                            \\
			                    & =   (-1)^{q_i} w_{noise}  \left(  (A^T A)_{n,q_i \frac{T}{2}} -   (A^T A)_{n,(q_i+1)\frac{T}{2}} \right)                  \\
			                    & = (-1)^{q_i} w_{noise}
			\left( N-2|n-q_i\frac{T}{2}| - N + 2|n- (q_i+1)\frac{T}{2}| \right)                                                                             \\
			                    & = (-1)^{q_i} 2 w_{noise}
			\left( -|n-q_i\frac{T}{2}|   +|n- (q_i+1)\frac{T}{2}| \right)                                                                                   \\
			                    & = (-1)^{q_i}2 w_{noise} \cdot
			\begin{cases}
				(n-q_i\frac{T}{2}) - (n -  (q_i+1) \frac{T}{2}) = \frac{T}{2}                    & \mbox{ if } n \leq q_i \frac{T}{2}                           \\
				- (n-q_i\frac{T}{2}) - (n -  (q_i+1) \frac{T}{2}) =  -2n + (2q_i + 1)\frac{T}{2} & \mbox{ if } q_i \frac{T}{2} \leq n \leq (q_i +1) \frac{T}{2} \\
				-(n-q_i\frac{T}{2}) + (n -  (q_i+1) \frac{T}{2}) = -\frac{T}{2}                  & \mbox{ if }  n \geq (q_i +1) \frac{T}{2}
			\end{cases} \\
			                    & = (-1)^{q_i}2 w_{noise} \cdot
			\begin{cases}
				\frac{T}{2}                                    & \mbox{ if } n \leq q_i \frac{T}{2}                           \\
				-2\textrm{rem}(\frac{T}{2},q_i) +  \frac{T}{2} & \mbox{ if } q_i \frac{T}{2} \leq n \leq (q_i +1) \frac{T}{2} \\
				-\frac{T}{2}                                   & \mbox{ if }  n \geq (q_i +1) \frac{T}{2}
			\end{cases}
			\\ &= (-1)^{q_i} w_{noise} \cdot
			\begin{cases}
				T                                    & \mbox{ if } n \leq q_i \frac{T}{2}                           \\
				-4\textrm{rem}(\frac{T}{2},q_i) +  T & \mbox{ if } q_i \frac{T}{2} \leq n \leq (q_i +1) \frac{T}{2} \\
				-T                                   & \mbox{ if }  n \geq (q_i +1) \frac{T}{2}
			\end{cases}.
		\end{aligned}
	\end{equation}

	If $q_i \frac{T}{2} \leq n \leq (q_i+1)\frac{T}{2}$ then $q_n = q_i$, which makes

	\begin{equation}\label{eq:q_n=q_inoise}
		\begin{aligned}
			(-1)^{q_i}\left(T-4\mathrm{rem}\left(\frac{T}{2},q_i\right) \right) & =(-1)^{q_i}T
			-4(-1)^{q_i}\mathrm{rem}\left(\frac{T}{2},q_i\right)                                                                                                                      \\
			                                                                    & =(1-2\cdot\mathbf{1}\{q_i \mathrm{odd}\})T + 4(-1)^{q_i+1} \mathrm{rem}\left(q_i,\frac{T}{2}\right) \\
			                                                                    & = T+2(A^Th_{k,T})_n.
		\end{aligned}
	\end{equation}

	where the last equality follows from  equation \eqref{eq:A^Th_k,Tn_simp} in lemma \ref{lemma:A^Th_k,T}.

	An example of $A^TAz_{noise}$ is plotted in figure \ref{fig:z_noise}. Plugging in \eqref{eq:q_n=q_inoise} simplifies \eqref{eq:A^TAz_noise_init} to

	\begin{equation}
		\begin{aligned}
			(A^T A z_{noise})_n & =w_{noise}
			\begin{cases}
				(-1)^{q_i}T       & \mbox{ if } n \leq q_i \frac{T}{2}                           \\
				T+2(A^Th_{k,T})_n & \mbox{ if } q_i \frac{T}{2} \leq n \leq (q_i +1) \frac{T}{2} \\
				(-1)^{q_i+1}T     & \mbox{ if }  n \geq (q_i +1) \frac{T}{2}
			\end{cases}.
		\end{aligned}
	\end{equation}

	\begin{figure}[ht]
		\begin{tikzpicture}
			\centering
			\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
				\addplot[ycomb,color=black,solid,mark=*]
				plot coordinates{
						(1,5)
						(2,5)
						(3,5)
						(4,5)
						(5,5)

						(6,5)
						(7,5)
						(8,5)
						(9,5)
						(10,5)

						(11,5)
						(12,5)
						(13,5)
						(14,5)
						(15,5)
						(16,5)
						(17,5)
						(18,5)
						(19,5)
						(20,5)

						(21,5)
						(22,3)
						(23,1)
						(24,-1)
						(25,-3)

						(26,-5)
						(27,-5)
						(28,-5)
						(29,-5)
						(30,-5)

						(31,-5)
						(32,-5)
						(33,-5)
						(34,-5)
						(35,-5)

						(36,-5)
						(37,-5)
						(38,-5)
						(39,-5)
						(40,-5)
					};

				%special point
				\addplot[ycomb, color=red,solid,mark=*]
				plot coordinates{
						(24,-1)
					};

			\end{axis}
		\end{tikzpicture}
		\caption{$\frac{1}{2w_{noise}}A^TAz_{noise}$ with $T=10$, noise at index $i=17, q_i=\textrm{rem}(i=17,\frac{T}{2}=5)=3$.}
		\label{fig:z_noise}
	\end{figure}


	The periodic solution $z_{cycle}$ contributes:

	If $n \leq \frac{T}{2}$:

	\begin{equation}
		\begin{aligned}
			(A^T Az_{cycle})_n & = w_{cycle} \sum_{j=2}^{2k-2} (-1)^{j}\left(N-2\left|n-j\frac{T}{2}\right|\right)                                                                                                    \\
			                   & = w_{cycle} \sum_{j=2}^{2k-2} (-1)^{j}\left(N+2\left(n-j\frac{T}{2}\right)\right)                                                                                                    \\
			                   & = w_{cycle}\left(N + 2(n-T) +  \sum_{j=3}^{2k-2} (-1)^{j}\left(N+2\left(n-j\frac{T}{2}\right)\right)  \right)                                                                        \\
			                   & = w_{cycle}\left(N + 2(n-T) +  \sum_{j=3, odd}^{2k-2} (-1)^{j}\left(N+2\left(n-j\frac{T}{2}\right)   \right)  + (-1)^{j+1}\left(N+2\left(n-(j+1)\frac{T}{2}\right) + \right) \right) \\
			                   & = w_{cycle}\left(N + 2(n-T) +  \sum_{j=3, odd}^{2k-2} (-1)^{j} \left(N+2\left(n-j\frac{T}{2}\right)    - \left(N+2\left(n-(j+1)\frac{T}{2}\right)   \right) \right) \right)          \\
			                   & = w_{cycle}\left(N + 2(n-T) -  \sum_{j=3, odd}^{2k-2}\left(N+2\left(n-j\frac{T}{2}  \right)  - \left(N+2\left(n-(j+1)\frac{T}{2}\right)   \right) \right) \right)                    \\
			                   & = w_{cycle}\left(N + 2(n-T) -2\sum_{j=3, odd}^{2k-2}  \frac{T}{2} \right)                                                                                                            \\
			                   & = w_{cycle}\left(N + 2(n-T) - \frac{2k-4}{2} T \right)                                                                                                                               \\
			                   & = w_{cycle}\left(N + 2(n-T) - (k-2) T \right)                                                                                                                                        \\
			                   & = 2w_{cycle}n.
		\end{aligned}
	\end{equation}

	Similarly if $n \geq N-\frac{T}{2}$:

	\begin{equation}
		\begin{aligned}
			(A^T Az_{cycle})_n & = w_{cycle} \sum_{j=2}^{2k-2} (-1)^{j}\left(N-2\left|n-j\frac{T}{2}\right|\right)                                                                               \\
			                   & = w_{cycle} \sum_{j=2}^{2k-2} (-1)^{j}\left(N-2\left(n-j\frac{T}{2}\right)\right)                                                                               \\
			                   & = w_{cycle}\left(N - 2(n-T) -  \sum_{j=3, odd}^{2k-2} \left(N-2\left(n-j\frac{T}{2}\right) - \left(N-2\left(n-(j+1)\frac{T}{2} \right) \right) \right)  \right) \\
			                   & =  w_{cycle}\left(N - 2(n-T) + (k-2)T \right)                                                                                                                   \\
			                   & = 2w_{cycle}(N-n).
		\end{aligned}
	\end{equation}

	If $\frac{T}{2} \leq n \leq N - \frac{T}{2}$: %used to evalute sum as \floor ... \rfloor since q_n comes in between upper and lower sum limits

	\begin{equation}
		\begin{aligned}
			(A^T Az_{cycle})_n & = w_{cycle} \sum_{j=2}^{2k-2} (-1)^{j}\left(N-2\left|n-j\frac{T}{2}\right|\right)                                                                                                                                                                                                               \\
			                   & =  w_{cycle} \left(N + \sum_{j=2}^{2k-2} (-1)^{j}\left(-2\left|n-j\frac{T}{2}\right|\right) \right)                                                                                                                                                                                             \\
			                   & =  -w_{cycle} \left(-N + 2\sum_{j=2}^{2k-2} (-1)^{j} \left|n-j\frac{T}{2}\right| \right)                                                                                                                                                                                                        \\
			                   & =  -w_{cycle} \left(-N + 2 \left( \sum_{j=2}^{q_n} (-1)^{j} \left|n-j\frac{T}{2}\right| + \sum_{j=q_n +1}^{2k-2} (-1)^{j} \left|n-j\frac{T}{2}\right| \right) \right)                                                                                                                           \\
			                   & =  -w_{cycle} \left(-N + 2 \left( \sum_{j=2}^{q_n} (-1)^{j} \left(n-j\frac{T}{2}\right) - \sum_{j=q_n +1}^{2k-2} (-1)^{j} \left(n-j\frac{T}{2}\right) \right) \right)                                                                                                                           \\
			                   & =  -w_{cycle} \left(-N + 2 \left( n\mathbf{1}\{q_n \textrm{even}\} + \sum_{j=2}^{q_n} (-1)^{j} \left(-j\frac{T}{2}\right) - \left( n\mathbf{1}\{q_n \textrm{odd}\} + \sum_{j=q_n +1}^{2k-2} (-1)^{j}   \left(-j\frac{T}{2}\right) \right) \right) \right)                                       \\
			                   & =  -w_{cycle} \left(-N + 2 \left( n (-1)^{q_n} + \frac{T}{2} \left( \sum_{j=q_n +1}^{2k-2} (-1)^{j} j - \sum_{j=2}^{q_n} (-1)^{j} j   \right) \right) \right)                                                                                                                                   \\
			                   & =  -w_{cycle} \left(-N + 2 \left( n (-1)^{q_n} + \frac{T}{2} \left( (q_n+1) \mathbf{1}\{q_n \textrm{ odd}\} + \left \lfloor \frac{2k-2-q_n}{2} \right \rfloor  -  \left( q_n \mathbf{1}\{q_n \textrm{ even}\} -  \left \lfloor \frac{q_n-1}{2} \right \rfloor   \right) \right) \right) \right) \\
			                   & =  -w_{cycle} \left(-N + 2 \left( n (-1)^{q_n} + \frac{T}{2} \left( q_n (-1)^{q_n+1} + \mathbf{1}\{q_n \textrm{ odd}\} + \left \lfloor \frac{2k-2-q_n}{2} \right \rfloor +   \left \lfloor \frac{q_n-1}{2} \right \rfloor   \right) \right) \right)                                             \\
			                   & =  -w_{cycle} \left(-N + 2 \left( n (-1)^{q_n} + \frac{T}{2} \left( q_n (-1)^{q_n+1} + \mathbf{1}\{q_n \textrm{ odd}\} + k-2  \right) \right) \right)                                                                                                                                           \\
			                   & =  -w_{cycle} \left(-N + 2 \left( (-1)^{q_n} \left( n  - q_n \frac{T}{2} \right)+  \mathbf{1}\{q_n \textrm{ odd}\}\frac{T}{2} + k\frac{T}{2}- T  \right) \right)                                                                                                                                \\
			                   & =  -w_{cycle} \left(-N + 2  (-1)^{q_n} \textrm{rem}(n,\frac{T}{2}) +  \mathbf{1}\{q_n \textrm{ odd}\}T + N - 2T  \right)                                                                                                                                                                        \\
			                   & = -w_{cycle}\left( (\mathbf{1}\{q_n \textrm{ odd}\} - 2)T  + 2  (-1)^{q_n} \textrm{rem}(n,\frac{T}{2}) \right)                                                                                                                                                                                  \\
			                   & = w_{cycle}\left( (2-\mathbf{1}\{q_n \textrm{ odd}\} )T  + 2  (-1)^{q_n+1} \textrm{rem}(n,\frac{T}{2}) \right).
		\end{aligned}
	\end{equation}





	\begin{figure}[ht]
		\begin{tikzpicture}
			\centering
			\begin{axis}[axis x line=middle, axis y line=middle, xticklabels={,,}, xlabel = {$x_1$}]
				\addplot[ycomb,color=black,solid,mark=*]
				plot coordinates{
						(1,0)
						(2,2)
						(3,4)
						(4,6)
						(5,8)

						(6,10)
						(7,12)
						(8,14)
						(9,16)
						(10,18)

						(11,20)
						(12,18)
						(13,16)
						(14,14)
						(15,12)

						(16,10)
						(17,12)
						(18,14)
						(19,16)
						(20,18)

						(21,20)
						(22,18)
						(23,16)
						(24,14)
						(25,12)

						(26,10)
						(27,12)
						(28,14)
						(29,16)
						(30,18)

						(31,20)
						(32,18)
						(33,16)
						(34,14)
						(35,12)

						(36,10)
						(37,8)
						(38,6)
						(39,4)
						(40,2)
					};

			\end{axis}
		\end{tikzpicture}
		\caption{$\frac{1}{w_{cycle}}A^TAz_{cycle}$ with $T=10$.}
		\label{fig:z_cycle}
	\end{figure}

	To summarize,

	\begin{equation}\label{eq:A^TAzcycle}
		\begin{aligned}
			(A^TAz_{cycle})_n & = w_{cycle} \cdot
			\begin{cases}
				2n                                                                                   & \mbox{ if } n \leq \frac{T}{2}                      \\
				(2-\mathbf{1}\{q_n \textrm{ odd}\} )T  + 2  (-1)^{q_n+1} \textrm{rem}(n,\frac{T}{2}) & \mbox{ if } \frac{T}{2} \leq n \leq N - \frac{N}{2} \\
				2(N-n)                                                                               & \mbox{ if } n \geq N- \frac{T}{2}                   \\
			\end{cases} \\
			                  & = w_{cycle} \cdot
			\begin{cases}
				-(A^T h_{k,T})_n     & \mbox{ if } n \leq \frac{T}{2}                      \\
				2T + (A^T h_{k,T})_n & \mbox{ if } \frac{T}{2} \leq n \leq N - \frac{N}{2} \\
				-(A^T h_{k,T})_n     & \mbox{ if } n \geq N- \frac{T}{2}                   \\
			\end{cases}.
		\end{aligned}
	\end{equation}


	In the second equality of  \eqref{eq:A^TAzcycle}, we used equations \eqref{eq:A^Th_k,Tn_cases},\eqref{eq:A^Th_k,Tn_simp} in lemma \ref{lemma:A^Th_k,T}.

	An example of $A^TAz_{cycle}$ is plotted in figure \ref{fig:z_cycle}.



	Therefore, if the noise occurs between the first and last half-period,

	\begin{equation}
		\begin{aligned}
			(A^T A z)_{n} & =
			\begin{cases}
				4nw_{bdry} + (-1)^{q_i} w_{noise}T + 2nw_{cycle}                                        & \mbox{ if } n \leq \frac{T}{2}                              \\

				2Tw_{bdry} + (-1)^{q_i} w_{noise}T + w_{cycle}\left(2T + (A^T h_{k,T})_n\right)         & \mbox{ if } \frac{T}{2} \leq n \leq q_i \frac{T}{2}         \\

				2Tw_{bdry} + w_{noise}(T+2(A^Th_{k,T})_n)  + w_{cycle}\left(2T + (A^T h_{k,T})_n\right) & \mbox{ if } q_i\frac{T}{2} \leq n \leq (q_i+1) \frac{T}{2}  \\

				2Tw_{bdry} + (-1)^{q_i+1} w_{noise}T + w_{cycle}\left(2T + (A^T h_{k,T})_n\right)       & \mbox{ if } (q_i+1) \frac{T}{2} \leq n \leq N - \frac{N}{2} \\

				2(N-n)w_{bdry} + (-1)^{q_i+1} w_{noise}T + 2w_{cycle}(N-n)                              & \mbox{ if } n \geq N- \frac{T}{2}                           \\
			\end{cases} \\
			              & =
			\begin{cases}
				(-1)^{q_i} w_{noise}T- (2w_{bdry} + w_{cycle} )(A^T h_{k,T})_n                       & \mbox{ if } n \leq \frac{T}{2}                              \\

				(2(w_{bdry}  + w_{cycle}) + (-1)^{q_i} w_{noise})T + w_{cycle}(A^T h_{k,T})_n        & \mbox{ if } \frac{T}{2} \leq n \leq q_i \frac{T}{2}         \\

				(2(w_{bdry} + w_{cycle})+w_{noise}) T +  (2w_{noise}    + w_{cycle} ) (A^Th_{k,T})_n & \mbox{ if } q_i\frac{T}{2} \leq n \leq (q_i+1) \frac{T}{2}  \\

				(2(w_{bdry}  + w_{cycle}) + (-1)^{q_i+1} w_{noise})T  + w_{cycle} (A^T h_{k,T})_n    & \mbox{ if } (q_i+1) \frac{T}{2} \leq n \leq N - \frac{N}{2} \\

				(-1)^{q_i+1} w_{noise}T - (2w_{bdry}+w_{cycle})(A^T h_{k,T})_n                       & \mbox{ if } n \geq N- \frac{T}{2}                           \\
			\end{cases}
		\end{aligned}
	\end{equation}

	Suppose $\beta < \frac{T}{2}$.

	%\textcolor{red}{todo: at least for no noise case, if $\beta \geq \frac{T}{2}$ then I think we get all 0, from dual formulation for y being feasible. I think we might have a condition related to s?}

	Now set

	\begin{equation}
		\begin{aligned}
			w_{bdry}  & = -\left(1-\frac{3}{2}\frac{\beta}{T}\right) < 0 \\
			w_{cycle} & = 1-2\frac{\beta}{T}>0                           \\
			w_{noise} & = (-1)^{q_i+1} \frac{s}{T}
		\end{aligned}
	\end{equation}

	Observe

	\begin{equation}
		\begin{aligned}
			-(2w_{bdry}+w_{cycle}) & = -(-2 + 3\frac{\beta}{T} + 1-2\frac{\beta}{T}) = 1 - \frac{\beta}{T}      \\
			2(w_{bdry}+w_{cycle})  & = 2(-1+\frac{3}{2}\frac{\beta}{T} + 1-2\frac{\beta}{T}) = -\frac{\beta}{T}
		\end{aligned}
	\end{equation}

	So

	\begin{equation}
		\begin{aligned}
			(A^T Az)_n & =
			\begin{cases}
				-s + (1-\frac{\beta}{T}) (A^T h_{k,T})_n                                                                           & \mbox{ if } n \leq \frac{T}{2}                              \\

				(-\frac{\beta}{T} - \frac{s}{T})T + (1-2\frac{\beta}{T})(A^T h_{k,T})_n                                            & \mbox{ if } \frac{T}{2} \leq n \leq q_i \frac{T}{2}         \\

				(-\frac{\beta}{T}+(-1)^{q_i+1}\frac{s}{T}) T +  (2(-1)^{q_i+1}\frac{s}{T}    + 1-2\frac{\beta}{T} ) (A^Th_{k,T})_n & \mbox{ if } q_i\frac{T}{2} \leq n \leq (q_i+1) \frac{T}{2}  \\

				(-\frac{\beta}{T} + \frac{s}{T})T  + (1-2\frac{\beta}{T}) (A^T h_{k,T})_n                                          & \mbox{ if } (q_i+1) \frac{T}{2} \leq n \leq N - \frac{N}{2} \\

				s +(1-\frac{\beta}{T})(A^T h_{k,T})_n                                                                              & \mbox{ if } n \geq N- \frac{T}{2}
			\end{cases} \\
			           & =
			\begin{cases}
				-s + (1-\frac{\beta}{T}) (A^T h_{k,T})_n                                     & \mbox{ if } n \leq \frac{T}{2}                              \\

				-s -\beta  + (1-2\frac{\beta}{T})(A^T h_{k,T})_n                             & \mbox{ if } \frac{T}{2} \leq n \leq q_i \frac{T}{2}         \\

				(-1)^{q_i+1}s -\beta+  (1+\frac{2}{T}((-1)^{q_i+1}s -\beta) ) (A^Th_{k,T})_n & \mbox{ if } q_i\frac{T}{2} \leq n \leq (q_i+1) \frac{T}{2}  \\

				s-\beta   + (1-2\frac{\beta}{T}) (A^T h_{k,T})_n                             & \mbox{ if } (q_i+1) \frac{T}{2} \leq n \leq N - \frac{N}{2} \\

				s +(1-\frac{\beta}{T})(A^T h_{k,T})_n                                        & \mbox{ if } n \geq N- \frac{T}{2}
			\end{cases}                                       \\
			           & =(A^T \delta_{s,i})_n +
			\begin{cases}
				(1-\frac{\beta}{T}) (A^T h_{k,T})_n                                                                                        & \mbox{ if } n \leq \frac{T}{2}                              \\

				-\beta  + (1-2\frac{\beta}{T})(A^T h_{k,T})_n                                                                              & \mbox{ if } \frac{T}{2} \leq n \leq q_i \frac{T}{2}         \\

				s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) +(-1)^{q_i+1}s -\beta+  (1+\frac{2}{T}((-1)^{q_i+1}s -\beta) ) (A^Th_{k,T})_n & \mbox{ if } q_i\frac{T}{2} \leq n \leq (q_i+1) \frac{T}{2}  \\

				-\beta   + (1-2\frac{\beta}{T}) (A^T h_{k,T})_n                                                                            & \mbox{ if } (q_i+1) \frac{T}{2} \leq n \leq N - \frac{N}{2} \\

				(1-\frac{\beta}{T})(A^T h_{k,T})_n                                                                                         & \mbox{ if } n \geq N- \frac{T}{2}
			\end{cases}.
		\end{aligned}
	\end{equation}

	Recall that in lemma \ref{lemma:A^Th_k,T}, $\textrm{rem}\left(n,\frac{T}{2}\right) \in [\frac{T}{2}]$. So

	\begin{equation}
		0< 2 \frac{1}{T}  \textrm{rem}\left(n,\frac{T}{2}\right) \leq 1
	\end{equation}

	with equality on $\leq $ achieved when $n=\frac{T}{2}$.

	So if $q_n$ is odd, then

	\begin{equation}
		0< (-1)^{q_n+1} 2 \frac{1}{T}  \textrm{rem}\left(n,\frac{T}{2}\right) \leq 1,
	\end{equation}

	and if $q_n$ is even, then

	\begin{equation}
		0 >  (-1)^{q_n+1} 2 \frac{1}{T}  \textrm{rem}\left(n,\frac{T}{2}\right) \geq -1
	\end{equation}

	with $n=\frac{T}{2}$ turning the righthand side nonstrict inequalities into equalities.

	Therefore by equation \eqref{eq:A^Th_k,Tn_simp} in lemma \ref{lemma:A^Th_k,T},

	\begin{equation}
		\begin{aligned}
			-\frac{1}{T}(A^T h_{k,T})_n & =  -\mathbf{1}\{q_n \textrm{ odd}\}   + 2 \frac{1}{T}  (-1)^{q_n+1} \textrm{rem}\left(n,\frac{T}{2}\right) \\
			                            & \begin{cases}
				                              1> \cdot \geq 0  & \mbox{ if } q_n \mbox{ is odd }  \\
				                              0 < \cdot \leq 1 & \mbox{ if } q_n \mbox{ is even } \\
			                              \end{cases}.
		\end{aligned}
	\end{equation}

	with  $n=\frac{T}{2}$ achieving equality in the nonstrict inequalities.

	When $n \leq \frac{T}{2}$, the quotient $q_n=0$ is even, so

	\begin{equation}
		\begin{aligned}
			(A^T h_{k,T})_n < \left(1-\frac{\beta}{T}\right)(A^T h_{k,T})_n = (A^T h_{k,T})_n - \beta \frac{1}{T}(A^T h_{k,T})_n
			\leq  (A^T h_{k,T})_n + \beta.
		\end{aligned}
	\end{equation}

	with the upper inequality achieved when $n=\frac{T}{2}$. Note $z_{\frac{T}{2}}= w_{bdry}<0$.

	When $n \geq N-\frac{T}{2}$, the quotient $q_n=2k-1$ is odd, so

	\begin{equation}
		\begin{aligned}
			(A^T h_{k,T})_n \leq \left(1-\frac{\beta}{T}\right)(A^T h_{k,T})_n = (A^T h_{k,T})_n - \beta \frac{1}{T}(A^T h_{k,T})_n
			<  (A^T h_{k,T})_n + \beta.
		\end{aligned}
	\end{equation}
	%this case can get subsumed by below. 


	When $\frac{T}{2} < n < N-2\frac{T}{2}$,

	\begin{equation}
		\begin{aligned}
			-\beta + \left(1-2\frac{\beta}{T}\right)(A^T h_{k,T})_n & = -\beta + (A^T h_{k,T})_n - 2\beta \frac{1}{T}(A^T h_{k,T})_n          \\
			                                                        & \begin{cases}
				                                                          \geq -\beta+(A^T h_{k,T})_n          & \mbox{ if } q_n \mbox{ is odd }  \\
				                                                          \leq -\beta+(A^T h_{k,T})_n + 2\beta & \mbox{ if } q_n \mbox{ is even }
			                                                          \end{cases} \\
			=                                                       & \begin{cases}
				                                                          \geq (A^T h_{k,T})_n  -\beta & \mbox{ if } q_n \mbox{ is odd }  \\
				                                                          \leq (A^T h_{k,T})_n +\beta  & \mbox{ if } q_n \mbox{ is even } \\
			                                                          \end{cases}
		\end{aligned}
	\end{equation}

	with equality achieved when $n=(q_n+1)\frac{T}{2}$. Note that the sign of $z_{(q_n)\frac{T}{2}}$ is $(-1)^{q_n}$. So if $z_n>0$ then $q_n$ is even, and equality is achieved at $n = (q_n+1)\frac{T}{2}$, which is odd, at which $-\beta + \left(1-2\frac{\beta}{T}\right)(A^T h_{k,T})_n  = (A^T h_{k,T})_n  -\beta $. Similarly, for $z_n<0$, $-\beta + \left(1-2\frac{\beta}{T}\right)(A^T h_{k,T})_n  = (A^T h_{k,T})_n  +\beta $. \textcolor{red}{todo: check and plot}

	Now, when $q_i \frac{T}{2} \leq n \leq (q_i+1)\frac{T}{2}$, we have $q_i=q_n$ and so

	\begin{equation}
		\begin{aligned}
			(-1)^{q_i+1} (A^T h_{k,T})_n & = (-1)^{q_i+1}  ( -\mathbf{1}\{q_i \textrm{ odd}\}T  + 2 (-1)^{q_i+1} \textrm{ rem}(n,\frac{T}{2}) ) \\
			                             & = -\mathbf{1}\{q_i \textrm{ odd}\}T  + 2  \textrm{ rem}(n,\frac{T}{2})                               \\
			                             & \begin{cases}
				                               \leq 0 \mbox{ if }  q_n \mbox{ is odd}  \\
				                               \leq T \mbox{ if }  q_n \mbox{ is even} \\
			                               \end{cases}
		\end{aligned}
	\end{equation}

	So when $q_i \frac{T}{2} \leq n \leq (q_i+1)\frac{T}{2}$,

	\begin{equation}
		\begin{aligned}
			 & s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) +(-1)^{q_i+1}s -\beta+  (1+\frac{2}{T}((-1)^{q_i+1}s -\beta) ) (A^Th_{k,T})_n                                                                    \\
			 & =
			s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) +(-1)^{q_i+1}s -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n + \frac{2}{T}(-1)^{q_i+1}s(A^Th_{k,T})_n                                                 \\
			 & =
			s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) +(-1)^{q_i+1}s -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n + \frac{2}{T}s (-\mathbf{1}\{q_i \textrm{ odd}\}T  + 2  \textrm{ rem}(n,\frac{T}{2}))    \\
			 & =
			s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) +(-1)^{q_i+1}s -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n + 2s (-\mathbf{1}\{q_i \textrm{ odd}\}  + \frac{2}{T}  \textrm{ rem}(n,\frac{T}{2}))     \\
			 & =
			s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) +(-1)^{q_i+1}s -\mathbf{1}\{q_i \textrm{ odd}\}(2s) -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n    + (2s)\frac{2}{T}  \textrm{ rem}(n,\frac{T}{2})) \\
			 & =
			s(\mathbf{1}\{ n<i\}-\mathbf{1}\{ n\geq i\}) -s -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n    + (2s)\frac{2}{T}  \textrm{ rem}(n,\frac{T}{2}))                                                  \\
			 & =
			-2s\mathbf{1}\{ n\geq i\}  -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n    + (2s)\frac{2}{T}  \textrm{ rem}(n,\frac{T}{2}))                                                                       \\
			 & =
			-\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n    + 2s(\frac{2}{T}  \textrm{ rem}(n,\frac{T}{2}))  -\mathbf{1}\{ n\geq i\})                                                                         \\
			 & \begin{cases}
				   >  -\beta+ (1-\frac{2}{T}\beta)(A^Th_{k,T})_n \mbox{ if } q_i \frac{T}{2} < n < i            \\
				   \leq -\beta+  (1-\frac{2}{T}\beta)(A^Th_{k,T})_n  \mbox{ if } i \leq n <  (q_i+1)\frac{T}{2} \\
			   \end{cases}                                                                                                  \\
		\end{aligned}
	\end{equation}

	with equality achieved when $n \in \{q_i \frac{T}{2} ,  (q_i+1)\frac{T}{2} \}$.

	So in all cases, if the noise occurs not at the first or last half-period, and the regularization is small enough, then $-\beta \leq |A^TAz -A^Ty| = |A^TAz - (A^T \delta_{s,i} + A^T h_{k,T})| \leq \beta$ with equality achieved at indices $n$ corresponding to the appropriate sign of $z_n$:

	\begin{equation}
		\begin{aligned}
			(A^T y-A^T Az)_n  =
			\begin{cases}
				\beta \mbox{ if } z_n > 0  \\
				-\beta \mbox{ if } z_n < 0 \\
				\in [-\beta, \beta] \mbox{ else }
			\end{cases}
		\end{aligned}
	\end{equation}


\end{proof}


==> unused/old_lasso_deriv.tex <==
%original lasso derivation. Updated to unify with deeper layer ReLU

\subsection{Rescaling the \nc{} training problem}
%Let $\mathcal{L}_{\mathbf{y}}:\mathbb{R}^N \to R$ be an arbitrary convex, lower semicontinuous loss function. 

\iftoggle{long}{We will use the following lemma to reformulate our \nc{} training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro} in propositions \ref{prop:2layerhomrescale} and \ref{parLlayernn_signdet}.}


\begin{lemma}\label{lemma:L2toL1rescale}
	Let $g_i: \Theta \to \mathbb{R}^N$ be a function of a collection $\params \in \Theta$ of variables, $i \in [m]$. 
	Consider 

	\begin{equation}
		\label{equ:psign_no_wreg_gen}
		\begin{aligned}
			\min_{\boldsymbol{\alpha} \in \mathbb{R}^m, \mathbf{u} \in \mathbb{R}^{m}, \params \in \Theta}  \mathcal{L}_{\mathbf{y}}\left( \sum_{i=1}^m \alpha_i u_i g_i(\params)  \right) + \frac{\beta}{2} \sum_{i=1}^m ( u_i^2 + \alpha_i^2).
		\end{aligned}
	\end{equation}

	where $u_i$ is independent of the variables in $\theta$. Problem \eqref{equ:psign_no_wreg_gen} is equivalent to

	\begin{equation}\label{eq:gen_rescale}
		\begin{aligned}
			\min_{ \boldsymbol{\alpha} \in \mathbb{R}^m, \params \in \Theta} \mathcal{L}_{\mathbf{y}} \left(\sum_{i=1}^m \alpha_i  g_i(\params)  \right) + \beta ||\boldsymbol{\alpha}||_1. \end{aligned}
	\end{equation}
\end{lemma}

\iftoggle{long}{\proofsketch{
	We use the identity $a^2+b^2\geq2|ab|$ to relate $l_2$ norms to $l_1$ norms, and then use the fact that this makes $\alpha_i$ and $u_i$ always appear as a product, and therefore there is redundancy in having both variables. So we can ``reallocate" the value of $u_i$ to $\alpha_i$ and remove $u_i$ from the problem.
}}

\begin{proof}

	Consider

	\begin{equation}
		\label{equ:psign'mult_gen}
		\begin{aligned}
			\min_{\boldsymbol{\alpha'} \in \mathbb{R}^m, \boldsymbol{u' \in \mathbb{R}^{m}}, \theta' \in \Theta} \mathcal{L}_{\mathbf{y}} \left( \sum_{i=1}^m \alpha'_i u_i' g_i(\theta')  \right) + \beta \sum_{i=1}^m |u'_i||\alpha'_i|. \end{aligned}
	\end{equation}

	Let $t^*$ and $r^*$ be the optimal values of \eqref{equ:psign_no_wreg_gen} and \eqref{equ:psign'mult_gen}, respectively. Since $ u_i^2 + \alpha_i^2 \geq 2|u_i| |\alpha_i|$, $ t^* \geq r^*$. On the other hand, for any solution $\alpha', u', \theta'$ and the value it achieves in problem \eqref{equ:psign'mult_gen}, setting $ u_i=\zeta_i^{-1} u_i',  \alpha_i=\zeta_i \alpha_i', \theta=\theta'$ where $\zeta_i = \sqrt{|\frac{\alpha_i'}{u_i'}|}$ attains an equal value in problem \eqref{equ:psign_no_wreg_gen}. This is because $u_i \alpha_i = u_i' \alpha_i'$ and $ (\zeta^{-1} u_i)^2 + (\zeta \alpha_i) ^2 = 2|\zeta^{-1} u_i| |\zeta \alpha_i| = |u_i| |\alpha_i|$. So $t^* \geq r^*$. Hence $t^* =r^*$, ie \eqref{equ:psign_no_wreg_gen} and \eqref{equ:psign'mult_gen} are equivalent.
	Since $\alpha'_i$  and $u'_i$ appear as a product in \eqref{equ:psign'mult_gen}, set $\alpha_i = \alpha'_i u'_i$. %makes $|s_i||\alpha_i|=$
	%In other words, the weight of $s$ was reallocated to $\alpha$.

\end{proof}

\begin{remark}\label{remk:rescale_pos_const}
\cref{eq:gen_rescale} still holds with the constraint $\mathbf{u} \in \mathbb{R}^{m}$  in \eqref{equ:psign_no_wreg_gen} by the same proof but with $\boldsymbol{u'} \in \mathbb{R}_+^{m}$ in \eqref{equ:psign'mult_gen}.
\end{remark}

\subsubsection{Rescaling the neural net for homogeneous activation functions, $2$ layers}

\begin{lemma}\label{prop:2layerhomrescale}
	Suppose $\sigma(z)$ is homogeneous (\cref{app_section:act_func}).
	The $2$-layer, $d$-dimensional training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro}:

	\begin{equation}\label{eq:train_hom}
		\begin{aligned}
			\min_{\boldsymbol{\alpha}\in \mathbb{R}^m, \mathbf{b} \in \mathbb{R}^m, \mathbf{w_i} \in \mathbb{R}^d} & \mathcal{L}_{\mathbf{y}} \left( \sum_{i=1}^m\alpha_i\sigma(\mathbf{X} \mathbf{w_i}+b_i\mathbf{1}) \right)
			+\frac{\beta}{2}\sum_{i=1}^m(\alpha_i^{2}+||\mathbf{w_i}||_2^{2}),
		\end{aligned}
	\end{equation}

	is equivalent to

	\begin{equation}\label{eq:train_hom_rescaled}
		\begin{aligned}
			\min_{\boldsymbol{\alpha}\in \mathbb{R}^m,  \mathbf{b} \in \mathbb{R}^m, \mathbf{w_i} \in \mathbb{R}^d: ||\mathbf{w_i}||_2=1} & \mathcal{L}_{\mathbf{y}} \left( \sum_{i=1}^m\alpha_i\sigma(\mathbf{X} \mathbf{w_i}+b_i \mathbf{1}) \right)
			+\beta||\boldsymbol{\alpha}||_1.
		\end{aligned}
	\end{equation}
\end{lemma}

\proofsketch{ Since $\sigma$ is homogeneous, the magnitude $||\mathbf{w_i}||_2$ can be pulled out of  $\sigma$. Since $b_i$ is unconstrained, this does not change the problem and \cref{lemma:L2toL1rescale} gives the result.}

\begin{proof}
 
 If $\mathbf{w_i}=0$ then the neuron $\sigma(\mathbf{xw_i}+b_i)=\sigma(b_i)$ can be incorporated into the bias term $\xi$. So assume $\mathbf{w_i} \neq \mathbf{0}$.
Let $u_i = ||\mathbf{w_i}||_2, \mathbf{v_i} = \frac{\mathbf{w_i}}{||\mathbf{w_i}||_2}, c_i = \frac{b_i}{||\mathbf{w_i}||_2}$. Since $\sigma$ is homogeneous, $\sigma(\mathbf{\mathbf{X} w_i} + b_i \mathbf{1})=
\iftoggle{long}{||w_i||_2\sigma(\mathbf{X} \frac{w_i}{||w_i||_2} + \frac{b_i}{||w_i||_2}) =}
 u_i\sigma\left(\mathbf{\mathbf{X} v_i }+ \frac{b_i}{u_i} \mathbf{1}\right)$. 
 \iftoggle{long}{Note $u_i$ and $v_i$ are independent of each other.}
The training problem \eqref{eq:train_hom} becomes,

	\begin{equation}\label{eq:train_hom_varchange}
		\begin{aligned}
			\min_{\mathbf{u} \in \mathbb{R}_+^m, \mathbf{b} \in \mathbb{R}^m, \boldsymbol{\alpha} \in \mathbb{R}^m, \mathbf{v_i} \in \mathbb{R}^d:||\mathbf{v_i}||_2 = 1} & \mathcal{L}_{\mathbf{y}} 
   \left( \sum_{i=1}^m \alpha_i u_i \sigma \left(\mathbf{\mathbf{X} v_i}+ \frac{b_i}{u_i}\mathbf{1} \right) \right)
			+\frac{\beta}{2}\sum_{i=1}^m(\alpha_i^{2}+u_i^{2}).
		\end{aligned}
	\end{equation}

	
 \iftoggle{long}{ so \eqref{eq:train_hom_varchange} is equivalent to

	\begin{equation}\label{eq:train_hom_bchange}
		\begin{aligned}
			\inf_{u \in {\mathbb{R}^m}^{>0}, b \in \mathbb{R}^m,\alpha \in \mathbb{R}^m, v_i \in \mathbb{R}^d: ||v_i||_2 = 1, i \in [m]} & \mathcal{L}_{\mathbf{y}} \left(\sum_{i=1}^m \alpha_i u_i \sigma\left(\mathbf{x_n v_i}+ c_i \right) \right)
			+\frac{\beta}{2}\sum_{i=1}^m(|\alpha_i|^{2}+||u_i||_2^{2}).
		\end{aligned}
	\end{equation}

 	which is the same as \eqref{equ:psign_no_wreg_gen} with $\Theta = \{v_i, c_i: i \in [m]\}, g(\Theta)=\sigma(x v_i+ c_i)$. Applying lemma \ref{lemma:L2toL1rescale}, we get that \eqref{eq:train_hom_bchange} is equivalent to

	\begin{equation}\label{eq:hom_rescale}
		\begin{aligned}
			\min_{\alpha \in \mathbb{R}^m, c_i \in \mathbb{R}, w_i \in \mathbb{R}^{d}: ||w_i||_2=1, i \in [m]} \mathcal{L}_{\mathbf{y}} \left(\sum_{i=1}^m \alpha_i  \sigma(x v_i + c_i)  \right) + \beta ||\alpha||_1 \end{aligned}
	\end{equation}

	Renaming variables produces \eqref{eq:train_hom}.
}
Note $\mathbf{v_i}, u_i$ are independent. Since $b_i$ is unregularized, we can apply a change of variables $b_i \to {b_i}{u_i}=c_i$. Then apply \cref{lemma:L2toL1rescale} and \cref{remk:rescale_pos_const} with $\theta = \{\mathbf{v_i}, c_i: i \in [m]\}, g_i(\theta)=\sigma(\mathbf{X v_i}+ c_i \mathbf{1})$.

\end{proof}

\subsubsection{Rescaling the neural net for sign-determined activation functions, $L \geq 2$ layers}


\begin{lemma}\label{lemma:combine_amp_with_w}
	The $L$-layer parallel neural network \eqref{parLlayernn_signdet} for activations that are sign determined (\cref{app_section:act_func}) can be equivalently written as
	\begin{equation}\label{nn_unrolled}
		\nn{L}{\mathbf{x}} = \sum_{i=1}^{m_L} \sigma_{\sul{i}{L-1}} \left ( {\mathbf{\Tilde{x}^{(i,L-2)}}} \tWul{i}{L-1} \right) \alpha_i,
	\end{equation}
	where every activation in the hidden layers has amplitude parameter 1:  for all $l \in [L-2], i \in [m_L]$,
	\begin{equation}\label{x_unrolled}
		\mathbf{\tilde{x}^{(i,l)}}:= \left[ \sigma_{\mathbf{s}=\mathbf{1}}\left( \mathbf{x^{(i,l-1)}} \tWul{i}{L-1}  \right) , \mathbf{1} \right]
	\end{equation}
	and
	\begin{equation}\label{w_unrolled}
		\tWul{i}{l} :=  \mathrm{Diag} \left( \left[{\sul{i}{l-1}}^T, 1 \right] \right) \Wul{i}{l} .
	\end{equation}

	where $\sul{i}{l-1} $ are trainable parameters independent of activation functions.

\end{lemma}

\proofsketch{
The amplitude parameters can be absorbed into the weight matrices.
}

\begin{proof}

	Note that  $\sigma_{\sul{i}{l-1}}\left(  \sxul{i}{l-1} \Wul{i}{l} \right) = \sigma_{s=\mathbf{1}}\left(\mathbf{ \sxul{i}{l-1} } \Wul{i}{l} \right) \mathrm{Diag} (\sul{i}{l-1})$.

	Then for every layer $l \in [L-2]$,
	\begin{equation}
		\begin{aligned}
			\sxul{i}{l+1} & = \left[ \sigma_{ \sul{i}{l+1}}\left(  \sxul{i}{l} \Wul{i}{l+1} \right) , \mathbf{1} \right]                                                                                         \\
			            & = \left[ \sigma_{\sul{i}{l+1}}\left( \left[\sigma_{s=\mathbf{1}}\left( \sxul{i}{l-1} \Wul{i}{l} \right) \mathrm{Diag} ( \sul{i}{l}), \mathbf{1}\right] \Wul{i}{l+1} \right) , \mathbf{1} \right]          \\
			            & =\left[ \sigma_{ \sul{i}{l+1} }\left( \left[\sigma_{s=1}\left(  \sxul{i}{l-1} \Wul{i}{l} \right) , \mathbf{1}\right] \mathrm{Diag} 
               \begin{pmatrix}
                   \sul{i}{l} \\
                   1
               \end{pmatrix}
               \Wul{i}{l+1} \right) , \mathbf{1} \right] \\
			            & =\left[ \sigma_{ \sul{i}{l+1}}\left( \left[\sigma_{s=1}\left(  \sxul{i}{l-1}\Wul{i}{l} \right) , \mathbf{1} \right]  \tWul{i}{l+1} \right) , \mathbf{1} \right].                           \\
		\end{aligned}
	\end{equation}

	Therefore at the last layer,

	\begin{equation} \label{neuron_unrolled}
		\begin{aligned}
			\sigma_{ \sul{i}{L-1}}\left( \sxul{i}{L-2} \Wul{i}{L-1}\right)  & =\sigma_{\sul{i}{L-1}}\left( \tsXul{i}{L-2}  \tWul{i}{L-1} \right).
		\end{aligned}
	\end{equation}

	Linearly combining \eqref{neuron_unrolled} over the $m_L$ neurons at the final layer gives \eqref{nn_unrolled}.

\end{proof}

\begin{lemma}\label{prop:sign-det_rescale}
	Suppose $\sigma(z)$ is sign-determined.
	Consider the parallel neural net training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro} for $L$ layers:

	\begin{equation}
		\label{equ:nn_train_signdetinput}
		\begin{aligned}
			\min_{\boldsymbol{\alpha} \in \mathbb{R}^{m_L},   \Wul{i}{l},  \sul{i}{l}: l \in [L-1], i \in [m_L] } \mathcal{L}_{\mathbf{y}}(f_L(\mathbf{X};\theta) ) + \beta/2 \left ( ||\boldsymbol{\alpha}||^2_2  +  \sum_{i=1}^{m_L} \sum_{l=1}^{L-1} ||\Wul{i}{l}_{1:m_{l-1}, 1:m_l}||^2_F
			+ ||\sul{i}{l}||^2_2 \right),
		\end{aligned}
	\end{equation}

	where $\Wul{i}{l}_{1:m_{l-1}, 1:m_l}$ denotes all but the last row of $\Wul{i}{l}$.

	Problem \eqref{equ:nn_train_signdetinput} is equivalent to

	\begin{equation}
		%\label{equ:nn_train_signdetinput_rescale}
		\begin{aligned}
			\min_{\boldsymbol{\alpha} \in \mathbb{R}^{m_L}, \mathbf{W^{(i,l)}}:  i \in [m_L], l \in [L-1]} \mathcal{L}_{\mathbf{y}}( f_L(X) ) + \beta ||\alpha||_1
		\end{aligned}
	\end{equation}

	where every activation function $\sigma_s(z)$ has amplitude parameter $s=1$.
\end{lemma}

\iftoggle{long}{\proofsketch{
	Since $\sigma_s$ depends only on the sign of its input, the norm of the layer weights don't change the neuron output and therefore the weights can be removed from the regularization penalty. By lemma \ref{lemma:combine_amp_with_w}, the hidden layer amplitudes can be absorbed into the weight matrices when training. The final layer amplitude parameters $s^{(i,L-1)}$ remain, and these act as $u_i$ in lemma \ref{lemma:L2toL1rescale}, which we then apply.
}}


\begin{proof}

Apply \cref{remk:signdet_inweights0} and then \cref{lemma:combine_amp_with_w}. This makes \eqref{equ:nn_train_signdetinput} is equivalent to

	\begin{equation}
		\begin{aligned}
			\min_{\boldsymbol{\alpha} \in \mathbb{R}^{m_L},  \Wul{i}{l}, \sul{i}{L-1}: l \in [L-1], i \in [m_L] } \mathcal{L}_{\mathbf{y}}(f_L(\mathbf{X};\theta) ) + \beta/2 \left ( \sum_{i=1}^{m_L} \left(\ssul{i}{L-1}\right)^2 + \alpha_i^2 \right),
		\end{aligned}
	\end{equation}

where all the inner amplitude parameters are $1$.
Next apply \cref{lemma:L2toL1rescale} with $u_i = \ssul{i}{L-1}, \params=\{\Wul{i}{l} : l \in [L-1], i \in [m_l] \}, g(\params)=\sigma_{s=1}\left (\mathbf{ \Xul{i}{L-2} \Wul{i}{L-1}} \right)$. 

\iftoggle{long}{
Let $i \in [m_L], l \in [L-1]$.  For each neuron $j \in m_l$, $\sigma^{(l)}_j(z)$ is one of two values depending only on the sign of $z$. Minimizing over $W^{(i,l)}_{1:m_{l-1},1:m_1}$ is equivalent to instead minimizing over the independent variables $u^{(i,l)} = ||W^{(i,l)_{1:m_{l-1},1:m_1}}||_F \in \mathbb{R}, v^{(i,l)}:= \frac{W^{(i,l)}_{1:m_{l-1},1:m_1}}{||W^{(i,l)}_{1:m_{l-1},1:m_1}} \in \{A \in \mathbb{R}^{m_{l-1} \times m_l}: ||A||_F = 1 \}$. The bias variables in the last rows of $W^{(i,l)}$ are not regularized and therefore can be freely rescaled: $ \Tilde{W}^{(i,l)}_{m_{l-1}+1,1:m_l} = \frac{1}{u^{(i,l)}}W^{(i,l)}_{m_{l-1}+1,1:m_l}$. Therefore the hidden layer output $X^{(i,l)}=\left[ \sigma_{s^{(i,l)}}\left( X^{(i,l-1)} W^{(i,l)} \right) , \mathbf{1} \right] =\left[ \sigma_{s^{(i,l)}} \left( u^{(i,l)}
			\begin{pmatrix}
					v^{(i,l)} \\
					{\Tilde{W}}^{(i,l)}_{m_{l-1}+1,1:m_l}
				\end{pmatrix}
			X^{(i,l-1)}   \right), \mathbf{1} \right] =\left[ \sigma_{s^{(i,l)}} \left(
			\begin{pmatrix}
					v^{(i,l)} \\
					\Tilde{W}^{(i,l)}_{m_{l-1}+1,1:m_l}
				\end{pmatrix}
			X^{(i,l-1)}   \right), \mathbf{1} \right] $ does not depend on $u^{(i,l)}$. Therefore, the regularization penalty $u^{(i,l)}=||W^{(i,l)_{1:m_{l-1},1:m_1}}||_F $ will send $u^{(i,l)} \to 0$ in the optimal solution, making the penalty zero and thus redundant.

	%, so normalizing $W^{(i,l)}_{1:m_{l-1},1:m_l}$ by $||W^{(i,l)}_{1:m_{l-1},1:m_1}||_F$ so that its Frobenuis norm is $1$ and making a change of variables to rescale the last row $W^{(i,l)}_{m_{l-1}+1,1:m_1}$ of $W^{(i,1)}$ does not change the hidden layer output $X^{(i,l)}=\sigma_{s^{(i,l)}}(X^{(i,l-1)}W^{(i,l)})$. In other words, let $\Tilde{W}^{(i,l)}_{1:m_{l-1}, 1:m_l}=\frac{1}{||W^{(i,l)}_{1:m_{l-1}, 1:m_l}||_F}W^{(i,l)}, \Tilde{W}^{(i,l)}_{m_{l-1}+1,1:m_l}=$ 

	%$X^{(i,l)} = \left[ \sigma_{s^{(i,l)}}\left( x^{(i,l-1)} W^{(i,l)} \right) , \mathbf{1} \right] = \left[ \sigma_{s^{(i,l)}}\left( \sum_{j=1}^{m_{l-1}} x^{(i,l-1)} W^{(i,l)}_{1:m_,j}\right) , \mathbf{1} \right]$

	Similarly, for each hidden layer $l \in [L-1]$ before the last layer and neuron $j \in [m_l]$ we can also normalize $s^{(i,l)}$ by $||s^{(i,l)}||_2$ and again rescale the last row of $W^{(i,l+1)}$ by $||s^{(i,l)}||_2$ without changing the output $X^{(i,l+1)}$.

	Therefore, the regularization terms $||W^{(i,l)}_{1:m_{l-1}, 1:m_l}||^2_F$ for $l \in [L]$ and $ ||s^{(i,l)}||^2_2 $ for  $l \in [L-1]$ become redundant in the minimization.
	So the only regularization term that remains is $\sum_{i=1}^{m_L}||s^{(L)}||^2_2 + \alpha_i^2$. Therefore, plugging in \eqref{parLlayernn_signdet} into $f_L$ makes problem \eqref{equ:nn_train_signdetinput_rescale} equivalent to

	\begin{equation}
		\label{equ:nn_train_signdetinput_simp}
		\begin{aligned}
			\min_{\substack{\alpha \in \mathbb{R}^{m_L},  s^{(i,l)}: ||s^{(i,l)}||_2=1, i \in [L-2], \\  W^{(i,l)}: ||W^{(i,l)}||_F=1, l \in [L-1], i \in [m_L] }} &\mathcal{L}_{\mathbf{y}}\left(\sum_{i=1}^{m_L} s^{(i,L-1)} \sigma_{s=1} \left ( X^{(i,L-2)} W^{(i,L-1)}_{1:m_{1-1}, 1:m_l} \right) \alpha_i  \right)
			+ \beta/2 \left ( \sum_{i=1}^{m_L}||s^{(L)}||^2_2 + \alpha_i^2 \right).
		\end{aligned}
	\end{equation}



	By lemma \ref{lemma:L2toL1rescale} with $u_i = s^{(i,L-1)}, \Theta=\{W^{(i,l)}: l \in [L-1], i \in [m_l] \}, g(\Theta)=\sigma_{s=1}\left ( x^{(i,L-2)} W^{(i,L-1)} \right)$, problem \ref{equ:nn_train_signdetinput_simp} is equivalent to

	\begin{equation}
		\label{equ:nn_train_signdetinput_simp}
		\begin{aligned}
			\min_{\substack{ \alpha \in \mathbb{R}^{m_L}, s^{(i,l)}:  ||s^{(i,l)}||_2=1, i \in [L-2], \\ W^{(i,l)}: ||W^{(i,l)}_{1:m_{1-1}, 1:m_l}||_F=1, l \in [L-1], i \in [m_L] }} \mathcal{L}_{\mathbf{y}}\left(\sum_{i=1}^{m_L}  \sigma_{s=1} \left ( X^{(i,L-2)} W^{(i,L-1)} \right) \alpha_i  \right) + \beta ||\alpha||_1 .
		\end{aligned}
	\end{equation}

	Problem \ref{equ:nn_train_signdetinput_simp} can be written according to lemma \ref{lemma:combine_amp_with_w} and equations  \ref{nn_unrolled}, \ref{x_unrolled}, \ref{w_unrolled} as

	\begin{equation}
		\label{equ:nn_train_signdetinput_simp_unrolled}
		\begin{aligned}
			\min_{\substack{ \alpha \in \mathbb{R}^{m_L},  s^{(i,l)}:  s^{(i,l)}, i \in [L-2], \\ W^{(i,l)} :||W^{(i,l)}_{1:m_{1-1}, 1:m_l}||_F=1, l \in [L-1], i \in [m_L]} } \mathcal{L}_{\mathbf{y}}\left(\sum_{i=1}^{m_L}  \sigma_{s=1} \left ( \tilde{X}^{(i,L-2)} \tilde{W}^{(i,L-1)} \right) \alpha_i  \right) + \beta ||\alpha||_1 .
		\end{aligned}
	\end{equation}


	The amplitude parameters always appear as a product with the next layer weights, so they can be combined into one variable $W^{(i,L-1)}=  \tilde{W}^{(i,l)} =  \mathrm{Diag} ([{s^{(i,l-1)}}^T, 1]) W^{(i,l)}$ \eqref{w_unrolled} with the corresponding redefinition $ X^{(i,l)}= \left[ \sigma_{s=1}\left( X^{(i,l-1)} w^{(i,l)} \right) , \mathbf{1} \right]$. So \eqref{equ:nn_train_signdetinput_simp_unrolled} becomes

	\begin{equation}
		\label{equ:nn_train_signdetinput_f}
		\begin{aligned}
			\min_{\alpha \in \mathbb{R}^{m_L},   W^{(i,l)}: ||W^{(i,l)}_{1:m_{1-1}, 1:m_l}||_F=1, l \in [L-1], i \in [m_L] } \mathcal{L}_{\mathbf{y}} \left(\sum_{i=1}^{m_L}  \sigma_{s=1} \left ( X^{(i,L-2)} W^{(i,L-1)} \right) \alpha_i  \right) + \beta ||\alpha||_1,
		\end{aligned}
	\end{equation}

	where all the amplitude parameters $s^{(i,l)}_j=1$.


	For sign-determined activation functions (sign, threshold), the general neural network $f_L(X)$ is invariant to the weight norms $||W^{(i,l)}||_F$. And the norm weights $||W^{(i,l)}||_F$ are not penalized in \eqref{equ:nn_train_signdetinput_f}. So we can rescale the bias weights $||W^{(i,l)}_{m_{l},1:m_l}||_F$ and normalize by $||W^{(i,l)}_{1:m_{l-1},1:m_l}||_F$, to turn training problem \eqref{equ:nn_train_signdetinput_f} into an equivalent problem where $||W^{(i,l)}_{1:m_{l-1},1:m_l}||_F$ is unconstrained.

}
	
\end{proof}

\begin{proposition}
	\label{lemma:tree_rescale}
	%The tree network $f_L = f^{L, \Theta^L}={f_L}_{\textrm{tree}}$ with a sign-determined activation can be rescaled similarly.

	Consider the training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro} for a tree neural net (\cref{app_subsection:tree_nn_def}) %\eqref{eq:nonconvex_generic_loss_gen_L_tree} 
	with $L$ layers and a sign-determined activation:

	\begin{equation}
		\label{equ:nn_train_signdetinput_tree}
		\begin{aligned}
			\min_{\boldsymbol{\alpha} \in \mathbb{R}^{m_L},  \mathbf{w^{(l)}}, \ssul{i}{l} \in \theta} \mathcal{L}_{\mathbf{y}}(f_L(\mathbf{X};\theta) ) + \frac{\beta}{2} \left (  \sum_{\mathbf{w^{(l)}, s^{(l,i)}} \in \theta} ||{\mathbf{w^{(l)}}}_{1:m_{l}}||^2_2
			+  \left(\ssul{i}{l} \right)^2 \right)
		\end{aligned},
	\end{equation}

	where $\mathbf{w^{(l)}}_{1:m_{l}}$ denotes all but the last (bias) element of $\mathbf{w^{(l)}}$. %and $\regparams$ contains all layer weights excluding bias terms of the form $w^{(l)}_{m_{l}}$ and $\xi$ as defined in \eqref{def:tree_networks}. %not writing \xi anyway and w^l vector is in \theta not \regparams

	Problem \eqref{equ:nn_train_signdetinput_tree} is equivalent to

	\begin{equation}
		%\label{equ:nn_train_signdetinput_rescale}
		\begin{aligned}
			\min_{\boldsymbol{\alpha} \in \mathbb{R}^{m_L}, \mathbf{w^{(l)}} \in \theta } \mathcal{L}_{\mathbf{y}}( \nn{L}{\mathbf{X}} ) + \beta ||\boldsymbol{\alpha}||_1,
		\end{aligned}
	\end{equation}

	where every activation function $\sigma_s(z)$ has amplitude parameter $s=1$.

\end{proposition}


\begin{proof}
	The proof is analogous to that of  \cref{prop:sign-det_rescale}.
Apply \cref{remk:signdet_inweights0tree} so that only the outer layer parameters $\ssul{i}{L-1}, \boldsymbol{\alpha}$ are regularized. Then decomposing $\sigma_{\ssul{i}{l-1}}(z)=\ssul{i}{l-1}\sigma(z)$, we note that for the inner layers since $\ssul{i}{l-1}w^{(l)}_i$ always appear as a product, they can be combined into one variable. So the inner layer activations become the standard $\sigma_{s=1}(z)$ and the only amplitude parameters remaining are for the outer layer: $\ssul{i}{L-1}$. Then apply \cref{lemma:L2toL1rescale}.

\iftoggle{long}{
	For each layer $l \in [L]$, and each unit $i \in [m_l]$, the subtree network $f^{(l-1)}(\mathbf{X}; \theta^{l-1,i})=\mathbf{1}w^{(l)}_{m_l + 1}+ \sum_{j=1}^{m_{l-2}} \sigma_{s^{l-2,i,j}}(f^{(l-2), \Theta^{l-2,i,j}})w^{(l-1)}_{i,j}
	$ is invariant to the total magnitude of the weight terms excluding bias in the previous layer $l-1$, ie $\sum_{j=1}^{m_{l-2}} ||w^{(l-1,i,j)}_{1:m_{l-2}}||^2_2$ and to the magnitude of the sign parameters, ie $\sum_{j=1}^{m_{l-2}}(s^{l-2,i,j})^2$. %And the bias terms are unpenalized and can be rescaled without affecting the training loss $\mathcal{L}_{\mathbf{y}}(f^{(L),\Theta^{L}})$. 
	So the regularization penalty will send the magnitudes of the non-bias weights and sign parameters to zero, making the regularization also zero.
	% So except for the final layer $L$, we can set each penalty term to one: $\sum_{j=1}^{m_{l-2}} ||w^{(l-1,i,j)}_{1:m_{l-2}}||^2_2 = \sum_{j=1}^{m_{l-2}}{s^{l-2,i,j}}^2 = 1$, removing their regularization. 
	So the only regularization term that remains is $\sum_{i=1}^{m_L} ({w^{(l)}_i})^2$.


	As similar to lemma \eqref{lemma:combine_amp_with_w}, for every layer $l \in [L]$ and subnetwork $i \in [m_l]$ the variables variables $ s^{l-1,i}w^{(l)}_i$ always appear as a product, so they can be absorbed into one variable, making the amplitude parameters all be $1$, so that each activation is the function $\sigma_{s=1}(x)$. Finally, apply lemma  \ref{lemma:L2toL1rescale} to turn the $l_2$ penaty into the $l_1$ penalty $ \beta \sum_{i=1}^{m_L} |w^{(L)}_{i}| = \beta ||\alpha||_1$.

	As similar to the proof of lemma \ref{prop:sign-det_rescale}, the above rescaling constrained the total norm of the weights in each layer to $1$. For sign-determined activation functions (sign, threshold), the general neural network $f_L(X)$ is invariant to the norms of the weights. So we can rescale the bias and normalize by the weights to leave the weights unconstrained. %weight norms $||W^{(l)}||_F$. %And the norm weights $||W^{(l)}||_F$ are not penalized in \eqref{equ:nn_train_signdetinput_f}. 
	%So we can rescale the bias weights $||w^{(l)}_{m_{l}+1}||_2$ and normalize by $||w^{(l)}_{1:m_{l}}||_2$, to leave $||w^{(l)}_{1:m_{l}}||_2$ unconstrained.
}
\end{proof}


\subsubsection{general rescaled training problem}

%Let $\theta_s \subset \theta$ be the set of training parameters consisting of just the layer weights $\mathbf{w}$, neuron biases and final layer coefficients $\alpha \in \mathbb{R}^{m_L}$ (no amplitude parameters $s$ or external bias $\xi$). 
Let $\Theta_s \subset \Theta$ be the parameter space with the constraint that all activation amplitudes are $1$, and if $L=2$, the last hidden layer weights $\mathbf{w^{(i)}}$ have unit norm $||\mathbf{w^{(i)}}||_2=1$. If the activation is sign-determined, then the weight norms can be constrained or not (\cref{remk:signdet_inweights0}, \cref{remk:signdet_inweights0tree}). % the parallel network, %if $L\leq 2$ 
	% the weights $W^{(i,L-1)}$ of the last hidden layer satisfy $||W^{i,L-1}||_F=1$. %, where the norm of each layer weight (which is a matrix for parallel networks and a vector for tree networks) excluding bias is $1$.

	%   Specifically, 

	% \begin{equation}\label{def:theta'_par}
	% \begin{aligned}
	%     \Theta' &:= \Theta - \{s_j: s_j \in \Theta \}
	% \end{aligned}
	% \end{equation}

	%  Specifically for the parallel network, 
	%  \begin{equation}\label{def:theta'_par}
	%   \begin{aligned}
	%        \Theta' &:= \{ \alpha \in \mathbb{R}^{m_L}, W^{(i,l)}: ||W^{(i,l)}_{1:m_{1-1}, 1:m_l}||_F=1, i \in [m_L], l \in [L-1]\}.
	%   \end{aligned}
	%   \end{equation}
	%   And for the tree network,
	%       \begin{equation}
	%   \begin{aligned}
	%        \Theta' &:= \{\alpha \in \mathbb{R}^{m_L}, w^{(l)} \in \Theta: ||w^{(l)}_{1:m_{1}}||_2=1, i \in [m_L], l \in [L-1]\}.
	%    \end{aligned}
	%    \end{equation}

	%did not include $\xi$ becuase in the training problem, that is part of the loss. w^l there are many of them in the tree network.

\begin{theorem}\label{thrm:rescaling}

	The general, $d$-dimensional \nc{} training problem  \eqref{eq:nonconvex_generic_loss_gen_L_intro} for the case of $L=2$ layers with leaky ReLU, ReLU, absolute value, sign, or threshold activations and for the case of $L\geq2$-layer tree or parallel networks with sign and threshold activations is equivalent to

	\begin{equation}\label{equ:nn_train_signdetinput_rescale}
		\begin{aligned}
			\min_{\theta \in \Theta_s} \mathcal{L}_{\mathbf{y}}( \nn{L}{\mathbf{X}} ) + \beta ||\boldsymbol{\alpha}||_1.
		\end{aligned}
	\end{equation}

\end{theorem}

\begin{proof}
Leaky ReLU, ReLU, and absolute value are homogeneous activations, while sign and threshold are sign-determined activations (\cref{app_section:act_func}). Apply \cref{prop:2layerhomrescale} for leaky ReLU, ReLU, and absolute value activations.
Apply \cref{prop:sign-det_rescale} and \cref{lemma:tree_rescale} for sign and threshold activations.

\iftoggle{long}{Note that for $L=2$ layers, problem \ref{eq:train_hom} is the same as \eqref{equ:nn_train_signdetinput_rescale}.
	Proposition \ref{prop:2layerhomrescale} for $L=2$ parallel layers prove the result for  homogeneous activations which include leaky ReLU, ReLU and absolute value.

	For sign and threshold activations, note that the norms of the weights and neuron biases do not affect the activations. So proposition \ref{prop:sign-det_rescale} and \ref{lemma:tree_rescale}  for $L\geq 2$-layer parallel and tree sign-determined activation functions prove the result.}

	
\end{proof}






\subsection{Derivation of the dual of the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale}}





\begin{lemma}\label{lemma:dual_of_rescaled}
\iftoggle{long}{Let $\Theta' \subset \Theta_s$ be the set of parameters consisting of bias terms, and layer weights for just one branch $i$ of the last layer $L$.

	Specifically for parallel networks,

	\begin{equation}
		\begin{aligned}
			\Theta' & :=
			\begin{cases}
				\{W^{(1,l)}:  l \in [L-1]\}     & \mbox{ if } L>2 \\
				\{w^i: i \in m_l, ||w^i||_2=1\} & \mbox{ if } L=2
			\end{cases}
		\end{aligned}
	\end{equation}

	For tree networks with $L>2$,  $\Theta'$ consists of all layer weight vectors $w^{(l)} \in \Theta$ that determine $f^{(L,1)}$ (or any other branch $f^{(L,i)}$).

}
	
	The dual of the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} for a neural net $f_L$ \eqref{eq:univ_NN} is

	\begin{equation}\label{gen_dual_gen_arch}
		\begin{aligned}
			\max_{{\lambda} \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( {\lambda} )                                            \\
			\text{ s.t. }                   & \max_{\theta \in \Theta_s}\left |{\lambda}^T \sigma \left ( \sful{1}{L-1}\left(\mathbf{X}; \params^{(L-1)} \right)\right) \right| \leq \beta,
		\end{aligned}
	\end{equation}

	
 where $f^*(\mathbf{x}):=\max_{\mathbf{x}} \{ \mathbf{z}^T \mathbf{x} - f(\mathbf{x}) \}$ denotes the convex conjugate of a function $f$.
The constraint in \eqref{gen_dual_gen_arch} involves just one unit $\sful{1}{L-1}$ of the tree/parallel net; for a $2$-layer net this is just one neuron. For parallel nets \eqref{gen_dual_gen_arch} it is
	\begin{equation}\label{gen_dual}
		\begin{aligned}
			\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda )                                                                      \\
			\text{ s.t. }                   & 
   \max_{\theta \in \Theta_s} \left|\lambda^T \sigma \left ( \mathbf{X^{(L-2)} }\Wul{i}{L-1} \right) \right| \leq \beta.
   %\max_{\mathbf{}W^{(1,l)} \in \Theta'} \left|\lambda^T \sigma \left ( \mathbf{X^{(L-2)} W^{(1,L-1)}}\right) \right| \leq \beta.
			% \text{ s.t. }&  \max_{W^{(1,l)}: ||W^{(l)}_{1:m_{1-1}, 1:m_l}||_F=1,  l \in [L-1]} \left|\lambda^T \sigma \left ( X^{(L-2)} W^{(L-1)}\right) \right| \leq \beta
		\end{aligned}
	\end{equation}

\end{lemma}

\begin{proof}

	Rewrite \eqref{equ:nn_train_signdetinput_rescale} as,

	\begin{equation}\label{gen_prep_to_dual}
		\begin{aligned}
			% \min_{\alpha \in \mathbb{R}^{m_L}, W^{(i,l)}: ||W^{(i,l)}_{1:m_{1-1}, 1:m_l}||_F=1, i \in [m_L], l \in [L-1]} 
			\min_{\theta \in \Theta_s}
			              & \mathcal{L}_{\mathbf{y}}( \mathbf{z} ) + \beta ||\boldsymbol{\alpha}||_1 \\
			\text{ s.t. } & \mathbf{z} = f_L(\mathbf{X};\theta).
		\end{aligned}
	\end{equation}

	The Lagrangian of problem \eqref{gen_prep_to_dual} is

	\begin{equation}\label{gen_lag}
		\begin{aligned}
			% L\left(\lambda,\alpha, W^{(i,l)}: i \in [m_L], l \in [L-1]\right) 
			L\left(\lambda, \boldsymbol{\alpha}, \Theta_s - \{\boldsymbol{\alpha}\}\right)
			 & = \mathcal{L}_{\mathbf{y}}( \mathbf{z} ) + \beta ||\boldsymbol{\alpha}||_1  - \lambda^T \mathbf{z} + \lambda^T f_L(\mathbf{X};\theta)                                                       \\
			 & = \mathcal{L}_{\mathbf{y}}( \mathbf{z} ) - \lambda^T\mathbf{z}  + \beta ||\boldsymbol{\alpha}||_1  + \sum_{i=1}^{m_L} \lambda^T \sigma \left (  \sful{i}{L-1}\left(\mathbf{X};\theta^{(L-1)} \right)\right) \alpha_i. 
		\end{aligned}
	\end{equation}

	Minimize the Lagrangian \eqref{gen_lag} over $\mathbf{z}$ and $\boldsymbol{\alpha}$ and use Fenchel duality \cite{boyd:2004}. The dual of \eqref{gen_prep_to_dual} is

	\begin{equation}\label{gen_dual_int}
		\begin{aligned}
			\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda ) \\
			\text{ s.t. }                   &
			% \max_{W^{(i,l)}: ||W^{(i,l)}_{1:m_{1-1}, 1:m_l}||_F=1, l \in [L-1]} 
			\max_{\theta \in \Theta_s}
			\left|\lambda^T \sigma \left ( \sful{i}{L-1} \left(\mathbf{X}; \theta^{(L-1)} \right) \right) \right| \leq \beta, i \in [m_L].
		\end{aligned}
	\end{equation}

	
	In the tree and parallel nets, each subnet $ \sful{i}{L-1}$ has the same architecture for all $i \in [m_L]$  (\cref{app_sec:parallel_nn_def}, \cref{app_subsection:tree_nn_def}). So the $m_l$ constraints in \eqref{gen_dual_int} collapse to just one constraint, and \eqref{gen_dual_int} becomes \eqref{gen_dual} as desired. For parallel architectures, plug in \eqref{par_def} for the neural net in \eqref{gen_dual}.
\iftoggle{long}{For parallel architectures, set $ \sful{i}{L-1}(X)=X^{(L-2,i)} W^{(L-1,i)}$ and $f^{(L-1)}(X)=X^{(L-2)} W^{(L-1)}$, ie just one copy of or subnetwork $ \sful{i}{L-1}(X)=X^{(L-2,i)} W^{(L-1,i)}$.}


\end{proof}

Now, we simplify the dual problem \eqref{gen_dual} for some different cases of the parallel versus tree architecture defining $f^{(L-1)}$, neural net depth $L$, data dimension $d$, and activation function $\sigma$ .

\subsection{$L=2$ layer, $d=1$-dimensional dual}


%for unbdd actvn: the original dual already implicitely has the constraint that lamnda^T1 = 0 (this comes from the scenario case when lambda is such that  the inf of the Lag is not -infinity.) but when we rewrite it we need to include this explicitely, bc otherwise no longer implied by just what we have. 

%\begin{proof}
%    Suppose $L=2,d=1$. Recall \cref{rk:L=2_d=1constraint}. Suppose $\lambda^*$ is optimal in problem \eqref{L=2_d=1_dual_finite} in \cref{lemma:dual_finite}. By the main theorem, this is the optimal value of the nonconvex problem. Let $I = \{n \in [N-1]: g_w(-w x_n) = g_w(-w x_{n+1})\}$. 
%    Observe for ReLU activation we can write $I = \{n \in [N-1]: \sum_{i=1}^n \lambda_i = 0 \}$ (\textcolor{red}{check}). For $n \in [N]$ suppose 
%    \begin{equation}
%    \tilde{x}_n 
%        \begin{cases}
%             = -w x_n \mbox{ if } n \notin I \\
%            \in -w [x_{n+1}, x_{n}] \mbox{ else }
%        \end{cases}. %x_i is descending
%    \end{equation}
%    \textcolor{red}{check endpoints }
%Consider \cref{L=2_d=1_dual_finite} where $x_n$ is changed to $\tilde{x_n}$. Then $\lambda^*$ is still feasible in the new version. 
%But the new version might give better max, with different lambda? So not actually the dual
%Then $\lambda^*$ achieves the same value in \cref{L=2_d=1_dual_finite} as the new version. Since $\lambda^*$ is optimal in \cref{L=2_d=1_dual_finite}, the new version is an upper bound. On the other hand the 
%\end{proof}

\begin{lemma}\label{lemma:dual_finite}
	For $L=2,d=1$, the dual in \cref{lemma:dual_of_rescaled} of the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} is equivalent to
	\begin{equation}\label{L=2_d=1_dual_finite}
		\begin{aligned}
			\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda )                       \\
			\text{ s.t. }                   & |\lambda^T \sigma(\mathbf{X}-x_n\mathbf{1})| \leq \beta, \quad   
			                                 |\lambda^T \sigma(x_n\mathbf{1}-\mathbf{X})| \leq \beta, n \in [N]    \\
			                                & \lambda^T \mathbf{1} = 0 \quad \text{ if $c_1 \neq 0$ or $c_2 \neq 0$},
		\end{aligned}
	\end{equation}

where $c_1, c_2$ are activation function slopes as defined in \cref{app_section:act_func}.
\end{lemma}

\proofsketch{
	The dual \eqref{gen_dual} constrains 
 \iftoggle{long}{ the single neuron output }
$\pm \lambda^T\sigma(\mathbf{X}w+b)$ over $w = \pm 1$. 
 \iftoggle{long}{where $w = \pm 1$}
  This is maximized when an argument to $\sigma$ is zero (covered by inequalities in \eqref{L=2_d=1_dual_finite}), or at $b \to \pm \infty$ (forbidden by $\lambda^T \mathbf{1}=1$.) 
 \iftoggle{long}{ The slope changes when the argument of $\sigma$ is $0$. So we only need to consider $b = \pm x_n$ for  $n \in [N]$ and make sure that at such $b$, $-\beta \leq \lambda^T \sigma(\pm \mathbf{X} +b) \leq \beta$.}
}

\begin{proof}
   For a $2$-layer network with $d=1$, we have $\mathbf{X} \in \mathbb{R}^N$, $m_0 = d+1=2, m_1= m_{L-1}= 1, \mathbf{X}^{(L-2)}=\mathbf{X}^{(0)}=[\mathbf{X},\mathbf{1}]$ and $ \Wul{i}{L-1}  =(w,b)^T \in \mathbb{R}^2$. 
\iftoggle{long}{ and each neuron is of the form $(w,b)^T \in \mathbb{R}^{2}$, where $w$ is the weight and $b$ is the bias of the neuron.} For fixed $\lambda, \mathbf{X}, w$, let $g_w: \mathbb{R} \to \mathbb{R}, g_w(b) = \lambda^T \sigma(\mathbf{X}w+b\mathbf{1})= \sum_{n=1}^N \lambda_n \sigma(x_n w + b) $. 
 We can write the constraint $ \max_{\theta \in \Theta_s} \left|\lambda^T \sigma \left ( \mathbf{X^{(L-2)} } \Wul{i}{L-1} \right) \right| \leq \beta$ in the dual \eqref{gen_dual} as

	\begin{equation}\label{L=2_d=1_dual}
		\begin{aligned}
		%	\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda )                                \\
			%\text{ s.t. }  
%   & \max_{b \in \mathbb{R}, w = \pm 1 } \lambda^T \sigma(\mathbf{X}w+b) \leq \beta \\
 %           &\max_{b \in \mathbb{R}, w = \pm 1 } -\lambda^T \sigma(\mathbf{X}w+b) \leq \beta.
          \max_{b \in \mathbb{R}, w = \pm 1 } g_w(b) \leq \beta \mbox{ and }
            \max_{b \in \mathbb{R}, w = \pm 1 } -g_w(b) \leq \beta.
		\end{aligned}
	\end{equation}
%When $L=2, d=1$, we have $\mathbf{X} \in \mathbb{R}^N$, the layer sizes are $m_0 = d+1=2, m_1= m_{L-1}= 1, \mathbf{X}^{(L-2)}=\mathbf{X}^{(0)}=[\mathbf{X},\mathbf{1}], \Wul{i}{L-1}  =(w,b)^T \in \mathbb{R}^2$. 
%\iftoggle{long}{ and each neuron is of the form $(w,b)^T \in \mathbb{R}^{2}$, where $w$ is the weight and $b$ is the bias of the neuron.} For fixed $\lambda, \mathbf{X}, w$, let $g_w: \mathbb{R} \to \mathbb{R}, g_w(b) = \lambda^T \sigma(\mathbf{X}w+b\mathbf{1})= \sum_{n=1}^N \lambda_n \sigma(x_n w + b) $. 
% We can write the constraint $ \max_{\theta \in \Theta_s} \left|\lambda^T \sigma \left ( \mathbf{X^{(L-2)} } \Wul{i}{L-1} \right) \right| \leq \beta$ in the dual \eqref{gen_dual} as,

%	\begin{equation}\label{L=2_d=1_dual}
%		\begin{aligned}
		%	\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda )                                \\
			%\text{ s.t. }  
%   & \max_{b \in \mathbb{R}, w = \pm 1 } \lambda^T \sigma(\mathbf{X}w+b) \leq \beta \\
 %           &\max_{b \in \mathbb{R}, w = \pm 1 } -\lambda^T \sigma(\mathbf{X}w+b) \leq \beta.
%          \max_{b \in \mathbb{R}, w = \pm 1 } g_w(b) \leq \beta \mbox{ and }
%            \max_{b \in \mathbb{R}, w = \pm 1 } -g_w(b) \leq \beta.
%		\end{aligned}
%	\end{equation}
Since $\sigma$ is piecewise linear (\cref{app_section:act_func}), so is $g_w$. So its subgradient is

	$\partial g_w(b) = \sum_{n: x_n w + b > 0} \lambda_n c_2 + \sum_{n: x_n w + b < 0} \lambda_n c_1 + \sum_{n: x_n w + b = 0} [\min\{c_1, c_2\}, \max \{ c_1, c_2\}].$

	Note that $\partial g$ and $\partial ({-g})=-\partial g$ only change at 
 \iftoggle{long}{ $b$ such that $x_n w + b =0$ for some $n\in[N]$, i.e., }
$b \in B_w:=\{-x_n w: n \in [N]\}$. 
\iftoggle{long}{ We define $b$ to be a global optimizer of $g$ if $g(b) = \max_{b' \in \mathbb{R}} g(b')$.}
So $g_w$ and $-g_w$ have global maximizers in $B_w$, as long as $\lim_{b \to \pm \infty} |g_w(b)| < \infty$, which is implied by \eqref{L=2_d=1_dual}.
\iftoggle{long}{
 So $B_w \cup \{-\infty, +\infty\}$ contains global maximizers of $g_w$ and $-g_w$. }
 Plugging in all possible $b \in B_w, w = \pm 1$ into $g_w(b) \leq \beta$ from \eqref{L=2_d=1_dual} gives the inequality constraints in \eqref{L=2_d=1_dual_finite}.
\iftoggle{long}{ So the constraint in the dual problem \eqref{L=2_d=1_dual} means for each possible value of $w=1$ or $w=-1$, it suffices to ensure that $|\lambda^T \sigma(Xw+b)|\leq \beta$ for all $b \in B$, which matches the inequality constraints in \eqref{L=2_d=1_dual_finite}.
 The set $\{-\infty, +\infty\}$ but not $B_w$ contains a global maximizer of $|g_w|$ if and only if $\max |g_w| = \infty$, which contradicts the constraints \cref{L=2_d=1_dual}. We have the following cases. If a maximizer is not in $B_w$ and is instead $\pm \infty$ then 
Next we derive the equality constraint in  \eqref{L=2_d=1_dual_finite}. Feasibility of the dual requires $\max_b |g_w(b)| < \infty$.
We consider two cases regarding whether $c_1, c_2$ are zero to determine if $B_w$ contains a global maximizer of $|g_w|$.
}
To make this equivalent to \eqref{L=2_d=1_dual} requires
a guarantee that $\lim_{b \to \pm \infty} |g_w(b)| < \infty$. We show this guarantee holds when $c_2=c_1=0$ but requires the constraint $\lambda^T \mathbf{1}=0$ otherwise. 

\iftoggle{long}{The equality constraint in \eqref{L=2_d=1_dual_finite} ensures that the condition $\lim_{b \to \pm \infty} |g_w(b)| < \infty$. We have two cases.}

 
	\textbf{Case 1}: Suppose $c_1\neq 0$ or $c_2 \neq 0$ (e.g., leaky ReLU) and $\lambda^T \mathbf{1} \neq 0$. If $c_1 \neq 0$ then $\lim_{b \to -\infty} |g_w(b)| =  \lim_{b \to \infty} |\sum_{n=1}^N \lambda_n(c_1 (x_n w+b) + d_1)| = \lim_{b \to \infty} | \lambda^T (wc_1\mathbf{X} + d_1\mathbf{1})  + c_1 b \lambda^T \mathbf{1} | < \infty$ if and only if $\lambda^T \mathbf{1} =0$. Similarly if $c_2 \neq 0$ then
  $\lim_{b \to \infty} |g_w(b)| = \infty$ 
 \iftoggle{long}{ $\lim_{b \to \infty} |g_w(b)| = \lim_{b \to \infty} | (wc_2x + d_2\mathbf{1}) + c_2  \lambda^T \mathbf{1} b| = \infty$ }
if and only if $\lambda^T \mathbf{1} =0$. Therefore $B_w$ contains a global maximizer of $|g_w|$ if and only if $\lambda^T\mathbf{1}=0$. 
\iftoggle{long}{In other words,  $\lambda^T \mathbf{1}=0$ ensures that the dual \eqref{L=2_d=1_dual} is feasible. }


\iftoggle{long}{So that strong duality can hold with the primal \eqref{equ:nn_train_signdetinput_rescale}.}


	\textbf{Case 2}: Suppose $c_2 = c_1 = 0$. Then $|g_w(b)|$ is bounded, and a global optimum exists in $B$.


So, the constraints in problems \eqref{L=2_d=1_dual} and \eqref{L=2_d=1_dual_finite} are equivalent.
\end{proof}

\begin{lemma}\label{lemma:lasso_without_simp}
	Suppose $L=2, d=1$. Let $\mathbf{A}$ be defined as in \cref{theo:1d_all}.
 \iftoggle{long}{Let $ \mathbf{A_+}, \mathbf{A_-} \in \mathbb{R}^{N \times N}$ be defined by $\mathbf{{A_+}}_{i,j}=\sigma(x_i-x_j), \mathbf{{A_-}}_{i,j}=\sigma(x_j-x_i)$.}
	 The bidual (dual of the dual) of the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} is

	\begin{equation}\label{gen_lasso_sol}
		\begin{aligned}
  \iftoggle{long}{\min_{\mathbf{z_+}, \mathbf{z_-} \in \mathbb{R}^N, \xi \in \mathbb{R}} & \mathcal{L}_{\mathbf{y}}(\mathbf{ A_+ z_+} +  \mathbf{A_- z_- } + \xi \mathbf{1} )+ \beta (||\mathbf{z_+}||_1 + ||\mathbf{z_-}||_1), 
			\quad \text{ where }                                      & \xi=0 \text{ if }  c_1=c_2=0,}
			\min_{\mathbf{z} \in \mathbb{R}^{2N}, \xi \in \mathbb{R}} & \mathcal{L}_{\mathbf{y}}(\mathbf{ A z} + \xi \mathbf{1} )+ \beta \|\mathbf{z}\|_1 
			\quad \text{ where }                                      & \xi=0 \text{ if }  c_1=c_2=0,
		\end{aligned}
	\end{equation}
and $c_1, c_2$ are activation function slopes as defined in \cref{app_section:act_func}. %Maybe this is confusing for $\xi$.


\end{lemma}

\iftoggle{long}{\proofsketch{
To take the bidual of \eqref{equ:nn_train_signdetinput_rescale} we take the dual of the dual problem \eqref{L=2_d=1_dual} by minimizing its Lagrangian. Intuitively, the primal and bidual resemble forms: the training loss $\mathcal{L}_{\mathbf{y}}$ that appeared in the primal \eqref{equ:nn_train_signdetinput_rescale} returns as is in the bidual, and like the primal the bidual contains $l_1$ penalties.
}
}

\begin{proof}
\cref{lemma:dual_finite} gives the dual as \eqref{L=2_d=1_dual_finite}, so we take its dual. 
%Denote the $n^{\textrm{th}}$ column of $A_+, A_-$ respectively  as ${a_+}_n = \sigma(X-x_n \mathbf{1}), {a_-}_n = \sigma(x_n \mathbf{1}-X)\in \mathbb{R}^n$.
\iftoggle{long}{By the definition of $A_+, A_-$ and lemma \ref{lemma:dual_finite}, }
Problem \eqref{L=2_d=1_dual_finite} can be written as

	\begin{equation} \label{L=2_d=1_dual_as_min}
		\begin{aligned}
			-\min_{\lambda \in \mathbb{R}^N} & \mathcal{L}_{\mathbf{y}}^*( \lambda )                        \\
			\text{ s.t. }
 %  \iftoggle{long}{ |\lambda^T \mathbf{A_+}| \leq \beta \mathbf{1}^T, \quad       
%			                                  |\lambda^T \mathbf{A_-}|\leq \beta \mathbf{1}     }
                                    & | \lambda^T \mathbf{A}| \leq \beta \mathbf{1}^T \\
                                    & \lambda^T \mathbf{1} = 0 \quad \text{ if $c_1 \neq 0$ or $c_2 \neq 0$}
		\end{aligned},
	\end{equation}




	where $\mathbf{1} \in \mathbb{R}^{2N}$. The Lagrangian of the negation of \eqref{L=2_d=1_dual_as_min} with bidual variables $\mathbf{z} \in \mathbb{R}^{2N}, \xi \in \mathbb{R}$ is

	\begin{equation} \label{bidual_Lag}
		\begin{aligned}
			L(\lambda, \mathbf{z},\xi)   %&= \mathcal{L}_{\mathbf{y}}^*(\lambda) + (\beta |\mathbf{z}|^T \mathbf{1}-\lambda^T \mathbf{A z} )  - \xi \lambda^T \mathbf{1} \\
			   % & = -\lambda^T( \mathbf{A z} + \xi \mathbf{1}) + \mathcal{L}_{\mathbf{y}}^*(\lambda) + \beta \|\mathbf{z}\|_1,
         & = \mathcal{L}_{\mathbf{y}}^*(\lambda) - \lambda^T( \mathbf{A z} + \xi \mathbf{1}) - \beta \|\mathbf{z}\|_1,
		\end{aligned}
	\end{equation}

	where $\xi=0$ if $c_1=c_2=0$.
 \iftoggle{long}{ , e.g. if the activation $\sigma(x)$ is a sign or threshold.}
Equation \eqref{bidual_Lag} holds because the constraint  $|\lambda^T \mathbf{A}| \leq \beta \mathbf{1}^T$ 
\iftoggle{long}{in \eqref{L=2_d=1_dual_as_min}}
i.e.,
\iftoggle{long}{$2N$ scalar constraints}
 $\lambda^T \mathbf{A} - \beta \mathbf{1}^T \leq \mathbf{0}^T, -\lambda^T \mathbf{A} - \beta \mathbf{1}^T \leq \mathbf{0}^T$ appears in the Lagrangian as $\lambda^T \mathbf{A}(\mathbf{z^{(1)}}-\mathbf{z^{(2)}}) -  \beta \mathbf{1}^T (\mathbf{z^{(1)}}+\mathbf{z^{(2)}}))$ with bidual variables $\mathbf{z^{(1)}}, \mathbf{z^{(2)}} \in \mathbb{R}^{2N}_+$, which are combined into one bidual variable $\mathbf{z} = \mathbf{z^{(1)}}-\mathbf{z^{(2)}}$. This makes $\mathbf{z^{(1)}}+\mathbf{z^{(2)}} = \|\mathbf{z}\|_1$. Then change variables $\mathbf{z}, \xi \to -\mathbf{z}, -\xi$ to get \eqref{bidual_Lag}. Since $\mathcal{L}^{**}=\mathcal{L}$ (\cref{assump:Loss_func}, \cite{Borwein:2000}), $\inf_{\lambda} L(\lambda, \mathbf{z},\xi) = -\mathcal{L}_y - \beta \|\mathbf{z}\|_1$ and negating its maximization gives \eqref{gen_lasso_sol}.

\iftoggle{long}{
This is equivalent to using one bidual variable $\mathbf{z} \in \mathbb{R}^N$, which can be split into a difference of nonnegative vectors $\mathbf{z^{(1)}},\mathbf{z^{(2)}}$: $\mathbf{z} = \mathbf{z^{(1)}}-\mathbf{z^{(2)}}$, with $||\mathbf{z}||_1 = \mathbf{z^{(1)}}+\mathbf{z^{(2)}}$. }
For $\mathbf{A}=\mathbf{A_+}$ we set $\mathbf{z}=\mathbf{z_+}$ and for $\mathbf{A}=\mathbf{A_-}$ we set $\mathbf{z}=\mathbf{z_-}$ to formulate the Lagrangian \eqref{bidual_Lag}.

\iftoggle{long}{Since $\mathcal{L}^*$ is convex and lower semicontinuous (\cref{assump:Loss_func}), $\mathcal{L}^{**}=\mathcal{L}$ \cite{Borwein:2000}. 
By Fenchel duality \cite{boyd:2004} and  $\mathcal{L}^{**}=\mathcal{L}$ (\cref{assump:Loss_func}, \cite{Borwein:2000}), the dual of \eqref{L=2_d=1_dual} is \eqref{gen_lasso_sol}.
}
\end{proof}

%%%

\iftoggle{long}{
\begin{remark}\label{rm:c_1=c_2=0}
	If $c_1 = c_2 = 0$, then the matrices $\mathbf{A_+}, \mathbf{A_-}$ reflect each other along the main diagonal:
By \cref{section:notation}, $x_i > x_j$ if $i < j$ so 
	\begin{equation}
		\begin{aligned}
  			{\mathbf{A_+}}_{i,j} & = \sigma(x_i - x_j) =
			\begin{cases}
				d_2   \mbox{ if } i \leq j  \\
				d_1 \mbox{ if } i > j
			\end{cases}, 
   \quad
			{\mathbf{A_-}}_{i,j} & = \sigma(x_j - x_i) = 
			\begin{cases}
				d_1 \mbox{ if } i < j \\
				d_2  \mbox{ if } i \geq j
			\end{cases}.
		\end{aligned}
	\end{equation}
\end{remark}
}
\begin{lemma}\label{lemma:sym_activation_simp}
	If $L=2,d=1$ and $\sigma$ is symmetric (\cref{app_section:act_func}) then the bidual in \cref{lemma:lasso_without_simp} is
	\begin{equation}\label{gen_lasso_sol_NxN}
		\begin{aligned}
			\min_{\mathbf{z} \in \mathbb{R}^N, \xi \in \mathbb{R}} & \mathcal{L}_{\mathbf{y}}( \mathbf{A_+ z} + \xi \mathbf{1} )+ \beta ||\mathbf{z}||_1, \quad 
			\text{ where }                                 \xi=0 \text{ if }  c_1=c_2=0.
		\end{aligned}
	\end{equation}
\end{lemma}

%normal sign would be symmetric and bounded

\begin{proof}
	Let $\mathbf{z}_+, \mathbf{z}_-$ be defined as in \cref{theo:1d_all}. Since $\sigma$ is symmetric, $\mathbf{A_+}=\mathbf{A_-}$. 
 \iftoggle{long}{ So since $z_+, z_-$ are unconstrained we may define one merged variable $z = z_+ + z_-$, and let $A=A_+$. }
 Apply a change of variable $\mathbf{z} = \mathbf{z_+} + \mathbf{z_-}$ in \eqref{gen_lasso_sol} so that $\mathbf{Az} = \mathbf{A_+z_+} + \mathbf{A_-z_-} = \mathbf{A}_+(\mathbf{z_+} + \mathbf{z_-})=\mathbf{A_+ z}$. 
\end{proof}

\begin{lemma}\label{lemma:sign_activation_simp}
	If $c_1=c_2=0 $ and $ d_1=-d_2 \neq 0$ (e.g. sign activation) the bidual in \cref{lemma:lasso_without_simp} is
 \iftoggle{long}{ problem \eqref{gen_lasso_sol} is equivalent to \eqref{gen_lasso_sol_NxN} but without a bias term $\xi$:}

	\begin{equation}\label{gen_lasso_sol_NxN_sign}
		\begin{aligned}
			\min_{\mathbf{z} \in \mathbb{R}^N, \xi \in \mathbb{R}} & \mathcal{L}_{\mathbf{y}}( \mathbf{A_+ z} )+ \beta ||\mathbf{z}||_1.
		\end{aligned}
	\end{equation}

\end{lemma}


%\proofsketch{
%The diagonal terms $(\mathbf{A_+})_{n,n}=(\mathbf{A_-})_{n,n} = \sigma(0)=d_2 \neq 0$ so $\mathbf{A_+} \neq - \mathbf{A_-}$. Nevertheless, in the dual in \cref{lemma:dual_finite}, the set of constraints $|\lambda^T \sigma(\mathbf{X}-x_n\mathbf{1})|\leq \beta, n \in [N]$ is the same as $|\lambda^T \sigma(x_n\mathbf{1}-\mathbf{X})|\leq \beta, n \in [N]$: the $n^{\text{th}}$ constraint in the former set of constraints is the same as the ${n-1}^{\text{th}}$ constraint in the latter set, and so are the first and last constraints in the former and latter sets, respectively. This collapses the constraint $|\lambda^T \mathbf{A}z| \leq \beta \mathbf{1}^T$ to $|\lambda^T \mathbf{A}_+ z| \leq \beta \mathbf{1}^T$.
%}

\begin{proof}
	%By \cref{rm:c_1=c_2=0}, 
 Let $d = d_1 = - d_2$. Let $g_+(n)=\left|\lambda^T \sigma(\mathbf{X}-x_n\mathbf{1}) \right|, g_-(n)=\left |\lambda^T \sigma(x_{n}\mathbf{1}-\mathbf{X}) \right|$.
 \iftoggle{long}{ for example $d_1 = -1, d_2=1$ in sign activation }
 By \cref{section:notation}, $i < j \implies x_i > x_j$, so for $n \in [N-1]$, the terms in the inequality constraints of \eqref{L=2_d=1_dual} are 
 \iftoggle{long}{
 $
			\left|\lambda^T \sigma(\mathbf{X}-x_n\mathbf{1}) \right|  =   \left |d_2 \sum_{i=1}^{n}  \lambda_i + d_1\sum_{i=n+1}^N  \lambda_i \right|$
	and
			$\left |\lambda^T \sigma(x_n\mathbf{1}-\mathbf{X}) \right|  = \left |d_1 \sum_{i=1}^{n-1}  \lambda_i + d_2 \sum_{i=n}^N  \lambda_i \right|$, for $n \in [N]$. 
   }
$
g_+(n)            =  |d| \left|- \sum_{i=1}^{n}  \lambda_i + \sum_{i=n+1}^N  \lambda_i \right| 
          %  =|d| \left| \sum_{i=1}^{n}  \lambda_i - \sum_{i=n+1}^N  \lambda_i \right|    
            =  g_-(n+1) 
$.
	And
 $ g_+(N)
        = |d| \left|\lambda^T \mathbf{1} \right|
		= g_-(1)
 $.
%$
%    \left |\lambda^T \sigma(x_{N}\mathbf{1}-\mathbf{X}) \right|
%        = |d| \left| \lambda^T \mathbf{1} \right|
%		= \left|\lambda^T \sigma(\mathbf{X}-x_1 \mathbf{1}) \right|  
%  $.
So 
 \iftoggle{long}{ if $c_1=c_2=0, d_1 = -d_2$ then }
the constraints $g_+(n) \leq \beta, n \in [N]$ are the same as
	$ g_-(n) \leq \beta, n \in [N]$. 
 \iftoggle{long}{ with $c_1=c_2=0$}
So \eqref{L=2_d=1_dual} reduces to

	\begin{equation}\label{L=2_d=1_dual_sign}
		\begin{aligned}
			\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda )                    \\
			\text{ s.t. }                   & |\lambda^T \sigma(X-x_n\mathbf{1})| \leq \beta, n \in [N],
			% & \lambda^T \mathbf{1} = 0 \quad \text{ if $c_1\neq0$ or $c_2\neq0$}
		\end{aligned}
	\end{equation}

	and taking the bidual as done in \cref{lemma:lasso_without_simp}
 \iftoggle{long}{ similarly as before for general $\sigma$ }
yields \eqref{gen_lasso_sol_NxN_sign}.
\end{proof}


==> unused/old_nn_architecture.tex <==
%old architectures. Changed to a nicer recursive definition
\section{Neural network architectures}
To simplify derivations, we write the $L$-layer standard, parallel and tree networks $f_L:\mathbb{R}^d \to \mathbb{R}$ all in the same form, defined recursively as
%
\begin{align} \label{eq:univ_NN}
	\nn{L}{\mathbf{x}}
	 & := \xi + \sum_{i=1}^{m_L} \sigma_{ \ssul{i}{L-1}} \left (  \sful{i}{L-1}\left(\mathbf{x}; \theta^{(L-1)} \right) \right) \boldsymbol{\alpha}_i,
\end{align}

where for $l \in [L]$, $ \sful{i}{l}$ depends on the output of the previous $(l-1)^{th}$ layer. 
\iftoggle{long}{, with $f^{(1,i)}$ depending on $x$.}
The next sections define $\sful{i}{l}$ for specific architectures.
The coefficients $\{\boldsymbol{\alpha}_i\}_{i=1}^K$ are the linear combination weights at the output layer, with $\boldsymbol{\alpha}_i \in \mathbb{R}^{m_{L-1}}$. 
%And $\xi \in \mathbb{R}$ as the final bias term outside of the network and. %For $l \in [L-1]$, $W^{(i,l)} \in \mathbb{R}^{(1+m_{l-1}) \times m_l}$ are the $l^{th}$ layer weights.
The parameter $\sigma_{\sul{i}{l}}=({\sigma_{\ssul{i}{l}}}_1 , \dots, {\sigma_{\ssul{i}{l}}}_{m_l})$ defines the activation function for the $m_l$ neurons at layer $l$ and subnetwork $i$, and is parametrized by $ \sul{i}{l}\in \mathbb{R}^{m_l}$. For neural networks that use the same activation for all neurons, such as leaky ReLU, ReLU, and absolute value, we drop the subscript on $\sigma$ and denote all the activations as simply $\sigma(x)$.
%
We next consider specific cases of $\sful{i}{l}$, as well as final and initial layer sizes.
%

\iftoggle{long}{
\subsection{standard neural network}
%
We define a standard $L$-layer neural network $f_L = {f_L}_{\textrm{std}}$ by \eqref{eq:univ_NN} with the following parameters:
%
\begin{equation}
	\begin{aligned}
		m_0       & := d.                                                                                                                \\
		m_L       & :=1.                                                                                                                 \\
		\mathbf{W^{(l)}}   & \in \mathbb{R}^{(1+m_{l-1}) \times m_l} \mbox{ are weights of layer } l.                                             \\
		\mathbf{x^{(0)}}   & :=[\mathbf{x},1] \in \mathbb{R}^{1 \times (d+1)}.                                                                             \\
		\mathbf{x^{(l)}}   & := \left[ \sigma_{s^{(l)}} \left( \mathbf{x^{(l-1)} W^{(l)}} \right) , \mathbf{1} \right] \in \mathbb{R}^{1\times (1+m_{l})}. \\
		\sful{1}{l}\left(\mathbf{x};\theta^{(l)}\right) & := \mathbf{x^{(l-1)}W^{(l)}} \in \mathbb{R}^{m_l}.                                                                            \\
		\boldsymbol{\alpha}    & \in \mathbb{R}^{m_{L-1}}.
	\end{aligned}
\end{equation}
In other words, a standard $L$-layer neural network is ${f_L}_{\textrm{std}}:\mathbb{R}^d \to \mathbb{R}$,
\begin{equation}  \label{eq:std_NN}
	\begin{aligned}
	 \nn{L,\textrm{std}}{\mathbf{x}} & := \xi + \sigma_{s^{(L-1)}} \left ( \mathbf{x^{(L-2)} W^{(L-1)}} \right) \alpha.
		% &= \xi + \sum_{i=1}^{m_{L-1}} \sigma_{s^{(L-1,i)}} \left ( x^{(L-2)} W^{(L-1)}_i \right) \alpha_i,
	\end{aligned}
\end{equation}

The external bias $\xi$, layer weights $\mathbf{W^{(l)}}$ (and any amplitude parameters $s^{(l)}$ if the activation function uses them) are the trainable parameters: $\theta = \{\xi, \mathbf{W^{(l)}}, s^{(l)}: l \in [L-1] \}$.
%\begin{remark}
%    For the standard neural network, $m_0 = d, m_L=1$. 
%\end{remark}
Note we can also write the standard network \eqref{eq:std_NN} as

\begin{equation}  \label{eq:std_NN_alt}
	\begin{aligned}
		{f_L}_{\textrm{std}}(\mathbf{x};\theta)
		 & = \xi + \sum_{i=1}^{m_{L-1}} \sigma_{s^{(L-1,i)}} \left (\mathbf{ x^{(L-2)} W^{(L-1)}}_i \right) \alpha_i,
	\end{aligned}
\end{equation}

where for layer $l \in [L]$, $\mathbf{W^{(l-1)}}_i \in \mathbb{R}^{m_l}$ is the $i^{\textrm{th}}$ column of the layer weight matrix $\mathbf{W^{(l-1)}} \in \mathbb{R}^{(1+m_{l-2}) \times m_{l-1}}$, corresponding to the $i^{\textrm{th}}$ neuron of layer $l-1$.

\subsection{Parallel neural network}\label{app_sec:parallel_nn_def}

Now consider a parallel neural network architecture which consists of $m_L$ standard neural subnetworks in parallel. For $l \in [L-1], i \in [m_l]$ let $\mathbf{W^{(l,i)}} \in \mathbb{R}^{(1+m_{l-1}) \times m_l}$ be the $l^{\textrm{th}}$ layer weights of the $i^{\textrm{th}}$ subnetwork including bias terms. We define a parallel $L$-layer neural network $f_L = {f_L}_{\textrm{par}}$ by  \cref{eq:univ_NN} where,
%
\begin{equation}\label{par_def}
	\begin{aligned}
		m_0            & := d.                                                                                                                      \\
		m_{L-1}        & := 1.                                                                                                                      \\
		\mathbf{\sxul{i}{l} }     & := \left[ \sigma_{ \sul{i}{l}} \left(\mathbf{\sxul{i}{l-1} \Wul{i}{l} } \right) , \mathbf{1} \right] \in \mathbb{R}^{1\times (1+m_{l})}, \\
		 \sxul{i}{0}   & :=(\mathbf{x},1) \in \mathbb{R}^{1 \times (d+1)},                                                                          \\
		\sful{i}{l}(\mathbf{x}; \theta^{(l)})      & := 
 \sxul{i}{l-1} \Wul{i}{l} \in \mathbb{R}^{m_l},                                                                               \\
		\alpha_i       & \in \mathbb{R}, \mbox{ for }  l  \in [L-1],  i \in [m_l].                  
	\end{aligned}
\end{equation}


%
Note that the $i^{\textrm{th}}$ neuron of the final layer evaluated on all the samples outputs a vector $ \Xul{i}{L-2} \Wul{i}{L-1} \in \mathbb{R}^N$.
In other words, we define a parallel neural network architecture with $L$ total layers ($L-1$ hidden layers) as $f_L:\mathbb{R}^d \to \mathbb{R}$,
\begin{align} \label{eq:generic_NN}
	{f_L}_{\textrm{par}}(\mathbf{x}; \theta) := \xi + \sum_{i=1}^{m_L} \sigma_{s^{(L-1,i)}} \left (  \Xul{i}{L-2} \Wul{i}{L-1}  \right) \alpha_i.
\end{align}



The bias $\xi$, layer weights $\Wul{i}{l}$ and any amplitude parameters $\sul{i}{l}$, if they are used by the activation function, are the trainable parameters: $\params = \{ \Wul{i}{l}, \sul{i}{l}, \xi: l \in [L-1], i \in [m_l] \}$.
For $l \in [L-2]$, the layer sizes $m_l$ are the same for the standard and parallel neural networks. The layer size $m_{L-1}$ in the standard neural network is the same as the layer size $m_L$ in the parallel neural network. The vice versa also holds (they are both 1). Therefore the vector $\boldsymbol{\alpha}$ containing the final output layer coefficients is $\boldsymbol{\alpha} \in \mathbb{R}^{m_{L-1}}$ for the standard network which is the same size as  $\boldsymbol{\alpha} \in \mathbb{R}^{m_{L}}$ for the parallel network.


\begin{remark}


	The $d$-dimension, $L$-layer parallel neural network for a sign-determined activation is written out as:

	\begin{equation}\label{parLlayernn_signdet}
		\begin{aligned}
			f_L(\mathbf{x};\theta) & = \sum_{i=1}^{m_L} \sigma_{\sul{i}{L-1} } \left ( \sxul{i}{L-2}\Wul{i}{L-1} \right) \alpha_i                                                                                                                                                                           \\
			       & = \sum_{i=1}^{m_L} \sigma_{\sul{i}{L-1} } \left( \cdots \left( \left[ \sigma_{ \sul{i}{2}}\left(\left[\sigma_{ \sul{i}{1}}\left( [\mathbf{x}, \mathbf{1}]  \Wul{i}{l} \right), \mathbf{1} \right] \right) \Wul{i}{2}, \mathbf{1} \right) \right ] \cdots \Wul{i}{L-1} \right) \alpha_i, \\
			       & \text{where for } i \in [m_L], l \in [L-1],  \sul{i}{l} \in \mathbb{R}^{m_l}, \sxul{i}{l} = \left[ \sigma_{\sul{i}{l}}\left( \sxul{i}{l-1} \Wul{i}{l}\right) , \mathbf{1} \right] \in \mathbb{R}^{1\times (1+m_{l})},                                                     \\
			       & \sxul{i}{0} =(\mathbf{x},\mathbf{1}) \in \mathbb{R}^{d\times 2};  
			        \text{ and for } l \in [L-1],  \Wul{i}{l} \in \mathbb{R}^{1+m_{l-1}\times m_l},  \boldsymbol{\alpha} \in \mathbb{R}^{m_L}.                                                                                                                                                            \\
		\end{aligned}
	\end{equation}

\iftoggle{long}{ 

 If the weight matrices and amplitude parameters are the same across units within each layer, then the parallel neural net becomes equivalent to a standard neural net.
If for each layer $l \in [L-1]$ before the final layer, all parallel units $i,j \in [m_L]$ have the same weight matrices and amplitude parameters, $\Wul{i}{l}= \Wul{j}{l}=:\mathbf{W^{(l)}}, \sul{i}{l}= \sul{j}{l}=:\mathbf{s^{(l)}}$ and we let $\mathbf{W^{(L-1)}}:=\left[\Wul{1}{L-1},\cdots, \Wul{m_L}{L-1}\right] \in \mathbb{R}^{1+m_{L-2}, m_{L-1}}$ then the layer outputs also satisfy $ \sxul{i}{l}= \sxul{j}{l}=: \mathbf{x^{(l)}}$, so if $\boldsymbol{\alpha}$ is divided my $m_L$ then the parallel neural network reduces to a non-parallel version $f_L(x)=m_L \sigma_{\mathbf{s^{(L-1)}}}(\mathbf{x^{(L-2)}})\mathbf{W^{(L-1)}}$. } 

A standard neural network is a parallel neural network with just one parallel unit, or whose weight matrices and amplitudes are the same over parallel units.
On the other hand, a parallel neural network can be transformed to a standard non-parallel neural network by aggregating parallel weight matrices into a block diagonal matrix for each layer (\cref{section:par2std}).

\end{remark}




\subsection{Tree neural network}\label{app_subsection:tree_nn_def}


For clarity, here we denote the parameter set $\theta^{(L)}$ of the neural network explicitly. The tree neural network has a recursive tree structure. Each node $i$ in layer $l$ is the root of another tree subnet with $l$ layers, and the set $\theta^{(l,i)}$ collects all parameters in this subnet. The set $\theta^{(l)}$ collects all parameters from the subnets of layer $l$. 
%
%
Denote  the  $i^{\textrm{th}}$ element of the vector $\mathbf{w^{(l)}}$ by $\mathbf{w^{(l)}}_i$. Denote $\thetaul{i}{l}, \ssul{i}{l}$ to indicate an $i^{\textrm{th}}$ independent copy of $\theta^{(l)}$ and $s^{(l)}$, respectively.
%
The $L$-layer tree network $f_L= {f_L}_{\textrm{tree}}(\mathbf{x};\theta)=: f^{(L)}(\mathbf{x}, \theta^{(L)})$ has the following parameters in \eqref{eq:univ_NN}:

\begin{equation}\label{def:tree_networks}
	\begin{aligned}
		m_1               & := d.                                                                                                            \\
		\mathbf{w^{(l)}}           & \in \mathbb{R}^{m_l+1}, l \in [L].                                                                               \\
		\ssul{i}{l}        & \in \mathbb{R}, l \in [L], i \in [m_l].                                                                          \\
		\theta^{(1)}          & := \{\mathbf{w^{(1)}} \}.                                                                                                 \\
		f^{(1)}(\mathbf{x};\theta^{(1)})
		                  & := [\mathbf{x}, 1] \mathbf{w^{(1)}} \in \mathbb{R}.                                                                  \\
		\theta^{(l)}          & := \bigcup_{i=1}^{m_{l-1}} \theta^{(l-1,i)}  \bigcup_{i=1}^{m_l} \{\ssul{i}{l-1}\} \bigcup \{ \mathbf{w^{(l)}} \}.          \\
		f^{(l)}(\mathbf{x}; \theta^{(l)}) & :=  \mathbf{w^{(l)}}_{m_l + 1}+ \sum_{i=1}^{m_{l}} \sigma_{\ssul{i}{l-1}}\left(f^{(l-1)}\left(\mathbf{x}; \thetaul{i}{l-1}\right)\right)\mathbf{w^{(l)}}_i \in \mathbb{R}, \mbox{ for } l \in [L]-\{1\}.                                                                                                 \\
	%	f^{(L-1)}(\mathbf{x}, \theta^{(L-1,i)})       & := f^{(L-1), \Theta^{(L-1,i)}} \in \mathbb{R}.                                                                   \\
		\boldsymbol{\alpha  }          & := \mathbf{w^{(L)}}_{1:m_L} \in \mathbb{R}^{m_L}.                                                                         \\
		\xi               & := \mathbf{w^{(L)}}_{m_L+1} \in \mathbb{R}.
	\end{aligned}
\end{equation}

The layer weights $\sWul{i}{l} $ and any amplitude parameters $\ssul{i}{l}$ (if the activation function uses them) of every level of every sub-tree network and the bias $\xi$ are the trainable parameters.
%Note $m_1 \in \mathbf{N}, w^{(L)}_{1:m_L} \in \mathbb{R}^{m_L}, w^{(L)}_{m_L+1} \in \mathbb{R} $  as defined in the tree network \eqref{def:tree_networks} plays the role of $m_0, \alpha, \xi$ in the parallel network \eqref{eq:generic_NN}, respectively. %Unlike the parallel network \eqref{eq:generic_NN}, the tree network \eqref{def:tree_networks} does not constrain $m_{L-1}$ to be $1$.
For example, the tree network evaluated on data matrix $\mathbf{X} \in \mathbb{R}^{N \times d}$ gives the tree subnetworks,

\begin{equation}\label{ex:tree_nn}
	\begin{aligned}
		% \Theta_1 &= \{W^{(1)} \in \mathbb{R}^{d }\} \\
		%f^{(1), \Theta^1} &= %\sum_{i=1}^d X_{1:N,i} W^{(1)}_i \\
		% &= X W^{(1)} \in \mathbb{R}^{N }\\
		\theta^{(2)}          & = \bigcup_{i=1}^{m_1} \thetaul{i}{1} \bigcup_{i=1}^{m_2} \{  \ssul{i}{1}\} \bigcup \{ \mathbf{w^{(2)}} \} .                                                     \\
		f^{(2)}(\mathbf{X};\theta^{(2)}) & = \mathbf{1}w^{(2)}_{m_2 + 1} + \sum_{i=1}^{m_2} \sigma_{ \ssul{i}{1}} \left (f^{(1)}\left(\mathbf{X}; \thetaul{i}{1}\right) w^{(2)}_i \right)                                                 \\
		& =
		\left[\cdots \sigma_{ \ssul{i}{1}}\left(f^{(1)}\left(\mathbf{X}, \thetaul{i}{1}\right)\right) \cdots \mathbf{1}\right] \mathbf{w^{(2)}}                        \\
	   & = \left[\cdots \sigma_{\ssul{i}{l}}\left([\mathbf{X}, \mathbf{1}]\sWul{i}{1}\right)\cdots \mathbf{1} \right] \mathbf{w^{(2)}}                                                                    \\
		& = [\sigma_{\Tilde{s}^{1}}([\mathbf{X},\mathbf{1}]\mathbf{\tilde{W}^{(1)}}),\mathbf{1}] \mathbf{w^{(2)}} ={f_2}_{\textrm{par}}(\mathbf{X};\theta^{(2)}) \in \mathbb{R}^{N},                          \\
		& \text{ where } \mathbf{\tilde{W}^{(1)}}=[ \sWul{1}{1}\cdots \sWul{m_1}{1} ] \in \mathbb{R}^{(1+d) \times m_1},                                                   
		\Tilde{s}^{1}      = [\ssul{1}{1},\cdots, \ssul{m_2}{1}]^T.                                                                                                                   \\
		\theta^{(3)}          & = \bigcup_{i =1}^{m_2}  \thetaul{i}{2}\bigcup_{i=1}^{m_3} \{ s^{(2,i)}\}  \bigcup \{ \mathbf{w^{(3)}} \} .                                                    \\
		f^{(3)}(\mathbf{X}; \theta^{(3)}) & = \mathbf{1}w^{(3)}_{m_3 + 1} 
 + \sum_{i=1}^{m_3} \sigma_{ \ssul{i}{2}}\left(f^{(2)}\left( \mathbf{X};\theta^{(2,i)}\right) \right) w^{(3)}_i                                                   \\
		%&= [\cdots \sigma(f^{(2,\Theta^{2,i})})\cdots] W^{(3)}\\
		%&= [\cdots \sigma(\sigma(X\tilde{W}^{(1,i)})W^{(2,i)})\cdots] W^{(3)}\\
		& = \mathbf{1}w^{(3)}_{m_3 + 1} + \sum_{i=1}^{m_3} \sigma_{\ssul{i}{2}} \left (\left [ \sigma_{ \ssul{i}{1}}([X,\mathbf{1}] \tWul{i}{l} ,\mathbf{1} \right] \sWul{i}{2}  \right) w^{(3)}_i \\
		                  & = {f_3}_{\textrm{par}}(\mathbf{X}; \params^{(3)}).                                                                                                                         \\
		\theta^{(4)}          & = \bigcup_{i=1}^{m_3} \thetaul{i}{3} \bigcup_{i=1}^{m_4} \{ \ssul{i}{3}\} \bigcup \{ \mathbf{w^{(4)}} \}.                                                     \\
		f^{(4)}(\mathbf{X}; \theta^{(4)}) & = \mathbf{1}w^{(4)}_{m_4 + 1}+ \sum_{i=1}^{m_4} \sigma_{ \ssul{i}{3}}\left(f^{(3)}\left(\mathbf{X}; \thetaul{i}{3}  \right)\right)w^{(4)}_i .                                                 \\
		                  & \vdots                                                                                                                                             \\
		\theta^{(L)}          & = \bigcup_{i=1}^{m_{L-1}} \thetaul{i}{L-1}\bigcup_{i=1}^{m_l} \{\ssul{i}{L-1} \} \bigcup \{\mathbf{ w^{(L)}} \} .                                                     \\
		f^{(L)}(\mathbf{X}; \theta^{(L)}) & =   \mathbf{1}w^{(L)}_{m_L + 1} + \sum_{i=1}^{m_{L}} \sigma_{\ssul{i}{L-1} }\left(f^{(L-1)}\left( \mathbf{X}; \thetaul{i}{L-1} \right)\right)w^{(L)}_i,                       
	\end{aligned}
\end{equation}

where $\tWul{i}{l}$ indicates an $i^{\textrm{th}}$ independent copy of $\mathbf{\tilde{W}^{(1)}}$.

%W's are defined ++ here. maybe better to change notation so that alphas are turned into W's to be consistent throughout, and just label alpha = W_L.also here they are vec, unless tilde for matrix

\subsection{Remarks}
	For the tree neural network, $m_l$ is defined for $l \in [L]$, and $m_1=d$. In contrast, the standard and parallel networks defined $m_l$ for $l \in \{0,\cdots,L\}$ and set $m_0=d$.
	For $l \in \{0, \cdots, L-2\}$, $m_l$ in the parallel neural network is the same as $m_{l+1}$ in the tree neural network. $m_L$ is the same in the parallel and tree networks. So $\boldsymbol{\alpha} \in \mathbb{R}^{m_L}$ in the parallel network is the same size as $ \boldsymbol{\alpha} = \mathbf{w^{(L)}_{1:m_L}} \in \mathbb{R}^{m_L}$ in the tree network.
	In the tree network \eqref{def:tree_networks}, $\ssul{i}{l}\in \mathbb{R}$ is a scalar and   $ \sWul{i}{l} \in \mathbb{R}^{l}$ are vectors, while in the parallel networks \eqref{eq:generic_NN}, $ \sul{i}{l}$  is a vector and $ \Wul{i}{l}$ is a matrix.
As shown in \cref{ex:tree_nn}, the $2$-layer neural network is equivalent for the standard, parallel 
\iftoggle{long}{${f_2}_{\textrm{par}}(X)$} 
and tree 
\iftoggle{long}{$f^{(2),\theta^2}$ } 
networks. The $3$-layer neural network is equivalent for the parallel 
\iftoggle{long}{${f_3}_{\textrm{par}}(X)$,}
 and tree 
 \iftoggle{long}{ $f^{(3),\theta^3}$ }
networks. However unlike the $2$-layer network $\nn{2,\textrm{tree}}{\mathbf{x}} =\nn{2,\textrm{par}}{\mathbf{x}}= \sigma(\mathbf{x {W}^{(1)}})\mathbf{W^{(2)}}$, the $3$-layer tree network 
\iftoggle{long}{$f^{(3),\theta^3}=f_3(X)$ }
${f_3}_{tree}$
is no longer in the same matrix-vector product form,
\iftoggle{long}{form of a product of a 
vector $\mathbf{w^{(3)}} \in \mathbb{R}^{3}$ with a $N \times {m_3}$ matrix, }
and so a $L\geq 4$-layer tree network $f^{(L)}(\mathbf{x}; \theta^{(L)})$ is no longer equivalent to the parallel network ${f_L}_{\textrm{par}}(\mathbf{x}; \theta^{(L)})$.


==> unused/oldsign_par_tree.tex <==
%replaced after changing to nicer recursive architecture def

\section{$L \geq 2$ parallel layer neural net with sign activation }\label{app_section:3lyr_sign}

In this section, 
%(\cref{app_section:3lyr_sign}), 
we assume the neural net has a parallel architecture, with $L \geq 2$ layers.
%
\iftoggle{long}{\textbf{Problem formulation}}
%
%put formulation since main paper was just about 3 layers
The \nc{} regularized training problem for a $L$-layer parallel neural net is
\begin{align} \label{eq:nonconvex_generic_lossL_Lyr}
	%   % \min_{\Theta} \frac{1}{2}\| f_L(X)-y\|_2^2 + \frac{\beta}{2} \|\Theta\|_2^2,
	\min_{\params \in \Theta} \mathcal{L}_{\mathbf{y}}( f_L(\mathbf{X};\theta)) + \frac{\beta}{2} \|\regparams\|_2^2,
\end{align} %put in appendix not main paper because we don't talk about bigger than L, becomes unnecessary since for sign deeper nets dont help. but need to talk about more layers in the proof to get to that point
where $\theta=\{\boldsymbol{\alpha}, \mathbf{W^{(i,l)}}, s^{(i,l)}: i \in [m_L], l \in [L]\}$ and $\sigma(x)=s^{(i,l)} \mathrm{sign}(x)$ is the activation of the neurons in the $i^{\mathrm{th}}$ parallel unit of the $l^{\mathrm{th}}$ layer.









\begin{proof}[\textbf{Proof of \cref{thm:deeper_sign_par}}] 
Apply \cref{prop:lasso_equiv_primal} and  \cref{prop:m_1_more_layers_same_size}. 
%
	\iftoggle{todos}{\textcolor{red}{todo: fix last prop so that last layer can be $m_2 \neq m_1$}}
%
\end{proof}

\begin{proof}[\textbf{Proof of  \cref{thm:3lyr_sign_tree}}]
	\cref{lemma:lasso_sign_L} analogously holds for the tree neural net. And \cref{prop:lasso_equiv_primal} also holds similarly for the tree neural net, as a map from the \lasso{} solution to the neural net satisfying $f_L(\mathbf{X};\theta)=\mathbf{Az}$ exists by construction of the dictionary set ${A_{L}}_{tree}$. So the \lasso{} problem is equivalent to the training problem  \eqref{eq:nonconvex_generic_loss_gen_L_intro} for a tree network.
	The dictionary is given by \cref{prop:prod_m_tree}.
\end{proof}



\subsection{Hyperplane arrangement set definitions and notation for sign activation, $L$ parallel layers}\label{def:H(Z)}

Define the hyperplane arrangement set for a matrix $\mathbf{Z} \in \mathbb{R}^{N\times m }$ as
%
%\begin{align*}
%\mathcal{H} := \bigcup \big \{ \%{\mathrm{sign}(X w)\} \,:\, w \in \mathbb{R}^d %\big \},
%\end{align*}
\begin{align}\label{eq:Hdef}
	%\mathcal{H}(\mathbf{\mathbf{Z}}) :=  \big \{ \mathrm{sign}([\mathbf{Z}, \mathbf{1}] \mathbf{w}) \in \mathbb{R}^{N}\,:\, \mathbf{w} \in \mathbb{R}^{m+1} \big \},
 \mathcal{H}(\mathbf{\mathbf{Z}}) :=  \big \{ \mathrm{sign}(\mathbf{Z} \mathbf{w}) \in \mathbb{R}^{N}\,:\, \mathbf{w} \in \mathbb{R}^{m} \big \} \subset \{-1,1\}^N,
\end{align} %making bias explicit


where the sign function is defined in \cref{section:notation}.
The set $\mathcal{H}(\mathbf{Z})$ denotes all possible $\{+1,-1\}$ labelings of the samples $\{\mathbf{z}_i\}_{i=1}^N$ by a linear classifier $\mathbf{w} \in \mathbb{R}^{m}$. Its size is upper bounded by
$
	|\mathcal{H}(\mathbf{Z})| \le 2 \sum_{k=0}^{r-1} {N-1 \choose k}\le 2r\left(\frac{e(n-1)}{r}\right)^r \leq 2^N,
$
where $r:=\mbox{rank}(\mathbf{Z})\leq \min(N,m)$ \cite{cover1965geometrical, stanley2004introduction}. %Tolga

For a set of vectors $H$, denote $[H]$ to be a matrix whose columns are elements of $H$. Consider sequences $\{S_l\}_{l=0}^{L-2}$ of sets $S_l$ of size $|S_l| \leq m_l$ satisfying $S_{l} \subset  \mathcal{H}(\left[[S_{l-1}],\mathbf{1}\right])$, with $S_0$ being the set of columns of $[\mathbf{X}, \mathbf{1}]$. Let ${A_L}_{par}(\mathbf{X})$ be the union of all possible $\mathcal{H}(S_{L-2})$ formed this way. 
%For a parallel network, since $m_{L-1}=1$, $S_{L-1}$ will be a singleton set.

\begin{remark}
    For notational convenience, we drop the parallel unit superscript $i=1$ on the weight matrices when discussing ${A_L}_{par}$, e.g. in the proofs of \cref{lemma:sign_rewritedual}, \cref{prop:m_1_more_layers}, and \cref{prop:m_1_more_layers_same_size}. 
\end{remark}

\iftoggle{long}{

Next, we define the $L$-layer hyperplane arrangement matrix recursively. Let $\mathcal{H}^{(0)}_{S_0}(\mathbf{X}) = \mathbf{X}$.
For $l \in [L]$, given a matrix $\mathcal{H}^{(l)}_{\{S_j\}_{j=1}^{l}}(\mathbf{X)} \in \mathbb{R}^{N \times |S_l|}$ and a subset of its hyperplane arrangements $S_{l+1} \subset \mathcal{H}\left(  \mathcal{H}^{(l)}_{\{S_j\}_{j=1}^{l}}\left(\mathbf{X}\right) \right)$, let  $\mathcal{H}^{(l+1)}_{\{S_j\}_{j=1}^{l+1}}(\mathbf{X)} = [S_{l+1}] \in \mathbb{R}^{N \times |S_{l+1}|}$ be the concatenation of those arrangements.  
Taking all possible such sequences of sets $\{S_j\}_{j=1}^L$, 
define the $L$-layer dictionary as 

	\begin{equation}\label{def:A_L(X)}
		A_L(X) := \bigcup_{\{S_j:j\in[L-3],|S_j|\leq m_j \}} S_L.
	\end{equation}


the concatenation of their corresponding $L$-layer hyperplane arrangement matrices. \\


Alternatively:


For a vector set $H=\{h_1, \dots, h_{|H|} \} \subset \mathbb{R}^d $ and an ordered subset $S \subset H$, let $[H]_S \in \mathbb{R}^{d \times |S|}$ be the horizontal concatenation of the vectors in $S$ in order. 
For a matrix $\mathbf{Z}$, let $\tilde{H}_S(\mathbf{Z}) =[[\mathcal{H}(\mathbf{Z})]_{S},  \mathbf{1}] $ 
\iftoggle{long}{denote the matrix formed by concatenating $[\mathcal{H}(\mathbf{Z})]_{S}$ with a column of ones}.



Now, denote $\tilde{H}^{(L-1)}_{S_j:j\in[L-1]}(\mathbf{X}) = \tilde{H}^{(L-1)}_{S_{L-1}} \circ \tilde{H}^{(L-1)}_{S_{l-2}} \circ \cdots \circ \tilde{H}^{(1)}_{S_1}(\mathbf{X})$ as the composition of $\tilde{H}_S$ with itself $L-1$ times, where the $j^{\text{th}}$ time uses a subset $S_{j-1} \subset \mathcal{H}\left([(\tilde{H}^{(j-1)}_{S_j} \circ \cdots \circ \tilde{H}^{(1)}_{S_1})(\mathbf{X}),\mathbf{1}]\right)$.


	We define the $L$-layer dictionary set,

	\begin{equation}\label{def:A_L(X)}
		A_L(X) := \bigcup_{\{S_j:j\in[L-3],|S_j|\leq m_j \}} \mathcal{H}(\tilde{H}^{(l)}_{S_j:j\in[l]}(X)).
	\end{equation}



%, where $\bigsqcup$ denotes taking a union . 
\begin{remark}
	The union in equation \ref{def:A_L(X)} is taken over all possible sequences of $S_1, \dots, S_{L-3}$, where $S_j$ is constrained by the previous $S_i$ for $i < j$, which in turn depends on $X$.
	Propositions \ref{prop:m_1_more_layers_same_size}, \ref{prop:m_1_more_layers} will show that for a fixed number of training samples $N$, regardless of their actual values $x_1,\dots,x_N$, $A_L(X)$ is the same set and with easily enumerable elements.
	%each s_j is constrained by previous s_j-1.
\end{remark}
}

\begin{lemma}\label{lemma:sign_rewritedual}
	The parallel net dual \eqref{gen_dual} in \cref{lemma:dual_of_rescaled} can be written as

	\begin{equation}\label{dsignpar_gen}
		\begin{aligned}
			\max_{\lambda} & -  \mathcal{L}( \lambda )                                   \\
			               & \text{ s.t. } \max_{\mathbf{h} \in {A_L}_{par}(\mathbf{X})} |\lambda^T \mathbf{h} | \leq \beta
		\end{aligned}
	\end{equation}

\end{lemma}

\iftoggle{long}{
\proofsketch{
Consider the maximization constraint of the dual problem \eqref{gen_dual}. We replace the layer weight variables $W^{(i,l)}$ by all vectors that $\sigma(x^{(L-2)}W^{(L-1)})$ can possibly be over all feasible $W^{(i,l)}$, and collect them into the set $A_L(X)$ as their feasible set.
}
}

\begin{proof}
Consider the maximization constraint of the dual problem \eqref{gen_dual}.  %For notational convenience, we drop the parallel unit superscript $i=1$ on the weight matrices. %For $j \in [m_{l}]$, denote the $j^{\textrm{th}}$ column of a matrix by subscript $J$. 
For $l \in [L-2]$, $\mathbf{X^{(l)}} = \left[ \sigma \left(\mathbf{ X^{(l-1)} W^{(l)}} \right) , \mathbf{1} \right] = [[S_l], \mathbf{1}]$ where $S_l \subset \mathcal{H}(\mathbf{X^{(l-1)}}) = \mathcal{H}([[S_{l-1}],\mathbf{1}])$. And so $\sigma\left(\mathbf{X^{(L-2)} W^{(L-1)}}\right) \in \mathcal{H}\left(\mathbf{X^{(L-2)}}\right) = \mathcal{H}([[S_{L-2}],\mathbf{1}])$. Therefore $\{ \sigma\left(\mathbf{X^{(L-2)} W^{(L-1)}}\right) : \theta \in \Theta_s\} = {A_L}_{par}(\mathbf{X})$.
%
%
\iftoggle{long}{
$\{\sigma\left(\mathbf{X^{(L-2)} W^{(1,L-1)}}\right): \theta \in \Theta_s\} = \bigcup_{\theta \in \Theta_s} \mathcal{H}(\mathbf{X}^{(L-2)}) = \bigcup S_{L-1} $ and $\mathbf{X}^{(L-2)} = [\sigma(\mathbf{{X}^{(L-3)}W^{(L-2)}}),\mathbf{1}]$

	%If $l \in [L-1]$ and the amplitude parameters of the activation functions are all one, then for some collection of subsets $S_j: j \in [l]$ corresponding to the weights in each $j^{\text{th}}$ layer, the output of the ${}^{\text{th}}$ hidden layer 
	For $i \in [m_{L-2}]$, denote $W^{(L-2)}_{i}$ as the $i^{\textrm{th}}$ column of  $W^{(L-2)}$, corresponding to the weights of the $i^{\textrm{th}}$ neuron in layer $L-2$. If the amplitude parameters of the activation functions are all one, then for some sets $S_1, \dots, S_{[L-3]}$, the input to the second to last layer is $X^{(L-2)} = [\sigma_{s=1}(X^{(L-3)}W^{(L-2)}), \mathbf{1}] = [ \sigma_{s=1}(X^{(L-3)}W^{(L-2)}_1), \dots,  \sigma_{s=1}(X^{(L-3)}W^{(L-2)}_{m_{L-2}}), \mathbf{1}] = [[\mathcal{H}(X^{(L-3)})]_{S_{L-3}},  \mathbf{1}] = \tilde{H}_{S_{L-3}}(X^{(L-3)})=\tilde{H}_{S_{L-3}}(\tilde{H}_{S_{L-4}}(X^{(L-4)}))=\cdots = \tilde{H}^{(L-3)}_{S_j:j\in[L-3]}(X^{(0)})=\tilde{H}^{(L-3)}_{S_j:j\in[L-3]}(X)$ can be written in terms of $L-3$ function compositions on the input matrix $X$. Given a fixed feasible $X^{(L-2)}$ and its corresponding sets $S_j:j \in [L-3]$, the set of all possible vectors $\sigma(X^{(L-2)}w)$ generated over all possible vectors $w \in \mathbb{R}^{1+m_{L-2}}$ is, by definition of $\mathcal{H}$, equal to $\mathcal{H}(\tilde{H}^{(l)}_{S_j:j\in[l]}(X))$. So the set of all possible $\sigma(X^{(L-2)}w)$ vectors over all vectors $w$ and all possible, feasible $X^{(L-2)}$ (generated by all possible  $W^{(i,l)}$) is their union $A_L(X)$, as defined in equation \ref{def:A_L(X)}. Therefore we can replace $\sigma(X^{(L-2)W^{(L-1)}})$ in the maximization constraint of the dual problem \eqref{gen_dual} by vectors $h \in A_L(X)$ to get the equivalent problem \ref{dsignpar_gen}.
}
\end{proof}

\begin{assumption}\label{Hstartswith1}
    Without loss of generality by multiplying vectors by $-1$, we will assume that the vectors in $\mathcal{H}(\mathbf{Z})$ start with first element being nonnegative. Then \cref{lemma:sign_rewritedual} still holds due to $\lambda^T \mathbf{h}$ being enclosed in absolute value.
\end{assumption}


\begin{lemma}\label{lemma:lasso_sign_L}
	Let $\mathbf{A}=[{A_L}_{par}(\mathbf{X})]$. The dual  \eqref{dsignpar_gen} is equivalent to the \lasso{} problem
	\begin{equation}\label{signLLasso_gen}
		\begin{aligned}
			\min_\mathbf{z} & \quad \mathcal{L}_{\mathbf{y}}( \mathbf{Az}) + \beta||\mathbf{z}||_1.
		\end{aligned}
	\end{equation}
\end{lemma}

\begin{proof}
	Problem \eqref{dsignpar_gen} is the dual of \eqref{signLLasso_gen}, and since the problems are convex with feasible regions that have nonempty interior, by Slater's condition, strong duality holds \cite{boyd:2004}. %or just take dual. clarify dual and bidual are convex, primal is not. so strong duality need to show directly
\end{proof}


\begin{remark}
	As can be seen by \cref{lemma:lasso_sign_L}, the set $A_{L,par} $ consists of all possible sign patterns at the final layer, up to multiplying by $-1$, in a parallel network.
\end{remark}



\begin{proposition}\label{prop:reconstruct_primal_L}
	Consider $\mathbf{A}$ as defined in \cref{lemma:lasso_sign_L}. Suppose $m_L \geq \| \mathbf{z} \|_0$. We can construct a parallel neural network $f$ %as defined in %\eqref{parLlayernn_cpt} 
	with $\sigma(z)=\textrm{sign}(z)$ such that $f_L(\mathbf{X};\theta)=\mathbf{Az}$ which achieves the same objective in the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} as the \lasso{} problem \eqref{signLLasso_gen}.
\end{proposition}

\begin{proof}
Let $I$ be the set of indices where $\mathbf{z}$ is nonzero. Let $\mathbf{z}'=\mathbf{z}_I, \mathbf{A}' = \mathbf{A}_I$. Let $\mathbf{a}'_i$ be the $i^{th}$ column of $\mathbf{A}'$. Since $\mathbf{a}'_l \in A_L(\mathbf{X})$, there is a sequence of sets $\{S^{(i)}_l\}_{l=1}^{L-2}$ that correspond to a sequence of matrices ${\mathbf{W}'}^{(i,l)}$ such that
\[
		f(\mathbf{X}) =  %\sigma(X^{(L-1)}W^{(L)})z' =
		\sum_{i=1}^{m_L}z'_i \sigma \left( \mathbf{ {X'}^{(i,L-2)} W'^{(i,L-1)}} \right) = \sum_{i=1}^{m_L}z'_i \mathbf{a'}_i=\sum_{i=1}^{|A_L|}z_i \mathbf{a}_i= \mathbf{Az},
\]
	achieves the same objective in \eqref{equ:nn_train_signdetinput_rescale} as in the \lasso{} problem \eqref{signLLasso_gen} with $\boldsymbol{\alpha}=\mathbf{z'},  \mathbf{W^{(i,l)}}= \mathbf{{{W}'}^{(i,l)}}$, and $ \mathbf{X^{(L-2)}}= \mathbf{{X'}^{(L-2)}}$. This construction uses similar ideas as the proof of \cref{lemma:sign_rewritedual}.


 \iftoggle{long}{
	Denote $W^{(l)}_i$ as the $i^{\textrm{th}}$ column of $W^{(l)}$, which contains the weights for the $i^{\textrm{th}}$ neuron of layer $l$.


 
 
 Let $z' \in \mathbb{R}^{m^L}$ be $z$ with $m_L - m^*\geq 0$ of its zero elements removed. Let $A' \in \mathbb{R}^{n \times m_L}$ be the matrix consisting of columns of $A$ that have the same index as the indices of $z$ that were used to make $z'$. Since each $i^{\textrm{th}}$ column $A'_i$ of $A'$ is in $A_L(X)$, there exists  a sequence of sets $S_j: j \in [L-1]$ and a sequence of matrices $ \tilde W^{(i,l-1)}: l \in [L-1]$ such that $\tilde X^{(i,l)} = \sigma([\tilde X^{(i,l-1)}, \mathbf{1}] \tilde W^{(l-2)}_i ) $ is a submatrix of $ \tilde{H}^{(l)}_{S_j:j\in[l]}(X)$ for $ l \in [L-2]$; in particular there exists a vector $\tilde W^{(i,L-1)} \in \mathbb{R}^{m_{L-2} }$ such that $A'_i = \sigma(\tilde X^{(i,L-2)} W^{(i,L-1)})$.
	So the parallel neural network,

	\begin{equation}
		f(X) =  %\sigma(X^{(L-1)}W^{(L)})z' =
		\sum_{i=1}^{m_L}z'_i \sigma({{\tilde X^{(i,L-2)}}}  \tilde W^{(i,L-1)}) = \sum_{i=1}^{m_L}z'_i (A')_i=\sum_{i=1}^{|A_L|}z_i (A)_i=Az,
	\end{equation}

	achieves the same objective in the primal \eqref{equ:nn_train_signdetinput_rescale} as the Lasso problem \eqref{signLLasso_gen} with $\alpha=z',  W^{(i,l)}= \tilde{W}^{(i,l)} , X^{(L-2)}=\tilde X^{(L-2)}$. Note we can normalize all the weights $W^{(i,L-1)}_i$ to achieve  $||W^{(i,L-1)}_i||_F=1$ to satisfy the primal \eqref{equ:nn_train_signdetinput_rescale} constraints.
}
\end{proof}

\begin{remark}
   \cref{prop:reconstruct_primal_L} gives a reconstruction from \lasso{} to the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} for an arbitrary number of layers $L$. \cref{prop:reconstruct_primal_L} is proved without relying on what the specific elements of $\mathbf{A}$ are, so that it is clear how a similar statement for the tree network holds. However, for practical use, the reconstruction given in \cref{prop:reconstruct_primal_L} can be simplified and made explicit as shown in \cref{thm:3lyr_sign_reconstruction} for $L=3$ layers.
\end{remark}

\iftoggle{long}{
\begin{remark}
	If $A_2(\mathbf{X})$ contains all vectors with $k$ switches for some $k \in [N]$, eg $k=1$ for $1$-dimensional data, and $m_1 = \cdots = m_{L-1}=m$ then for each $i \in [m]$ we can find $W^{(l)}_i $ directly in order $O(\min\{km_1,N\})=O(N)$ time by decomposing a $m_1$ switch vector into $1$-switch vectors as described in \cref{section:1D_dictionary}. If $L=3$ layers, then for $d=1$ dimensions, $\mathbf{X^{(1)}}$ is a matrix whose columns are one switch vectors in $\{-1,1\}$ and each column of $W^{(2)}_i$ is also a vector in $\{-1,1\}$.
\end{remark}
}

\begin{proposition}\label{prop:lasso_equiv_primal}
	For $L$-layer networks with sign activation, the \lasso{} problem \eqref{signLLasso_gen} problem and the original training problem \eqref{eq:nonconvex_generic_lossL_Lyr} are equivalent.
\end{proposition}

\begin{proof}
The proof is similar to that of \cref{theo:1d_all}.
     Let $t^*, r^*, d^*, f^*, l^*$ be the optimal values of the training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro}, rescaled problem \eqref{equ:nn_train_signdetinput_rescale},  problem \eqref{gen_dual}, problem \eqref{dsignpar_gen}, and the \lasso{} problem \eqref{signLLasso_gen}, respectively. 
     By \cref{thrm:rescaling}, the training problem \eqref{eq:nonconvex_generic_loss_gen_L_intro} is equivalent to its rescaling \eqref{equ:nn_train_signdetinput_rescale}.
     By \cref{lemma:dual_of_rescaled}, the dual of the rescaled problem  \eqref{equ:nn_train_signdetinput_rescale} is \eqref{gen_dual}. 
     By \cref{lemma:sign_rewritedual}, the dual problem \eqref{gen_dual} is equivalent to \eqref{dsignpar_gen}. By \cref{lemma:lasso_sign_L}, \eqref{dsignpar_gen} is equivalent to the \lasso{} problem \eqref{signLLasso_gen}.
    
    So by weak duality, $l^* = f^* \leq d^* \leq r^* = t^*$. On the other hand, \cref{prop:reconstruct_primal_L} gives a map from the \lasso \eqref{signLLasso_gen} to the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} that achieves the same objective value.
    \iftoggle{long}{ achieves the same function error $||y-f_L(X)||^2_2=||y-Az||^2_2$ and regularization penalty $\beta||\alpha||_1=\beta||z||_1$. 
    }
    So $l^* = r^* = t^*$ (strong duality holds).
\end{proof}

\iftoggle{long}{\begin{proof}
	Proposition \ref{prop:reconstruct_primal_L} gives a map from the LASSO problem \eqref{signLLasso_gen} problem to the \nc{} primal \eqref{equ:nn_train_signdetinput_rescale} that achieves the same function error $||y-f_L(X)||^2_2=||y-Az||^2_2$ and regularization penalty $\beta||\alpha||_1=\beta||z||_1$.  Since the LASSO problem \eqref{signLLasso_gen} is the bidual and hence a lower bound on the primal \eqref{equ:nn_train_signdetinput_rescale}, the mapping that the primal \eqref{equ:nn_train_signdetinput_rescale} can achieve any value of the LASSO problem \eqref{signLLasso_gen} shows that they are equivalent.
\end{proof}}



%\begin{lemma}
%Let dimension $d=1$. Let $z_3, d_3$ be the optimal solution and value of the LASSO problem with $L=3$. There exists a solution $z_2$ of the primal problem \eqref{equ:nn_train_signdetinput_rescale} with $L=2$ that achieves $d_3$.
%and regularization parameter $\beta=\beta_3$. There exists a regularization parameter $\beta_2=g(\beta_3)$ such that the optimal value $d_2$ of the LASSO problem with $L=3$ and $\beta=\beta_2$ satisfies $d_2 \leq d_3$. Then the LASSO problems with their respective regularization parameters are equivalent.
%\end{lemma}

%\section{2 versus 3 layer neural nets, 1D \label{section:3lyr_m1x2lyr}}

%\begin{remark}
%    Given the solution to the rescaled or original training problem, an optimal solution to the other problem can be found with the same resulting neural network.
%\end{remark}

%we found optimal solution in the rescaled problem. There is an optimal solution to original problem with the same nn. This is in fact the nn that we construct. Our reconstructed nn is Az. We make another nn that is also Az, and so we can rescale it to be optimal in the original problem without changing the number of neurons. Here we only deal with the function.

%\proofsketch{We rewrite a 3 layer network as a 2 layer network with a different $\beta$. Then any 3 layer network is also feasible in the 2 layer network training problem with a regularization parameter $\beta$ that is $m_1$ times greater. }

\begin{proof}[\textbf{Proof of \cref{cor:3lyr_m1x2lyr} }]
    %Given an optimal $3$ layer network in the original training problem, it can be rescaled to be optimal in the 

    
	%By \cref{prop:lasso_equiv_primal}, an optimal neural network to the rescaled training problem \eqref{equ:nn_train_signdetinput_rescale} can be constructed from the $L=3$ layer LASSO problem \eqref{signLLasso_gen}. Let $m_2^* = ||z^*||_0$ be the number of nonzero optimal bidual variables in \eqref{signLLasso_gen}. For convenience, let $\mathbf{z}$ be the subvector of nonzero elements of $\mathbf{z^*}$. By lemma \ref{lemma:decomp_english} and the construction of such an optimal neural network for the rescaled problem in the proof of proposition \ref{prop:reconstruct_primal_L},  \\ 
By the equivalence of the training problem to a \lasso{} model, the $2$-layer \lasso{} dictionary matrix is a submatrix of the $3$-layer dictionary matrix, so $p^*_{L=3,\beta} \leq p^*_{L=2,\beta}$. By the equivalence of the training problem to the rescaled problem, to show $p^*_{L=2,\beta} \leq p^*_{L=3,m_1\beta}$, it suffices to show that given an optimal fitting loss $\mathcal{L}_{\mathbf{y}}(f_{3}(\mathbf{X};\theta^{(3)}))$ and weight penalty $\|\boldsymbol{\alpha^{(3)}}\|_1$ for the $3$-layer rescaled training problem \eqref{equ:nn_train_signdetinput_rescale}, there exists an equivalent $2$-layer net $f_{2}(\mathbf{X};\theta^{(2)}) = f_{3}(\mathbf{X};\theta^{(3)})$ with weight penalty $\|\boldsymbol{\alpha^{(2)}}\|_1 \leq m_1 \|\boldsymbol{\alpha^{(3)}}\|_1$. Here, $\params^{(L)}$ and $\boldsymbol{\alpha}^{(L)}$ denote an architecture with $L$ layers.
Let $\mathbf{z}^*$ be optimal in the $3$-layer \lasso{} \eqref{thm_eq:3lyrsign}. Let $m_3^* = ||\mathbf{z^*}||_0$ and let $\mathbf{z} \in \mathbb{R}^{m_3^*}$ be the subvector of nonzero elements of $\mathbf{z^*}$.
 \cref{thm:3lyr_sign_reconstruction} and its proof provide weights $\Wul{i}{1}, \bul{i}{1} \in \mathbb{R}^{1 \times m_1}$ and $\Wul{i}{2} \in \mathbb{R}^{m_1}, \bul{i}{2} \in \mathbb{R}$ such that $\Xul{i}{2}\Wul{i}{2} + \bul{i}{2} \mathbf{1} \in \{-2,0\}^N$ and the output of an optimal $3$-layer neural net evaluated on $\mathbf{X}$ is
 \iftoggle{long}{ the first layer output is the matrix }
% $\xul{i}{l}=[\sigma(\mathbf{X} \Wul{i}{l}), \mathbf{1}] \in \{-1,1\}^{N \times (1+m_1)}$
 \iftoggle{long}{, whose columns are $1$-switch vectors in $\{-1,1\}^N$, 
 and $\Xul{i}{1}\Wul{i}{2}\in \{-2,0\}^N$ and an output of the optimal neural network for the rescaled \eqref{equ:nn_train_signdetinput_rescale} evaluated on all the training data is }
  %rescaled but that doesn't matter, the neural net evaluates to the same function and optimal objective is the same.

 %Since $\xul{i}{l}=[\sigma(\mathbf{X} \Wul{i}{l}), \mathbf{1}] \in \{-1,1\}^{N \times (1+m_1)}$. 
%ignore last [1] actually

	\begin{equation*}\label{eq:2layerto3layer_int}
		\begin{aligned}
			%m^* <2N?
			\nn{3}{\mathbf{X}} & =
			\sum_{n=1}^{m_3^*} z_i \sigma \left(\Xul{i}{2} \Wul{i}{2} + \mathbf{1} \cdot \bul{i}{2}\right) \\      
			                  & =   \sum_{i=1}^{m_2^*} z_i \left( \Xul{i}{2} \Wul{i}{2} + \mathbf{1} \cdot \bul{i}{2}+\mathbf{1}\right)                                                                  \\
			                     & = \sum_{i=1}^{m_3^*} z_i \left(  \sigma \left( \mathbf{X} \Wul{i}{1} + \mathbf{1} \cdot \bul{i}{1}  \right )\Wul{i}{2} + \mathbf{1} \cdot \bul{i}{2} +\mathbf{1} \right)                                                \\
			                     %& = \sum_{i=1}^{m_2^*} z_i \left(  [\sigma(X^{(i,0)} W^{(i,1)}), \mathbf{1}]\begin{bmatrix}
				                                                                                       %W^{(i,2)}_{1:m_1} \\
				                                                                                       %W^{(i,2)}_{m_1+1}
			                                                                                       %%+\mathbf{1} \right)                                                                                                                                                 \\
			       %    & = \sum_{i=1}^{m_2^*} z_i \left(  \sigma(\xul{i}{0} \Wul{i}{1} ) \Wul{i}{2}_{1:m_1} + \Wul{i}{2}_{m_1+1} \mathbf{1} +\mathbf{1} \right)                     \\
		%	           & = \sum_{i=1}^{m_2^*} z_i \left(  \sigma(\xul{i}{0}\Wul{i}{1} ) \Wul{i}{2}_{1:m_1} +  (1+ \Wul{i}{2}_{m_1+1}) \mathbf{1} \right)                            \\
			   %        & = \left( \sum_{i=1}^{m_2^*} z_i(1+W^{(i,2)}_{m_1+1}) \right) \mathbf{1}  + \sum_{i=1}^{m_2^*} \sigma(X^{(i,0)}  W^{(i,1)}) z_i W^{(i,2)}_{1:m_1}       \\
			%           & = \left( \sum_{i=1}^{m_2^*} z_i(1+\Wul{i}{2}_{m_1+1}) \right) \mathbf{1}  + \sum_{i=1}^{m_2^*} \sigma([\mathbf{X}, \mathbf{1}]  \Wul{i}{1}) z_i \Wul{i}{2}_{1:m_1} \\
			           & = \sigma \left(\mathbf{X} 
              \underbrace{\left[ \Wul{1}{1}\cdots \Wul{m_3^*}{1}\right]}_{\mathbf{W}} + \mathbf{1} \cdot 
              \underbrace{\left[ \bul{i}{1}, \cdots, \bul{i}{m_3^*}\right]}_{\mathbf{b}}
              \right)
              \underbrace{
			\begin{bmatrix}
				 & z_1  \Wul{1}{2}           \\
				 & \vdots                           \\
				 & z_{m_3^*}  \Wul{m_3^*}{2}
			\end{bmatrix}
   }_{\boldsymbol{\alpha}}
   +
  \mathbf{1} \underbrace{\sum_{i=1}^{m_3^*} z_i \left(1+ \bul{i}{2} \right)}_{\xi},
		\end{aligned}
	\end{equation*}

	% \begin{equation}
	%    f_2(x)=\sigma_s(xW_0+b)\alpha + \xi=\sigma([x,1]W)\alpha + \xi,
	%\end{equation}

which is the output of a $2$-layer network evaluated on $\mathbf{X}$ with $m=m_1m^*_2$ neurons, $\mathbf{W} \in \mathbb{R}^{2 \times m}, \boldsymbol{\alpha} \in \mathbb{R}^{m}, \xi \in \mathbb{R}$.
\iftoggle{long}{

	which matches the form of a $2$-layer network defined by \eqref{eq:2layernn} with $m=m_1m^*_2$ neurons, $\xi =  \sum_{i=1}^{m_2^*} z_i(1+ \Wul{i}{2}_{m_1+1} )$, and $\boldsymbol{\alpha} = \begin{bmatrix}
			 & z_1  \Wul{1}{2}_{1:m_1}            \\
			 & \vdots                           \\
			 & z_{m_2^*} \Wul{m_2^*}{2}_{1:m_1}
		\end{bmatrix} \in \mathbb{R}^{m}$ , and $\mathbf{W} =\left[\Wul{1}{1} \cdots \Wul{m_2^*}{1}\right]  \in \mathbb{R}^{2 \times m}$.
Note $z_i \Wul{i}{2} \in \mathbb{R}^{m_1}$.
}
	By the proof of \cref{thm:3lyr_sign_reconstruction}, the nonzero elements of $\Wul{i}{2}$ are $\pm 1$, so the weight penalty in the rescaled problem \eqref{equ:nn_train_signdetinput_rescale} for this $2$-layer net is $\|\boldsymbol{\alpha}^{(2)}\|_1=  \|\boldsymbol{ \alpha}\|_1 \leq m_1 \| \mathbf{z}^* \|_1 = m_1 \| \boldsymbol{\alpha}^{(3)} \|_1 $.
% $ ||\boldsymbol{ \alpha}||_1 =  \left \| \begin{bmatrix}
%			 & z_1  W^{(1,2)}_{1:m_1}           \\
%			 & \vdots                           \\
%			 & z_{m_2^*}  W^{(m_2^*,2)}_{1:m_1}
%		\end{bmatrix} \right \|_1 = \sum_{i=1}^{m^*_2} |z_i| || W^{(i,2)}_{1:m_1} ||_1 = \beta \sum_{i=1}^{m^*_2} |z_i| m_1  =  m_1 \beta \sum_{i=1}^{m^*_2} |z_i|$ which is the outer weight $l_1$ norm $\sum_{i=1}^{m^*_2} |z_i|$ of the original rescaled 3 layer neural net scaled up by the first layer size, $m_1$. %Note $\left[ W^{(1,1)}\cdots W^{(1,2N)}\right] \in \mathbb{R}^{N \times 2N m_1}$, although columns may be removed if the corresponding $z_i$ is $0$.
%  The rescaled 3 layer net can then be unrescaled to be optimal in the original training problem without changing the function.
%
\end{proof}



\section{$L\geq 3$ layer tree neural networks with sign activation}





	%Let $\mathbf{Z}$ be a matrix whose columns are in $\{-1,1\}^N$. Denote subsets $Z_S \subset Z$ with size $|S| = m$. Denote $[Z_S: |S|\leq m]$ to be the matrix which is the the concatenation of matrices $Z_S$. to be the matrix consisting of columns from $Z_S$. 
 Recall the set $\mathcal{H}$ defined in \eqref{eq:Hdef}. We define a matrix-to-matrix operator
	\begin{equation} %H acts on a matrix not a set of matrices!
		J^{(m)}(\mathbf{Z}) := \left[ \bigcup_{|S| \leq m} \mathcal{H}([\mathbf{Z}_S, \mathbf{1}]) \right],
	\end{equation}

which is the concatenation of all possible hyperplane arrangement patterns classifying up to $m$ columns of $\mathbf{Z}$.
Define ${A_L}_{\textrm{tree}}(\mathbf{X}) $ to be the set of columns in $J^{(m_{L-1})}\circ \cdots \circ J^{(m_{2})}(\mathcal{H}([\mathbf{X},\mathbf{1}])) $.
   %& = \mathcal{H}\left( J^{(m_{L-2})}\circ \cdots \circ J^{(m_{2})}(\mathcal{H}([\mathbf{X},\mathbf{1}])) \right).

	%which is $J$ composed with itself $L-2$ times. %check if L-2 or off by 1

\begin{lemma}
	The  dual problem \eqref{gen_dual_gen_arch} in \cref{lemma:dual_of_rescaled} for tree neural networks  is equivalent to

	\begin{equation}\label{gen_dual_tree_A}
		\begin{aligned}
			\max_{z \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}^*( \lambda )                         \\
			\text{ s.t. }             & \max_{\mathbf{h} \in {A_L}_{\textrm{tree}}(\mathbf{X})} |\lambda^T \mathbf{h}| \leq \beta.
		\end{aligned}
	\end{equation}
\end{lemma}

\iftoggle{long}{
\proofsketch{
	The proof follows from the recursive definition of the tree structure neural network. Note the standard and parallel networks lack this recursion.
}
}

\begin{proof}
	Recall the recursive tree architecture in \cref{app_subsection:tree_nn_def}. The set of all possible first layer outputs is $f^{(1)}(\mathbf{X};\theta^{(1)})= [\mathbf{X}, 1] \mathbf{w^{(1)}} $ is $\mathcal{H}([\mathbf{X},\mathbf{1}])$. For  $l \in [L-1]-\{1\}$, the 
matrix of all possible $l^{th}$ layer outputs  
 $f^{(l)}\left(\mathbf{X}; \theta^{(l)}\right) :=  w^{(l)}_{m_l + 1}\mathbf{1} + \sum_{i=1}^{m_{l}} \sigma\left(f^{(l-1)}\left(\mathbf{X};\theta^{(l-1,i)}\right)\right)w^{(l)}_i \in \mathbb{R}^N$ is $J^{(m_l)}$ applied to the matrix of  all possible $(l-1)^{th}$ layer outputs. Finally, plug in the penultimate layer $f^{(L-1)}\left(\mathbf{X}; \theta^{(L-1)}\right)$ into \eqref{gen_dual_gen_arch}.

 \iftoggle{long}{
 $f^{(l), \Theta^l}(X) = w^{(l)}_{m_l + 1}\mathbf{1} + \sum_{i=1}^{m_{l}} \sigma_{s^{l-1,i}}(f^{(l-1), \Theta^{l-1,i}})w^{(l)}_i \in \mathbb{R}^N $ and at the final layer, $f^{(L-1)}(X) = f^{(L-1), \Theta^{(L-1)}}(X) \in \mathbb{R}^N$. So given layer $l \in [L-2]$ and the set $Z$ of all possible vectors of the form $f^{(l, \Theta^{l-1})}(X)$, i.e., possible outputs at layer $l-1$, any possible $f^{(l)}(X)$ at the next layer $l$ is a linear combination of $m_l$ vectors from $Z$, which is a vector in $J(Z)$. And any linear combination of $m_l$ vectors from $Z$ is also a feasible output $f^{(l)}(X)$  at layer $l$. When $l=2$, by a similar argument as for the parallel networks, the set of all possible outputs at the final layer is $\mathcal{H}(X)$. By recursing, the set of all possible $f^{(L-1)}(X)$ becomes $J$ applied to $\mathcal{H}(X)$ for $L-2$ times.
 }
\end{proof}

\begin{lemma}\label{prop:prod_m_tree}
	${A_L}_{\textrm{tree}}(\mathbf{X})$ contains all vectors in $\{-1,1\}^N$ with up to $\prod_{l=1}^L m_l$ switches.
\end{lemma}

\begin{proof}
For notational convenience, in this proof we denote ${A_l}_{tree}(\mathbf{X})$ as $A_l$. Let $p_k = \prod_{l=1}^k m_l$.
	We use induction on the layer $l$. The base case when $l=2$ holds by \cref{prop:H_oneswitch}.
	%    For $l \in [L]$, let $A_l=\bigcup_{\{S_j:j\in[j],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X), p_l=\prod_{j=1}^{l} m_j$
	Now suppose \cref{prop:prod_m_tree} holds when $l=k \in [L-1]$. Observe $[A_{k}] \subset A_{k+1}$ as a submatrix, so if $p_k \geq N-1$, then \cref{prop:prod_m_tree} holds for $l=k+1$. So suppose $p_k < N-1$. Then $A_k$ contains all vectors in $\{-1,1\}^N$ with at most  $p_k$ switches. 

	%    The argument follows closely as that of proposition \ref{prop:m_1switches}.
	Let $\mathbf{h} \in {A_{k+1}}$.  
 The set ${A_{k+1}}$ contains all columns in $J^{(m_{k+1})}([A_{k}])$. So, there exist $\mathbf{w} \in \mathbb{R}^{m_{k+1}}, b \in \mathbb{R}$ and a submatrix $\mathbf{Z}:=[A_k]_S$ where $|S| \leq m_{k+1}$
and $\mathbf{h} = \sigma(\mathbf{\mathbf{Z} w} + b \mathbf{1})$. Each of the at most $ m_{k+1}$ columns of $\mathbf{Z}$ has at most $p_k$ switches, so the $N$ rows of $[\mathbf{Z}, \mathbf{1}]$ change at most $\min \{N-1, m_{k+1}p_k=p_{k+1}\}$ times. So $[\mathbf{Z},\mathbf{1}]$ and hence $\mathbf{h}=\sigma([\mathbf{Z},\mathbf{1}])$ changes value at most $\min \{N-1,p_{k+1}\}$ times.
Conversely, 
%let $\mathbf{h} \in \{-1,1\}^N$ with $p_{k+1} \in \{ n, \cdots N-1\}$ switches. 
by \cref{lemma:decomp_english}
	with 
 %$[[A_k]_S: |S|\leq m_k]=A_k$ and 
 $p=p_k, m = m_{k+1}$, the set $A_{k+1}$ of all columns in $J^{(m_{k+1})}([A_k])$ contains all vectors with at most $p_k m_{k+1}=p_{k+1}$ switches. So \cref{prop:prod_m_tree} holds for $l=k+1$. By induction, it holds for $l=L$ layers.














\end{proof}




==> unused/parallel_vs_std_scratch.tex <==
%not sure if this made sense

\section{Discussion: parallel versus standard neural networks}\label{app_sec:par_vs_std_nn_strong_duality}

A parallel neural net can be converted to a standard neural net, as described in the appendix. However, for $L\geq3$ layers with sign activation, the Lasso dictionary matrix of the parallel neural net depends on the number of neurons, which changes under conversion. So the Lasso dictionary may no longer apply to the converted neural network. Therefore, applying the Lasso problem for a standard neural net requires more careful consideration.

Weak duality between the training problem and the Lasso problem holds for the standard neural network. In deriving the Lasso equivalence to the nonconvex training problem (proof in appendix), the only step where the architecture choice of parallel and tree structures instead of a standard neural network is needed is in the reconstruction of an optimal neural network with more than two layers from the Lasso solution. This reconstruction improves weak duality to strong duality.

In fact, appendix \ref{app_sec:counterex_beta20} contains an example where if $\beta \to 0$ then the standard neural net can fail to achieve strong duality. In this counterexample, $m<N$. \iftoggle{todos}{\textcolor{red}{todo: read through, fix reference}} \\

However, if the number of neurons $m > N$, the number of samples, then a standard neural network can achieve strong duality, as discussed in appendix  \ref{app_sec:std_nn_m>N}. Even if $m < N$, there are cases such as with the square wave label (theorem \ref{}) where the optimal parallel neural net has only one unit that is active, and is therefore equivalent to a standard neural net.



\subsection{shattering}%but we have a better scenario than shattering: we know exactly what the matrix looks like.

\iftoggle{todos}{\textcolor{red}{todo: Fix/remove, cite Tolga's paper on shattering.}}

Suppose the data shatters, ie $A=\bigcup_{\{S_j:j\in[l],|S_j|\leq 1+m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X)$ contains all possible vectors in $[-1,1]^N$ then strong duality holds for the nonparallel neural network as well. The dual problem \ref{dsignLpar} becomes

\begin{equation}\label{dsignLparshatter}
	\begin{aligned}
		\max_{\lambda \in \mathbb{R}^N} & -\mathcal{L}_{\mathbf{y}}( \lambda )                              \\
		                                & \text{ s.t. } \max_{h \in \{-1,1\}^{N}} |\lambda^T h | \leq \beta
	\end{aligned}
\end{equation}

which is simplified to

\begin{equation}\label{dsignLparshattersimp}
	\begin{aligned}
		-\min_{\lambda \in \mathbb{R}^N} & \mathcal{L}_{\mathbf{y}}( \lambda )    \\
		                                 & \text{ s.t. } ||\lambda||_1 \leq \beta
	\end{aligned}
\end{equation}

which is the projection of $\lambda$ towards $y$ on to the $l_1$ ball of radius $\beta$.

%Let $\lambda^*$ be the optimal solution to problem \eqref{dsignLparshattersimp}. Let $S = \{n \in [N]: \lambda_n > 0 \}$. 

%Let an optimal $h$ be $h^*:= \text{sign}(h) = h^* \in \mathrm{argmax}_{h \in \{-1,1\}^N }\{\lambda^T h\} \subset \{-1,1\}^N = A_L(X)$. 

%Then let $H^* := \mathrm{argmax}_{h \in \{-1,1\}^N }\{\lambda^T h\} = \{h: \text{ if } \lambda_n \neq 0 \text{ then } h_n = \text{ sign}(\lambda_n), \text{ for } n\in [N] \}$. 

%Let $\alpha = \lambda$. 
%By definition of $A_L(X)$, for every $h \in H^*$, there exists weights $W^{(1)},\cdots, W^{(L-2)}$ and vector $W^{(L-2)}$ and corresponding $X^{(1)}, \cdots, X^{(L-2)}$ such that $\sigma(X^{(L-2)}W^{(L-2)}) = h^*$, and so $|{\lambda^*}^T \sigma(X^{(L-2)}W^{(L-2)}) |=|{\lambda^*}^T h| = ||\lambda^*||_1 \leq \beta $. 

%Then $||\lambda^*||_1 = |\lambda^* h^*||_1 $


%If we can find $w \in \mathbb{R}^{m_{l-1}+1}$ such that  Then for every $n \in S$, $\text{ sign}(\lambda_n)=h^*_n =  \sigma(x_n^{(L-2)}w)$.

%$\lambda^T h = \sum_{n \in [N]}\lambda_n \sigma(X^{(L-2)}w)_n = \sum_{n \in S}\lambda_n \sigma(X^{(L-2)}w)_n = \sum_{n \in S}\lambda_n \sigma(x_n^{(L-2)}w)$



%from the dual \eqref{gen_prep_to_dual}, $z^*= \mathcal{L}_{\mathbf{y}}(X) = \sum_{i=1}^{m_L}\alpha_i \sigma(X^{(L-2)}W^{(L-1)}) = $.

%If $\mathcal{L}_{\mathbf{y}}(z)=\frac{1}{2}||z-y||^2_2$ then this projection is 

\subsection{Strong duality also holds for standard neural nets if $m \geq N$}\label{app_sec:std_nn_m>N}

Note that for $1D$ data, given the same neural net first hidden layer size $m_1$, adding more layers can only decrease the expressability of the output: $A_{L+1}(X) \subset A_{L}(X)$. So the only way for the data to shatter is for the data to shatter on the first hidden layer.

%\iftoggle{todos}{
%\textcolor{red}{todo: how to go from $\lambda$ back via sign of each component which is same for h. and solve for $\lambda$ if L2 loss}
%}\\



We can also see this from the Lasso problem. Consider a standard nonparallel neural network with $m_1, \cdots, m_L$ neurons in each layer, ie the same number as that of each parallel unit in the parallel neural net. This standard neural net has   $m_L$ times as less neurons as the parallel one, but taking the bidual of the training problem results in the same LASSO problem and dictionary matrix.

Now suppose there exists possible neuron weights $W^{(1)},\cdots, W^{(L)}$ such that $X^{(L-1)}$ has rank $N$. Then for any matrix $A'$ consisting of a subset of columns from the dictionary matrix $A$, there exists $W^{(L)}$ such that $X^{(L-1)}W^{(L)} = A'=\sigma(A')$. Hence we can construct a standard nonparallel neural network $f(X)=\sigma(X^{(L-1)}W^{(L)})z = Az$ with $z=\alpha$ and the same number of neurons $m_1, \cdots, m_L$ as the layers of each parallel unit of the parallel neural network, and achieves the same function value in the primal. So strong duality holds for the standard neural network as well.  Therefore a parallel structure is not necessary for achieving minimal training loss in this case.

One way for this to occur is if for some $2 \leq l < L$, there exist weights $W^{(1)},\cdots, W^{(l)}$ such that $X^{(l)}$ has full rank and $m_l = m_{l+1} = \cdots = m_L$. i.e., the size of the layers do not change henceforth. Then setting each $W^{(l')}$  for $l < l' < L$ to be the identity matrix to preserve the full column rank of $X^{(l)}$ at $N$ means $X^{(L-1)}$ will have full rank. In the case of $1D$ data, the additional layers between the third and last layer can essentially just be identity matrices that preserve the expressability of the neural network from layer to layer.

In the case of $1D$ data, this can occur if the first layer has enough neurons relative to the number of samples. Suppose $m_1 \geq N$ and dimension $d=1$ and layer sizes satisfy $N-1 = m_1 = m_2 = \cdots = m_L$. By proposition \ref{prop:m_1_more_layers_same_size} there exists $X^{(1)}$ and $W^{(2)}$ such that $X^{(2)} = [\sigma(X^{(1)}) , \mathbf{1}]$ has full column rank.

Note if $A$ is not full rank, the LASSO problem is not strictly convex and there may be multiple possible neural networks. The generalizability of each of these possible networks is an area for future research.



\subsection{If $m<N$ then when $\beta \to 0$, strong duality may not hold for standard neural net}\label{app_sec:counterex_beta20}

%when the penultimate hidden layer size



However, if the number of neurons is not enough, specifically the penultimate hidden layer size $m_{L-1} < N-1$ %and the cardinality of the LASSO solution $||z^*||_0$ 
for $1D$ data, then depending on the training data and labels, strong duality might not hold for the standard nonparallel neural network. The standard neural network results in the same Lasso problem, but the Lasso problem may achieve a lower objective value than the primal for the standard neural network.

As the regularization penalty decreases $\beta \to 0$, the Lasso problem approaches satisfying $Az=y$:

\begin{equation}
	\begin{aligned}
		\min_z & ||z||_1                 \\
		       & \text{ such that } Az=y
	\end{aligned}
\end{equation}



In this low-regularization regime, we show a counterexample as follows.

\textcolor{red}{ is this example sufficient? even if $\beta \neq 0$, is this counterexample enough? we do have $||\alpha||_1=||z||_1$}

Let the number of samples be $N=3, X \in \mathbb{R}^3$. Suppose the neural network has layer sizes $m_1=1, m_2=2$. By proposition \ref{prop:m_1switches}, up to permutation of columns, the dictionary matrix $A$ consists of $1$ in the upper right corner including the diagonal and $-1$ elsewhere, and therefore the column span of $A$ is all of $\mathbb{R}^3$ by lemma \ref{lemma:A_full_rk}.

So for any $y$, we can solve $z=A^{-1}y$ and from the LASSO problem we can construct a parallel neural network to achieve perfect interpolation of the data. However, the nonparallel neural network is of the form  
%but actually, ${f_{3,std}}(\mathbf{x}; \theta) :=  \sigma \left ( \left[ \sigma \left([\mathbf{x},1] \mathbf{W^{(1)}} \right), \mathbf{1}  \right ]   \mathbf{W^{(2)}}\right) \alpha + \xi$ \\
$f(X)=\sigma(X^{(1)}W^{(2)})\alpha$ where $X^{(1)}=\sigma([X, \mathbf{1}]W^{(1)}) W^{(2)} \in \mathbb{R}^2$. %So $X^{(1)}$ is one of the columns of $A$, concatenated with a column of ones, which is a matrix that consists of two of the columns of $A$. 
Then  $\sigma(X^{(1)}W^{(2)})$ has size $3 \times 2$ and therefore does not have full column rank. Therefore there exists $y \in \mathbb{R}^3$ for which no such $\alpha \in \mathbb{R}^2$ satisfies $\sigma(X^{(1)}W^{(2)})\alpha=y$.

The counterexample can be generalized to any any dimension $d$, number of layers $m_L$, number of samples $N$, training data $X \in \mathbb{R}^{N \times d}$ where the dictionary matrix $A$ has full rank but $m_{L-1}<N$.




==> unused/reludiagram.tex <==

%below is correct if a1 is just x_j1. Also not necessary. Also not using f^{L,sigma}_{s,j,k} notation anymore.
 \begin{figure}[t]
%todo: magenta and red look too similar
    \centering
    \scalebox{0.9}{
     \noindent\makebox[\textwidth]{
\begin{tikzpicture}
    \pgfmathsetmacro{\hint}{8} %horizontal interval spacing
    \pgfmathsetmacro{\vint}{-4} %vertical interval spacing
    \pgfmathsetmacro{\scale}{0.25}
    \pgfmathsetmacro{\hbias}{-2*\hint}
    \pgfmathsetmacro{\labelv}{0}
    \pgfmathsetmacro{\labelh}{-15}


    \begin{scope}[scale=\scale, shift={(0*\hint+0.5*\hbias,-2*\vint)}]
         %\node[] (graphs) at (-3,\labelv) {\lasso{} feature $\reludiccol{L}$ plotted over $x_i$};
        \draw[gray] (-58,\labelv-3) -- (10,\labelv-3);
	\end{scope}
 
     \begin{scope}[scale=\scale, shift={(-4*\hint,-1.5*\vint)}]
        %\incline{magenta};
         \node[] (init) at (3,-3) {};
	\end{scope}
 
    %left half
%    \begin{scope}[scale=\scale, shift={(-4*\hint,0)}]
%        \decline{magenta};
%        \node[] (0upper) at (3,3) {};
%        \node[] (0lower) at (3,-3) {};
%	\end{scope}
 %
    \begin{scope}[scale=\scale, shift={(-6*\hint,\vint)}]
        \decrelu{\acolor}{\ashape};
        \node[] (00upper) at (3,3) {};
        \node[] (00lower) at (3,-3) {};
	\end{scope}
 %
%    \begin{scope}[scale=\scale, shift={(-4*\hint,2*\vint)}]
%        \downshiftdecrelu{orange}{magenta};
%        \node[] (000upper) at (3,3) {};
%        \node[] (000lower) at (3,-3) {};
%	\end{scope}
 %
%    \begin{scope}[scale=\scale, shift={(-2.5*\hint,3*\vint)}]
%        \downshiftdecrelu{orange}{magenta};
%        \node[] (0001upper) at (3,3) {};
%        \node[] (0001lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(-5.5*\hint,3*\vint)}]
%        \negincrelu{orange}{magenta};
%        \node[] (0000upper) at (3,3) {};
%        \node[] (0000lower) at (3,-3) {};
%	\end{scope}
%
    \begin{scope}[scale=\scale, shift={(-5*\hint,4*\vint)}]
        \decrelu{\bcolor}{\snegshape};
        \node[] (00010upper) at (3,3) {};
        \node[] (00010lower) at (3,-3) {};
	\end{scope}
    \begin{scope}[scale=\scale, shift={(-7*\hint,4*\vint)}]
        \incrampfromzero{\bcolor}{\snegshape}{\acolor}{\ashape};
        \node[] (00000upper) at (3,3) {};
        \node[] (00000lower) at (3,-3) {};
	\end{scope}
%
%    \begin{scope}[scale=\scale, shift={(-6.5*\hint,5*\vint)}]
%        \incramp{orange}{red}{magenta};
%        \node[] (00000_0upper) at (3,3) {};
%        \node[] (00000_0lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(-4.5*\hint,5*\vint)}]
%        \downshiftincramp{orange}{magenta};
%        \node[] (00000_1upper) at (3,3) {};
%        \node[] (00000_1lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(-2.5*\hint,5*\vint)}]
%        \downshiftdecrelu{yellow}{orange};
%        \node[] (00010_0upper) at (3,3) {};
%        \node[] (00010_0lower) at (3,-3) {};
%	\end{scope}
 %
%    \begin{scope}[scale=\scale, shift={(-7*\hint,6*\vint)}]
%        \decramp{orange}{red}{magenta};
%        \node[] (00000_00upper) at (3,3) {};
%        \node[] (00000_00lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(-6*\hint,6*\vint)}]
%        \incramp{orange}{red}{magenta};
%        \node[] (00000_01upper) at (3,3) {};
%        \node[] (00000_01lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(-5*\hint,6*\vint)}]
%        \upshiftdecramp{orange}{magenta};
%        \node[] (00000_10upper) at (3,3) {};
%        \node[] (00000_10lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(-4*\hint,6*\vint)}]
%        \downshiftincramp{orange}{magenta};
%        \node[] (00000_11upper) at (3,3) {};
%        \node[] (00000_11lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(-3*\hint,6*\vint)}]
%        \negincrelu{yellow}{orange};
%        \node[] (00010_00upper) at (3,3) {};
%        \node[] (00010_00lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(-2*\hint,6*\vint)}]
%        \downshiftdecrelu{yellow}{orange};
%        \node[] (00010_01upper) at (3,3) {};
%        \node[] (00010_01lower) at (3,-3) {};
%	\end{scope}
 %
    \begin{scope}[scale=\scale, shift={(-7.5*\hint,7*\vint)}]
        \decramptozero{\bcolor}{\snegshape}{\ccaprampcolor}{\snegshape}
        \node[] (00000_000upper) at (3,3) {};
        \node[] (00000_000lower) at (3,-3) {};
	\end{scope}
    \begin{scope}[scale=\scale, shift={(-6.5*\hint,7*\vint)}]
        \incrampfromzero{\ccaprampcolor}{\snegshape}{\acolor}{\ashape};
        \node[] (00000_010upper) at (3,3) {};
        \node[] (00000_010lower) at (3,-3) {};
	\end{scope}
%    \begin{scope}[scale=\scale, shift={(-5*\hint,7*\vint)}]
%        \upshiftdecramp{orange}{magenta};
%        \node[] (00000_100upper) at (3,3) {};
%        \node[] (00000_100lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(-4*\hint,7*\vint)}]
%        \zerofunc{};
%        \node[] (00000_110upper) at (3,3) {};
%        \node[] (00000_110lower) at (3,-3) {};
%	\end{scope}
    \begin{scope}[scale=\scale, shift={(-5.5*\hint,7*\vint)}]
        \incrampfromzero{\crelucolor}{\snegshape}{\bcolor}{\snegshape};
        \node[] (00010_000upper) at (3,3) {};
        \node[] (00010_000lower) at (3,-3) {};
	\end{scope}
    \begin{scope}[scale=\scale, shift={(-4.5*\hint,7*\vint)}]
        \decrelu{\crelucolor}{\snegshape};
        \node[] (00010_010upper) at (3,3) {};
        \node[] (00010_010lower) at (3,-3) {};
	\end{scope}
 
%%%%%%%%%% right half
%    \begin{scope}[scale=\scale, shift={(4*\hint+\hbias,0)}]
%        \incline{magenta};
%        \node[] (1upper) at (3,3) {};
%        \node[] (1lower) at (3,-3) {};
%	\end{scope}
 %
    \begin{scope}[scale=\scale, shift={(0*\hint+\hbias,\vint)}]
        \increlu{\acolor}{\ashape};
        \node[] (10upper) at (3,3) {};
        \node[] (10lower) at (3,-3) {};
	\end{scope}
%
%    \begin{scope}[scale=\scale, shift={(4*\hint+\hbias,2*\vint)}]
%        \downshiftincrelu{magenta}{blue};
%        \node[] (100upper) at (3,3) {};
%        \node[] (100lower) at (3,-3) {};
%	\end{scope}
%
%    \begin{scope}[scale=\scale, shift={(2.5*\hint+\hbias,3*\vint)}]
%        \negdecrelu{magenta}{blue};
%        \node[] (1000upper) at (3,3) {};
%        \node[] (1000lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(5.5*\hint+\hbias,3*\vint)}]
%        \downshiftincrelu{magenta}{blue};
%        \node[] (1001upper) at (3,3) {};
%        \node[] (1001lower) at (3,-3) {};
%	\end{scope}
 %
    \begin{scope}[scale=\scale, shift={(-1*\hint+\hbias,4*\vint)}]
        \decramptozero{\acolor}{\ashape}{\bcolor}{\sposhape};  
        \node[] (10000upper) at (3,3) {};
        \node[] (10000lower) at (3,-3) {};
	\end{scope}
    \begin{scope}[scale=\scale, shift={(1*\hint+\hbias,4*\vint)}]
        \increlu{\bcolor}{\sposhape};
        \node[] (10010upper) at (3,3) {};
        \node[] (10010lower) at (3,-3) {};
	\end{scope}
%
%    \begin{scope}[scale=\scale, shift={(1.5*\hint+\hbias,5*\vint)}]
%        \decramp{magenta}{green}{blue};
%        \node[] (10000_0upper) at (3,3) {};
%        \node[] (10000_0lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(3.5*\hint+\hbias,5*\vint)}]
%        \downshiftdecramp{magenta}{blue}; 
%        \node[] (10000_1upper) at (3,3) {};
%        \node[] (10000_1lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(5.5*\hint+\hbias,5*\vint)}]
%        \downshiftincrelu{blue}{cyan};
%        \node[] (10010_0upper) at (3,3) {};
%        \node[] (10010_0lower) at (3,-3) {};
%	\end{scope}
 %
%    \begin{scope}[scale=\scale, shift={(1*\hint+\hbias,6*\vint)}]
%        \incramp{magenta}{green}{blue};
%        \node[] (10000_00upper) at (3,3) {};
%        \node[] (10000_00lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(2*\hint+\hbias,6*\vint)}]
%        \decramp{magenta}{green}{blue};
%        \node[] (10000_01upper) at (3,3) {};
%        \node[] (10000_01lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(3*\hint+\hbias,6*\vint)}]
%        \upshiftincramp{magenta}{blue};
%        \node[] (10000_10upper) at (3,3) {};
%        \node[] (10000_10lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(4*\hint+\hbias,6*\vint)}]
%        \downshiftdecramp{magenta}{blue};
%        \node[] (10000_11upper) at (3,3) {};
%        \node[] (10000_11lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(5*\hint+\hbias,6*\vint)}]
%        \negdecrelu{blue}{cyan};
%        \node[] (10010_00upper) at (3,3) {};
%        \node[] (10010_00lower) at (3,-3) {};
%	\end{scope}
%    \begin{scope}[scale=\scale, shift={(6*\hint+\hbias,6*\vint)}]
%        \downshiftincrelu{blue}{cyan};
%        \node[] (10010_01upper) at (3,3) {};
%        \node[] (10010_01lower) at (3,-3) {};
%	\end{scope}
 %
    \begin{scope}[scale=\scale, shift={(-1.5*\hint+\hbias,7*\vint)}]
        \incrampfromzero{\ccaprampcolor}{\sposhape}{\bcolor}{\sposhape};
        \node[] (10000_000upper) at (3,3) {};
        \node[] (10000_000lower) at (3,-3) {};
	\end{scope}
    \begin{scope}[scale=\scale, shift={(-0.5*\hint+\hbias,7*\vint)}]
        \decramptozero{\acolor}{\ashape}{\ccaprampcolor}{\sposhape};
        \node[] (10000_010upper) at (3,3) {};
        \node[] (10000_010lower) at (3,-3) {};
	\end{scope}
%    \begin{scope}[scale=\scale, shift={(3*\hint+\hbias,7*\vint)}]
%        \upshiftincramp{magenta}{blue};
%        \node[] (10000_100upper) at (3,3) {};
%        \node[] (10000_100lower) at (3,-3) {};
%	\end{scope}
%     \begin{scope}[scale=\scale, shift={(4*\hint+\hbias,7*\vint)}]
%        \zerofunc{};
%        \node[] (10000_110upper) at (3,3) {};
%        \node[] (10000_110lower) at (3,-3) {};
%	\end{scope}
    \begin{scope}[scale=\scale, shift={(0.5*\hint+\hbias,7*\vint)}]
        \decramptozero{\bcolor}{\sposhape}{\crelucolor}{\sposhape};
        \node[] (10010_000upper) at (3,3) {};
        \node[] (10010_000lower) at (3,-3) {};
	\end{scope}
    \begin{scope}[scale=\scale, shift={(1.5*\hint+\hbias,7*\vint)}]
        \increlu{\crelucolor}{\sposhape};
        \node[] (10010_010upper) at (3,3) {};
        \node[] (10010_010lower) at (3,-3) {};
	\end{scope}
 
 %% arrows
 %
\path[->, draw = black] (init) edge (00upper);
\path[->, draw = black] (init) edge (10upper);
 %left half 
%\path[->, draw = black] (0lower) edge (00upper);
 %
\path[->, draw = black] (00lower) edge (00000upper); 
\path[->, draw = black] (00lower) edge (00010upper); 
 %
%\path[->, draw = black] (000lower) edge (0000upper);
%\path[->, draw = black] (000lower) edge (0001upper);
%
%\path[->, draw = black] (0000lower) edge (00000upper);
%\path[->, draw = black] (0001lower) edge (00010upper);
%
\path[->, draw = black] (00000lower) edge (00000_000upper);
\path[->, draw = black] (00000lower) edge (00000_010upper);
\path[->, draw = black] (00010lower) edge (00010_000upper);
\path[->, draw = black] (00010lower) edge (00010_010upper);
%
%\path[->, draw = black] (00000_0lower) edge (00000_00upper);
%\path[->, draw = black] (00000_0lower) edge (00000_01upper);
%\path[->, draw = black] (00000_1lower) edge (00000_10upper);
%\path[->, draw = black] (00000_1lower) edge (00000_11upper);
%\path[->, draw = black] (00010_0lower) edge (00010_00upper);
%\path[->, draw = black] (00010_0lower) edge (00010_01upper);
%
%\path[->, draw = black] (00000_00lower) edge (00000_000upper);
%\path[->, draw = black] (00000_01lower) edge (00000_010upper);
%\path[->, draw = black] (00000_10lower) edge (00000_100upper);
%\path[->, draw = black] (00000_11lower) edge (00000_110upper);
%\path[->, draw = black] (00010_00lower) edge (00010_000upper);
%\path[->, draw = black] (00010_01lower) edge (00010_010upper);

 %right half 
% \path[->, draw = black] (1lower) edge (10upper);
 %
\path[->, draw = black] (10lower) edge (10000upper);
\path[->, draw = black] (10lower) edge (10010upper);
 %
%\path[->, draw = black] (100lower) edge (1000upper);
%\path[->, draw = black] (100lower) edge (1001upper);
%
%\path[->, draw = black] (1000lower) edge (10000upper);
%\path[->, draw = black] (1001lower) edge (10010upper);
%
\path[->, draw = black] (10000lower) edge (10000_000upper);
\path[->, draw = black] (10000lower) edge (10000_010upper);
\path[->, draw = black] (10010lower) edge (10010_000upper);
\path[->, draw = black] (10010lower) edge (10010_010upper);
%\path[->, draw = black] (10000lower) edge (10000_1upper);
%\path[->, draw = black] (10010lower) edge (10010_0upper);
%
%\path[->, draw = black] (10000_0lower) edge (10000_00upper);
%\path[->, draw = black] (10000_0lower) edge (10000_01upper);
%\path[->, draw = black] (10000_1lower) edge (10000_10upper);
%\path[->, draw = black] (10000_1lower) edge (10000_11upper);
%\path[->, draw = black] (10010_0lower) edge (10010_00upper);
%\path[->, draw = black] (10010_0lower) edge (10010_01upper);
%
%\path[->, draw = black] (10000_00lower) edge (10000_000upper);
%\path[->, draw = black] (10000_01lower) edge (10000_010upper);
%\path[->, draw = black] (10000_10lower) edge (10000_100upper);
%\path[->, draw = black] (10000_11lower) edge (10000_110upper);
%\path[->, draw = black] (10010_00lower) edge (10010_000upper);
%\path[->, draw = black] (10010_01lower) edge (10010_010upper);

%legend

%    \node[] (dic) at (0,0) {$\left(s^{(3)}\left( \left( s^{(2)} \left( \left(  s^{(1)} \left(x - a \right) \right)_+ -b\right) \right)_+ -c \right)\right)_+$ where $s^{(l)} \in \{-1, 1\}, a \in \mathbb{R}, b \geq 0, c \geq 0$.};
    
\begin{scope}[scale=\scale, shift={(0*\hint+1.1*\hbias,8*\vint)}]
    \draw (-5*\hint, 2) -- (4.1*\hint+\hbias, 2) -- (4.1*\hint+\hbias,-6) -- (-5*\hint, -6) -- cycle;
    
    \node [\ashape, scale=0.5, fill=\acolor, label=right:{\small $a_1$  %($ x_{j_1}$ if $k=0$ and $2x_{j_2}-x_{j_1}$ if $k=1$)
    }] (\acolor) at (-4.5*\hint, 0) {};

    %col 1
    \node [\snegshape, scale=0.5, fill=\bcolor, label=right:{\small $\min 
    \{a_1, x_{j_2} \}$}] (\bcolor) at (-3.9*\hint, 0) {};
    \node [\snegshape, scale=0.5, fill=\crelucolor, label=right:{\small $\min\{a_1, x_{j_2}, x_{j_3} \}$}] (\crelucolor) at (-3.9*\hint, -2) {};
    \node [\snegshape, scale=0.5, fill=\ccaprampcolor, label=right:{\small $\min \{ a_1, \max \{ x_{j_3}, \min \{a_1, x_{j_2} \} \} \}$}] (\ccaprampcolor) at (-3.9*\hint, -4) {};

    %col 2
    \node [\sposhape, scale=0.5, fill=\bcolor, label=right:{\small $\max \{a_1, x_{j_2} \}$}] (blue) at ((1.3*\hint+\hbias, 0) {};
    \node [\sposhape, scale=0.5, fill=\crelucolor, label=right:{\small $\max\{a_1, x_{j_2}, x_{j_3} \}$}] (cyan) at ((1.3*\hint+\hbias, -2) {};
    \node [\sposhape, scale=0.5, fill=\ccaprampcolor, label=right:{\small $\max \{ a_1, \min \{ x_{j_3}, \max \{a_1, x_{j_2} \} \} \} $}] (green) at ((1.3*\hint+\hbias, -4) {};
    
\end{scope}

%labels
\begin{scope}[scale=\scale, shift={(-6*\hint,-2*\vint)}]
        \node[] (f) at (\labelh,\labelv) {\small layers $L$};
\end{scope}
    \begin{scope}[scale=\scale, shift={(-4*\hint,-2*\vint)}]
        %\incline{magenta};
          \node[] (graphs) at (3,\labelv) {\lasso{} feature $\reludicfun{L}(\mathbf{X})$};;
	\end{scope}
%\begin{scope}[scale=\scale, shift={(-6*\hint,-1*\vint)}]
%        \node[] (l1) at (\labelh,\labelv) {\small $(x-a)$};
%\end{scope}
%\begin{scope}[scale=\scale, shift={(-8*\hint,0)}]
%        \node[] (l1) at (\labelh,\labelv) {\small $s^{(1)}(x-a)$};
%\end{scope}
\begin{scope}[scale=\scale, shift={(-6*\hint,1*\vint)}]
        \node[] (l1) at (\labelh,\labelv) {\small $2$};
\end{scope}
%\begin{scope}[scale=\scale, shift={(-8*\hint,2*\vint)}]
%        \node[] (l1) at (\labelh,\labelv) {\small $\left(s^{(1)}\left(x-a\right)\right)_+-b$};
%\end{scope}
%\begin{scope}[scale=\scale, shift={(-8*\hint,3*\vint)}]
%        \node[] (l1) at (\labelh,\labelv) {\small $s^{(2)}\left(\left(s^{(1)}\left(x-a\right)\right)_+-b\right)$};
%\end{scope}
\begin{scope}[scale=\scale, shift={(-6*\hint,4*\vint)}]
        \node[] (l1) at (\labelh,\labelv) {\small $3$};
\end{scope}
%\begin{scope}[scale=\scale, shift={(-8*\hint,5*\vint)}]
%        \node[] (l1) at (\labelh,\labelv) {\small $s^{(2)}\left(\left(s^{(1)}\left(x-a\right)\right)_+-b\right)_+ -c $};
%\end{scope}
%\begin{scope}[scale=\scale, shift={(-8*\hint,6*\vint)}]
%        \node[] (l1) at (\labelh,\labelv) {\small $s^{(3)}\left(s^{(2)}\left(\left(s^{(1)}\left(x-a\right)\right)_+-b\right)_+ -c \right)$};
%\end{scope}
\begin{scope}[scale=\scale, shift={(-6*\hint,7*\vint)}]
        \node[] (l1) at (\labelh,\labelv) {\small $4$};
\end{scope}


\end{tikzpicture}
}
}
\caption{
%For each function of $x$ labeled on the left, its possible graphs are drawn on the right, for the various combinations of parameters $s^{(l)} \in \{-1,1\}$ and $b,c \geq 0$. 
%The rows of arrows from top to second from the bottom represent the following sequence repeated twice: taking a ReLU, subtracting $a,b$ or $c$, and scaling by $s{(l)}$. 
%The last row of arrows takes a ReLU again. 
%In all other cases, the arrows pointing to the right and left represent the cases $s^{(l)} \geq 0$ and $s^{(l)} \leq 0$, respectively. 
The $L^{th}$ row consists of possible graphs of the dictionary function $\reludicfun{L}(x)$ where $\sigma$ is ReLU and $\mathbf{s}$ is varied. The point $a_1$ is as defined in \cref{def:RELU dic func}.
Arrows point to the right and left to represent the cases $s_{l} \geq 0$ or $s_{l} \leq 0$, respectively, for $l \in [L-1]$. 
%If the kink points coincide, the feature vector reduces to the all-zero vector.
%The colored dots mark the zeros and kink points.
}
\label[figure]{fig:relu_evol_simp}
\end{figure}



==> unused/scratch.tex <==

\section{motivation for threshold 2 layer critical solution (Note works for feature that has highest inner product with y, but for the other features need to go through more careful analysis with subgradients.)}

Suppose the error is not too large: $S > -1$ if $q_i$ is odd and $s<1$ if $q_i$ is even. And assume $y=h_{k,T}+\delta_{s,i}$.

Note if  $|y^T a_j|$ is maximized for columns $a_j$ of $A$ if $a_j$ switches in the middle of a period. We can do a change of variables by negative $z$ so that we assume the columns of $A$ begin with first element being $-1$, to match the form of $h_{k, T}$. Then at the critical $\beta = \beta_c$, for any column $a_j$ of the dictionary matrix $A$ that has a switch at some $q_n\frac{T}{2}+1$ for odd $q_n \in [2(k-1)]$, ie in the middle of the $q_n^{th}$ half-cycle. %in the 3-layer case we are assuming no sign changes, so just add s. q always starts at 0.

Then, since the error $s$ does not change the sign of $y_i$, for such a $j$,

\begin{align*}
    y^T a_j &= (h_{k,T} + \delta_{s,i})^T a_j \\
    &= h_{k,T}^T a_j + \delta_{s,i}^T a_j\\
    &= T + s(-1)^{\mathbf{1}_{q_n\geq q_i}}
\end{align*}

which is maximized in absolute value if $q_n < q_i$ if $s>0$ and $q_n > q_i$ if $s>0$.

Suppose $s=0$. Then $|y^T a_j|=T = \mbox{argmax}{a_j}|y^T a_j|$ is maximized for all columns of $A$ that switch at $q_n\frac{T}{2}+1$, for odd $n$. And $\beta_c = T$. If all such $a_j$ were active at the critical $\beta$,  their coefficients $z_j>0$. Let $\Tilde{I}$ be a $N \times k-1$ matrix with for odd $j$, $\Tilde{I}_{\frac{T}{2}j+1,j} = 1$  and $0$ in all other elements. Let $\Tilde{A}=A\Tilde{I}$ be the submatrix of $A$, taking the columns with indices odd multiples of $\frac{T}{2}$. \textcolor{red}{ ($T/2$ or $T/2 + 1$?) }.  Let $\Tilde{z} = \Tilde{I}^Tz$ denote a subvector $z$ with only the elements at every odd multiple of $\frac{T}{2}$. So for large enough $\beta$, 

\begin{align*}
    \min \frac{1}{2}||\Tilde{A}\Tilde{z}-y||^2_2 + \beta \mathbf{1}^T \Tilde{z} 
\end{align*}

which is solved by setting the gradient to $0$:

\begin{align*}
    \Tilde{A}^T(\Tilde{A}\tilde{z}-y) + \beta\mathbf{1}&=0\\
    \tilde{z} &= (\Tilde{A}^T\Tilde{A})^{-1}(\Tilde{A}^Ty-\beta\mathbf{1})\\
    &=  (\Tilde{A}^T\Tilde{A})^{-1}(\beta_c \mathbf{1}-\beta\mathbf{1})\\
     &(\beta_c - \beta)_+ (\Tilde{A}^T\Tilde{A})^{-1}\mathbf{1}.\\
\end{align*}

since $a_j^T y T  >0$ so that $a_j^T y = \beta_c$ for all maximizing $a_j$.


Note if $z = \frac{(\beta_c - \beta)_+}{||a_j||^2_2}e_j \geq \mathbf{0}$ where $a_j = \mbox{argmax}_[a_k] |a_k^T y|$ then for any $k \neq j$, since $||a_k||_2 = ||a_j||_2$ and $|a_j^Ty| \geq |a_k^Ty|$,

\begin{equation}
    \begin{aligned}
      (A^T(Az-y))_k &= a_k^T(Az-y) \\
      &= a_k^T(\frac{(\beta_c - \beta)_+}{||a_j||^2_2}a_j-y) \\
      &= (\beta_c - \beta)_+\frac{a_k^T a_j}{||a_j||^2_2} - a_k^Ty \\
      & \in [(\beta_c - \beta)_+(-1)-|a_j^Ty|,(\beta_c - \beta)_+(1)+|a_j^Ty|]\\
      &=  [-(\beta_c - \beta)_+-\beta_c,(\beta_c - \beta)_+ +\beta_c]\\
      &= [\beta -2\beta_c, 2\beta_c - \beta ]
    \end{aligned}
\end{equation}

Note that $2\beta_c - \beta \geq \beta_c - \beta \geq 0$. So  $|(A^T(Az-y))_k| \leq 2\beta_c - \beta$ which is at most $\beta$ if $2\beta_c - \beta \leq \beta$ ie $\beta_c \leq \beta$, which is not true unless $\beta_c = \beta$.

\begin{equation}
    \begin{aligned}
      \frac{(\beta_c - \beta)_+}{N}a_j-y &= 
      \begin{cases}
          ( \frac{(\beta_c - \beta)_+}{N}-1) \mbox{ if }j \leq \frac{T}{2} \\
          (-\frac{(\beta_c - \beta)_+}{N}-1) \mbox{ if odd cycle, }j \geq \frac{T}{2},  \\
           (-\frac{(\beta_c - \beta)_+}{N}+1) \mbox{ if even cycle, }j \geq \frac{T}{2},  \\
      \end{cases}    
    \end{aligned}
\end{equation}

%So $|(A^T(Az-y))_k| \leq |\beta-2\beta_c|$. So for $|(A^T(Az-y))_k| \leq \beta$ it suffices that $0 \leq \beta - 2\beta_c \leq \beta$  or $0 \leq 2\beta_c - \beta \leq \beta$. Since $\beta \leq \beta_c$ we have $\beta \leq \beta_c \leq 2\beta_c$ and so the condition is satisfied.

%a_k^Ty could be very negative! If all but one is flipped ie shifted by T


To check that $\Tilde{z} \geq 0$ it suffices to show that $(\Tilde{A}^T\Tilde{A})^{-1}\mathbf{1} \geq 0$. Note $\Tilde{I}^T A^T A \Tilde{I}$ subsamples the matrix $A^TA$ at intervals of $T^{th}$ in the columns and then the rows starting at $\frac{T}{2}$.

From equation \eqref{eq:A^TA_writtenout}

\begin{equation}
 \setcounter{MaxMatrixCols}{20}
\begin{aligned}
    \Tilde{I}^T A^T A \Tilde{I}
 &=  \Tilde{I}^T\begin{pmatrix}
    N   & N-2 & N-4 & \cdots & 2 & 0 & -2 & \cdots & 6-N  & 4-N & 2-N   \\
    N-2 & N   & N-2 & \cdots & 4 & 2 &  0 & \cdots & 8-N  & 6-N & 4-N   \\
    N-4 & N-2 & N   & \cdots & 6 & 4 & 2 & \cdots  & 10-N & 8-N & 6-N   \\
    \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
    6-N & 8-N & 10-N & \cdots & 2 & 4 & 6 & \cdots & 8-N & 6-N & 4-N   \\
    4-N & 6-N & 8-N & \cdots &  0 & 2 & 4 & \cdots & 6-N  & 4-N & 2-N   \\
    2-N & 4-N & 6-N & \cdots & -2 & 0 & 2 & \cdots & 4-N  & 2-N & N
    \end{pmatrix}\Tilde{I} \\
    &=  \begin{pmatrix}
    N   & N-2T & N-4T & \cdots & 2T & 0 & -2T & \cdots & 6T-N  & 4T-N & 2T-N   \\
    N-2T & N   & N-2T & \cdots & 4T & 2T &  0 & \cdots & 8T-N  & 6T-N & 4T-N   \\
    N-4T & N-2T & N   & \cdots & 6T & 4T & 2T & \cdots  & 10T-N & 8T-N & 6T-N   \\
    \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
    6T-N & 8T-N & 10T-N & \cdots & 2T & 4T & 6T & \cdots & 8T-N & 6T-N & 4T-N   \\
    4T-N & 6T-N & 8T-N & \cdots &  0 & 2T & 4T & \cdots & 6T-N  & 4T-N & 2T-N   \\
    2T-N & 4T-N & 6T-N & \cdots & -2T & 0 & 2T & \cdots & N-4T  & N-2T & N
    \end{pmatrix}\\
    \end{aligned}
\end{equation}

which has inverse

\begin{equation}
    \setcounter{MaxMatrixCols}{20}
\begin{aligned}
     (\Tilde{I}^T A^T A \Tilde{I})^{-1} &= \frac{1}{4T}
    \begin{pmatrix}
         2 & -1 & 0 & 0 & 0 & \cdots & 0 &  0 &1 \\
        -1 & 2 & -1 & 0 & 0 & \cdots & 0 & 0 & 0 \\
        0 & -1 & 2 & -1 &  0 & \cdots & 0 & 0 & 0\\
        0 & 0 & -1 & 2 &  -1 & \cdots & 0 & 0 & 0\\
        \vdots & \vdots &\vdots &\vdots &\vdots  &\ddots & \vdots & \vdots & \vdots \\
        0 & 0 & 0 & 0  & 0 & \cdots & -1 & 2 & -1 \\
        1 & 0 & 0 & 0  & 0 & \cdots & 0 & -1 & 2 \\
    \end{pmatrix}.\\ 
\end{aligned}
\end{equation}



%Not on diagonal: $-(N-jT) + 2(N-(j+2)T) - (N-(j+4)T) = jT -2(j+2)T +(j+4)T = jT - 2jT -4T +jT + 4T = 0$. 


So 

\begin{equation}
    \begin{aligned}
         (\Tilde{I}^T A^T A \Tilde{I})^{-1}\mathbf{1} &= \frac{1}{2T}
         \begin{pmatrix}
             1 \\
             0 \\
             \vdots \\
             0 \\
             1
         \end{pmatrix}
         & \geq \mathbf{0}
    \end{aligned}
\end{equation}

So for large enough $\beta \leq \beta_c$ in the critical zone,

\begin{equation}\label{2lyr_z_betac}
    z = (\beta_c - \beta)(\Tilde{I}^T A^T A \Tilde{I})^{-1}\mathbf{1} = \frac{(\beta_c - \beta)}{2T}
         \begin{pmatrix}
             1 \\
             0 \\
             \vdots \\
             0 \\
             1
         \end{pmatrix}
\end{equation}

Since the data is sorted in descending order $x_1 > x_2 > \cdots > x_N$ by assumption \ref{}, the dictionary matrix $A \in \{-1,1\}^{N \times N}$ is of the form 

\begin{equation}
A = 
    \begin{pmatrix}
    1 & 1 & 1 & 1 &\cdots & 1 & 1 \\
    -1 & 1 & 1 & 1 &\cdots & 1 & 1 \\
    -1 & -1 & 1 & 1 &\cdots & 1 & 1 \\
    -1 & -1 & -1 & 1 &\cdots & 1 & 1 \\
    -1 & -1 & -1 & -1 &\cdots & 1 & 1 \\
     \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
    -1 & -1 & -1 & -1 &\cdots & -1 & 1 
    \end{pmatrix}.
\end{equation}



Note
\begin{align*}
(\Tilde{A}^T\Tilde{A})^{-1}\mathbf{1}&=( \Tilde{I}^T A^T A  \Tilde{I})^{-1} \mathbf{1} 
\end{align*}


%where we used that for all columns $a_j$ in $\Tilde{A}$, $a_j^Ty = \beta_c = T$, and if $\beta > \beta_c$ then the optimal solution is $z=0$.

%Note $Az = \frac{1}{2T}(\tilde{a}_1 + \tilde{a}_k)$.

Now, suppose $\beta \in [\frac{T}{2},T]$. We evaluate $ A^T(Az-y) + \beta \partial g(z)$ with $z$ such that $z_j=\tilde{z}_j$ for $j=\frac{T}{2}+1\mod T$ and inserted into $z_j=0$ otherwise. 
Let $a_j$ be the column $j$ of $A$.





So 

\begin{equation}
   \begin{aligned}
       |(Az-y)_j| =\begin{cases}
        1-\frac{(\beta_c - \beta)_+}{T} &\mbox{if} j \leq \frac{T}{2}\\
        1&\mbox{if} j \in [\frac{T}{2}+1,N-\frac{T}{2}]\\
         1-\frac{(\beta_c - \beta)_+}{T}&\mbox{if} j > N-\frac{T}{2} \\
    \end{cases} 
\end{aligned} 
\end{equation}



    



So

\begin{align*}
    (A^T(Az-y) + \beta \partial g(z))_j &= (A^T(Az-y))_j +\beta \partial g(z)_j \\
    &= a_j^T (Az-y) + \beta\partial g(z)_j \\
    &= a_j^T (\frac{1}{2T}(\beta_c - \beta)_+(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})-y) + \beta \partial g(z)_j \\
     &= a_j^T (\frac{1}{2T}(\beta_c - \beta)_+(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})) - a_j^T y + \beta \partial g(z)_j \\
   % &= a_j^T (\frac{1}{2T}(\beta_c - \beta)_+(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})) - \beta_c + \beta \partial g(z)_j \\
\end{align*}

If $j \in \{\frac{T}{2}, N- \frac{T}{2}\}$, then 

\begin{equation}
    a_{\frac{T}{2}}^T a_{N-\frac{T}{2}} = \frac{T}{2} + \frac{T}{2} - (N-T) = 2T-N
\end{equation}

and  $z_j>0$ and $a_j^T y = \beta_c$, so

\begin{align*}
    (A^T(Az-y) + \beta \partial g(z))_j 
    &= (\frac{1}{2T}(\beta_c - \beta)_+(N+  a_{\frac{T}{2}}^T a_{N-\frac{T}{2}}))   -\beta_c + \beta  \\
      &= (\frac{1}{2T}(\beta_c - \beta)_+(N+ 2T-N) - \beta_c  + \beta \\
      &= \frac{1}{2T}(\beta_c - \beta)_+(2T) - \beta_c  + \beta \\
      &= 0 \mbox{ if } \beta < \beta_c 
\end{align*}

By remark \ref{remark:2lyr_pred_betac},  for all columns $a_j$ of $A$, $|a_j^T(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})|$ is maximized if $(a_j)_k = 1$ at the $\frac{T}{2}$ indices $k$ when  $(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})_k=2$, and $(a_j)_k = -1$ at the $\frac{T}{2}$ indices indices when $(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})_k=-2$. Therefore $|a_j^T(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})|\leq \frac{T}{2}(2)(1) + \frac{T}{2}(-2)(-1) + (N-T)(0) =2T$. So $\frac{1}{2T}(\beta_c - \beta)_+(a_j^T(a_{\frac{T}{2}} + a_{N-\frac{T}{2}}) \in (\beta_c - \beta)_+[-1, 1] = [\beta_c - \beta, \beta - \beta_c]$. Also, for any column $a_j$ of $A$, $-\beta_c \leq a_j^T y \leq \beta_c$.

So for $j \notin \{\frac{T}{2},N-\frac{T}{2}\}$ we have $z_j=0$ so 

\begin{align*}
    (A^T(Az-y) + \beta \partial g(z))_j 
    &= \frac{1}{2T}(\beta_c - \beta)_+(a_j^T(a_{\frac{T}{2}} + a_{N-\frac{T}{2}}   -a_j^Ty + \beta[-1,1]  \\
      &= \frac{1}{2T}(\beta_c - \beta)_+(a_j^T(a_{\frac{T}{2}} + a_{N-\frac{T}{2}}) + [-\beta-a_j^Ty, \beta - a_j^Ty]\\
      & \supset [(\beta -\beta_c) + -\beta+\beta_c, (\beta_c - \beta) + \beta - \beta_c] \\
      & \supset \{0\}
\end{align*}

as desired.

So $\mathbf{0} \in A^T(Az-y) + \beta \partial g(z)$.

If $z_j=0$, 

\begin{align*}
    (A^T(Az-y))_j &= a_j^T (Az-y) \\
    &= a_j^T (\frac{1}{2T}(\beta_c - \beta)_+(a_{\frac{T}{2}} + a_{N-\frac{T}{2}})-y)  \\
     &= \frac{1}{2T}(\beta_c - \beta)_+ a_j^T(a_{\frac{T}{2}} + a_{N-\frac{T}{2}}) - a_j^T y \\
     & \in [-\frac{2T}{2T}(\beta_c - \beta)_+-\beta_c, \frac{2T}{2T}(\beta_c - \beta)_+ +\beta_c]
  \end{align*}



\textcolor{red}{If $\beta<\beta_c$ is too small, what breaks?}


\textcolor{red}{TODO: fix $A^TA$ for noncritical $\beta$ derivation}


We get exactly the two endpoints.

\section{initial specific work }



\section{Convex neural network approximation}
Consider the regularized training problem to
\begin{equation}\label{equ:p0}
\begin{aligned}
    \inf_{w,b,\alpha} &\frac{1}{2}\sum_{n=1}^N \norm{\sum_{i=1}^m\alpha_i\sigma(w_i^Tx_n+b_i)-y_n}_2^2\\
    &+\frac{\beta}{2}\sum_{i=1}^m(|\alpha_i|^{\theta}+|w_i|^{\theta}).
\end{aligned}
\end{equation}
Here $\sigma(z)$ is the activation function and $\beta>0$ is a regularization parameter. Possible choice of $\sigma$ include $\sigma(z)=|z|$ and $\sigma(z)=z_+$. We assume that $\sigma(z)$ is degree-$p$ homogeneous, i.e., 
$$
\sigma(c z)= c^p z,
$$
for all $c>0$. 
By properly rescaling the parameters, we can reformulate \eqref{equ:p0} as follows.
\begin{proposition}
Suppose that $\theta=\theta(p)$. The regularized problem \eqref{equ:p0} is equivalent to
\begin{equation}\label{equ:p}
\begin{aligned}
    \inf_{w,b,\alpha} &\frac{1}{2}\sum_{n=1}^N \norm{\sum_{i=1}^m\alpha_i\sigma (w_i^Tx_n+b_i)-y_n}_2^2\\
    &+ \tilde \beta\|\alpha\|_1,
    \text{ s.t. }\|w_i\|_2\leq 1, i\in[m],
\end{aligned}
\end{equation}
where $\tilde \beta=c(\theta)\beta$. 
\end{proposition}
\begin{proof}
Let $\zeta\in \mbR^n$ satisfying $\zeta_i>0$. Consider
\begin{equation}
    w_i'=\zeta_i w_i, b_i'=\zeta_i b_i, \alpha_i'=\zeta_i^{-p}\alpha_i.
\end{equation}
We note that 
$$
\sum_{i=1}^m\alpha_i'\sigma ((w_i')^Tx_n+b_i')=\sum_{i=1}^m\alpha_i\sigma (w_i^Tx_n+b_i).
$$
We can compute that
\begin{equation}
\begin{aligned}
&\sum_{i=1}^m(|\alpha_i'|^{\theta}+|w_i'|^{\theta})\\
=&\sum_{i=1}^m(\zeta_i^{-p\theta}|\alpha_i|^{\theta}+\zeta_i^{\theta}|w_i|^{\theta})\\
=&\sum_{i=1}^m
\end{aligned}
\end{equation}
\end{proof}
Let $z_n=\sum_{i=1}^m\alpha_i\sigma(w_i^Tx_n+b_i)$.  Denote $X=x_{1:n}$, $Y=y_{1:n}$ and $Z=z_{1:n}$. Then, we can rewrite \eqref{equ:p} as
\begin{equation}\label{equ:p_repeat}
\begin{aligned}
    \inf_{w,b,\alpha} &\;\frac{1}{2}\|Z-Y\|_F^2+\tilde \beta\|\alpha\|_1,\\
    \text{ s.t. }& z_n=\sum_{i=1}^m\alpha_i\sigma(w_i^Tx_n+b_i),n\in[N]\\
    & \|w_i\|_2 = 1, i\in[m].
\end{aligned}
\end{equation}
We derive the dual problem of \eqref{equ:p} as follows.
\begin{proposition}
The dual problem of \eqref{equ:p} writes
\begin{equation}\label{equ:d}
\begin{aligned}
\max_\lambda&-\frac{1}{2}\|\lambda+y\|_2^2, \\
\text{ s.t. }&\max_{w,b:\|w\|_2= 1} |\lambda^T\sigma(Xw+b)|\leq  \tilde \beta.
\end{aligned}
\end{equation}

\end{proposition}


\begin{proposition}
Suppose that $\sigma(z)=|z|$ or $\sigma(z)=(z)_+$. The dual problem \eqref{equ:d} is equivalent to
\begin{equation}\label{equ:d_simple}
\begin{aligned}
\max_\Lambda&-\frac{1}{2}\|\Lambda+Y\|_2^2,\\
\text{ s.t. } &|\lambda^T\sigma(X-x_n\bone)|\leq  \frac{\tilde \beta}{2},n\in[N],\\
&|\lambda^T\sigma(x_n\bone-X)|\leq  \frac{\tilde \beta}{2},n\in[N],\\
&\lambda^T\bone = 0.
\end{aligned}
\end{equation}
% Here $x_{\pi(1)}< x_{\pi(2)}<\dots<x_{\pi(n)}$ be the re-ordering of $\{x_i\}_{i=1}^n$ and 
\end{proposition}

\begin{proposition}\label{prop:bd}
Suppose that $\sigma(z)=|z|$. The bi-dual problem follows
\begin{equation}\label{equ:bd}
\begin{aligned}
   \min_{z,\xi} \frac{1}{2} \norm{Y-Az+\xi \bone}_2^2-\frac{1}{2}\|Y\|_2^2+\beta\sum_{n=1}^N\|z\|_1,
\end{aligned}
\end{equation}
where $A\in\mbR^{n\times n}$ is defined by $A_{i,j}=|x_i-x_j|$. 
\end{proposition}
\begin{proof}
Consider the Lagrangian function
\begin{equation} \label{equ:Lag}
\begin{aligned}
&L(\Lambda,z_{0}, z_1,\xi) \\
=&\frac{1}{2}\norm{\Lambda+Y}_2^2-\sum_{n=1}^Nz_{0,n}\pp{\lambda^T(X-x_n\bone)_+-\beta}\\
&-\sum_{n=1}^Nz_{1,n}\pp{\lambda^T(x_n\bone-X)_+-\beta}+\xi\Lambda^T\bone\\
=&\frac{1}{2}\norm{\Lambda+Y}_2^2+\xi\Lambda^T\bone+\beta\sum_{n=1}^N(z_{0,n}+z_{1,n})\\
&-\sum_{n=1}^Nz_{0,n}\lambda^T(X-x_n\bone)_+-\sum_{n=1}^Nz_{1,n}\lambda^T(X-x_n\bone)_+\\
=&\frac{1}{2}\norm{\Lambda+Y}_2^2+\xi\Lambda^T\bone+\frac{\tilde \beta}{2}\sum_{n=1}^N(z_{0,n}+z_{1,n})\\
&-\lambda_n^T\sum_{n=1}^N \pp{z_{0,n}(X-x_n\bone)_++z_{1,n}(x_n\bone-X)_+}\\
\end{aligned}
\end{equation}
Here $z_{0},z_{1},z\in\mbR^n$. The dual function writes 
\begin{equation}
\begin{aligned}
    &-\min_{\Lambda} L(\Lambda,z,\xi) \\\\
    =&\frac{1}{2} \norm{Y-\sum_{n=1}^N\pp{z_{0,n}(X-x_n\bone)_++z_{1,n}(x_n\bone-X)_+}+\xi \bone}_2^2-\frac{1}{2}\|Y\|_2^2+\beta\sum_{n=1}^N\|z\|_1
\end{aligned}
\end{equation}
This completes the proof.
\end{proof}

The following proposition gives the mapping of a bidual solution to a primal solution. A direct corollary is that the strong duality holds, i.e., $P=D$. 
\begin{proposition}\label{prop:bidual_to_primal}
Let $A\in\mbR^{N\times N}$ defined by $A_{i,j}=|x_i-x_j|$. Suppose that we have $z\in\mbR^N$, $\xi \in \mathbf{R}$. Let $m^* = ||z||_0$. If the number of neurons in the primal non-convex problem satisfies $m \geq m^*$ then we can construct a network as defined $f_\theta$ in the primal with $\sigma(z)=|z|$ to satisfy that $f_\theta(X)=Az+\xi$.
\end{proposition}
\begin{proof}
Consider the following neural network. Let $w_n=1$ and $b_n=-x_n$. Then, we consider
\begin{equation}
    f_\theta(X)=\sum_{n=1}^{N} z_n|w_nX+b_n|+\xi
\end{equation}
Then, we have $f_\theta(X)=Az+\xi$. 
\end{proof}

\begin{proposition}
Suppose that $\sigma(z)=|z|$. The bi-dual problem writes
\begin{equation}
\begin{aligned}
\min_{u_i,u_i',b_i,b_i'}& \norm{\sum_{i=1}^p D_i(X(u_i-u_i')+b_i-b_i')-y}_2^2+\tilde{\beta}\sum_{i=1}^p(\|u_i\|_2+\|u_i'\|_2),\\
\text{ s.t. }& D_i(Xu_i+b_i\bone)\geq 0, D_i(Xu_i'+b_i'\bone)\geq 0,
\end{aligned}
\end{equation}
where $D_1,\dots,D_p$ are the enumeration of $\{\diag(\mathrm{sign}(Xu))|u\in\mbR^n\}$.
\end{proposition}

\begin{theorem}
Suppose that $\sigma(z)=|z|$. Suppose that the neural network has at most $m$ neurons. Then, the primal problem is equivalent to 
\begin{equation}
\begin{aligned}
\min_{u_i,u_i'}& \norm{\sum_{i=1}^p D_i(X(u_i-u_i')+b_i-b_i')-y}_2^2+\tilde{\beta}\sum_{i=1}^p(\|u_i\|_2+\|u_i'\|_2),\\
\text{ s.t. }& D_i(Xu_i+b_i\bone)\geq 0, D_i(Xu_i'+b_i'\bone)\geq 0,\\
&\|\bmbm{U&b}\|_0+\|\bmbm{U'&b'}\|_0\leq 1,
\end{aligned}
\end{equation}
It is also equivalent to
\begin{equation}
    \min_{z,\xi} \frac{1}{2} \norm{Y-Az+\xi \bone}_2^2-\frac{1}{2}\|Y\|_2^2+\beta\sum_{n=1}^N\|z\|_1,\text{ s.t. } \norm{\bmbm{z\\\xi}}_0\leq m
\end{equation}
\end{theorem}


If the activation $\sigma(z)$ is symmetric, for example absolute value $\sigma(z)=|z|$, then we can set $A=A_+ \in \mathbf{R}^{N \times N}$. If $A$ is full rank then the objective in \eqref{equ:bd} is strictly convex, so there is a unique solution. When the regularizer $\beta \to 0$, and there are enough neurons $m \geq m^*$ or the number of neurons is unconstrained, the primal problem becomes 

\begin{equation}\label{eq:absval_beta0}
    \min_{z,\xi} \frac{1}{2} \norm{Y-Az+\xi \bone}_2^2
\end{equation}

Let $\Bar{A} $  be the sum of the rows of $A$ and $\Bar{Y}=\sum_{i=1}^N y_i$. Let $\tilde{A}=A-\Bar{A},\tilde{Y}=Y-\Bar{Y} $.
Then if $\Tilde{A}$ is full rank, \eqref{eq:absval_beta0} has the unique bidual solution $z^* = \Tilde{A}^{-1}\tilde{Y}, \xi^* = \Tilde{Y}-\Tilde{A}z^*$.

\iftoggle{todos}{
\textcolor{red}{todo: simulations}
    }
\section{ideas}


-Should $(\cdot)_+$ be $ |\cdot|$ in proof of equation \ref{equ:bd}?

-For general piecewise linear $\sigma(z)$, equation \ref{equ:bd} holds with $A_{i,j} = \sigma(x_i-x_j)$ and $\sigma(\cdot)$ instead of $(\cdot)_+$ and $A_0z_0+A_1 z_1$

-Simpler to remove $||Y||^2_2$ in equation \ref{equ:bd}? (just style)

-Prop \ref{prop:bidual_to_primal} holds with $|\cdot|$ replaced by general $\sigma(\cdot)$



\section{2-layer leaky Relu}

Since $\sigma(z)$ is degree-p homogenous, the sign of $\sigma(b+x_i)$ and its derivative depends only on the sign of $b+x_i$ \textbf{red}{(todo: show)}. So if $\sigma(z)$ is piecewise linear, $\sigma(b \pm x_i)$ only has two linear pieces, with a kink when $b \pm x_i=0$. So $\lambda^T \sigma(b-X)$ is piecewise linear and only has kinks when $b \pm x_i=0$ for $i \in [n]$. And when $\lambda^T X^j=0$ for $j \in \{0, \dots, p-1\}$, there is a finite optimum $\max_{b} |\lambda^T \sigma(b \pm X)| < \infty$, and so these kinks are the only possible maximizers of $|\lambda^T \sigma(b \pm X)| $. Therefore problem \ref{equ:d_simple} holds when $\sigma(z)$ is piecewise linear. $\sigma(z)$ is piecewise linear for example when $\sigma(z) = z_+$ or $|z|$ or leaky Relu. 

Suppose the activation function is a leaky Relu. For some $a, b \in \mathbf{R}$

\begin{equation}
\begin{aligned}
      \sigma(z) &= 
    \begin{cases}
        az \mbox{ if } z > 0 \\
        cz \mbox{ else }
    \end{cases} \\
      &= (a\mathbf{1}_{z>0}+c\mathbf{1}_{z<0})z
\end{aligned}
\end{equation}

When $a=0,b=1$, the activation function is Relu $\sigma(z) = z_+$. When $a=1,b=-1$, the activation function is absolute value $\sigma(z) = |z|$. When $0<b<a$ the activation function is the sterotypical leaky Relu. So from the above discussion, piecewise linear is equivalent to leaky Relu, but we exclude $c=0$ with Relu below for analysis.

\begin{proposition}\label{prop:bd_gen}
For general piecewise linear activation $\sigma$, the bi-dual problem follows
\begin{equation}\label{equ:bd_gen}
\begin{aligned}
   \min_{z_0, z_1 \in \mathbf{R^{\geq 0}}^n, \xi \in \mathbf{R}} \frac{1}{2} \norm{Y-A_0 z_0 -A_1 z_1 +\xi \bone}_2^2-\frac{1}{2}\|Y\|_2^2+\beta\sum_{n=1}^N\|z_0\|_1+\|z_1\|_1,
\end{aligned}
\end{equation}
where $A_0, A_1 \in\mbR^{n\times n}$ are defined by ${A_0}_{i,j}= a(x_i-x_j)\mathbf{1}\{(x_i-x_j)\}$, ${A_1}_{i,j}= -c(x_i-x_j)\mathbf{1}\{(x_j-x_i)\}$. 
\end{proposition}

Proof is almost same as for proposition \ref{prop:bd_gen}.

Change variables $\tilde{z}_0 = a z_0, \tilde{z}_1 = -c z_1$. 

Assume samples are ordered $x_1 \leq \dots \leq x_n$. Let $A$ be a $n \times 2n$ matrix of nonnegative entries where 

\begin{equation}
A_{i,j}=
    \begin{cases}
        x_i - x_j \mbox{ if } i \leq j \leq n \\
        x_j - x_{i-n} \mbox{ if } n < j < i+n \\
        0 \mbox{ else }
    \end{cases}
\end{equation}


So the matrix $A$ has horizontal bands sliding to the down and right. In other words, $A$ took the matrix with $i,j$ element $x_i - x_j$, and shifted the bottom left triangle horizontally to the right of the top right triangle. 

Let $\Tilde{z} = [\tilde{z_1}, \tilde{z_0}]^T$ be the $2n$ vector where $\tilde{z_1},\tilde{z_0}$ are vertically stacked on top of each other. Let $D$ be a matrix whose first $n$ diagonal elements are $\frac{1}{|c|}$ and last $n$ are $\frac{1}{|a|}$. Then the primal is equivalent to

\begin{equation}
\begin{aligned}
   \min_{z \in \mathbf{R}^{2n}, \xi \in \mathbf{R}} \frac{1}{2} \norm{Y-A z +\xi \bone}_2^2-\frac{1}{2}\|Y\|_2^2+\beta || D z ||_1 \\
\end{aligned}    
\end{equation}


%\textbf{Remark}

%If $\beta \xrightarrow[]{} 0$ then we can merge $z_0+z_1 = z$ which is either nonnegative or unconstrained. The optimal bidual variables will be the same for any leaky Relu activation with the same sign of $c$ and $a$:

%\begin{equation}
%\begin{aligned}
%   \min_{z \in \mathbf{R}^n, \xi \in \mathbf{R}} \frac{1}{2} \norm{Y-A z +\xi \bone}_2^2 \\
%\end{aligned}    
%\end{equation}

%which can be solved analytically.


\section{2-layer NN with threshold activation}

Suppose the activation is a threshold activation: $\sigma_s(z) = s \mathbf{1}\{ z \geq 0 \}$ and the training problem is 


\begin{equation}
\label{equ:psign}
\begin{aligned}
   \min_{w, b, s, \alpha} \frac{1}{2} \sum_{n=1}^N || \sum_{i=1}^m \alpha_i \sigma_{s_i}(w_i^Tx_n+b_i) - y_n||^2_2 + \beta/2 \sum_{i=1}^m ( {w_i}_2^2 + s_i^2 + \alpha_i^2)
\end{aligned}
\end{equation}

Then $\sigma_s(cz) = s \mathbf{1}\{ cz \geq 0 \} = \sigma_s(z) $ is not degree-$p$ homogenous. However, we have a similar proposition and proof as equation \ref{equ:p}.

\begin{proposition}\label{prop:sign_thresh_scaled}
%Suppose that $\theta=\theta(p)$. 
The regularized problem \eqref{equ:psign} is equivalent to
\begin{equation}\label{equ:psignscaled}
\begin{aligned}
    \inf_{w :w_i =\pm 1,b,\alpha \in \mathbf{R}^m} &\frac{1}{2}\sum_{n=1}^N \norm{\sum_{i=1}^m\alpha_i \sigma_{s=1} (w_i^Tx_n+b_i)-y_n}_2^2 +  \beta\|\alpha\|_1
\end{aligned}
\end{equation}
%where $\tilde \beta=c(\theta)\beta$. 
\end{proposition}

\begin{proof}

Note $\sigma_{s_i}(w_i^Tx_n+b_i)=\sigma_{s_i}(\frac{w_i}{||w_i||_2}^Tx_n+\frac{b_i}{||w_i||_2})$ in the loss function takes only two values (namely in $\{0,s_i\}$, although the actual values do not matter) neither of which depends on $||w_i||_2$. Also $b_i$  is not regularized, so can be changed to a new rescaled variable without affecting the problem. So the regularization penalty $||w||^2_2$ will be made zero. So problem \eqref{equ:psign} is equivalent to

\begin{equation}
\label{equ:psign_no_wreg}
\begin{aligned}
   \min_{w, b, s, \alpha} \frac{1}{2} \sum_{n=1}^N || \sum_{i=1}^m \alpha_i \sigma_{s_i}(w_i^Tx_n+b_i) - y_n||^2_2 + \beta/2 \sum_{i=1}^m ( s_i^2 + \alpha_i^2).
\end{aligned}
\end{equation}

Let

\begin{equation}
\label{equ:psign'mult}
\begin{aligned}
   \min_{w, b, s', \alpha'} \frac{1}{2} \sum_{n=1}^N || \sum_{i=1}^m \alpha'_i \sigma_{s_i'}(w_i^Tx_n+b_i) - y_n||^2_2 + \beta \sum_{i=1}^m |s'_i||\alpha'_i| \end{aligned}
\end{equation}

be problem \eqref{equ:psign_no_wreg} with a multiplicative instead of additive regularization. Since $ s_i^2 + \alpha_i^2 \geq 2|s_i| |\alpha_i|$, the problem values satisfy $ \eqref{equ:psign_no_wreg} \geq\eqref{equ:psign'mult} $. On the other hand, for any solution $s', \alpha', w', b'$ and cooresponding value of problem \eqref{equ:psign'mult}, problem \eqref{equ:psign_no_wreg} can achieve an equal (as good as) value by setting $\zeta_i = \sqrt{|\frac{\alpha_i'}{s_i'}|},  s_i=\zeta_i^{-1} s_i',  \alpha_i=\zeta_i \alpha_i', w=w', b=b'$. This is because $s_i \alpha_i = s_i' \alpha_i'$ so the loss function is unchanged and $ (\zeta^{-1} s_i)^2 + (\zeta \alpha_i) ^2 = 2|\zeta^{-1} s_i| |\zeta \alpha_i| = |s_i| |\alpha_i|$ is so the regularization term is unchanged. So the problem values satisfy $ \eqref{equ:psign_no_wreg} \leq\eqref{equ:psign'mult} $, and hence they are equivalent.

Since $\alpha'_i$  and $s'_i$ always appear as a product in \eqref{equ:psign'mult}, changing to new variables $s_i=\frac{s_i'}{|s_i'|}, \alpha_i=\alpha_i'|s_i'|$ gives %makes $|s_i||\alpha_i|=$

\begin{equation}
\begin{aligned}
   \min_{w, b, s:|s_i|=1, \alpha} \frac{1}{2} \sum_{n=1}^N || \sum_{i=1}^m \alpha_i \sigma_{s_i}(w_i^Tx_n+b_i) - y_n||^2_2 + \beta ||\alpha||_1 \end{aligned}
\end{equation}

which is equivalent to problem \eqref{equ:psign'mult}. In other words, the weight of $s$ was reallocated to $\alpha$.

\end{proof}

As noted above, the threshold activation $\sigma_s$ does not depend on $||w_i||_2$. So may assume $||w_i||_2=1$. For 1D data, this gives

\begin{equation} 
\begin{aligned}
    \inf_{w: w_i = \pm 1,b,\alpha} &\frac{1}{2}\sum_{n=1}^N \norm{\sum_{i=1}^m\alpha_i \sigma_{s=1} \{ w_i x_n+b_i\}-y_n}_2^2 +  \beta\|\alpha\|_1
\end{aligned}
\end{equation}

ie

\begin{equation} \label{equ:thresh_primal_rewrite}
\begin{aligned}
    \inf_{w: w_i = \pm 1,b,\alpha} &\frac{1}{2} \norm{z-y}_2^2 +  \beta\|\alpha\|_1 \\
    &\mbox{such that } z_n = \sum_{i=1}^m\alpha_i \sigma_{s=1} \{ w_i x_n+b_i\}, n \in [N]
\end{aligned}
\end{equation}

which is the same as the primal problem \ref{equ:p} and hence has the same dual as equation \ref{equ:d} but with activation being threshold $\sigma(z) = \mathbf{1}\{z\}=\sigma_{s=1}(z)$, and $\tilde{\beta}=\beta$. Note that deriving the dual depended on $\alpha$ being a L1 penalty in the objective and linear in the constraint, and did not depend on the specific form of $\sigma(z)$; the Lagrangian was minimized nontrivially when $\alpha=0$, regardless of $w,b$.

For fixed $w_i \in \{-1,1\}$, the finite piecewise linear function  $\sum_{i=1}^m\alpha_i \sigma_{s=1} \{ w_i x_n+b_i\}$ with threshold activation $\sigma_{s=1}$ is maximized over $b_i$ at its transition points or kinks when $w_i x_n + b_i =0$. (ie, the subgradient can only be zero at these kinks, since everywhere else, the subgradient is just the linear slope $\sum_{i=1}^j \alpha_i$ unless that slope is zero, in which case the adjacent kink suffices). Plugging this in to the dual problem \ref{equ:d} gives the following.

\begin{proposition}\label{prop:sign_thresh_dual}
Suppose that $\sigma(z)= s \mathbf{1}\{z\geq 0\}$. The dual problem \eqref{equ:d} is equivalent to
\begin{equation}\label{equ:d_simple_sign}
\begin{aligned}
\max_\Lambda&-\frac{1}{2}\|\Lambda+Y\|_2^2,\\
\text{ s.t. } &|\lambda^T\mathbf{1}\{X-x_n\bone\}|\leq  \beta,n\in[N],\\
&|\lambda^T \mathbf{1}\{x_n\bone-X\}|\leq  \beta ,n\in[N] %other prob should also just be beta not beta/2?
\end{aligned}
\end{equation}
% Here $x_{\pi(1)}< x_{\pi(2)}<\dots<x_{\pi(n)}$ be the re-ordering of $\{x_i\}_{i=1}^n$ and 
\end{proposition}

Note that unlike equation \ref{equ:d_simple} where the activation $\sigma(z)$ is unbounded over $z$, we don't need $\lambda^T\bone = 0$ because $\sigma(w_ix_n+b_i)=\mathbf{1}\{w_ix_n+b_i\} \in \{0,1\}$.

Suppose the samples are ordered $x_1 \leq ... x_n \leq ... x_N$.
For every $n \in [N]$, $x_i - x_n \geq 0$ iff $i \geq n$, and $x_n - x_i \geq 0$ iff $n \geq i$. So $\lambda^T\mathbf{1}\{X-x_n\bone\} = \sum_{i=n}^N \lambda_i$ and $\lambda^T \mathbf{1}\{x_n\bone-X\}= \sum_{i=1}^{n} \lambda_i$. %overlap at n

So,

\begin{proposition} \label{prop:sign_thresh_dual2}
Suppose that $\sigma(z)= s \mathbf{1}\{z\geq 0\}$. The dual problem \eqref{equ:d} is equivalent to
\begin{equation}\label{equ:d_simple_sign_repeat}
\begin{aligned}
\max_\Lambda&-\frac{1}{2}\|\Lambda+Y\|_2^2,\\
\text{ s.t. } &
|\sum_{i=1}^n \lambda_i| \leq \beta, n \in [N]\\
&|\sum_{i=n}^N \lambda_i| \leq \beta, n \in [N]
\end{aligned}
\end{equation}
% Here $x_{\pi(1)}< x_{\pi(2)}<\dots<x_{\pi(n)}$ be the re-ordering of $\{x_i\}_{i=1}^n$ and 
\end{proposition}

Proposition \ref{prop:bd} and its proof still follows, except there is no $\lambda^T \mathbf{1}=0$ constraint, so that there is no $\xi$ and hence no  bias term in the bidual. (Also, replace absolute value activation with the appropriate activation $\sigma(z) = \mathbf{1}\{z\}$.) And since the activation $\sigma(z) = \mathbf{1}\{z\}$ is not symmetric, the two dual variable vectors $z_0, z_1$ remain, corresponding to coefficients in matrices $A_0$ and $A_1$ as follows.

\begin{proposition}\label{prop:bd_sign}
Suppose that $\sigma(z)=s \mathbf{1}(z)$. The bi-dual problem follows
\begin{equation}\label{equ:bd_sign}
\begin{aligned}
   \min_{z_0, z_1 \in \mathbf{R}^n} \frac{1}{2} \norm{Y-A_0 z_0 + A_1 z_1}_2^2-\frac{1}{2}\|Y\|_2^2+\beta\sum_{n=1}^N\|z\|_1,
\end{aligned}
\end{equation}
where $A_0, A_1 \in\mbR^{n\times n}$ is defined by ${A_0}_{i,j}= \mathbf{1}\{x_i-x_j\}, {A_1}_{i,j}= \mathbf{1}\{x_j-x_i\}$. 
\end{proposition}

If the samples are ordered in ascending order $x_1 \leq \dots x_n \leq \dots x_N$ then $A_1$ is an upper right triangular matrix of ones, and $A_0$ is a bottom left triangular matrix of ones. 

Let $A = [A_1 A_0]$ be a $n \times 2n$ matrix with $A_1$ and $A_0$ horizontally stacked next to each other. $A$ consists of $n$ horizontal bands of $n+1$ ones along the diagonal. Let $z = [z_1 z_0]$ be a $2n$ vector where $z_1,z_0$ are vertically stacked on top of each other. Problem \ref{equ:bd_sign} is

\begin{equation}
\begin{aligned}
   \min_{z \in \mathbf{R}^{2n}} \frac{1}{2} \norm{Y-Az}_2^2-\frac{1}{2}\|Y\|_2^2+\beta||z||_1,
\end{aligned}
\end{equation}

\subsection{Minimal weight regularization with threshold activation} 

\iftoggle{todos}{
\textcolor{red}{todo: go through, check and rewrite nicer}
}

When $\beta \to 0$, the optimal solution converges to the lowest L1 norm solution to minimizing $||Y-Az||^2_2$, ie the solution to

\begin{equation} \label{equ:thresh_beta=0}
\begin{aligned}
   \min_{z \in \mathbf{R}^{2n}} ||z||_1, \mbox{ such that } Az=Y
\end{aligned}
\end{equation}

There are $n$ equations and $2n$ variables in $Az=y$. Suppose we know $n$ free variables $ z_{n+1},\dots,z_{2n}$. Then the last row of $Az=Y$ gives $\sum_{i=0}^n z_{i+n} = y_n$, so $z_n = y_n - \sum_{i=1}^n z_{i+n}$. The second to last row of $Az=Y$ gives $z_{n-1} = y_{n-1} - \sum_{i=0}^{n-1} z_{i+n} = y_{n-1} - (\sum_{i=0}^{n} z_{i+n} - z_{2n}) = y_{n-1} - y_n + z_{2n}$. The third to last row gives $z_{n-2} = y_{n-2} - \sum_{i=0}^{n-1} z_{i+n-1} =  y_{n-2}-(\sum_{i=0}^{n} z_{i+n-1} - z_{2n-1}) = y_{n-2} - y_{n-1} + z_{2n-1}$. Repeating, for $i \in [n-1]$ we get $z_i=y_i - y_{i+1} + z_{2n-i}$. So the total L1 penalty is $||z||_1 = \sum_{i=1}^{n} |z_n| + \sum_{i=n+1}^{2n} |z_n| = \sum_{i=1}^{n-1} |y_i - y_{i+1} + z_{2n-i}| + |y_n - \sum_{i=n+1}^{2n} z_i| +  \sum_{i=n+1}^{2n} |z_i| = \sum_{i=n+1}^{2n-1} |y_{2n-i} - y_{2n+1-i} + z_{i}| + |y_n - \sum_{i=n+1}^{2n} z_i| + \sum_{i=n+1}^{2n} |z_i| $. The optimal $z_{n+1},\dots, z_{2n}$ will be those that minimize this quantity: 

\begin{equation}
    ||z||_1 = \sum_{i=n+1}^{2n-1} |y_{2n-i} - y_{2n+1-i} + z_{i}| + |y_n - \sum_{i=n+1}^{2n} z_i| + \sum_{i=n+1}^{2n} |z_i|
\end{equation}
%$= y_1 - y_{n} +  \sum_{i=n+1}^{2n-1} |z_i| + \sum_{i=n}^{2n} z_i = y_1 - y_{n} +  z_n + z_{2n} + 2\sum_{i=n+1}^{2n-1} z_i   $ so any choice of $z_n, z_{n+1},\dots,z_{2n}$ that sum to $y_n$ is a solution to the unregularized $\beta=0$ problem. 

For $i \in \{n+1, \dots, 2n\}$, let $d_i = y_{2n-i}-y_{2n+1-i}$, $r_i = z_{i}$, $a = y_n$, $f(r)=\sum_{i=n+1}^{2n-1} |d_i + r_{i}| + |a - \sum_{i=n+1}^{2n} r_i| + \sum_{i=n+1}^{2n} |r_i| = ||z||_1$ which is convex in $r$. So we want $\textrm{argmin}_{r \in \mathbf{R}^n} f(r)$. 

The subgradient of $f(r)$ in each coordinate is

\begin{equation}
    \delta_{r_i} f(r) = 
    \begin{cases}
        \left \{ \mathbf{1}\{ i < 2n\} \textrm{sign}(d_i + r_i) - \textrm{sign}(a-r^T\mathbf{1}) + \textrm{sign}(r_i) \right \} \quad \mbox{ if } d_i + r_i \neq 0, a-r^T\mathbf{1} \neq 0, r_i \neq 0 \\
        %[-1,1]   - \textrm{sign}(a-r^T\mathbf{1}) + \textrm{sign}(r_i) \quad \mbox{ if } d_i + r_i = 0, a-r^T\mathbf{1} \neq 0, r_i \neq 0 \\
    \end{cases}
\end{equation}

and any of the $3$ terms ($\mathbf{1}\{ i < 2n\} \textrm{sign}(d_i + r_i), \textrm{sign}(a-r^T\mathbf{1})$ or $\textrm{sign}(r_i) $) is replaced by $[-1,1]$ if the corresponding function value ($d_i+r_i, a - r^T \mathbf{1}$ or $ r_i$) is $0$. Otherwise, each of the $3$ terms is $\pm 1$. So for $i < 2n$, if $d_i \neq 0$ then the subgradient $ \delta_{r_i} f(r)$ is either $\pm \{3\}, \pm\{1\}, [-1,1], [1,3]$ or $[-3,-1]$, which only contains $0$ if it is $[-1,1]$, which requires one of the three function values to be $0$ and the other two to be opposite sign. 

 For $i < n$, if $d_i = 0$ then the subgradient $ \delta_{r_i} f(r)$ is either $[1,3], [-3,-1], [-1,3]$ or $[-3,1]$, which only contains $0$ if it is the latter two, which requires $r_i=0$ and $a-r^T \mathbf{1} \neq 0$.

For coordinate $i=2n$, then the subgradient $ \delta_{r_n} f(r)$ is $\{0\}, \pm \{2\}, [0,2]$ or $ [-2,0]$ for which containing $0$ requires not being $\pm \{2\}$ which requires either $a -r^T \mathbf{1}=0$ or $r_n =0$.

The subgradient is $\delta_r f(r) = \Pi_{i=n+1}^{2n} \delta_{r_i} f(r) \subset \mathbf{R}^n$ which is $0$ at the minimizing $r$. 

Suppose $a \neq 0$. Let 

\begin{equation}
    \begin{aligned}
      I_{0} &= \{ i \in \{n+1,\dots,2n\}: d_i = 0 \}\\
      I_{1} &= \{ i \in \{n+1,\dots,2n\}: \textrm{sign}(d_i) = \textrm{sign}(a) \}\\
      I_{-1} &= \{ i \in \{n+1,\dots,2n\}: \textrm{sign}(d_i) \neq \textrm{sign}(a) \}
    \end{aligned}
\end{equation}

which partition $\{n+1,\dots,2n\}$.  If $a=0$ then use $\textrm{sign}(0)=1$ in the definitions of $I_0, I_1, I_{-1}$ above.
Note for all $i \in I_1 \cup I_{-1}$, $d_i \neq 0$.

Let 

\begin{equation}
\begin{aligned}
     (I,I')=
    \begin{cases}
        (I_{-1}, I_1) &\mbox{ if } I_1 = \emptyset \mbox{ and } a= 0\\
        (I_1, I_{-1}) &\mbox{ else }\\
        
    \end{cases}
\end{aligned}
\end{equation}

Note $I \neq \emptyset$. Set 

\begin{equation}
r_i = 
    \begin{cases}
       0 \mbox{ if } i=2n \mbox{ or } i \in I_0 \cup I' \\
       -d_i \mbox{ if } i \in I
    \end{cases}
\end{equation}

%, and if $I_1 \neq \emptyset$ then the rest of the argument follows. Otherwise all sample value gaps $d_i$ and $y_n$ have the same sign. In this case, swap the roles of $I_1$ and $I_{-1}$: set 

%\begin{equation}
%r_i = 
%    \begin{cases}
%       0 \mbox{ if } i=2n \mbox{ or } i \in I_0 \cup I_{1}\\
%       -d_i \mbox{ if } i \in I_{-1}=\{n+1,\dots,2n\} - I_1
%    \end{cases}
%\end{equation}

\textbf{Claim}: $0 \in \delta f(r)$.

\begin{proof}
    For the last coordinate $i=n$, $r_n=0$, and so $0 \in \delta_{r_n}f(r)$. So suppose $i < n$.

    Let $d=\min  I \neq 0$. 

    If $a\neq 0$ then $a$ and $d_i$ have the same sign for any $i \in I=I_1$. If $a=0$ then $I=I_{-1} \neq \emptyset$ so $a-r^T \mathbf{1} = \sum_{i \in I} d_i \neq 0$. We have $|a - r^T \mathbf{1}| =| a + \sum_{i \in I} d_i| \geq |d| > 0 $, so $a-r^T \mathbf{1} \neq 0$. In fact, $\textrm{sign}(a-r^T \mathbf{1}) = \textrm{sign}(d)  =  \textrm{sign}(d_i) = -\textrm{sign}(r_i)$ for any $i \in I$. %check again

    Suppose $i \in I$. Then we set $r_i = -d_i$, so $d_i + r_i = 0$. And since $i \notin I_0$, $0 \neq -d_i = r_i$. And $\textrm{sign}(a-r^T \mathbf{1}) = \textrm{sign}(d_i) = -\textrm{sign}(r_i)$. So $0 \in \delta_{r_n}f(r)$.

    Finally, suppose $i \in I'$. Then $r_i=0$ and $a-r^T \mathbf{1} \neq 0$. Since $i \notin I_{0}$, $0 \neq d_i = d_i + r_i $. And $\textrm{sign}(a-r^T \mathbf{1}) = \textrm{sign}(a) = -\textrm{sign}(d_i) = -\textrm{sign}(d_i+0)= -\textrm{sign}(d_i+r_i)$. So $0 \in \delta_{r_i}f(r)$.
\end{proof}

If the sign of the gap between consecutive sample values is the same as that of the last sample value, then the corresponding dual free variable is the gap between consecutive sample values, which determines the corresponding dual variable.

For $i > n$, if $i \in I$ then $z_{i}=r_i=y_{2n+1-i}-y_{2n-i}$ and for $i < n$, if $2n-i \in I$ then $z_i = y_i - y_{i+1} + z_{2n-i} = y_i - y_{i+1} + r_{2n-i} = y_i - y_{i+1} - d_{2n-i} = y_i - y_{i+1} + y_{2n+1-(2n-i)} - y_{2n-(2n-i)}= y_i - y_{i+1} + y_{1+i} - y_{i}=0$. Otherwise, the reverse situation occurs: if $i > n$ then $z_i = 0$ and for $i < n$, $z_i=y_i - y_{i+1}$ .

To summarize, the optimal $z$ when $\beta \to 0$ that solves problem \ref{equ:thresh_beta=0} is:

\begin{equation}
\begin{aligned}
 z_i = 
    \begin{cases}
        y_{2n+1-i}-y_{2n-i} \quad &\mbox{ if } i \in I  \\
        0 \quad &\mbox{ if } 2n-i \in I \mbox{ or } i \in I_0 \cup I' \mbox{ or } i=2n\\
        y_i - y_{i+1} &\mbox{ if } 2n-i \in I_0 \cup I'
    \end{cases}   
\end{aligned}
\end{equation}


\section{2 layer NN with sign activation}



Define

\begin{equation}
    \textrm{sign}(z)=
    \begin{cases}
        1 \mbox{ if } z \geq 0\\
        -1 \mbox{ else}
    \end{cases}
\end{equation}

Note that we define $\textrm{sign}(0)=1$.

\begin{lemma}
 Proposition \ref{prop:sign_thresh_scaled} holds for the sign activation $\sigma_s(z) = s \cdot \textrm{sign}(z)$.
\end{lemma}

The proof is the same as that for proposition \ref{prop:sign_thresh_scaled}, using the fact that $\sigma_s(z)$ is invariant under scaling $z$ by a positive scalar.

By the same argument as for threshold activation $\sigma_s(z)=s \mathbf{1}\{z\}$, equation \ref{equ:thresh_primal_rewrite} holds for sign activation $\sigma_s(z) = s \cdot \textrm{sign}(z)$. Also by the same argument as for threshold activation, propositions \ref{prop:sign_thresh_dual}, \ref{prop:bd_sign}  hold for $\textrm{sign}(\cdot)$ replacing the activation function $\mathbf{1}(\cdot)$. Moreover, we can make a change of variables $z'_1 = -z_1$ and then $z_{0,n}\sigma(X-x_n \mathbf{1})+z_{1,n}\sigma(x_n \mathbf{1}-X) = (z_{0,n}+z'_{1,n})\sigma(X-x_n \mathbf{1})$ in equation  \ref{equ:Lag} so that $A$ is replaced by $A_0$, and we get a result similar to proposition \ref{prop:bd}:

\begin{proposition}\label{prop:bd_sign_simp}
Suppose that $\sigma_s(z)=s \cdot \textrm{sign}(z)$. The bi-dual problem follows
\begin{equation}
\begin{aligned}
   \min_{z \in \mathbf{R}^n} \frac{1}{2} \norm{Y-Az }_2^2-\frac{1}{2}\|Y\|_2^2+\beta\sum_{n=1}^N\|z\|_1,
\end{aligned}
\end{equation}
where $A\in\mbR^{n\times n}$ is defined by $A_{i,j}= \textrm{sign}\{x_i-x_j\}$. 
\end{proposition}

$A$ is invertible, as shown in the proof of proposition \ref{prop:m_1switches} for inverting the matrix $H$. So the  objective in problem \eqref{prop:bd_sign_simp} is strictly convex and therefore admits a unique optimal solution.

\iftoggle{todos}{
\textcolor{red}{todo: make invertability its own lemma}
}

If $\beta \to 0$ and the training samples are such that $Y$ is in the span of the columns of $A$, then the neural net will converge to the minimum $L1$ norm interpolation  $z = A^{-1}y$ of the training samples. 

\section{sign activation for $L>2$ hidden layers}

We follow the same approach as \citep{wang2021parallel} %threshold nn paper
and focus on the one-dimensional data case.

Consider the neural network with $m_L$ parallel units, each consisting of $L$ hidden layers, each of which consists of $m_l$ hidden neurons. %Let $\alpha=(\alpha_1, \dots, \alpha_{m_2} )^T \in \mathbf{R}^{m_2}$ and
For parallel unit $i \in [m_L]$ and hidden layer $l \in [L]$, let $s^{(i,l)} \in \mathbf{R}^{(l)}$ and the vector-valued activation function $\sigma_{s^{(i,l)}}(z)$ be the scalar-valued activation function $\sigma_{s^{(i,l)}_j}(z_j)$ applied to each coordinate $j$ of $z$. 

Define a parallel neural network $f_L: \mathbf{R}^d \to \mathbf{R}$ by

\begin{equation}\label{parLlayernn_cpt}
\begin{aligned}
     f_L(x) &= \sum_{i=1}^{m_L} \sigma_{s^{(i,L)}} \left ( x^{(i,L-1)} W^{(i,L)} \right) \alpha_i\\
     &= \sum_{i=1}^{m_L} \sigma_{s^{(i,L)}} \left( \cdots \left( \sigma_{s^{(i,2)}}\left(\sigma_{s^{(i,1)}}\left( (x, \mathbf{1}) W^{(i,1)} \right), \mathbf{1} \right)W^{(i,2)}, \mathbf{1} \right) \cdots W^{(i,L)} \right) \alpha_i \\
    &\text{where for } i \in [m_L], l \in [L-1], s^{(i,l)} \in \mathbf{R}^l, x^{(i,l)} = \left( \sigma_{s^{(i,l)}}\left( x^{(i,l-1)} W^{(i,l)} \right) , \mathbf{1} \right) \in \mathbf{R}^{1\times (1+m_{l})}, x^{(i,0)}=(x,\mathbf{1}) \in \mathbf{R}^{d\times 2}\\
    & m_0=d, \alpha \in \mathbf{R}^{m_L}\\
    &\text{for } l \in [L-1], W^{(i,l)} \in \mathbf{R}^{1+m_{l-1}\times m_l}\\
    &\text{for } i \in [m_L], W^{(i,L)} \in \mathbf{R}^{1+m_{L-1}}
\end{aligned}
\end{equation}

As a special case, if for all layers $l \in [L-1]$ before the last layer and for all parallel units $i,j \in [m_L]$, the weight matrices and amplitude parameters satisfy $W^{(i,l)}=W^{(j,l)}=:W^{(l)}, s^{(i,l)}_i=s^{(i,l)}=:s^{(l)}$ and we let $W^{(L)}:=[W^{(1,L)},\cdots,W^{(m_L,L)}] \in \mathbf{R}^{1+m_L-1, m_L}$ then the layer outputs also satisfy $x^{(i,l)}=x^{(j,l)}=:x^{(l)}$, so if $\alpha$ is divided my $m_L$ then the parallel neural network reduces to a non-parallel version $f_L(x)=m_L \sigma_{s^{(L)}}(x^{(L-1)})W^{(L)}$. Conversely, a parallel neural network is equivalent to a standard non-parallel neural network with larger weight matrices by combining each set of weight matrices of parallel neurons as block diagonal elements of one large weight matrix for the combined neuron (see remark \eqref{remk:par_nn_to_std}).

For training data vector $X \in \mathbf{R}^{N \times d}$ consisting of $N$ samples of $d$-dimensional data, denote $f_L(X)=(f_L(x_1),\dots,f_L(x_N))^T \in \mathbf{R}^{N \times d}$ and note that in this case $X^{(0)} \in \mathbf{R}^{N \times d+1}$ is the vector $X$ with a column of ones appended. Each layer $l$ appends a column of ones to the output of the previous layer to account for the bias term in each neuron of that layer $l$.


Suppose the neural network $f_L$ is trained on the following problem generalizing \eqref{equ:psign} to $L$ hidden layers: 

\begin{equation}
\label{equ:psignLpar}
\begin{aligned}
   \min_{\alpha \in \mathbf{R}^{m_L},  W^{(i,l)} s^{(i,l)}: l \in [L], i \in [m_L] } \frac{1}{2} || f_L(X) - y||^2_2 + \beta/2 \left ( ||\alpha||^2_2  +  \sum_{i=1}^{m_L} \sum_{l=1}^L ||{W^{(i,l)}_i}_{1:m_{1-1}, 1:m_l}||^2_F
    + ||s^{(i,l)}||^2_2 \right)
\end{aligned}
\end{equation}

where $W^{(i,l)}_{1:m_{1-1}, 1:m_l}$ denotes all but the last row of $W^{(i,l)}$. The last row of $W^{(i,l)}$ which are variables corresponding to the bias terms of the neurons, which are unregularized. Only regularizing the non-bias weights is consistent with the neural network in \eqref{equ:psign} that had $L=1$ hidden layer. 

We can rescale parameters to simplify \eqref{equ:psignLpar} and change the weight penalty to $L1$. 

\begin{proposition}
    Problem \ref{equ:psignL} is equivalent to 

\begin{equation}
\label{equ:psignL_simppar}
\begin{aligned}
   \min_{\alpha \in \mathbf{R}^{m_L}, s^{(i,l)}=1, W^{(i,l)}: ||W^{(i,l)}||_F=1, i \in [m_L], l \in [L-1]} \frac{1}{2} || f_L(X) - y||^2_2 + \beta ||\alpha||_1
\end{aligned}
\end{equation}
\end{proposition}

So the amplitude parameters $s^{(i,l)}$ do not need to be trained and can just be set to $1$.

\begin{proof}
    Let $i \in [m_L], l \in [L]$. The bias variables in the last rows of $W^{(i,l)}$ are not regularized and therefore can be rescaled. For each neuron $j \in m_l$, $\sigma^{(l)}_j(z)$ is one of two values depending only on the sign of $z$, so normalizing $W^{(i,l)}_{1:m_{l-1},1:m_l}$ by $||W^{(i,l)}_{1:m_{l-1},1:m_1}||_F$ so that its Frobenuis norm is $1$ as in \eqref{equ:psignL_simppar} and making a change of variables to rescale the last row $W^{(i,l)}_{m_{l-1}+1,1:m_1}$ of $W^{(i,1)}$ does not change the hidden layer output $X^{(i,l)}=\sigma_{s^{(i,l)}}(X^{(i,l-1)}W^{(i,l)})$. 
    
    For each hidden layer $l \in [L-1]$ before the last layer, we can also normalize $s^{(i,l)}$ by $||s^{(i,l)}||_2$ and again rescale the last row of $W^{(i,l+1)}$ by $||s^{(i,l)}||_2$ without changing the output $X^{(i,l+1)}$. 
    
    Therefore, the regularization terms $||W^{(i,l)}_{1:m_{l-1}, 1:m_l}||^2_F$ for $l \in [L]$ and $ ||s^{(i,l)}||^2_2 $ for  $l \in [L-1]$ become redundant in the minimization. 
    So the only regularization term that remains is $\sum_{i=1}^{m_L}||s^{(L)}||^2_2 + \alpha_i^2$. Now, the same proof as for proposition \ref{prop:sign_thresh_scaled} holds to transform this L2 regularization into a L1 penalty on $\alpha$.
\end{proof}


Problem \ref{equ:psignL_simppar} is equivalent to 

\begin{equation}
\label{equ:psignL_intermedpar}
\begin{aligned}
   \min_{\alpha \in \mathbf{R}^{m_L}, s^{(i,l)}=1, W^{(i,l)}: ||W^{(i,l)}||_F=1, i \in [m_L], l \in [L-1]} & \frac{1}{2}  || Z - y||^2_2 + \beta ||\alpha||_1 \\
   &\text{ s.t. }
   Z = f_L(X)
\end{aligned}
\end{equation}

The Lagrangian of \eqref{equ:psignL_intermedpar} is 

\begin{equation}\label{Lag_par}
    L(\{s^{(i,l)}=1, W^{(i,l)}: i \in [m_L], l \in [L],\} \alpha, \lambda) = \frac{1}{2}  || Z - y||^2_2 + Z^T \lambda + \beta ||\alpha||_1 - \sum_{i=1}^{m_L} \alpha_i \left( \sigma_{s=1} \left( X^{(i,L-1)} {W^{(i,L)}} \right) \right)^T \lambda.
\end{equation}

From minimizing the Lagrangian \eqref{Lag_par} over $\alpha$, the dual of \eqref{equ:psignL_simppar} will have the constraint that for each $i \in [m_L]$,  $\max_{s^{(i,l)}=1, W^{(i,l)} \in \mathbf{R}^{1+m_{l-1} \times m_l}, W^{(i,L)} \in \mathbf{R}^{1+m_{L-1}}} |\lambda^T \sigma \left( X^{(i,L-1)}{W^{(i,L)}} \right) | \leq \beta $. However, the left hand side constraint does not depend on $i$, so it reduces to a single constraint. Therefore the dual of \eqref{equ:psignL_simppar} is

\begin{equation}\label{dsignL_sigmaspar}
\begin{aligned}
   \max_{\lambda} & -\frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } \max_{W^{(l)} \in \mathbf{R}^{1+m_{l-1} \times m_1}, w^{(L)} \in \mathbf{R}^{1+m_{L-1}}} |\lambda^T \sigma_{s=1} \left( X^{L-1}{w^{(L)}} \right) | \leq \beta 
\end{aligned}
\end{equation}

where for $l \in [L]$ we define $X^{(l)}=\left(\sigma_{s=1}(X^{(l-1)}W^{(l)}), \mathbf{1}\right), X^{(0)}=X$.



%Note $\left(\sigma \left( \sigma\left( X W^{(1)} \right) {W^{(2)}} \right)^T \lambda \right)_i$ is the inner product between $\lambda$ and the $i^{th}$ column of $\sigma \left( \sigma\left( X W^{(1)} \right) {W^{(2)}}\right) \in \mathbf{R}^{N \times m_2}$, which is $\sigma \left( \sigma\left( X W^{(1)} \right) {W^{(2)}_{1:m_1+1, i}}\right) \in \mathbf{R}^{N \times m_2}$ where ${W^{(2)}_{1:m_1+1, i}}$ is the $i^{th}$ column of $W^{(2)}$, corresponding to the weights from neuron $i$ in the second layer.




%The vector $w^{(2)}$ can be normalized by any positive scalar without changing $\sigma \left( \sigma\left( X W^{(1)} \right) {w^{(2)}} \right) $, so we may assume $||w^{(2)}||_2 =1$.

For a matrix $Z$ of some size $n \times d$, let $\mathcal{H}(Z)=\{ \sigma_{s=1}( Z w): w \in \mathbf{R}^d \}$ be the set of all length-$N$ sign pattern vectors, ie possible outputs of a single neuron taking in $n$ samples of dimension $d$. For example for the first hidden layer, if $Z=X$ then $n=N, d=2$. %As shown earlier, the elements of $\mathcal{H}$ can be concatenated next to each other to form a matrix whose columns are all $\{-1,1\}^N$ sequences with one sign switch. In the LASSO problem, as shown earlier by symmetry it suffices to consider such sequences starting with $1$.


For a set $H=\{h_1, \dots, h_{|H|} \} \subset \mathbf{R}^d $ of vectors and an ordered subset $S \subset H$ let $[H]_S$ denote the matrix formed by horizontally concatenating the vectors $h \in S$ one after another. Let $\tilde{H}_S(Z) =[[\mathcal{H}(Z)]_{S},  \mathbf{1}] $ denote the matrix formed by concatenating $[\mathcal{H}(Z)]_{S}$ with a column of ones.  Let $\tilde{H}^{(l)}_{S_j:j\in[l]}(X) = \tilde{H}^{(l)}_{S_l} \circ \tilde{H}^{(l-1)}_{S_{l-1}} \circ \cdots \circ \tilde{H}^{(1)}_{S_1}(X)$ denote composing $\tilde{H}_S$ with itself $l$ times, where the $j^{\text{th}}$ time uses a subset $S_{j-1} \subset \mathcal{H}\left([(\tilde{H}^{(j-1)}_{S_j} \circ \cdots \circ \tilde{H}^{(1)}_{S_1})(X),\mathbf{1}]\right)$.
If $l \in [L]$ and $s^{(l)}=1$, then for some collection of subsets $S_j: j \in [l]$ corresponding to the weights in each $j^{\text{th}}$ layer, the output of the $l^{\text{th}}$ hidden layer $X^{(l)} = \sigma_{s=1}(X^{(l-1)}W^{(l)}, \mathbf{1}) = [ \sigma_{s=1}(X^{(l-1)}W^{(l)}_1), \dots,  \sigma_{s=1}(X^{(l-1)}W^{(l)}_{m_l}), \mathbf{1}] = [[\mathcal{H}(X^{(l-1)})]_{S_l},  \mathbf{1}] = \tilde{H}_S(X^{(l-1)})=\tilde{H}_{S_l}(\tilde{H}_{S_{l-1}}(X^{(l-2)}))=\cdots = \tilde{H}^{(l)}_{S_j:j\in[l]}(X^{(0)})=\tilde{H}^{(l)}_{S_j:j\in[l]}(X)$ can be written in terms of $l$ function compositions on the input matrix $X$. So the set of all possible outputs of layer $l$ is $\bigcup_{\{S_j:j\in[l],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X)$. The union is taken over all possible sequences of $S_1, \dots, S_l$, where $S_j$ is constrained by the previous $S_i$ for $i < j$, which in turn depends on $X$. However, proposition \ref{prop:m_1_more_layers_same_size}, \ref{prop:m_1_more_layers} will show that for a fixed number of training samples $N$, regardless of their actual values $x_1,\dots,x_N$, $\bigcup_{\{S_j:j\in[l],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X)$ is the same set and with easily enumerable elements.
%each s_j is constrained by previous s_j-1.

Therefore the dual problem \eqref{dsignL_sigmaspar} is 

\begin{equation}\label{dsignLpar}
\begin{aligned}
   \max_{\lambda} & -\frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } \max_{h \in \bigcup_{\{S_j:j\in[l],|S_j|\leq 1+m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X)} |\lambda^T h | \leq \beta 
\end{aligned}
\end{equation}


Problem \eqref{dsignLpar} is the dual of and therefore equivalent to the LASSO problem

\begin{equation}\label{signLLasso}
\begin{aligned}
   \min_z & \frac{1}{2}  || Az- y||^2_2 + \beta||z||_1  \\
\end{aligned}
\end{equation}

where the ``dictionary" matrix $A=[\bigcup_{\{S_j:j\in[L],|S_j|\leq 1+m_j \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X)]$ is the matrix consisting of all possible sign patterns at the final layer.

Let $z^*$ be the optimal solution to the LASSO problem \eqref{signLLasso} and $m^* = ||z^*||_0$  be its cardinality. If the number of neurons in the final layer exceeds the number of nonzero elements of the optimal solution $z^*$ then we can reconstruct a parallel neural network from $z$.

Therefore we have a map from the LASSO problem \eqref{signLLasso} problem to the nonconvex primal \eqref{equ:psignL} that achieves the same function error $||y-f_L(X)||^2_2=||y-Az||^2_2$ and regularization penalty $\beta||\alpha||_1=\beta||z||_1$. We can normalize all the weights $W^{(l)}_i$ to achieve  $||W^{(l)}_i||_F=1$ to be feasible in the primal.  Since the LASSO problem \eqref{signLLasso} is the dual and hence a lower bound on the primal \eqref{equ:psignL}, the mapping that the primal \eqref{equ:psignL} can achieve any value of the LASSO problem \eqref{signLLasso} shows that they are equivalent.


\begin{proposition}
  Suppose $A \in \mathbf{R}^{n \times n}$ is as defined in \ref{signLLasso}. Suppose $m_L \geq m^*$. Suppose we have $z \in \mathbf{R}^{n}$. We can construct a parallel network $f$ as defined in \eqref{parLlayernn_cpt} with $\sigma(z)=\textrm{sign}(z)$ such that $f(X)=Az$.
\end{proposition}

\begin{proof}
Denote $W^{(l)}_i$ as the $i^{\textrm{th}}$ column of $W^{(l)}$, which contains the weights for the $i^{\textrm{th}}$ neuron of layer $l$. Let $z' \in \mathbf{R}^{m^L}$ be $z$ with $m_L - m^*\geq 0$ of its zero elements removed. Let $A' \in \mathbf{R}^{n \times m_L}$ be the submatrix consisting of columns of $A$ that have the same index as the indices of $z$ that were used to make $z'$. Since each $i^{\textrm{th}}$ column $A'_i$ of $A'$ is in $\bigcup_{\{S_j:j\in[L],|S_j|\leq 1+m_j \}} {\tilde{H}^{(l)}}_{S_j:j\in[l]}(X)$, there exists a vector $\tilde W^{(L)}_i$, a sequence of sets $S_j: j \in [L-1]$ and  $\tilde X^{(L-1)}_i = \tilde{H}^{(l)}_{S_j:j\in[l]}(X)$ such that $A'_i = \sigma(\tilde X^{(L-1)}_i W^{(L)}_i)$.  
So the parallel neural network 

\begin{equation}
    f(X) =  %\sigma(X^{(L-1)}W^{(L)})z' =
    \sum_{i=1}^{m_L}z'_i \sigma({{\tilde X^{(L-1)}}} _i \tilde W^{(L)}_i) = \sum_{i=1}^{m_L}z'_i (A')_i=\sum_{i=1}^{n}z_i (A)_i=Az
\end{equation}

 is feasible in the primal with $\alpha=z',  W^{(L)}_i= \tilde {W^{(L)}_i}, X^{(L-1)}=\tilde X^{(L-1)}$.

\end{proof}

\subsection{strong duality for nonparallel neural networks}

Suppose the data shatters, ie $A=\bigcup_{\{S_j:j\in[l],|S_j|\leq 1+m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X)$ contains all possible vectors in $[-1,1]^N$ then strong duality holds for the nonparallel neural network as well. The dual problem \ref{dsignLpar} becomes

\begin{equation}\label{dsignLparshatter}
\begin{aligned}
   \max_{\lambda \in \mathbf{R}^N} & -\frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } \max_{h \in [-1,1]^{N}} |\lambda^T h | \leq \beta 
\end{aligned}
\end{equation}

which is simplified to

\begin{equation}\label{dsignLparshattersimp}
\begin{aligned}
   -\min_{\lambda \in \mathbf{R}^N} & \frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } ||\lambda||_1 \leq \beta 
\end{aligned}
\end{equation}

which is the projection of $\lambda$ towards $y$ on to the $L_1$ ball of radius $\beta$.

\iftoggle{todos}{
\textcolor{red}{todo: correct?}

\textcolor{red}{todo: how to go from $\lambda$ back}
}

We can also see this from the Lasso problem. Consider a standard nonparallel neural network with $m_1, \cdots, m_L$ neurons in each layer, ie the same number as that of each parallel unit in the parallel neural net. This standard neural net has   $m_L$ times as less neurons as the parallel one, but results in the same LASSO problem and dictionary matrix.

Now suppose there exists possible neuron weights $W^{(1)},\cdots, W^{(L)}$ such that $X^{(L-1)}$ has rank $N$. Then for any matrix $A'$ consisting of a subset of columns from the dictionary matrix $A$, there exists $W^{(L)}$ such that $X^{(L-1)}W^{(L)} = A'=\sigma(A')$. Hence we can construct a standard nonparallel neural network $f(X)=\sigma(X^{(L-1)}W^{(L)})z = Az$ with $z=\alpha$ and the same number of neurons $m_1, \cdots, m_L$ as the layers of each parallel unit of the parallel neural network, and achieves the same function value in the primal. So strong duality holds for the standard neural network as well.  Therefore a parallel structure is not necessary for achieving minimal training loss in this case.

One way for this to occur is if for some $2 \leq l < L$, there exist weights $W^{(1)},\cdots, W^{(l)}$ such that $X^{(l)}$ has full rank and $m_l = m_{l+1} = \cdots = m_L$. i.e., the size of the layers do not change henceforth. Then setting each $W^{(l')}$  for $l < l' < L$ to be the identity matrix to preserve the full column rank of $X^{(l)}$ at $N$ means $X^{(L-1)}$ will have full rank. In the case of $1D$ data, the additional layers between the third and last layer can essentially just be identity matrices that preserve the expressability of the neural network from layer to layer. 

In the case of $1D$ data, this can occur if the first layer has enough neurons relative to the number of samples. Suppose $m_1 \geq N$ and dimension $d=1$ and layer sizes satisfy $N-1 = m_1 = m_2 = \cdots = m_L$. By proposition \ref{prop:m_1_more_layers_same_size} there exists $X^{(1)}$ and $W^{(2)}$ such that $X^{(2)} = [\sigma(X^{(1)}) , \mathbf{1}]$ has full column rank.

Note if $A$ is not full rank, the LASSO problem is not strictly convex and there may be multiple possible neural networks. The generalizability of each of these possible networks is an area for future research.
 
 
\iftoggle{todos}{
\subsection{expressibility of parallel versus standard neural networks for $1D$ data  $m_{L-1}<N$}
}
%when the penultimate hidden layer size



 However, if the number of neurons is not enough, specifically the penultimate hidden layer size $m_{L-1} < N-1$ %and the cardinality of the LASSO solution $||z^*||_0$ 
 for $1D$ data, then depending on the training data and labels, strong duality might not hold for the standard nonparallel neural network. The standard neural network results in the same Lasso problem, but the Lasso problem may achieve a lower objective value than the primal for the standard neural network.

 As the regularization penalty decreases $\beta \to 0$, the Lasso problem approaches satisfying $Az=y$: 

 \begin{equation}
 \begin{aligned}
          \min_z & ||z||_1\\
          &\text{ such that } Az=y
 \end{aligned}
 \end{equation}
 
In this low-regularization regime, we show a counterexample as follows.

\textcolor{red}{ is this example sufficient? even if $\beta \neq 0$, is this counterexample enough? we do have $||\alpha||_1=||z||_1$}

 Let the number of samples be $N=3, X \in \mathbf{R}^3$. Suppose the neural network has layer sizes $m_1=1, m_2=2$. By proposition \ref{prop:m_1switches}, up to permutation of columns, the dictionary matrix $A$ consists of $1$ in the upper right corner including the diagonal and $-1$ elsewhere, and therefore the column span of $A$ is all of $\mathbf{R}^3$ 
 \iftoggle{todos}{
 (\textcolor{red}{todo:make invertability as its own theorem}). 
 }
 So for any $y$, we can solve $z=A^{-1}y$ and from the LASSO problem we can construct a parallel neural network to achieve perfect interpolation of the data. However, the nonparallel neural network is of the form $f(X)=\sigma(X^{(1)}W^{(2)})\alpha$ where $X^{(1)}=\sigma([X, \mathbf{1}]W^{(1)}) W^{(2)} \in \mathbf{R}^2$. %So $X^{(1)}$ is one of the columns of $A$, concatenated with a column of ones, which is a matrix that consists of two of the columns of $A$. 
 Then  $\sigma(X^{(1)}W^{(2)})$ has size $3 \times 2$ and therefore does not have full column rank. Therefore there exists $y \in \mathbf{R}^3$ for which no such $\alpha \in \mathbf{R}^2$ satisfies $\sigma(X^{(1)}W^{(2)})\alpha=y$.

 The counterexample can be generalized to any any dimension $d$, number of layers $m_L$, number of samples $N$, training data $X \in \mathbf{R}^{N \times d}$ where the dictionary matrix $A$ has full rank but $m_{L-1}<N$.



\subsection{dictionary matrix for 1D data}

 Let the (original $1D$) training samples be ordered $x_1 > \dots > x_N$. Assume there are no repeat samples, ie that $x_i \neq x_j$ for $i \neq j$.


For any length $m \in \mathbf{N}$ and sequence of $m$ integers $1 < I_1 < I_2 < \dots < I_m \leq N$, let $h(I_1,\dots,I_m) \in \mathbf{R}^N$ be the vector such that at each index $n \in [N]$,

\begin{equation}
    \begin{aligned}
        h(I_1,\dots,I_m)_n = 
        \begin{cases}
            1 \text{ if }  n \in [I_{2i}, I_{2i+1}) \text{ for some }  i \in \mathbf{Z} \\
            -1 \text{ else }
        \end{cases}
    \end{aligned}
\end{equation}

In other words, $h(I_1,\dots,I_m)$ starts at $1$ and alternates $m$ times between $1$ and $-1$, switching values at each successive index $I_i$. 

For any $1 < i \leq m$, $h(i)-\mathbf{1}$ is $-2$ if at indices $\geq i$ and $0$ otherwise. So we have the unit cliff vector 

\begin{equation}
    \begin{aligned}
        h(i)=\sigma(h(i)-\mathbf{1}). 
    \end{aligned}
\end{equation}

For any indices $1 < i < j \leq m$, the vector $h(i,j)$ dips to $-1$ between indices $i$ and $j-1$ and is $1$ elsewhere. The vector $h(i)-h(j)$ dips to $-2$ between indices $i$ and $j-1$ and is $0$ elsewhere. So, the one-dip vector $h(i, j)$ can be decomposed into single-switch vectors $h(i)$ and $h(j)$ as the unit dip vector

\begin{equation}
\begin{aligned}
       h(i, j) &= 
       \sigma(h(i)-h(j))
\end{aligned}
\end{equation}




For $1\leq a\leq b \leq m$, define the vector $\mathbf{1}[a,b] \in \mathbf{R}^m$ to be, for indices $i \in [m]$,

\begin{equation}
    \mathbf{1}[a,b]_i = 
    \begin{cases}
        1 \mbox{ if } i \in [a,b]\\
        0 \mbox{ else } 
    \end{cases}
\end{equation}
\iftoggle{todos}{
\textcolor{red}{(only used $\mathbf{1}[a,b]$ in 1switch, 2 switch examples so might not need)}
}
We have the unit ``cliff" (a negative step) vector $\frac{1}{2}(h(i)-\mathbf{1}) = -\mathbf{1}[i,m] \leq 0$ and the unit ``dip" (a negative bump) vector $ \frac{1}{2}(h(i)-h(j)) = -\mathbf{1}[i,j-1] \leq \mathbf{0}$.
Note for any nonpositive vectors $a,b \in {\mathbf{R}^{N}}^{\leq0}, \sigma(a+b)=\sigma(a)+\sigma(b)$. 


\subsubsection{span of $k$-switch vectors}


\begin{lemma}\label{lemma:h+h-}
    Let $\mathcal{I} = \{I_1, \cdots, I_{2m} \} \subset [N]$ be a vector with $2m$ switches. There exist $h^+(\mathcal{I}), h^-(\mathcal{I}) \in [-1,1]^N$ each with $m$ switches such that $h(\mathcal{I})=\sigma(h^+ - h^-)$.
\end{lemma}

\begin{proof}
    
Let 

\begin{equation}
    \begin{aligned}
        (m^+, m^-) &= 
        \begin{cases}
            (2m-1, 2m  ) \text{ if } m \text{ is odd}\\
            (2m, 2m-1) \text{ if } m  \text{ is even}\\
        \end{cases}
    \end{aligned}
\end{equation}

\begin{equation}
    \begin{aligned}
        h^+(\mathcal{I}) &= h(I_1, I_4, I_5,I_8,I_9,I_{12},I_{13},\cdots,I_{4i},I_{4i+1},\cdots, I_{m^+})\\
        h^-(\mathcal{I}) &= h(I_2, I_3,I_6,I_7,\cdots, I_{4i+2},I_{4i+3},\cdots, I_{m^-})\\
    \end{aligned}
\end{equation}

Note $h^+$ and $h^-$ each have $m$ switches. 

We have

\begin{equation}
    \begin{aligned}
        h(I_1,\cdots, I_{2m}) 
        &= \sigma \left(h^+ - h^- \right).\\
    \end{aligned}
\end{equation}

In other words, the ``hills" (the indices where the vectors are $1$) of two $m$-switch vectors $h^+$ and $h^-$ are interleaved to form a vector $ h(I_1,\cdots, I_{2k}) $ with $2m$ switches. 

\end{proof}

\begin{lemma}
     Let $\mathcal{I} = \{I_1, \cdots, I_{r} \} \subset [N]$ be a vector with $1 \leq r\leq 2k-1$ switches. There exist $h^+(\mathcal{I}), h^-(\mathcal{I}) \in [-1,1]^N$ each with at most $k$ switches such that $h(\mathcal{I})=\sigma(h^+ - h^-)$.
\end{lemma}

\begin{proof}
    If $r$ is even, let $r^+=r^-=\frac{r}{2}$. If $r$ is odd, let $r^+ = \frac{r+1}{2}, r^- = \frac{r-1}{2}$. So $r^+ \geq r^-, r = r^+ + r^-$ and $r^+ - r^- \in \{0,1\}$. 
    If $r^+=r^-$ then define $m^+,  m^-$ in the same way as lemma \ref{lemma:h+h-}.
    If $r^+ = r^- + 1$, then let $m^+=r$. Let $m^-=m^+-2$ if $r^+$ is odd, else let $r^-=m^+-1$.

    Define $h^+, h^-$ in the same way as lemma \ref{lemma:h+h-}.
\end{proof}

\begin{lemma}
 Let $I_0 = \mathbf{1}$. For a subset $\mathcal{I }= \{I_1, \cdots, I_k\} \subset [N]$ such that $1 < I_1 < \cdots < I_k \leq N$, denote $h(\mathcal{I}) = h(I_1, \cdots, I_k)$.
Let $m_1,m_2 \in \mathbf{N} $. Let $k \in [m_1 m_2]$. Let $1 < I_1 < \cdots < I_{k} \leq N$. 

There exists $w \in \mathbf{R}^{m_2}$ and $m_2$ subsets $\mathcal{I}^{(i)} \subset N$ each of size at most $|S_i| \leq m_1$ such that $h(I_1,\cdots, I_{k}) = \sigma \left(\sum_{i=1}^{m_2} w_i h(\mathbf{I}^{(i)}) \right)$.
\end{lemma}

\begin{proof}
    By the fundamental theorem of arithmetic, there exist nonnegative integers $q,r$ such that $r<2m_1$ and $k = q(2m_1)+r$. Since $r < q$
    For $i \in [q]$, let $\mathcal{I}^{(i)} = I_{1+(i-1)2m_1},I_{2+(i-1)2m_1},\cdots,I_{i(2m_1)}$ be the $i^{th}$ chunk of $2m_1$ indices in $[k]$. Let $\mathcal{I}_{q+1} = \{I_{1+q(2m_1)},I_{2+q(2m_1)},\cdots, I_k\}$.
    By lemma \ref{lemma:h+h-},

    \begin{equation}
        \begin{aligned}
            h(I_1, \cdots, I_k) &= \sigma \left( h^+(\mathcal{I}_{q+1})- h^-(\mathcal{I}_{q+1})+ \sum_{i=1}^q h^+ (\mathcal{I}^{(i)}) - h^- (\mathcal{I}^{(i)})\right) \\
        \end{aligned}
    \end{equation}

    which contains $2(q+1) \leq 2\frac{k}{2m_1} \leq 2\frac{m_1 m_2}{2m_1}=m_2$ vectors of the form $h^+$ or $h^-$, each of which have at most $m_1$ switches. 
\end{proof}

\subsubsection{decomposing into one switch vectors}

We can add more dips to the vector by combining one-dip vectors as follows. Suppose $m$ is even. Let $I_1< \dots < I_m$.

For any $m \in \mathbf{N}, I \in [N]^m$, $h(I)$ falls to $-1$ at $I_i$ for odd index $i$ and rises to $1$ at even $i$ and is constant at all other indexes in between. Hence an arbitrary $m$-switch vector in $\{-1,1\}^N$ can be decomposed as

\begin{equation}
    \begin{aligned}
        h(I)  &= \sigma(h(I)-\mathbf{1})\\
        &=\sigma \left( -\mathbf{1}[I_1, I_2] -\mathbf{1}[I_3, I_4] \cdots - \mathbf{1}\{m \textrm{ is even} \}\mathbf{1}[I_{m-1}, I_m] - \mathbf{1}\{m \textrm{ is odd}\}\mathbf{1}[I_{m-1},m]\right)\\
        &= \sigma\left(\mathbf{1}\{m \textrm{ is odd} \}(h(I_m) -\mathbf{1})  + \sum_{i=1}^{\lfloor \frac{m}{2} \rfloor} h(I_{2i-1})- h(I_{2i}) \right)\\
        &= \sigma\left( [\sigma([X, \mathbf{1}] W^{(1)}, \mathbf{1}]) w\right)\\
        &= \sigma\left( X^{(1)} w\right)
    \end{aligned}
\end{equation}

where $W^{(1)} \in \mathbf{R}^{2 \times m}$ with $i^{th}$ column being $(1,-x_i)^T$, $X^{(1)}=[h(I_1)\cdots h(I_m)]$, and $w \in \mathbf{R}^{m+1}$ is defined as, for indices $i \in [m+1]$,

\begin{equation}
w_i=
    \begin{cases}
        1 \mbox{ if } i \mbox{ is odd}, i \leq m\\
        -1 \mbox{ if } i \mbox{ is even}, i \leq m\\
        -1 \mbox{ if } i=m+1, m \mbox{ is  odd }\\
        0 \mbox{ if } i=m+1, m \mbox{ is  even }\\
    \end{cases}
\end{equation}

%$1$ at odd indices up to $m$, and $-1$ at even indices up to $m$ and if $m$ is even then $0$ at the last index $m+1$.


\subsubsection{decomposing into two- switch vectors}

We have the unit dip vector %in the middle

\begin{equation}
    \begin{aligned}
    h(i,j)
        &= \sigma(h(i,j)-\mathbf{1})\\
        &= \sigma(-\mathbf{1}[i,j-1])
    \end{aligned}
\end{equation}

and the unit double-dip vector that is $-1$ between $[I_i, I_{m-i}-1]$ and $[I_{i+1},I_{m-(i+1)}]$ and $0$ elsewhere:

\begin{equation}
    \begin{aligned}
    h(I_i, I_{i+1}, I_{m-i}, I_{m-(i+1)})&= \sigma(h(I_i, I_{m-i})-h(I_{i+1}, I_{m-(i+1)}))\\
     &=\sigma(-\mathbf{1}[I_i, I_{i+1}-1] - \mathbf{1}[I_{m-i},I_{m-(i+1)}-1])
    \end{aligned}
\end{equation}

and the unit 3-switch vector

\begin{equation}
\begin{aligned}
h(I_{m-2},I_{m-1},I_m)&=
    \sigma(h(I_{m-2})-h(I_{m-1})+h(I_m)-\mathbf{1})\\
    &= \sigma(h(I_{m-2},I_{m-1}) + h(I_m)-\mathbf{1})\\
    &=\sigma(-\mathbf{1}[I_{m-2},I_{m-1}]-\mathbf{1}[I_{m},m])
\end{aligned}
\end{equation}

Now consider up to $2$-switch vectors.
If $m$ is even, then we can decompose the first half of the vector $h(I_1,\cdots,I_{m/2})$ into one-switch vectors, and then symmetrically reflect the one switch vectors to form two-switch vectors.

Case 1: $m \equiv 0 \mod 4 $.
Then $m$ is even and $m/2$ is divisible by $2$, then

\begin{equation}
    \begin{aligned}
        h(I) &=
        \sigma(\sum_{i \in [m/2], i \textrm{ odd}} h(I_i, I_{m-i})-h(I_{i+1}, I_{m-(i+1)}))
    \end{aligned}
\end{equation}

which decomposes $h(I)$ into nested layers of $2$-switch vectors. 

Case 2: $m \equiv 2 \mod 4 $.
Then $m$ is even and $m/2$ is odd,

\begin{equation}
    \begin{aligned}
        h(I) &=
        \sigma(h(I_m) - \mathbf{1} + \sum_{i \in [\frac{m-1}{2}], i \textrm{ odd}} h(I_i, I_{m-i})-h(I_{i+1}, I_{m-(i+1)}))
    \end{aligned}
\end{equation}

Case 3: $m \equiv 1 \mod 4 $.
Then $m$ is odd and $(m-3)/2$ is odd. 

\begin{equation}
\begin{aligned}
     h(I) = h(I_{m-2})+h(I_{m-1},m)+
        \sigma(h(I_m) - \mathbf{1} + \sum_{i \in [\frac{m-3}{2}], i \textrm{ odd}} h(I_i, I_{m-i})-h(I_{i+1}, I_{m-(i+1)}))
\end{aligned}
\end{equation}

Case 4: $m \equiv 3 \mod 4 $.
Then $m$ is odd and the half of the remaining vector $(m-3)/2$ is even. 

\begin{equation}
    \begin{aligned}
          h(I) &= h(I_{m-2})+h(I_{m-1},m)+
        \sigma(\sum_{i \in [m/2], i \textrm{ odd}} h(I_i, I_{m-i})-h(I_{i+1}, I_{m-(i+1)}))
    \end{aligned}
\end{equation}


\iftoggle{todos}{
 \textcolor{red}{todo: fix $l$ vs $l-1$ indices on $\mathbf{H}$}
}


 \textcolor{red}{todo if time: picture}

 Note that $\bigcup_{\{S_j:j\in[j],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[L]}(X)$ is a set of vectors in $[-1,1]^N$. For $1D$ data, we can further characterize this collection of vectors by the number of switches they can have.

\begin{proposition}\label{prop:H_oneswitch}
    For dimension $d=1$ and activation function $\sigma(z)=\text{sign}(z), X \in \mathbf{R}^{n \times 1}, \mathcal{H}(X)$ consists of all length $N$ sequences of $\pm1$  with up to one switch.
\end{proposition}

\begin{proof}
    The zero-switch vector $\mathbf{1}=\sigma(\mathbf{0})=\sigma(X \mathbf{0}) \in \mathcal{H}(X)$.

    Let $h \in \mathcal{H}(X)-\{ \mathbf{1}\}$, so $h$ switches at least once. There exists $w^{(1)}=(w,b) \in \mathbf{R}^2$ such that $h=Xw^{(1)}$. %$h_1 = \sigma(x_1 w + b) =1$ so $x_1 w +b > 0$ so $w>0$. 
    Let $i = \min \{j \in [N]: h_i = -1 \}>1$ be the first index for which $h$ switches. So $x_{i}w+b < 0 \leq x_{i-1}w+b  $. So $x_{i} w < x_{i-1}w$. On the other hand by our ordering, $x_i \leq x_{i-1}$. So we must have $w>0$. $\sigma(z)$ is monotone nondecreasing. So for all $j > i$, $h_j = \sigma((Xw)_j) = \sigma((x_j,1)(w,b)^T) = \sigma(x_j w + b) \leq \sigma(x_i w + b) = \sigma(h_i)=-1$, so $h_j =-1$. So every $h \in \mathcal{H}$ switches at most once.

    Now, let $h \in [-1,1]^N$ be a vector such that $h_1=1$. Let $i \in N$ and suppose $h$ switches once, at index $i>1$, so $ h_i =-1$. Let $w=1,b=-x_{i-1}, w^{(1)}=(w,b)$. Then for $j<i$, $x_j w+b = x_j - x_{i-1} \geq x_{i-1} - x_{i-1} = 0$ so $h_j = \sigma((x_j,1)w^{(1)})=1$. And for $j\geq i$, $x_j w+b = x_j - x_{i-1} \leq x_{i} - x_{i-1} < 0$ so $h_j = -1$. So every vector in $[-1,1]^N$ that starts with $1$ and switches once is in $\mathcal{H}$.
\end{proof}

We can extend this to adding one more layer.

\begin{proposition}\label{prop:m_1switches}
    For dimension $d=1$, activation function $\sigma(z)=\text{sign}(z), X \in \mathbf{R}^{N \times 1}, \bigcup_{\{S_j:j\in[1],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X) = \cup_{|S|\leq m_1} \mathcal{H}\left([\mathcal{H}\left(X\right)]_S, \mathbf{1}]\right)$ consists of all length $N$ sequences of $\pm1$ with at most $\min\{N-1,m_1\}$ switches.
\end{proposition}

%ones is probably redundant since always in anyways, but this just makes sure that no matter X^l and s_l-1, we always have the option to include bias, since technically s_l could depend on s_l-1.

\begin{proof}
    Let $h \in \cup_{|S|\leq m_1} \mathcal{H}\left([\mathcal{H}\left(X\right)]_S, \mathbf{1}]\right)$. So there exists $w \in \mathbf{R}^{n}$ with $n\leq m_1 + 1$ and a matrix $Z \in \mathbf{R}^{N \times n}$ that has $n-1\leq m_1$ columns from $\mathcal{H}(X)$ and one column that is a vector of all ones, such that $h=\sigma(Zw)$. By proposition \ref{prop:H_oneswitch}, each of the $n-1$ columns of $Z$ from $\mathcal{H}(X)$ has at most one switch, and the column of ones has no switch, so the matrix $Z$ has at most $n$ unique rows. Therefore the vector $Zw$ has at most $ n$ unique elements and $n-1\leq m_1$ switches between unique elements. Hence $h=\sigma(Zw)$ has at most $m_1$ switches. So every vector $h \in [\cup_{|S|=m_1} \mathcal{H}([\mathcal{H}(X))]_{m_1}]$ has at most $m_1$ switches.

    Conversely, let $h \in [-1,1]^N$ be such that $h_1=1$ and $h$ has $n \leq m_1-1$ switches.  For $i \in [n-1]$, let $h'^{(i)} \in [-1,1]^n$ be the vector such that $h^{(i)}_j=\text{sign(i-j)}$, ie $h^{(i)}_j=1$ if $j\leq i$ and $-1$ otherwise.  Let $h^{(n)} = \mathbf{1} \in \mathbf{R}^n$.  Let $H' = [h'^{(1)} \cdots h'^{(n)}] \in \mathbf{R}^{n \times n}$ be the matrix where the $h'^{(i)}$ are concatenated next to each other. $H'$ consists of $1$'s in the upper right corner including the diagonal and $-1$'s in the lower left corner. 
    
    We will add $N-n$ rows to $H' \in \mathbf{R}^{n \times n}$ to form a new matrix $H \in \mathbf{R}^{N \times n}$ as follows. For every index $i>1$ such that $h_{i-1}=h_{i}$,  expand $H'$ by inserting another copy of $H'$'s corresponding row $\tilde{h'}$ right beneath itself, so that the indices that $h$ switches at are exactly the indices at which the rows of $H$ change.

    Note that H has $n \leq m_1 $ columns, so is a valid output matrix $X^(1)$ of the first hidden layer. 
    
    Let $h^{(i)} \in \mathbf{R}^N$ denote the $i^{th}$ column of $H$. As in $H'$, the columns of $H$ still only switch at most once. So by proposition \ref{prop:H_oneswitch}, for $i \in [n]$, $h^{(i)} \in \mathcal{H}(X)$. Denote the $i^{th}$ row of $H$ as $\tilde{h}_i$. 
    Let $I \subset [N]$ be the set of indices for which a row of $H$ changes, ie $\tilde{h}_{i-1} \neq \tilde{h}_i$ for $i \in I$. Note $|I|=n$. Let $I$ be an (descending) ordered set, with $I_j$ being the $j^{th}$ row at which $H$ changes rows. %$H$ consists of ones in the upper right corner including the diagonal, and $-1$ elsewhere, including the bottom $N-n$ rows. 
    
    Now, let $w^{(1)} \in \mathbf{R}^{n}$ be defined as follows. For $i \in [n-1]$, let $w^{(1)}_{i} = \frac{h_{I_i} - h_{I_{i+1}}}{2}$. And let $w^{(1)}_{n} = \frac{h_{I_1}+h_{I_n}}{2}$. Then for $i \in [n]$, $(Hw^{(1)})_{I_i} = \tilde{h}_{I_i}^T w = \sum_{j=1}^{i-1} (-1) w_j + \sum_{j=i}^{n-1} (1) w_j + w_n = -\frac{1}{2}\sum_{j=1}^{i-1} (h_{I_j} - h_{I_{j+1}})  + \frac{1}{2}\sum_{j=i}^{n-1} (h_{I_j} - h_{I_{j+1}}) + \frac{h_{I_1}+h_{I_n}}{2} = \frac{1}{2}(-(h_{I_1}-h_{I_i}) + (h_{I_i}-h_{I_n}) + (h_{I_n}+h_{I_1}))=h_{I_i}$. 
    And for every $i \in [N]-I$, let $j = \max\{k \in I: j \leq i\}$ be the previous index in $I$ that has the same row in $H$ as row $j$ and the same element in $h$ as that at index $j$; then $(Hw)_i = \tilde{h}_i^T w = \tilde{h}_j^T w = h_j = h_i$. So $Hw^{(1)}=h$. Since $h \in [-1,1]^N$, we have  $\sigma(Hw^{(1)})=\sigma(h)=h$, so $h \in \cup_{|S|\leq m_1+1} \mathcal{H}\left([\mathcal{H}\left(X\right)]_S, \mathbf{1}]\right)$. 
    
    %not using switch property of sigma and -1, 1: holds for any vector. And we never used that for any arbitrary subset of columns we can find a w,b such that we get the full number of switches.
\end{proof}

If we add more layers however, the number of switches does not increase.



\begin{proposition}\label{prop:m_1_more_layers}
    For dimension $d=1$, activation function $\sigma(z)=\text{sign}(z), X \in \mathbf{R}^{N \times 1}$, every vector in $\bigcup_{\{S_j:j\in[j],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[L]}(X)$ has at most $\min \{N-1, m_1\}$ switches.
\end{proposition}

\begin{proof}
Let $W^{(1)} \in \mathbf{R}^{2 \times m_1}$. For any vector $w \in \mathbf{R}^2$, $Xw$ has at most 1 switch. $XW^{(1)}$ has $m_1+1$ columns, so $[XW^{(1)}, \mathbf{1}]$ has at most $\min\{N, m_1+1\}$ unique rows. Let the indices of these unique rows be $r_1, ..., r_{n} \in [N]$ where $n\leq \min\{N,m_1\}$. So $X^{(1)} = \sigma([XW^{(1)},\mathbf{1}])$ only has changing rows at $r_1, ..., r_{n}$. Any other row $i \in [N]$ will be the same as the most recent row that changed, ie the row indexed by $\max\{ r_j: r_j < i\}$.

Now let $W^{(2)} \in \mathbf{R}^(m_1 +1 \times m_2)$. $X^{(1)}$ has changing rows only at $r_1, \dots, r_{n}$, so for any vector $w \in R^{m_1 + 1}$, the elements of the vector $X^{(1)}w $ can only switch at indices  $r_1, \dots, r_{n}$. This held for any $w \in \mathbf{R}^{m_1}$, so $X^{(1)} W^{(2)}$ only has at most $m_1$ unique rows, in particular again at rows $r_1, \dots, r_{n}$. So $X^{(2)} = \sigma([X^{(1)}W^{(2)}, \mathbf{1}])$ also only has changing rows at $r_1, \dots, r_{n}$.

Continuing the same way, $X^{(3)} = \sigma([X^{(2)}W^{(3)}, \mathbf{1}])$ can only have changing rows at $r_1, \dots , r_{n}$, etc and so does $X^{(L-1)} = \sigma([X^{(L-2)}W^{(L-1)}, \mathbf{1}])$.

So for any vector $w \in \mathbf{R}^{m_L}$, and any feasible $X^{(L-1)}$ (taken over all possible sequences of $W^{(1)}, \dots, W^{(L-1)}$), $X^{(L-1)}w$ will have only at most $m_1$ switches.

%    We use induction on $l$. The base case when $l=1$ is shown by proposition \ref{prop:m_1switches}.
%    For $l \in [L]$, let $A_l=\bigcup_{\{S_j:j\in[j],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[l]}(X), p_l=\prod_{j=1}^{l} m_j$
%    Suppose proposition \ref{prop:prod_m} holds when $l=k \in [L-1]$. Note $A_{k} \subset A_{k+1}$ so if $p_k \geq N-1$ then proposition \ref{prop:prod_m} holds proposition for $l=k+1$. So assume $p_k < N-1$. So $S_k$ contains all vectors in $[-1,1]^N$ with at most  $p_k$ switches. For layer $k+1$, $A_{k+1}=\bigcup_{S:|S|\leq m_{k+1}} \mathcal{H}([[\mathcal{H}(X^{(k)})]_S, \mathbf{1}])= \bigcup_{S:|S|\leq m_{k+1}} \mathcal{H} ([A_k]_S, \mathbf{1}])$. 

%    The argument follows closely as that of proposition \ref{prop:m_1switches}.

%    Let $h \in A_{k+1}$. So there exists $w \in \mathbf{R}^{m_{k+1}+1}$ and matrix $Z \in \mathbf{R}^{N \times (m_{k+1}+1)}$ whose first $m_{k+1}$ columns are from $A_k$ such that $h = \sigma(Zw)$. Each of the $m_{k+1}$ columns of $Z$ has at most $p_k$ switches, so the $N$ rows of $Z$ change at most $\min \{N-1, m_{k+1}p_k=p_{k+1}\}$ times. So $Zw$ and hence $h=\sigma(Zw)$ changes at most $\min \{N-1,p_{k+1}\}$ times.

%    Conversely, let $h \in [-1,1]^N$ with $n \leq p_{k+1}\leq N-1$ switches. $P_{k+1} \geq 1$ so $A_k$ includes vectors with a single switch. Therefore a similar argument as the rest of the proof of proposition \ref{prop:m_1switches} can be used to solve for $w$, so that $h \in A_{k+1}$.
\end{proof}

The following proposition provides a converse if the layers all have the same size.

\begin{proposition}\label{prop:m_1_more_layers_same_size}
Suppose $m_1 = \dots = m_L = m$.
    For dimension $d=1$, activation function $\sigma(z)=\text{sign}(z), X \in \mathbf{R}^{N \times 1}$, $\bigcup_{\{S_j:j\in[j],|S_j|\leq m_l \}} \tilde{H}^{(l)}_{S_j:j\in[L]}(X)$ contains all vectors in $[-1,1]^N$ with at most $\min \{N-1, m_1\}$ switches.
\end{proposition}

\begin{proof}
By proposition \ref{prop:m_1switches},
     for any $z \in [-1,1]^{N} $ with at most $\min \{N-1, m_1\}$ switches we can find a possible $X^{(1)} \in \mathbf{R}^{N \times (m+1)}$ and $W^{(2)} \in \mathbf{R}^{m+1 \times m}$ such that $X^{(1)} W^{(2)}=z=\sigma{(z)}$ so $X^{(2)}=z$. 

     For every $l \in \{3, \dots, L \}$ can set $W^{(l)} \in \mathbf{R}^(m \times m)$ to be the $m \times m$ identity matrix so that $X^{(L-1)}=X^{(1)}$. And then setting $W^{(L)}=W^{(2)} $ gives $\sigma(X^{(L-1)}W^{(L)}z) =\sigma(X^{(1)}W^{(2)}z) = \sigma(z)=z$.
\end{proof}

%proof is wrong: not recursive, X^(l) has to be legitamite.Given z \in R^{m_L}, I wanted to find a possible X^(L-1), w, alpha such that z =sigma( sigma(X^(L-1)W^(L))*alpha). In the first layer, we can find X*W^(1) whose column span contains any vector with at most m_L switches. If m_1=...=m_L this works for z with m_L switches at the L^th layer but if z has more switches, then I don't have a guarantee z is in the column span of X^(L-1)W^(L) which has m_L columns. I think for each neuron i if the vector X^(L-1)W^(L)_i is a particular vector with m_1*...*m_(L-1) switches then there is a 


\subsection{dictionary matrix for special cases of 2D data}


The $1D$ structure of the data is only used to explicitely construct the dictionary matrix $\tilde{S}_{j:j\in [L]}(X)$ as a collection of vectors with a certain number of switches governed by the product of the number of neurons in each layer. If the data is $2D$, in certain situations this structure can also be recovered. 

\subsubsection{upper half plane with no bias}
Suppose the training data is on the upper half plane of $\mathbf{R}^{2}$: $x_i \in \mathbf{R}^2, {x_i}_2 \geq 0$. Suppose none of the training data have the same angle from the origin. Let $x'_i = \angle x_i$. Assume angles go from $0$ to $2\pi$ counterclockwise from the positive $x$ axis. Order the data by decreasing angle from the origin, so that $x'_1 > x'_2 > \dots x'_N$. 

Then if we ignore the bias term, for any $w = (w_1, w_2)\in \mathbf{R}^2$ in the upper half plane, and $i \in [N]$, $w^T x_i \geq 0$ if and only if $x_i' \in [\angle w - \pi/2, \angle w + \pi/2]$. Since $x_i' \in [0, \pi]$, this condition is equivalent to $x_i' \leq \angle w+\pi/2$ if $\angle w \geq \pi/2$, and $x_i' \geq \angle w-\pi/2$ otherwise. Since $x'_1 > \dots > x'_N$, if $\angle w \leq \pi/2$ then $w^T x_i \geq 0$ if and only if $i \leq \max \{j \in [N]: x_j^T w \geq 0\}$. And if $\angle w \leq \pi/2$ then $w^T x_i \geq 0$ if and only if $i \geq \min \{j \in [N]: x_j^T w \geq 0\}$. If $w$ in the lower half plane, the data also splits analagously.

So $\mathcal{H}(X')$ will also consist of all vectors in $[-1,1]^N$ with one switch. Therefore a neural network without bias terms in the first layer will fit the LASSO problem with dictionary matrices following propositions \ref{prop:m_1_more_layers}, \ref{prop:m_1_more_layers_same_size}.


\subsubsection{data on a circle with bias}
Suppose the training data $x_i$ is normalized so that for all $i \in [N]$, $||x_i||_2=1$. This may occur from preprocessing steps %cite
or model layer batch normalization in the neural network. Then the $x'_i$ for which $w^T x_i \geq 0$ will also be consecutive, although it need not include the first or last samples $x_1, x_N$. Therefore $\mathbf{H}(X)$ will consist of all vectors in $[-1,1]^N$ with at most $2$ switches.  

%We will not assume that the elements of $\mathcal{H}$ all start with $1$. 

\iftoggle{todos}{
\textcolor{red}{todo: finish, more rigor}
}

%does the dictionary matrix A depend on m_1, ... m_{L-1}? In particular, the number of switches a column of A can have depends on m_1, ... m_{L-1}. 

\section{(almost same as nonparallel; don't use?) parallel, L hidden layers sign activation} 

Define a neural network $f_L:\mathbf{R} \to \mathbf{R}$ with $L$ hidden layers by

\begin{equation}\label{Llayernn_cpt}
\begin{aligned}
     f_L(x) &= \sigma_{s^{(L)}} \left( x^{(L-1)} W^{(L)} \right) \alpha\\
    &\text{where for }l \in [L-1], x^{(l)} = \left( \sigma_{s^{(l)}}\left( x^{(l-1)} W^{(l)} \right) , \mathbf{1} \right) \in \mathbf{R}^{1\times (1+m_{l})}, x^{(0)}=(x,1) \in \mathbf{R}^{1\times 2}\\
    & m_0=1, \alpha \in \mathbf{R}^{m_L}\\
    &\text{and for } l \in [L], W^{(l)} \in \mathbf{R}^{1+m_{l-1}\times m_l}
\end{aligned}
\end{equation}


Suppose the neural network $f_L$ is trained on the following problem generalizing \eqref{equ:psign} to $L$ hidden layers: 

\begin{equation}
\label{equ:psignL}
\begin{aligned}
   \min_{W^{(1)}, W^{(2)}, s^{(1)}, s^{(2)}, \alpha} \frac{1}{2} || f_L(X) - y||^2_2 + \beta/2 \left ( ||\alpha||^2_2  +  \sum_{l=1}^L ||W^{(l)}_{1:m_{1-1}, 1:m_l}||^2_F
    + ||s^{(l)}||^2_2 \right)
\end{aligned}
\end{equation}

where $W^{(l)}_{1:m_{1-1}, 1:m_l}$ denotes all but the last row of $W^{(l)}$. The last row of $W^{(l)}$ which are variables corresponding to the bias terms of the neurons, which are unregularized. Only regularizing the non-bias weights is consistent with the neural network in \eqref{equ:psign} that had $L=1$ hidden layer. 


\begin{proposition}
    Problem \ref{equ:psignL} is equivalent to 

\begin{equation}
\label{equ:psignL_simp}
\begin{aligned}
   \min_{s^{(l)}=1: l \in [L-1], W^{(l)}: ||W^{(l)}||_F=1, l \in [L], \alpha} \frac{1}{2} || f_L(X) - y||^2_2 + \beta ||\alpha||_1
\end{aligned}
\end{equation}
\end{proposition}

So the amplitude parameters $s^{(l)}$ do not need to be trained and can just be set to $1$.

\begin{proof}
    The bias variables in the last rows of $W^{(l)}$ are not regularized and therefore can be rescaled. For each hidden layer $l \in [L]$ and each neuron $j \in m_l$, $\sigma^{(l)}_j(z)$ is one of two values depending only on the sign of $z$, so normalizing $W^{(l)}_{1:m_{l-1},1:m_l}$ by $||W^{(l)}_{1:m_{l-1},1:m_1}||_F$ and making a change of variables to rescale the last row $W^{(l)}_{m_{l-1}+1,1:m_1}$ of $W^{(1)}$ does not change the output of the $l^{\text{th}}$ hidden layer $\sigma_{s^(l)}(X^{(l-1)}W^{(l)})$. For each hidden layer $l \in [L-1]$ we can also normalize $s^{(l)}$ by $||s^{(l)}||_2$ and again rescale the last row of $W^{(l+1)}$ by $||s^{(l)}||_2$ without changing the output of the ${l+1}^{\text{th}}$ hidden layer. Therefore, the regularization terms $||W^{(l)}_{1:m_{l-1}, 1:m_l}||^2_F$ for $l \in [L]$ and $ ||s^{(l)}||^2_2 $ for  $l \in [L-1]$ become redundant in the minimization. So the only regularization term that remains is $||\alpha||^2_2+||s^{(L)}||^2_2$. Now, the same proof as for proposition \ref{prop:sign_thresh_scaled} holds to transform this L2 regularization into a L1 penalty on $\alpha$.
\end{proof}

%\begin{proof}
%    The variables in the last rows of $W^{(1)}, W^{(2)}$ are not regularized and therefore can be rescaled. For each coordinate $j \in m_1$, $\sigma^{(1)}_j(z)$ is one of two values depending only on the sign of $z$, so normalizing $W^{(1)}_{1,1:m_1}$ by $||W^{(1)}_{1,1:m_1}||_F$ and making a change of variables to rescale the last row $W^{(1)}_{2,1:m_1}$ of $W^{(1)}$ does not change the output of the first hidden layer $\sigma_{s^(1)}(XW^{(1)})$. The same argument holds for normalizing the first $m_1$ rows of $W^{(2)}$ and rescaling its last row for the second hidden layer. We can also normalize $s^{(1)}$ by $||s^{(1)}||_2$ and again rescale the last row of $W^{(2)}$ by $||s^{(1)}||_2$ without changing the output of the second hidden layer. Therefore, the regularization terms $||W^{(2)}_{1:m_1, 1:m_2}||^2_F + ||W^{(1)}_{1,1:m_1}||^2_F + ||s^{(1)}||^2_2 $ become redundant in the minimization. So the only regularization term that remains is $||\alpha||^2_2+||s^{(2)}||^2_2$. Now, the same proof as for proposition \ref{prop:sign_thresh_scaled} holds to transform this L2 regularization into a L1 penalty on $\alpha$.
%\end{proof}

Problem \ref{equ:psignL_simp} is equivalent to 

\begin{equation}
\label{equ:psignL_intermed}
\begin{aligned}
   \min_{W^{(l)}: ||W^{(l)}||_F=1, s^{(l)}=1, \alpha} & \frac{1}{2}  || Z - y||^2_2 + \beta ||\alpha||_1 \\
   &\text{ s.t. }
   Z = f_L(X)
\end{aligned}
\end{equation}

The Lagrangian is 

\begin{equation}
    L(s^{(l)}=1, W^{(l)}, \alpha, \lambda) = \frac{1}{2}  || Z - y||^2_2 + Z^T \lambda + \beta ||\alpha||_1 - \alpha^T \left( \sigma_{s=1} \left( X^{(L-1)} {W^{(L)}} \right) \right)^T \lambda
\end{equation}


Note for $i \in [N], \left(\left( \sigma_{s=1} \left( X^{(L-1)} {W^{(L)}} \right) \right)^T \lambda \right)_i$ is the inner product between $\lambda$ and the $i^{th}$ column of $\sigma_{s=1} \left( X^{(L-1)} {W^{(L)}} \right) \in \mathbf{R}^{N \times m_L}$, which is $\sigma \left( X^{(L-1)}{W^{(L)}_{1:1+m_{1-1}, i}}\right) \in \mathbf{R}^{N \times m_L}$ where ${W^{(L)}_{1:1+m_{L-1}, i}}$ is the $i^{th}$ column of $W^{(L)}$, corresponding to the weights from neuron $i$ in the $L^{\text{th}}$ layer.

The dual of \eqref{equ:psignL_simp}  is 

\begin{equation}\label{dsignL_sigmas}
\begin{aligned}
   \max_{\lambda} & -\frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } \max_{s^{(l)}=1, W^{(1)} \in \mathbf{R}^{1+m_{l-1} \times m_1}, w^{(L)} \in \mathbf{R}^{1+m_{L-1}}} |\lambda^T \sigma \left( X^{L-1}{w^{(L)}} \right) | \leq \beta 
\end{aligned}
\end{equation}



\section{(redundant since generalized to L) sign activation nonparallel 2 hidden layers}

For $L=2$ hidden layers, for $x \in \mathbf{R}$ the neural network is

\begin{equation}\label{3layernn_cpt}
\begin{aligned}
     f_3(x) &= \sigma_{s^{(2)}}\left( \left(\sigma_{s^{(1)}}\left( X W^{(1)} \right) , \mathbf{1} \right) W^{(2)} \right) \alpha
\end{aligned}
\end{equation}

where $X = (x, 1) \in \mathbf{R}^{1 \times 2}, W^{(1)} \in \mathbf{R}^{2 \times m_1},  W^{(2)} \in \mathbf{R}^{m_1+1 \times m_2}, %b \in \mathbf{R}^{1 \times m_2}, 
\alpha \in \mathbf{R}^{m_2 \times 1}$.

For $L=2$ hidden layers, the training problem is

\begin{equation}
\label{equ:psign3}
\begin{aligned}
   \min_{W^{(1)}, W^{(2)}, s^{(1)}, s^{(2)}, \alpha} \frac{1}{2} || \sigma_{s^{(2)}}\left(\sigma_{s^{(1)}}\left( X W^{(1)} \right) {W^{(2)}}\right)\alpha - y||^2_2 + \beta/2 \left ( ||\alpha||^2_2  +  ||W^{(2)}_{1:m_1, 1:m_2}||^2_F + ||W^{(1)}_{1,1:m_1}||^2_F + ||s^{(1)}||^2_2 + ||s^{(2)}||^2_2\right)
\end{aligned}
\end{equation}

Where $W^{(1)}_{1,1:m_1}$  denotes the first row of $W^{(1)}$ and $W^{(2)}_{1:m_1, 1:m_2}$ denotes the first $m_1$ rows of $W^{(2)}$. These are the non-bias weights of two hidden layers, and for notational convenience the output of the innermost activation $\sigma_{s^(1)}$ attaches a vector of ones $\mathbf{1} \in \mathbf{R}^{2 \times 1}$ to the end of the output matrix.


For $L=2$ hidden layers, 

\begin{proposition}
    The training problem \eqref{equ:psign3} for $L=2$ hidden layers is equivalent to 

\begin{equation}
\label{equ:psign3_simp}
\begin{aligned}
   \min_{W^{(1)}, W^{(2)}, \alpha} \frac{1}{2} || \sigma \left(\sigma\left( X W^{(1)} \right) {W^{(2)}}\right)\alpha - y||^2_2 + \beta ||\alpha||_1
\end{aligned}
\end{equation}
\end{proposition}

where $\sigma(z) = \sigma_{s=1}(z) = \text{sign}(z)$.




For example, for $L=2$ hidden layers, problem \ref{equ:psign3_simp} is equivalent to 

\begin{equation}
\label{equ:psign3_intermed}
\begin{aligned}
   \min_{W^{(1)}, W^{(2)}, \alpha} & \frac{1}{2}  || Z - y||^2_2 + \beta ||\alpha||_1 \\
   &\text{ s.t. }
   Z = \sigma \left(\sigma\left( X W^{(1)} \right) {W^{(2)}}\right)\alpha 
\end{aligned}
\end{equation}


The Lagrangian of the $L=2$ hidden layer training problem is 

\begin{equation}
    L(W^{(1)}, W^{(2)}, \alpha, \lambda) = \frac{1}{2}  || Z - y||^2_2 + Z^T \lambda + \beta ||\alpha||_1 - \alpha^T \left( \sigma \left( \sigma\left( X W^{(1)} \right) {W^{(2)}} \right) \right)^T \lambda
\end{equation}

The dual of \eqref{equ:psign3_simp}  is 

\begin{equation}\label{dsign3_sigmas}
\begin{aligned}
   \max_{\lambda} & -\frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } \max_{W^{(1)} \in \mathbf{R}^{2 \times m_1}, w^{(2)} \in \mathbf{R}^{m_1+1}} |\lambda^T \sigma \left( \sigma\left( X W^{(1)} \right) {w^{(2)}} \right) | \leq \beta 
\end{aligned}
\end{equation}


For a $n \times d$ matrix $Z$, for every $h=\sigma(Zw) \in \mathcal{H}(Z)$, we have $-h = \sigma(Z(-w)) \in \mathcal{H}(Z)$. Let $l \in [L-1]$. Suppose $H=\sigma_{s=1}(X^{(l-1)}W^{(l)})$. Let $h$ be the $i^{th}$ column of $H$. Let $H'$ be $H$ except its $i^{th}$ column is $-h$. Let $w^{(l+1)} \in \mathbf{R}^{m_l+1}$ and $ \tilde w^{(l+1)} $ be $\tilde w^{(l+1)} $  except its $i^{th}$ element is negated. Then $\sigma(X^{(l-1)}W^{(l)})w^{(l+1)}=\sigma(X^{(l-1)}\tilde W^{(l)})w^{(l+1)}$. Since the constraint in problem \eqref{dsignL} maximizes over all feasible weights, it suffices to remove ``redundant" elements that are negations of each other from $\mathcal{H}(X^{(l)})$. So we restrict the definition of $\mathcal{H}(Z)$ by assuming that all $h \in \mathcal{H}(Z)$ start with $h_1 = 1$.


$\sigma\left( X W^{(1)} \right) {w^{(2)}}$ is a linear combination of up to $m_1 + 1$ columns of $\sigma\left( X W^{(1)} \right) \in \mathbf{R}^{N \times m_1}$. When $W^{(1)}$ ranges over all of $\mathbf{R}^{2 \times m_1}$, $\sigma\left( X W^{(1)} \right) {w^{(2)}}$ is the output of a neuron acting on up to $m_1 + 1$ subset of columns generated by $\sigma(X W^{(1)})$. The $i^{th}$ column of  $\sigma\left( X W^{(1)} \right) $ is $X W^{(1)}_{1:2, i}$, the output of the $i^{th}$ neuron in the first layer over all the training samples. So $\sigma\left( X W^{(1)} \right) {w^{(2)}}$ is a possible output of a neuron with weights $w^{(2)}$ taking in $N$ feature vectors of length $m_1+1$, ie the feature matrix $\sigma\left( X W^{(1)} \right)$. This is $\mathcal{H}$ acting on a $S=m_1+1$ size subset of $\mathcal{H}(X)$ whose elements are concatenated into into a matrix, denoted by $[\mathcal{H}(X))]_{S}$.


For every $h=\sigma(Xw) \in \mathcal{H}(X)$, we have $-h = \sigma(X(-w)) \in \mathcal{H}(X)$. Suppose $H=\sigma(XW^{(1)})$ with $i^{th}$ column being $h$, and $H'$ being $H$ except its $i^{th}$ column is $-h$. Let $w^{(2)} \in \mathbf{R}^{m_1+1} \tilde w^{(2)} $ be $\tilde w^{(2)} $  except its $i^{\text{th}}$ element is negated. Then $\sigma(XW^{(1)})w^{(2)}=\sigma(X\tilde W^{(1)})\tilde w^{(2)}$. So it suffices to remove ``redundant" elements from $\mathcal{H}(X)$ by assuming that all $h \in \mathcal{H}(X)$ start with $h_1 = 1$.

The dual of \eqref{dsign3_sigmas} is 

\begin{equation}\label{dsign3}
\begin{aligned}
   \max_{\lambda} & -\frac{1}{2}  || \lambda + y||^2_2 + ||y||^2_2  \\
   &\text{ s.t. } \max_{h \in \cup_{|S|\leq m_1+1} \mathcal{H}([\mathcal{H}(X))]_S} |\lambda^T h | \leq \beta 
\end{aligned}
\end{equation}

In the outermost $\mathcal{H}$, for $Z \in \mathbf{R}^{N \times m_1}$ define $\tilde{Z}=[Z \mathbf{1}]$ to be $Z$ with a vector of ones appended, and $\mathcal{H}(Z)=\{ \sigma(\tilde{Z} w): w \in \mathbf{R}^{m_1+1} \}$ to account for the bias term within the outermost $\sigma$ argument. \eqref{dsign3} is the dual of and therefore equivalent to the LASSO problem

\begin{equation}
\begin{aligned}
   \min_z & \frac{1}{2}  || Az- y||^2_2 + \beta||z||_1  \\
\end{aligned}
\end{equation}

where the ``dictionary" matrix $A=[\cup_{|S| \leq m_1+1} \mathcal{H}([\mathcal{H}(X))]_S ]$ is the matrix consisting of all possible second layer patterns.

\iftoggle{todos}{
    \textcolor{red}{todo: shattering}
}

\section{other}

\begin{lemma}
    Suppose  $\sigma(z) \xrightarrow[]{} \infty$ iff $|z| \to \infty$. Also suppose there exists $a > 0$ such that $\sigma(z)$ has a Taylor expansion at $a^+$ and $a^-$.  Then $\max_{b} |\lambda^T \sigma(Xw+b)| < \infty$ iff for every $j \in \{0, \dots, p-1\}$, $\sum_{i=1}^n \lambda_i x^j_i = 0$.
\end{lemma}

If $p=1$ as in $\sigma(z) = z_+$ or $\sigma(z) = |z|$, or leaky Relu, then this condition is just $\sum_{i=1}^n \lambda_i = 0$. If $X^j$ denotes elementwise exponentiation of vector $X$, then  we can write the finite maximum condition as $\lambda^T X^j=0$ for $j \in \{0, \dots, p-1\}$. 

\begin{proof}
Since $\sigma(z) \xrightarrow[]{} \infty$ iff $|z| \to \infty$, we have $ \max_{b} |\lambda^T\sigma(b \pm X)| = \infty$ only if $|b| \to \infty$. Observe $\lambda^T \sigma(b\pm X)= \sum_{i=1}^n \lambda_i \sigma(b \pm x_i) = \sum_{i=1}^n \lambda_i \sigma(\frac{|b|}{a}(\textrm{sgn(b)}a \pm \frac{a x_i}{|b|})) = \sum_{i=1}^n \lambda_i |\frac{b}{a}|^p \sigma(\textrm{sgn(b)}a \pm \frac{a x_i}{|b|})= \sum_{i=1}^n \lambda_i |\frac{b}{a}|^p  \sum_{j=0}^\infty \sigma^{(j)}(\textrm{sgn}(b)a) (\pm \frac{a x_i}{|b|})^j  =  \sum_{j=0}^{p-1} \sigma^{(j)}(\textrm{sgn}(b)a) |\frac{b}{a}|^{p-j}  \sum_{i=1}^n \lambda_i  x_i^j +  \sum_{i=1}^n \sum_{j=p}^\infty \lambda_i \sigma^{(j)}(\textrm{sgn}(b)a) \frac{x_i^j}{|\frac{b}{a}|^{j-p}} $ approaches $\pm \infty$ as $|b| \xrightarrow[]{} \infty$ iff for every $j \in \{0, \dots, p-1\}$, $\sum_{i=1}^n \lambda_i x^j_i = 0$. 
\end{proof}

\section{other} 

\begin{proposition}
    If $\sigma(z)=z_+$ and the optimal dual variables are all nonnegative ($\lambda \geq 0$) then the constraint in equation \ref{equ:d} reduces to
    $(x-x_1\mathbf{1})^T \lambda \leq \beta$ and  $(x_n\mathbf{1}-x)^T \lambda \geq -\beta$.
\end{proposition}

The constraint in equation \ref{equ:d} is that for all hyperplane arrangement patterns $D$,

\begin{equation}
\begin{aligned}
       \max_{w,b} & \quad a \sum_{i\in D} \lambda_i (x_i w + b) + c \sum_{i\in D^c} \lambda_i (x_i w + b) \quad \quad \leq \beta \\
       \text{ st } & |w|=1 \\
       &x_i w + b \geq 0 \text{ for all } i \in D\\
       &x_i w + b \leq 0 \text{ for all } i \in D^c
\end{aligned}
\end{equation}

(And similarly for the negative). %although accounted for by D^c?

Assume $x_1 < x_2 < \dots < x_N$. Then the hyperplane arrangements are for all $j \in \{0, \dots, N\}$, $D_j = \{x_i: i \leq j \}$ and $D^c$, ie for all $j \in \{0, \dots, N\}$, $D_j^c = \{x_i: i > j \}$.

If $w=1$, for each hyperplane arrangement $D_j$,

\begin{equation}
\begin{aligned}
       \max_{b} & \quad a \sum_{i\in D} \lambda_i (x_i + b) + c \sum_{i\in D^c} \lambda_i (x_i  + b) =  a \sum_{i\in D} \lambda_i x_i + c \sum_{i\in D^c} \lambda_i x_i  + b(a\sum_{i\in D} \lambda_i +c\sum_{i\in D^c} \lambda_i ) \leq \beta \\
       \text{ st } 
       &\max_{i \leq j} \{-x_i\} \leq b \leq \min_{i>j} \{-x_i\}  \\
\end{aligned}
\end{equation}

which is a linear program, and if is finite then $b \in \{\max_{i \leq j} \{-x_i\}, \min_{i>j} \{-x_i \} \}$. So for every $j \in \{0, \dots, N\}$, the hyperplane arrangement $D_j$ gives

\begin{equation}
    \begin{aligned}
     a \sum_{i\in D} \lambda_i x_i + c \sum_{i\in D^c} \lambda_i x_i  + \max \left \{ {\max_{i \leq j} \{-x_i\} (a\sum_{i\in D} \lambda_i +c\sum_{i\in D^c} \lambda_i ), \min_{i>j} \{-x_i\}  (a\sum_{i\in D} \lambda_i +c\sum_{i\in D^c} \lambda_i )} \right \} \leq \beta   
    \end{aligned}
\end{equation}

Similarly for $w=-1$ the hyperplane arrangement $D_j$ gives

\begin{equation}
    \begin{aligned}
     -a \sum_{i\in D} \lambda_i x_i - c \sum_{i\in D^c} \lambda_i x_i  + \max \left \{ {\max_{i \leq j} \{x_i\} (a\sum_{i\in D} \lambda_i +c\sum_{i\in D^c} \lambda_i ), \min_{i>j} \{x_i\} (a\sum_{i\in D} \lambda_i +c\sum_{i\in D^c} \lambda_i )} \right \} \leq \beta   
    \end{aligned}
\end{equation}

Let $\tilde{D}_i = (aD_i + c (I-D_i))$.

Then for $w=1$ and  hyperplane arrangement $D_j$,

\begin{equation}
    (\tilde{D}_j \lambda)^T x + \max \{  \max_{i \leq j} \{-x_i\}   \mathbf{1}^T \tilde{D}_j \lambda, \min_{i>j} \{-x_i\}  \mathbf{1}  \tilde{D}_j \lambda \} \leq \beta 
\end{equation}

which is equivalent to 

\begin{equation}
\begin{aligned}
      (\tilde{D}_j \lambda)^T x +  \max_{i \leq j} \{-x_i\}   \mathbf{1}^T \tilde{D}_j \lambda & \leq \beta \\
    (\tilde{D}_j \lambda)^T x +  \min_{i>j} \{-x_i\}  \mathbf{1}^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

ie

\begin{equation}
\begin{aligned}
       (x +  \max_{i \leq j} \{-x_i\}   \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (x +  \min_{i>j} \{-x_i\}  \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

Note $\max_{i \leq j} \{-x_i\} = -\min_{i \leq j} \{x_i\} = -x_1$. And $\min_{i>j} \{-x_i\} = -\max_{i>j} \{x_i\} = -x_n$. So the $w=1$ and $D_j$ hyperplane constraint is,

\begin{equation}
\begin{aligned}
       (x - x_1  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (x -  x_n\mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

By switching $D_j$ and $D_j^c$ (ie turning $i\leq j$ into $i>j$ and $i>j$ into $i \leq j$), for $w=1$ and $D_j^c$ arrangement gives


\begin{equation}
\begin{aligned}
       (x +  \max_{i > j} \{-x_i\}   \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (x +  \min_{i\leq j} \{-x_i\}  \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

ie

\begin{equation}
\begin{aligned}
       (x - x_{j+1}  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (x -  x_{j} \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

And for $w=-1$, plugging in $w=-1$ negates the sign of $x$, so the hyperplane arrangement $D_j$ gives 


\begin{equation}
\begin{aligned}
      (- x +  \max_{i \leq j} \{x_i\}   \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (-  x +  \min_{i>j} \{x_i\}  \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

ie 

\begin{equation}
\begin{aligned}
      (- x +  x_j  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (-  x + x_{j+1}  \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

By switching $D_j$ and $D_j^c$, for $w=-1$, hyperplane $D_j^c$ gives

\begin{equation}
\begin{aligned}
      (- x +  x_n  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (- x + x_1 \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
\end{aligned}
\end{equation}

All together collecting $w=1$ and $W=-1$ and $D_j, D_j^c$, for every $j \in \{0, \dots, n\}$ we have


\begin{equation}
\begin{aligned}
       (x - x_1  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (x -  x_n\mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
       (x - x_{j+1}  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (x -  x_j\mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\   
    (-x + x_{j}  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (-x +  x_{j+1} \mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\     (-x + x_1  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    (-x +  x_n\mathbf{1})^T  \tilde{D}_j \lambda 
\end{aligned}
\end{equation}

ie, for every $j \in \{0,\dots,n \}$, 

\begin{equation}
    \begin{aligned}
    -\beta \leq (x - x_1  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\
    -\beta \leq (x -  x_n\mathbf{1})^T  \tilde{D}_j \lambda  &\leq \beta \\
     -\beta \leq (x - x_{j}  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\ 
    -\beta \leq (x - x_{j+1}  \mathbf{1})^T \tilde{D}_j \lambda & \leq \beta \\ 
    \end{aligned}
\end{equation}

Note that in elementwise vector partial ordering, for each $j$,

$x-n \mathbf{1} \leq x-x_{j+1}\mathbf{1} \leq x-x_j\mathbf{1} \leq x -x_n\mathbf{1}$.

Special case: Suppose $c=0$, for example $\sigma(z)=z_+$. Suppose the optimal dual variables are all the same sign, eg $\lambda \geq 0$. This occurs? if the problem was to interpolate through all points, so the objective is $\lambda^T y$, and the labels are all positive so that the optimal $\lambda \geq 0$. 

The constraints would reduce to the most restrictive ones that make the coefficients on $\lambda$ the largest or smallest, ie $(x-x_1\mathbf{1})^T \lambda \leq \beta$ and  $(x_n\mathbf{1}-x)^T \lambda \geq -\beta$. There is also the $\lambda \geq 0$ constraint. This is like a deformed simplex. If the objective is to maximize $\lambda^T y$ and only one of the nonzero constraints is active (for example if the sign of $x_i$ is the same for all $i$) then we would put everything into one of the coordinates of $\lambda$, eg if $y= \mathbf{1}$ then $\lambda_i = \textrm{argmax} \beta/(x_i-x_1) = \beta/(x_n - x_1)$ so $i=n$ and all other  $y_i=0$. For general $y$, choose $\lambda_i = \textrm{argmax } \beta y_i/(x_i-x_1)  $.

\textbf{unused}\\

Suppose $\sum_{i=1}^n \lambda_i = 0$. Then for fixed $w$, $\sum_{i=1}^n \lambda_i (x_i w + b)_+$ is bounded and becomes flat at the first and last kink point. So for some $j \in [n]$,

\begin{align}
    \max_{b} \sum_{i=1}^n \lambda_i (x_i w + b)_+ &= \sum_{i=1}^n \lambda_i (x_i w - x_j w)_+ \\
    &= \sum_{i=1}^n \lambda_i ((x_i - x_j) w)_+ \\
    &= \sum_{i=1}^n \lambda_i |(x_i - x_j) | ( \textrm{sgn} (x_i - x_j)  w)_+ \\
    &= \sum_{x_i - x_j > 0} \lambda_i |(x_i - x_j) | ( \textrm{sgn} (x_i - x_j)  w)_+ + \sum_{x_i - x_j < 0} \lambda_i |(x_i - x_j) | ( \textrm{sgn} (x_i - x_j)  w)_+ \\    
\end{align}


